Occam Learning Meets Synthesis Through Unification

The generalizability of PBE solvers is the key to the empirical synthesis performance. Despite the importance of generalizability, related studies on PBE solvers are still limited. In theory, few existing solvers provide theoretical guarantees on generalizability, and in practice, there is a lack of PBE solvers with satisfactory generalizability on important domains such as conditional linear integer arithmetic (CLIA). In this paper, we adopt a concept from the computational learning theory, Occam learning, and perform a comprehensive study on the framework of synthesis through unification (STUN), a state-of-the-art framework for synthesizing programs with nested if-then-else operators. We prove that Eusolver, a state-of-the-art STUN solver, does not satisfy the condition of Occam learning, and then we design a novel STUN solver, PolyGen, of which the generalizability is theoretically guaranteed by Occam learning. We evaluate PolyGen on the domains of CLIA and demonstrate that PolyGen significantly outperforms two state-of-the-art PBE solvers on CLIA, Eusolver and Euphony, on both generalizability and efficiency.

==> sections/Background.tex <==
%!TEX root = ../CLIA.tex
\section{Preliminaries} \label{section:background}
In this section, we introduce some concepts that we build upon for the rest of this paper. 

\subsection{Programming by Example} \label{section:background-pbe}
\begin{definition}[Semantics Function] Given a program domain $\mathbb P$, an input domain $\mathbb I$, and an output domain $\mathbb O$, an oracle function $\sem{.}_{\mathbb P, \mathbb I, \mathbb O}: \mathbb P \rightarrow \mathbb I \rightarrow \mathbb O$ asociates a program $p$ and an input $I$ with an output, denoted as $\sem{p}_{\mathbb P, \mathbb I, \mathbb O}(I)$. 
\end{definition}

In this paper, we implicitly assume the existence of a universal semantics function $\sem{.}$ for any program, input and output domains. 

\textit{Programming by Example (PBE)}~\cite{} is a subproblem of program synthesis where the synthesis system is required to learn a program from a set of given input-output examples.

\begin{definition}[Programming by Example] Given a program domain $\mathbb P$, an input domain $\mathbb I$ and an output domain $\mathbb O$, a PBE task $T \in (\mathbb I \times \mathbb O)^*$ is a sequence of input-output examples.
	
Correspondingly, a PBE solver $\mathcal S: (\mathbb I \times \mathbb O)^* \rightarrow {\{\top\} \cup \mathbb P}$ is a function satisfying the following two conditions for any PBE task $T \in (\mathbb I \times \mathbb O)^*$:
\begin{itemize}
	\item (Correctness) If $\mathcal S(T)$ is a program, $\mathcal S(T)$ must be consistent with all examples in $T$:
	$$\mathcal {S}(T) \in \mathbb P \implies \forall (I, O) \in T, \sem{\mathcal {S}(T)}(I) = O$$
	\item (Completeness) If $\mathcal S(T) = \top$, all programs in $\mathcal P$ must violate at least one example in $T$:
	$$\mathcal {S}(T) = \top \iff \forall p \in \mathbb P, \exists (I, O) \in T, \sem{p}(I) \neq O$$
\end{itemize}
\end{definition}

Obviously, PBE tasks on input domain $\mathbb I$ cannot distinguish two programs if their semantics perform the same on all inputs in $\mathbb I$. We formalize this property as a relation between programs.

\begin{definition}[Semantically Equivalence] Two programs $p_1$ and $p_2$ are semantically equivalence on an input domain $\mathbb I$, written as $p_1 \sim_{\mathbb I} p_2$ if and only if $\forall I \in \mathbb I, \sem{p_1}(I) = \sem{p_2}(I)$.
\end{definition}
\subsection{Conditional Program Domain and Synthesis through Unification}
In this paper, we focus on a special kind of synthesis tasks where the program domain supports enough flexibility for \texttt{if-then-else} operators: We assume the program domain can be decomposed into two domains, for if-conditions and if-terms respectively, according the \texttt{if-then-else} operator.

\begin{definition}[Conditional Program Domain] A program domain $\mathbb P$ is a conditional program domain if and only if there exist two program domains $\mathbb P_c$ and $\mathbb P_t$ such that $\mathbb P$ is the smallest set of programs such that:
$$
\mathbb P = \mathbb P_t \cup \left\{\texttt{if}\ c\ \texttt{then}\ p_1\ \texttt{else}\ p_2\ |\ p_1, p_2 \in \mathbb P, c \in C(\mathbb P_c)  \right\}
$$
where $C(\mathbb P_c)$ is the set of all possible conditions, which is the smallest set such that:
$$
C(\mathbb P_c) = \mathbb P_c \cup \left\{c_1\ \texttt{and}\ c_2\ |\ c_1,c_2 \in C(\mathbb P_c)\right\} \cup  \left\{c_1\ \texttt{or}\ c_2\ |\ c_1,c_2 \in C(\mathbb P_c)\right\} \cup \{\texttt{not}\ c\ |\ c \in C(\mathbb P_c)\}
$$
\end{definition}

For convenience, we use a pair of program domains $(\mathbb P_c, \mathbb P_t)$ to denote a conditional program domain derived from it. 

\textit{Synthesis through Unification (STUN)}~\cite{DBLP:conf/cav/AlurCR15} is a framework for synthesizing from a conditional program domain. Given a conditional program domain $(\mathbb P_t, \mathbb P_c)$, the STUN framework synthesizes programs in two steps:
\begin{enumerate}
	\item It uses a term solver to synthesize a set of programs $P \subseteq \mathbb P_t$ such that for any possible input $I$, there is always a program $p \in P$ such that $\sem{p}[I]$ is a valid output.
	\item It uses a unifier to unify $P$ into a single program using conditions synthesized from $C(\mathbb P_c)$ and \texttt{if-then-else} operators.
\end{enumerate}
In this paper, we only consider the specialized version of the STUN framework on PBE tasks.

\begin{definition}[Term Solver] Given a program domain $\mathcal P_t$, a term solver $\mathcal T: (\mathbb I \times \mathbb O)^* \mapsto \{\top\} \cup \mathcal P(\mathbb P_t)$ is a function satisfying the following two conditions for any PBE task $T \in (\mathbb I, \mathbb O)^*$, where $\mathcal P(\mathbb P_t)$ represents the power set of $\mathbb P_t$:
	\begin{itemize}
		\item (Correctness) If $\mathcal T(T)$ is a set of programs, for each example, there is a program in $\mathcal T(T)$ consistent with it:
		$$\mathcal T(T) \subseteq \mathbb P_t \implies \forall (I,O) \in T, \exists p \in \mathcal T(T), \sem{T}(I) = O$$
		\item (Completeness) If $\mathcal T(T) = \top$,  all subsets of $\mathcal P_t$ must violate at least one example in $T$:
		$$\mathcal T(T) = \top \iff \forall P \subseteq \mathbb P_t, \exists (I,O) \in T, \forall p \in P, \sem{p}(I) \neq O$$
	\end{itemize}
\end{definition}

\begin{definition}[Unifier] Given a conditional program domain $\mathbb P = (\mathbb P_t, \mathbb P_c)$, a unifier $\mathcal U: \mathcal P(\mathbb P_t) \rightarrow (\mathbb I \times \mathbb O)^* \rightarrow \{\top\} \cup \mathbb P$ is a function such that for any set of programs $P \subseteq \mathbb P_t$, $\mathcal U(P)$ is a PBE solver for conditional program domain $(P, \mathbb P_c)$. 
\end{definition}

In the STUN framework, a synthesizer is a pair of a term solver $\mathcal T$ and a unifier $\mathcal U$. Given a PBE task $T$, the synthesizer simply returns $\mathcal U(\mathcal T(T))(T)$ as the result. In contrast to the correctness of this construction, which is straight-forward from the correctness of $\mathcal T$ and $\mathcal U$, the completeness of STUN is guaranteed only when the program domain is \textit{if-closed}, in which the conditions are expressive enough to correct the mistake made by the term solver. 

\begin{definition}[If-Closed] A conditional program domain is \textit{if-closed} if: $$\forall p_1, p_2 \in \mathbb P_t, \exists c \in C(\mathbb P_c), \forall I \in \mathbb I, \left(\sem{c}(I) \iff \sem{p_1}(I) = \sem{p_2}(I)\right)$$
\end{definition}

\begin{lemma} \label{lemma:completeness}  The STUN framework is complete for any if-closed conditional program domain $(\mathbb P_t, \mathbb P_c)$.
\end{lemma}

In this paper, we mainly focus on if-closed program domains. For other domains, STUN can be extended to complete by backtracking to the term solver when the unification fails, as done by many related works ~\cite{DBLP:conf/cav/AlurCR15, DBLP:conf/tacas/AlurRU17}.

\subsection{\textit{EuSolver}}
\textit{Eusolver}~\cite{DBLP:conf/tacas/AlurRU17} is a state-of-the-art synthesizer following the STUN framework. We shall briefly introduce the algorithm of \textit{Eusolver} as it motivates our work on the generalizability. 

\SetKwFunction{Enum}{Enumerate}
\SetKwFunction{Covered}{Covered}
\SetKwFunction{Learn}{LearnDT}
\SetKwFunction{Select}{SelectCond}

Algorithm \ref{alg:eusolver-term} shows the pseudo code of the term solver in \textit{Eusolver}. The term solver enumerates programs in domain $\mathbb P_t$ in the increasing order of the size (Line 4). For each program $p$, if there is not a program that satifies exactly the same subset of examples as $p$, $p$ will be included into the result (Lines 6-8). The enumeration ends when the enumerated programs are enough to cover all examples in $T$ (Line 9).

Algorithm \ref{alg:eusolver-uni} shows the pseudo code of the unifier in \textit{Eusolver}, which is from \textit{ID3}~\cite{DBLP:journals/ml/Quinlan86}, a standard multi-label decision tree learning algorithm. The unifier uses function \Learn{\variable{examples}} to recursively synthesize a program satisfying all examples in \variable{examples} (Lines 1-11). In each invocation, the unifier firstly try to use a term to cover all examples (Lines 2-4). Then, it picks up a condition $c$ in $\mathbb P_c$ based on some greedy strategy, and tries to synthesize a program in the form of \texttt{if} $(c)$ \texttt{then} $t$ \texttt{else} $f$ (Line $5$).  To form a correct program, program $t$ and $f$ must satisfy all examples on which $c$ is evaluated to true and false respectively (Lines 6-7). Therefore, the unifier recursively invokes $\Learn$ to synthesize proper programs $t$ and $f$ (Line $9$). 

\begin{figure}[t]
\begin{minipage}{.46\linewidth}
\begin{algorithm}[H]
	\small
	\caption{The term solver in \textit{Eusolver}.}
	\label{alg:eusolver-term}
	\LinesNumbered
	\KwIn{PBE task $T$ and domain $\mathbb P_t$.}
	\KwOut{A set of programs in $\mathbb P_t$ or $\top$.}
	\SetKwProg{Fn}{Function}{:}{}
	\Fn{\Covered{$p, T$}}{\Return $\left\{(I,O)\ |\ (I,O) \in T \wedge \sem{p}(I) = O\right \}$;}
	\variable{covered} $\gets \emptyset$; \ \ \variable{result} $\gets \emptyset$; \\
	\For{each $p \in \Enum{$\mathbb P_t$}$}{
		\If {$\forall p' \in \variable{result}, \Covered{$p, T$} \neq \Covered{$p', T$}$}{
			$\variable{covered} \gets \variable{covered} \cup \Covered{$p, T$}$; \\
			$\variable{result} \gets \variable{result} \cup \{p\}$;
		}
		\lIf {$\variable{covered} = T$}{\Return \variable{covered}}
	}
\Return $\top$;
\end{algorithm}
\ \ 
\end{minipage}
\begin{minipage}{.49\linewidth}
	\begin{algorithm}[H]
		\small
		\caption{The unifier in \textit{Eusolver}.}
		\label{alg:eusolver-uni}
		\LinesNumbered
		\KwIn{PBE task $T$, terms $P$, condition domain $\mathbb P_c$.}
		\KwOut{A valid program in $(P, \mathbb P_c)$ or $\top$.}{
		\SetKwProg{Fn}{Function}{:}{}
		\Fn{\Learn{$\variable{examples}$}}{
			\If {$\exists p \in P, \variable{examples} \subseteq \Covered{p, T} $}{\Return $p$;}	
			$c \gets \Select{$\variable{examples}, \mathbb P_c$}$; \\
			$\variable{tE} \gets \{(I, O) \in \variable{examples}\ |\ \sem{c}(I)\}$; \\
			$\variable{fE} \gets \{(I, O) \in \variable{examples}\ |\ \neg \sem{c}(I) \}$; \\
			\lIf {$\variable{tE} = \emptyset \vee \variable{fE} = \emptyset$}{\Return $\top$}
			$t \gets \Learn{$tE$};$\ \
			$f \gets \Learn{$fE$};$ \\
			\lIf {$t = \top \wedge f = \top$}{\Return $\top$}
			\Return \texttt{if} $(c)$ \texttt{then} $t$ \texttt{else} $f$; \\
		}
		\Return {\Learn{$T$}};
	}
	\end{algorithm}
\end{minipage}
\end{figure}
\todo{Example}

==> sections/Evaluation.tex <==
%!TEX root = ../CLIA.tex
\section{Evaluation}\label{section:evaluation}

To evaluate \mainname, we report several experiments designed to answer the following research questions:

\begin{itemize}
	\item \textbf{RQ1:} How does \mainname compare against existing solver for generalizability?
	
	
	\item \textbf{RQ2:} How quickly can \mainname arrive at a correct solution?
\end{itemize}

\subsection{Experimental Setup}

\noindent \textbf{Benchmark}

We combined two datasets, CLIA benchmark used in SyGuS-Comp \todo{add refer} comprised of 100 benchmarks and our benchmark of divide-and-conquer. Our benchmark focus on the combinator of information merge of two list. For example, with the maximum prefix sum $(mps)$, maximum suffix sum $(mts)$ and maximum segment sum $(mss)$ of both lists, we are able to obtain the maximum segment sum of the list concatenated with the combinator function $ mss = \max \left(mss_{1}, mss_{2}, mts_{1}+m p s_{2}\right)$. These tasks have significant application in the domain of parallel and concurency. In these tasks, the input are in the form $(l_1 args_1,l_2 args_1, \cdots, l_1 args_n,l_2 args_n)$ with $2n$ arguments in total. Our benchmarks are in CLIA domain for a type of fundamental questions about conbinator and have not been put forward yet. Since these tasks are with a great number of arguments and these arguments are not functionally symmetric, and for some are not necessarily used or should not be used in the optimal solutions, they are challenging for the current solvers. Solving these tasks with PBE is a essential step in AlgorithmSynthesis \todo{add refer} that we have not found other existing solver are able to solve this problem satisfactorily.



\noindent \textbf{Baseline Solvers}

We compare MaxFlash with four synthesizers, which are selected according to the following criteria. First, we compare \mainname with Eusolver because \mainname uses the same frame as Eusolver for deviding the whole synthesizing procedure into term solver and unifier. We also take CVC4 into comparison for its excellent performance in CLIA domain.

\begin{itemize}
	\item $Esolver$ \todo{add refer},  the winner of the PBE track in SyGuS-Comp 2014 \todo{add refer}, is the very basic solver of SyGus. $Esolver$ uses an enumerate method with many optimization techniques.
	
	
	\item $Eusolver$  \todo{add refer}, the winner of the PBE track in SyGuS-Comp 2016 \todo{add refer}. $Eusolver$ uses an optimized enumeration strategy which makes it especially efficient on synthesizing if-statements.

	\item $CVC4$ \todo{add refer}, the winner of the PBE-string track in SyGuS-Comp from 2017 to 2019 \todo{add refer} . $CVC4$ synthesizes programs by an SMT solver and an algorithm named counterexample-guided quantifier instantiation .

\end{itemize}

\subsection{Compared Approach}

We implemented $CEGIS$ and $RANDOM$ models to compare the generalizability for PBE tasks.

\begin{itemize}
	\item \textbf{$CEGIS.$} We initially provide an empty input for each solver. The result given is then checked with SMT solver. If the result fails, we add the counterexample from the SMT solver to our input and repeat the procedure. Otherwise, the PBE solver arrives at a correct solution and we record the time consumption and examples needed in the final input. This framework is to imitate the procedure of interactive synthesis. $CEGIS$ are intended to make all of the example provided useful for synthesize.
	
	
	\item \textbf{$RANDOM.$} An enough long list of examples with input values in given range are genarated randomly at first. Then we check how many examples random generated are capable with each solver to get correct solution with dichotomy. Such method is to simulate the random input environment and a determinate list of examples are useful to exclude the influence of different random seeds when comparing each solver. When a solver fail to give correct solution with the total list, we just assume the solver fail on this PBE task. This framework is closer to the motivation of \mainname, which attributes to the requirements of some systems for random inputs, though $RANDOM$ are naturally less efficient than $CEGIS$ since much of the random examples are redundant and futile.
\end{itemize}

When it comes to the comparison about efficiency, we removed the restrictions for PBE environment and simply provided each solver with the specification of the tasks. \mainname and Eusolver are inherently $CEGIS$ solver while DRYADSYNTH and cvc4 are not. Their function are based on domain-specific konwledge. This research question solely cares the efficiency of each solver in the conventional scenario rather than generalizability. 

All the following experiments set the time limit as 120 seconds and example number limit at $50000$ . Random generated input are range from $-50$ to $50$. For each test on a specific benchmark, we have run the testing solver $5$ times for an average result.


\subsection{Exp1: Comparison of generalizability(RQ1)}

\noindent \textbf{Procedure. } We respectively test the $CEGIS$ and $RANDOM$ models for PBE tasks. Due to the differences between the each solvers, the experiment settings are slightly different. $Eusolver$ and \mainname are inherently $CEGIS$ so we solely invoke them with the primitive specification for $CEGIS$ model. The other solver are not $CEGIS$ so we reply on external runner to generate counterexample for them interactievly. The $RANDOM$ model are settled as aforementioned.

\noindent \textbf{Results. } The results are showed in\ref{tab-exp1-and-exp2} drawn as Figure \ref{fig-exp1-and-exp2}. \mainname has overall satisfactory generalizability on our benchmarks. The model of $CEGIS$ and $RANDOM$ only yields slight difference in trend. $Esolver$ fails to solve enough benchmark for reasonable comparison.  $CVC4$ is not able to behave generalizability on even the simplest tasks. So we focus on the comparison with  $Eusolver$ .
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\begin{table}[ht]
	\scriptsize
	\renewcommand\arraystretch{1.5}% Please add the following required packages to your document preamble:
	% \usepackage{multirow}
		\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
			\hline
			\multirow{3}{*}{Solver} & \multicolumn{8}{c|}{$PBE$}                                                                                                                                                     & \multicolumn{3}{c|}{\multirow{2}{*}{Original}}                              \\ \cline{2-9}
			& \multicolumn{4}{c|}{$CEGIS$}                                                          & \multicolumn{4}{c|}{$RANDOM$}                                                          & \multicolumn{3}{c|}{}                                                       \\ \cline{2-12} 
			& solved & \begin{tabular}[c]{@{}c@{}}commonly\\ solved\end{tabular} & time   & example & solved & \begin{tabular}[c]{@{}c@{}}commonly\\ solved\end{tabular} & time    & example & solved & \begin{tabular}[c]{@{}c@{}}commonly\\ solved\end{tabular} & time   \\ \hline
			$PolyGen$               & 92     & 92                                                        & 1.0x   & 1.0x    & 88     & 88                                                        & 1.0x    & 1.0x    & 92     & 92                                                        & 1.0x   \\ \hline
			$Eusolver$              & 67     & 64                                                        & 5.745x & 2.014x  & 64     & 59                                                        & 17.085x & 2.018x  & 67     & 64                                                        & 5.745x \\ \hline
			$Esolver$               & 9      & 9                                                         & 3.442x & 0.842x  & 9      & 9                                                         & 47.769x & 1.251x  & 9      & 9                                                         & 5.175x \\ \hline
			$CVC4$                  &        &                                                           &        &         &        &                                                           &         &         & 100    & 92                                                        & 0.085x \\ \hline
		\end{tabular}
	\caption{The results of Exp1 and exp2. For each solver compared with \mainname, we only care about the benchmarks that both \mainname and that solver have sucessfully solved. For these commonly solved benchmarks, we present the average time consumption and examples needed of the baseline solver compared to \mainname. As $CVC4$ failed to work in the PBE environmentm, we do only present the part of Exp2}
	\label{tab-exp1-and-exp2}
	\end{table}

\begin{itemize}
	
	\item \mainname. \mainname solves almost all the benchmarks. In $CEGIS$ framework, \mainname solved most benchmarks within $100$ examples, while in $RANDOM$ framework, \mainname solved most of them within $1000$ examples. Synthesis process is finished in 100 seconds which guarantees acceptable efficiency and generalizability. 

	\item $Eusolver.$  $Eusolver$ possesses relatively considerable generalizability and is the best behaved base-line solver for PBE since it is based on $CEGIS$ inherently. $Eusolver$ solves over 60 benchmarks in all. However, \mainname outperforms $Eusolver$ both in time and examples to a great extent. $Eusolver$ solved highly visible less benchmark than \mainname.
	
	\item $Esolver.$ $Esolver $ are thought to have best generalizability in the nature of enumerative strategy. However, exponent time complexity makes it fail to solve most benchmarks since the input arguments are of a great numder and some solutions are too large for $Esolver$. $Esolver$ is able to solve 10 benchmark of 100 in all with very short solution.  $Esolver $ shows best generalizability in these simple cases as expected. Since $Esolver$ has similar behavior for $PBE$ and synthesis by specification, we only presents the result in Exp2.
	

	
	\item $CVC4.$ $CVC4$ are able to generate solutions for our benchmark with PBE. However, the solution generated are always overfitting to the each examples that we may conclude $CVC4$ loses almost all the generalizability. The expression generated by $CVC4$ is too large for z3 to verify, so we instead verify by examples, that is to calculate the expression on a reasonable set of random input and is enough to show the failure. On the case $Max_3$ which required the biggest of all three input arguments, the solution generated by $CVC4$ is merely to fit all the input points with a branch for each points and the accuracy under verify-by-examples is always less than $4\%$ from the beginning of CEGIS up to $100$ examples and the accuracy does not seem to grow. On the simpler case where we only have one input argument $x, 0 \leq x\le 100$  and the solution is $x+1$ , $CVC4$ yields the correct solution only after $100$ examples in $CEGIS$, which proves that $CVC4$ nearly sacrifices all of its generalizability for domain-specific ability.
	
	
\end{itemize}
\begin{figure}[ht]
	\centering  
	\vspace{-0.35cm} 
	\subfigtopskip=2pt 
	\subfigbottomskip=2pt
	\subfigure[\tiny Results of Exp 1 for CEGIS of example]{
		\label{exp1-cegis-example}
		\includegraphics[width=0.32\linewidth]{pics/exp1_cegis_example.png}}
	\subfigure[\tiny Results of Exp 1 for CEGIS of time]{
		\label{exp1-cegis-time}
		\includegraphics[width=0.32\linewidth]{pics/exp1_cegis_time.png}}
	\subfigure[\tiny Results of Exp 1 for RANDOM of example]{
		\label{exp1-random-example}
		\includegraphics[width=0.32\linewidth]{pics/exp1_random_example.png}}
	\subfigure[\tiny Results of Exp 1 for RANDOM of time]{
		\label{exp1-random-time}
		\includegraphics[width=0.32\linewidth]{pics/exp1_random_time.png}}
	\caption{The results of exp1 and exp2. For each approach, we sort its solved benchmarks in the increasing
		order of the time cost or number of examples needed. Scatter are added for every 10 benchmarks.}
	\label{fig-exp1-and-exp2}
\end{figure}

\subsection{Exp2: Comparison of efficiency(RQ2)}

\noindent \textbf{Procedure. } We managed to exploit the best performance of each solver without PBE constrains. For $CVC4$ specifically, the syntax limit are removed while the other solvers remains syntax-guilded.

\noindent \textbf{Results. }The results are drawn as Figure \ref{cegis}.  \mainname has a resonable time consumption for the benchmarks.

\begin{itemize}
	
	\item \mainname. \mainname has reasonable performance when compared out of PBE. Some exisiting solver has better efficiency, but on the other hand, they are short of generalizability. 
	
	\item $Esolver.$ $Esolver$ is of poor efficiency for the benchmark due to its pure enumerative strategy and such efficiency excludes the possibility to utilize its generalizability for real demand.
	
	\item $Eusolver.$ Eusolver is slowers than \mainname on most hard cases and is able to solve less cases than \mainname in the time limit. Thus, \mainname has better performance than $Eusolver$ in whole.
	
	\item $CVC4$. $CVC4$  is quite efficient when given specification for synthesis. That is because they apply a great amount of sophisticated domain knowledge and achieve great performancee on CLIA. Though they give up their  generalizability in exchange.
	
\end{itemize}

In conclusion, \mainname is capable to solve the benchmarks satisfactorily. None of the existing solver is able to surpass \mainname both in efficiency and generalizability. And \mainname is the only solver capable to solve some PBE problems according to our knowledge.

==> sections/Generalization.tex <==
%!TEX root = ../CLIA.tex
\section{Generalization Model} \label{section:model}
In this section, we shall introduce the generalization model considered in our paper.

\subsection{Definition}
To formally measure the generalizability of a PBE synthesizer, a generation model for all possible PBE tasks is necessary. In this paper, we model the PBE task generated from some application scenario $(\mathbb P, \mathbb I, \mathbb O)$ as a random variable relying on a distribution $D_p$ over the program domain $\mathbb P$, which  describes the probability for each program to be used in this application. 

Given distribution $D_p$, we assume a PBE task with $n$ examples is generated in three steps:
\begin{enumerate}
	\item A program $p$ is randomly drawn from the program domain $\mathbb P$ according to $D_p$.
	\item $n$ inputs $I_1, \dots, I_n$ are uniformly and independently drawn from the input domain $\mathbb I$.
	\item PBE task $(I_1, \sem{p}(I_1)), \dots, (I_n, \sem{p}(I_n))$ is returned as the result of the generation.
\end{enumerate}

In the rest of this paper, we use $\mathcal G[D_p]$ to denote the model derived from distribution $D_p$.

Given the generation model of PBE tasks, the generalizability of a solver can be naturally defined as the minimal number of examples required by the solver to achieve a limited error rate. 

\begin{definition}[Generalizability] Given a generation model $\mathcal G[D_p]$ and a PBE solver $\mathcal S$, the generalizability $\text{gen}[D_p, \mathcal S]: [0, 1] \rightarrow \mathbb Z^+$ is a function where $\forall \epsilon \in (0, 1]$, $\text{gen}[D_p, \mathcal S](\epsilon)$ is defined as the smallest integer such that:
	$$\forall n \geq \text{gen}[D_p, \mathcal S](\epsilon), \Pr_{p \sim D_p, I_1, \dots, I_n \sim U(\mathbb I)} \left[ \mathcal S\big((I_1, \sem{p}(I_1)), \dots, (I_n, \sem{p}(I_n)) \big) \not \sim_{\mathbb I} p \right] \leq \epsilon
	$$
where $U(\mathbb I)$ denotes the uniform distribution over the input domain $\mathbb I$.
\end{definition}

Though the definition of the generalizability is natural, it has two shortages for analyzing PBE solvers: (1) Precisely modeling the distribution $D_p$ itself is a hard task, and thus makes the calculation of the generalizability difficult; (2) The distribution over programs varies frequently as the context (such as a natural language description) changes, and thus the concrete value of the generalization error cannot comprehensively reflect the generalizability of a PBE solver.

Therefore, we further introduce the concept of \textit{generalization function}, which eliminates the usage of $D_p$ by assuming the target program is fixed.

\begin{definition}[Generalization Function] Given a PBE solver $\mathcal S$, the generalization function $\text{gen}[\mathcal S]: \mathbb P \times [0, 1] \rightarrow \mathbb Z^+$ is a function defined where $\forall p \in \mathbb P, \forall \epsilon \in (0, 1]$, $\text{gen}[\mathcal S](p, \epsilon)$ is defined as the smallest integer such that 
	$$
	\forall n \geq \text{gen}[\mathcal S](p, \epsilon),  \Pr_{I_1, \dots, I_n \sim U(\mathbb I)} \left[ \mathcal S\big((I_1, \sem{p}(I_1)), \dots, (I_n, \sem{p}(I_n)) \big) \not \sim_{\mathbb I} p \right] \leq \epsilon 
	$$
\end{definition}

The last concept we shall introduce in this section is named as \textit{distinguishable factor}, which is defined as the probability for a random input to distinguish two distinguishable programs. 
\begin{definition}[Distinguishable Factor] Given a program domain $\mathbb P$ and a input domain $\mathbb I$, distinguishable factor $\alpha_{\mathbb P, \mathbb I}$ is defined as the maximal possible number such that:
	$$
	\forall p_1, p_2 \in \mathbb P, \left(p_1 \not \sim_{\mathbb I} p_2 \implies \Pr_{I \sim U(\mathbb I)}\left[\sem{p_1}(I) \neq \sem{p_2}(I)  \right] \geq \alpha_{\mathbb P, \mathbb I}\right)
	$$
\end{definition}
%In our generalization model, the inputs are assumed to be independently selected among the whole input domain. Therefore, if a solver is trapped into a plausible program of which the semantics is extremely closed to the target one, it can be hard for the solver to be aware of this mistake unless a large number of programs are provided. 
The distinguishable factor actually provide a lower bound on the probability for the solver to exclude incorrect programs: For each incorrect program $p_w$ and a randomly selected example $e$, the probability for $p_w$ to violate $e$ is at least $\alpha_{\mathbb I, \mathbb O}$. For any program domain $\mathbb P$ and input domain $\mathbb I$, $|\mathbb I|^{-1}$ is a trivial lower bound of $\alpha_{\mathbb I, \mathbb O}$, as two distinguishable programs must differ on at least one input. Moreover, for some specific domains, the value of $\alpha_{\mathbb P, \mathbb O}$ can be much more larger, and can even be close to $1$, as shown in Lemma \ref{lemma:alpha}.

\begin{lemma} \label{lemma:alpha} The distinuishable factor for the domain $(\mathbb P^L_{n,m}, \mathbb I^L_{n,m})$ of bounded linear integer expressions with $n$ parameters is at least $1 - \frac{1}{m}$, where:
	$$
	\mathbb P^L_{n,m} = \left \{\lambda \left(x_1, \dots, x_n\right). \left(a_0 + \sum_{i=1}^n a_i x_i \right) \bigg| a_0, \dots, a_n \in \{0, 1, \dots, m\}\right\}\ \ \ \mathbb I ^L_{n,m} = \{0, 1, \dots, m \}^n
	$$
\end{lemma}
\begin{proof} \todo{complete it}. Bertrand's postulate (there is always a prime number in $[n,2n]$). Module $p$.
\end{proof}

In the rest of this paper, we implicitly assume the existence of a constant $\alpha > 0$ that is a lower bound for all referred $\alpha_{\mathbb P, \mathbb I}$. Under such an assumption, a universal generalization bound for all PBE solver and all domains can be established.

\begin{theorem} For any domain $(\mathbb P, \mathbb I, \mathbb O)$ and any PBE solver $\mathcal S$:
	$$\forall p \in \mathbb P, \forall \epsilon \in (0, 1], \left(\text{gen}[\mathcal S](p, \epsilon) \leq \ln_{1/(1- \alpha)} |\mathbb P| + \ln_{1/(1 - \alpha)} \left(\frac{1}{\epsilon}\right)\right)
	$$
which implies that $\text{gen}[\mathcal S](p, \epsilon) = O(\ln |\mathbb P|) + O\left(\ln (1/\epsilon)\right)$.
\end{theorem}

\subsection{Polynomial-Size  Generalizability}
\begin{definition}[Polynomial-Size Generalizability] \label{def:poly-gen} A PBE solver $\mathcal S$ has \textit{polynomial-size genralizability} if there exists a polynomial $g(x,y)$ such that:
	$$\forall p \in \mathbb P, \forall \epsilon (0, 1], \text{gen}[\mathcal S](p, \epsilon) \leq g(\text{size}(p), \ln(1 / \epsilon))$$
\end{definition}

\subsection{Generalizability of STUN}
Similiar to Definition \ref{def:poly-gen}, we define polynomial-size generalizability for term solvers and unifiers. 

\begin{definition}[Term Solver with Polynomial-Size Generalizability] A term solver $\mathcal T$ has \textit{polynomial-size generalizability} if there exists a pollynomial $g(x, y)$ such that $\forall p \in (\mathbb P_t, \mathbb P_c), \forall \epsilon \in [0, 1), \forall n \geq g(\text{size}(p), \ln(1 / \epsilon))$:
	$$\Pr_{I_1, \dots, I_n \sim U(\mathbb I)} \left[\exists I \in \mathbb I, \forall p' \in \mathcal T\big((I_1, \sem{p}(I_1)), \dots, (I_n, \sem{p}(I_n)) \big), \big(\sem{p}(I) \neq \sem{p'}(I)\big)\right] \leq \epsilon$$
\end{definition}

\begin{definition}[Unifier with Polynomial-Size Generalizability] A unifier $\mathcal U$ has 
	\textit{polynomial-size generalizability} if there exists a polynomial $g(x, y)$ such that $\forall P \subseteq \mathbb P_t, \forall p \in (P, \mathbb P_c), \forall \epsilon \in [0,1), \forall n \geq g(\text{size}(p), \ln(1/\epsilon))$:
	$$ \Pr_{I_1, \dots, I_n \sim U(\mathbb I)} \left[\mathcal U(P)\big((I_1, \sem{p}(I_1)), \dots, (I_n, \sem{p}(I_n)) \big) \not \sim_{\mathbb I} p\right] \leq \epsilon
	$$
\end{definition}

\begin{definition}[Size Preserving] \label{def:size-preserve}A PBE solver $\mathcal S$ is \textit{size-preserving} if there exists a polynomial $s(x, y)$ such that for any $p \in (\mathbb P_t, \mathbb P_c)$, for any $\epsilon \in [0, 1)$, and for any input sequence $I_1, \dots, I_n \in \mathbb I$:
$$ \Pr\left[\text{size}\left( \mathcal S\big((I_1, \sem{p}(I_1)), \dots, (I_n, \sem{p}(I_n))\big)\right) > s\left(\text{size}(p),  \ln \left(\frac{1}{\epsilon}\right)\right)\right] \leq \epsilon $$
\end{definition}

\begin{definition}[Size Preserving] \label{def:size-preserve}A term solver $\mathcal T$ is \textit{size-preserving} if there exists a polynomial $s(x, y)$ such that for any $p \in (\mathbb P_t, \mathbb P_c)$, for any $\epsilon \in [0, 1)$, and for any input sequence $I_1, \dots, I_n \in \mathbb I$:
	$$ \Pr\left[\text{sizesum}\left( \mathcal T\big((I_1, \sem{p}(I_1)), \dots, (I_n, \sem{p}(I_n))\big)\right) > s\left(\text{size}(p),  \ln \left(\frac{1}{\epsilon}\right)\right)\right] \leq \epsilon $$
where $\text{sizesum}(P)$ is defined as the total size of programs in $P$, i.e., $\sum_{p' \in P} \text{size}(p')$.
\end{definition}

\begin{theorem} \label{theorem:gen-stun}Suppose $\mathcal T$ and $\mathcal U$ be a term solver and a unifier. Let $\mathcal T'$ and $\mathcal U'$ be a term solver and a unifier constructed as following:
	$$
	\mathcal T'(e_1, \dots, e_n) = \mathcal T\left(e_1, \dots, e_{\lfloor \frac{n}{2}\rfloor}\right)\ \ \ \ \mathcal U'(P)(e_1, \dots, e_n) = \mathcal U(P)\left(e_{\lfloor \frac{n}{2} \rfloor + 1}, \dots, e_{n}\right)
	$$
Then the STUN solver induced by $\mathcal T'$ and $\mathcal U'$ has polynomial-size generalizability on $\mathbb P=(\mathbb P_t, \mathbb P_c)$ if: 
\begin{itemize}
	\item Program domain $\mathbb P$ is if-closed.
	\item Term solver $\mathcal T$ is size-perserving on $\mathbb P$.
	\item  Both of $\mathcal T$ and $\mathcal U$ has polynomial-size generalizability on $\mathbb P$.
\end{itemize}
\end{theorem}

\subsection{Generalizability of \textit{Eusolver}} \label{section:gen-eu}
\begin{lemma} The term solver in \textit{Eusolver} (Algorithm \ref{alg:eusolver-term}) has polynomial-size generalizability.
\end{lemma}
\begin{lemma} The unifier in \textit{Eusolver} {Algorithm \ref{alg:eusolver-uni}} does not have polynomial-size generalizability.
\end{lemma}
\begin{proof} For any integer $n > 0$, we construct a unification task $\texttt{maxn} = (P^n, \mathbb P_c^n, p_n)$ as following:
	$$
	P^n = \{x_1, \dots, x_n\}\ \ \ \mathbb P_c^n = \{x_i\leq x_j\ |\ 1 \leq i,j \leq n\}\ \ \ \sem{p_n}(x_1, \dots, x_n) = \max(x_1, \dots, x_n)
	$$
In domain $(P^n, \mathbb P_c^n)$, $p_n$ can be implemented as a program of size $O(n^2)$:
\begin{align*}
p_n = &\ \texttt{if}\ ((x_2 \leq x_1)\ \texttt{and}\ (x_3 \leq x_1)\ \texttt{and}\ \dots\ \texttt{and}\ (x_n \leq x_1))\ \texttt{then}\ x_1 \\
& \ \texttt{else if}\ ((x_3 \leq x_2)\ \texttt{and}\ (x_4 \leq x_2)\ \texttt{and}\ \dots\ \texttt{and}\ (x_n \leq x_2))\ \texttt{then}\ x_2 \\
&\ \dots \\
&\ \texttt{else if}\ (x_{n-1} \leq x_n)\ \texttt{then}\ x_{n-1}\ \texttt{else}\ x_n
\end{align*}

When synthesizing \texttt{if} conditions, the unifier in \textit{Eusolver} only considers boolean expressions in $\mathbb P_c^n$. Such a limitation can make the size of the resulting program exponentially larger:

\textbf{Claim: } For any program $p^*$ that only uses boolean expressions in $\mathbb P_c^n$ as \texttt{if} conditions:
\begin{center}
 $p^* \sim_{\mathbb I} p_n \implies$ $p^*$ uses \texttt{if-then-else} operator at least $\left(2^{n-1} - 1\right)$ times. 
\end{center}

\todo{the proof of this claim can be found in the appendix.}

According to Algorithm \ref{alg:eusolver-uni}, the unifier will return immediately when there is a program in $\mathbb P_t$ covering all remaining examples. Therefore, there must be at least two examples while synthesizing each \texttt{if} condition.  

Combining with the previous claim, we know that: to synthesize a correct program for task \texttt{maxn}, the unifier in \textit{Eusolver} requires at least $2^{n-1}$ examples. Therefore, we obtain that the unifer does not have polynomial-size generalizability.
\end{proof}

The same construction works also for proving the generalizability of \textit{Eusolver}.
\begin{theorem} \textit{Eusolver} does not have polynomial-size generalizability.
\end{theorem}

==> sections/Generalization2.tex <==
%!TEX root = ../CLIA.tex
\section{Generalization Model} \label{section:model}
In this section, we introduce the abstracted generalization model used in this paper. At the beginning, we introduce some necessary preliminaries on programming-by-example in Section \ref{section:pre-pbe}. Then, we define a natural and concrete model of the generalizability in Section \ref{section:concrete-gen}, and then abstracted it using assumptions in Section \ref{section:abstracted-gen}. After that, in Section \ref{section:gen-case}, we establish a case study to show how our abstracted model compare the generalizability of two PBE solvers. At last, motivated by the polynomial-time class $\mathsf P$, we introduce a coarse class of solvers with acceptable generalizability, namely \textit{polynomial-size generalizability}, in Section \ref{section:gen-class}.

\subsection{Preliminaries: Programming by Example}\label{section:pre-pbe}
\begin{definition}[Semantics Function] Given a program domain $\mathbb P$, an input domain $\mathbb I$, and an output domain $\mathbb O$, an oracle function $\sem{.}_{\mathbb P, \mathbb I, \mathbb O}: \mathbb P \rightarrow \mathbb I \rightarrow \mathbb O$ associates a program $p$ and an input $I$ with an output, denoted as $\sem{p}_{\mathbb P, \mathbb I, \mathbb O}(I)$. 
\end{definition}

In this paper, we implicitly assume the existence of a universal semantics function $\sem{.}$ for any program, input and output domains. 

Besides, we assume that domain $\mathbb P$ is defined by a regular tree grammar $G = \langle N, \Sigma, s_0, R \rangle$, where:
\begin{itemize}
	\item $N$ is a set of non-terminal symbols.
	\item $\Sigma$ is a set of terminal symbols that is disjoint from $N$. In $\Sigma$, each symbol $f$ is associated with an arity $k_f$. Specially, the arity is defined as $0$ for constants and input variables.
	\item $s_0 \in N$ represents the start symbol.
	\item $R$ is a set of production rules. All rules in $R$ are in the form of $(s, f (x_1, \dots, x_{k_f}))$ where $s, x_1, \dots, x_{k_f} \in N, f \in \Sigma$.  Rule $(s, f (x_1, \dots, x_{k_f}))$ represents that nonterminal symbol $s$ can be expanded to a function using operator $f$ and taking symbols $x_1, \dots, x_{k_f}$ as parameters. 
\end{itemize}
A program $p$ is inside regular tree grammar $G$ if there is no non-terminal symbol remaining in $p$ and $p$ can be produced by the start symbol $s_0$ directly or indirectly.

\textit{Programming by Example (PBE)} is a subproblem of program synthesis where the solver is required to learn a program from a set of given input-output examples.

\begin{definition}[Programming by Example] \label{def:pbe}Given a program domain $\mathbb P$, an input domain $\mathbb I$ and an output domain $\mathbb O$, a PBE task $T \in (\mathbb I \times \mathbb O)^*$ is a sequence of input-output examples.
	
	Correspondingly, a PBE solver $\mathcal S: (\mathbb I \times \mathbb O)^* \rightarrow {\{\top\} \cup \mathbb P}$ is a function satisfying the following two conditions for any PBE task $T \in (\mathbb I \times \mathbb O)^*$:
	\begin{itemize}
		\item (Soundness) If $\mathcal S(T)$ is a program, $\mathcal S(T)$ must be consistent with all examples in $T$:
		$$\mathcal {S}(T) \in \mathbb P \implies \forall (I, O) \in T, \sem{\mathcal {S}(T)}(I) = O$$
		\item (Completeness) If $\mathcal S(T) = \top$, all programs in $\mathbb P$ must violate at least one example in $T$:
		$$\mathcal {S}(T) = \top \iff \forall p \in \mathbb P, \exists (I, O) \in T, \sem{p}(I) \neq O$$
	\end{itemize}
\end{definition}



\subsection{Generalizability} \label{section:concrete-gen}
\textit{Generalizability} is a property defined for PBE solvers.  Intuitively, it represents the ability for a solver to learn the \textit{full} functionality of a hidden target program from a few number of examples. According to Definition \ref{def:pbe}, PBE tasks on input domain $\mathbb I$ cannot distinguish two programs if their semantics perform the same on all inputs in $\mathbb I$. Therefore, the best a PBE solver can do is to synthesize a program that is \textit{semantically equivalent} to the target program on the entire input domain. 

\begin{definition}[Semantically Equivalence] Two programs $p_1$ and $p_2$ are semantically equivalence on input domain $\mathbb I$, written as $p_1 \sim_{\mathbb I} p_2$ if and only if $\forall I \in \mathbb I, \sem{p_1}(I) = \sem{p_2}(I)$.
\end{definition}

In this paper, we model the PBE task in an application scenario $(\mathbb P, \mathbb I, \mathbb O)$ as a random variable relying on two distributions $D_p$ and $D_I$, describing the probability for each program to be taken as the target, and the probability for each input to be provided as an examples respectively.

Given distributions $D_p$, $D_I$, we assume a PBE task with $n$ examples is generated in three steps: 
\begin{enumerate}
	\item A program $p$ is randomly drawn from the program domain $\mathbb P$ according to $D_p$.
	\item $n$ inputs $I_1, \dots, I_n$ are independently drawn from the input domain $\mathbb I$ according to $D_I$.
	\item PBE task $(I_1, \sem{p}(I_1)), \dots, (I_n, \sem{p}(I_n))$ is returned as the result of the generation.
\end{enumerate}

With the generation model of PBE tasks, we define the generalizability as the minimal number of examples such that given a random PBE task, with a high probability, the solver is guaranteed to synthesize a program semantically equivalent to the target one.

\begin{definition}[Generalizability] \label{def:gen} Given a generation model $(D_p, D_I)$ and a PBE solver $\mathcal S$, the generalizability $\text{gen}[D_p, D_I, \mathcal S]: [0, 1] \rightarrow \mathbb Z^+$ is a function where $\forall \epsilon \in (0, 1)$, $\text{gen}[D_p, D_I, \mathcal S](\epsilon)$ is defined as the smallest integer such that:
	$$\forall n \geq \text{gen}[D_p, D_I, \mathcal S](\epsilon), \Pr_{p \sim D_p, I_1, \dots, I_n \sim D_I} \left[ \mathcal S\big((I_1, \sem{p}(I_1)), \dots, (I_n, \sem{p}(I_n)) \big) \not \sim_{\mathbb I} p \right] \leq \epsilon
	$$
\end{definition}

When $(D_p, D_I)$ is given, the following solver $S_{\text{opt}}[D_p, D_I]$ achieves the optimal generalizability:
$$ \mathcal S_{\text{opt}}[D_p, D_I](T) \coloneqq \arg\max_p D_p(p)\ \ s.t.\ \forall (I, O) \in T, \sem{p}(I) = O 
$$
Where $D_p(p)$ represents the probability of $p$ in distribution $D_p$. Specially, when there is no program that is consistent with all examples, $\mathcal S_{\text{opt}}[D_p, D_I](T)$ is defined as $\top$.

\begin{theorem} For any PBE solver $\mathcal S$, for any model $(D_p, D_I)$ and $\epsilon \in (0, 1)$,
	$$\text{gen}[D_p,D_I, \mathcal S_{\text{opt}}[D_p, D_I]](\epsilon) \leq \text{gen}[D_p, D_I, \mathcal S](\epsilon)
	$$
\end{theorem}

\subsection{Abstracted Generalizability} \label{section:abstracted-gen}
Though Definition \ref{def:gen} provides a natural definition for the generalizability, its usage is rather limited, as it requires distributions $D_p, D_I$ and domains $\mathbb P, \mathbb I, \mathbb O$ to be explicitly given. When designing a PBE solver, we would always expecet the solver to be generally efficient for different domains, or at least, for different tasks in the same domain. However, as these distributions and domains vary frequently from tasks to tasks, the current definition of generalizability is usually unavailable when we want to evaluate the overall efficiency of a solver. 

To improve this point, we abstract the distributions and domains with assumptions, and thus make the generalizability estimable even when concrete values of $D_p, D_I, \mathbb P, \mathbb I, \mathbb O$ are unavailable.

\subsubsection{Abstracting the program distribution} To reduce the reliance on the program distribution $D_p$, we use the principle of \textit{Ocam's Razor}: We assume that a realistic application scenario always prefer simpler programs than complex ones. Therefore, distribution $D_p$ should be biased to smaller programs. To formalize this assumption, we start by defining the size of a program.

\begin{definition} Given a regular tree grammar $\langle N, \Sigma, s_0, R \rangle$, the size $\text{size}_0(p)$ of program $p$ is defined as the number of production rules used to produce program $p$ from the start symbol $s_0$, i.e.:
	$$\text{size}_0(p)\coloneqq\left\{
	\begin{array}{lcl}
		1 &  & p \in N \\
		1 + \sum_{1}^{k_f} \text{size}_0(p_i) & & p = f(p_1, \dots, p_{k_f})
	\end{array}
	\right.
	$$
	The normalized size $\text{size}(p)$ of a program $p$ is defined as $\text{size}(p) \coloneqq \left(\ln |R|\right)\text{size}_0(p)$.
\end{definition}
The advantage of introducing \textit{normalized size} is that for any program $p$, the normalized size of $p$ provides an upper bound on the number of programs no larger than $p$.

\begin{lemma} \label{lemma:size}For any program domain $\mathbb P$, $\forall p \in \mathbb P$, 
	$ \left|\left\{p' \in \mathbb P\  |\ \text{size}(p') \leq \text{size}(p)\right\} \right| \leq \exp\left(\text{size}(p)\right)
	$.
\end{lemma} 

\begin{assumption}[Ocam's Razor] \label{ass:1} For a random program $p \sim D_p$, the expected number of programs no larger than $p$ is asymptotically smaller than the size of the program space in logarithmic unit:
	$$
	\ln \left( \mathbb E_{p \sim D_p} \big [\left|\left\{p'\ |\ \text{size}(p') \leq \text{size}(p)\right\}\right|\big] \right) = o\left(\ln |\mathbb P|\right)
	$$
	Specially, when $\mathbb P$ is an infinite program domain, we assume the expectation is bounded:
	$$
	\ln \left( \mathbb E_{p \sim D_p} \big [\left|\left\{p'\ |\ \text{size}(p') \leq \text{size}(p)\right\}\right|\big] \right) < + \infty
	$$
\end{assumption}

To remove the reliance on $D_p$ from the generalizability, we introduce the concept of \textit{generalization function},  which eliminates the usage of $D_p$ by assuming the target program is fixed.

\begin{definition}[Generalization Function] Given an input distribution $D_I$ and a PBE solver $\mathcal S$, the generalization function $\text{gen}[D_I,\mathcal S]: \mathbb P \times [0, 1] \rightarrow \mathbb Z^+$ is a function where $\forall p \in \mathbb P, \forall \epsilon \in (0, 1)$, $\text{gen}[D_I,\mathcal S](p, \epsilon)$ is defined as the smallest integer such that 
	$$
	\forall n \geq \text{gen}[D_I, \mathcal S](p, \epsilon),  \Pr_{I_1, \dots, I_n \sim D_I} \left[ \mathcal S\big((I_1, \sem{p}(I_1)), \dots, (I_n, \sem{p}(I_n)) \big) \not \sim_{\mathbb I} p \right] \leq \epsilon 
	$$
\end{definition}

\subsubsection{Abstracting the semantics.} To calculate the generalizability, we have to model the semantics of a program on a random example, and thus distribution $D_I$ and domains $\mathbb P, \mathbb I, \mathbb O$ are required. To improve this point, we observe that: In most cases, the semantics is used to calculate the probability for a random example to disprove some incorrect assertion on the semantics of the target program. 

\begin{example} \label{example:analysis}Suppose there are only two programs $\{p_1, p_2\} (p_1 \not \sim_{\mathbb I} p_2)$ in the program domain, and the solver $\mathcal S$ perfers $p_1$ when both programs are consistent with all examples. In the case that $p_2$ is selected as the target program, the generalizability of $\mathcal S$ is determined by the probability for a random example to disprove the incorrect assertion $\forall I, \left(\sem{p}(I) = \sem{p_1}(I)\right)$:
	$$
	\text{gen}[D_I, \mathcal S](p_2, \epsilon) = \left \lceil \ln \epsilon \bigg{/} \ln\left(1 - \Pr_{I \sim D_I}\left[\sem{p_2}(I) \neq \sem{p_1}(I)\right]\right) \right \rceil
	$$
	Therefore, to obtain an upper bound for the generalizability function, the only thing we need about the semantics is a lower bound for probability $\Pr_{I \sim D_I} \left[\sem{p_2}(I) \neq \sem{p_1}(I)\right]$. Suppose there is such a lower bound $\alpha \in (0, 1)$, then:
	
	$$
	\text{gen}[D_I, \mathcal S](p_2, \epsilon) \leq \left \lceil \frac{\ln \epsilon}{\ln \left(1 - \alpha\right)} \right \rceil \leq \left \lceil \frac{1}{\alpha} \ln \left(\frac{1}{\epsilon}\right) \right \rceil = O\left(\ln \left(\frac{1}{\epsilon}\right)\right)
	$$
\end{example}

Example \ref{example:analysis} shows that, to obtain an asymptotical upper bound for the generalizability, a probability lower bound can be used instead of concrete semantics. In this paper, to obtain an abstracted generalization model, we assume that there is a global lower bound $\alpha$ on the probability for a random input to disprove an incorrect assertion.

\begin{assumption} \label{ass:2} There exists a constant $\alpha \in (0, 1)$ such that for any logic formula $\varphi(I, p)$, where $I$ represents an input and $p$ represents the target program:
	$$
	\forall p \in \mathbb P, \left(\exists I \in \mathbb I, \left(\neg \varphi(I, p)\right) \implies \Pr_{I \sim D_I}\left[\neg \varphi(I, p)\right] \geq \alpha\right)
	$$
\end{assumption}
\todo{This assumption may be changed to distinguishable factor. Double check after the proof of the unifier is finished.}

When the size of the input domain $\mathbb I$ is limited, there is a trivial lower bound $\alpha = |\mathbb I|^{-1}$. Moreover, for some specific domains and formulas, there can be a much larger lower bound, as shown in Example \ref{example:bound}. However, in our abstracted model, we do not refer to these concrete values: We just treat the probabilities for all domains and all formulas equivalently as a constant $\alpha$, and tries to derive some general bound for the generalizability.

\begin{example} \label{example:bound}Let $\mathbb P^L_{n,m}, \mathbb I^{L}_{n,m}$ be the domain of linear integer expressions with $n$ parameters: 
	$$
	\mathbb P^L_{n,m} = \left \{\lambda \left(x_1, \dots, x_n\right). \left(a_0 + \sum_{i=1}^n a_i x_i \right) \bigg| a_0, \dots, a_n \in \{0, 1, \dots, m\}\right\}\ \ \ \mathbb I ^L_{n,m} = \{0, 1, \dots, m \}^n
	$$
	For any program $p' \in \mathbb P^L_{n,m}$,  the probability for disproving $\forall I, (\sem{p}(I) = \sem{p'}(I))$ is at least $1 - \frac{1}{m}$:
	$$
	\forall p \in \mathbb P^L_{n,m}, \left(\exists I \in \mathbb I, \left(\sem{p}(I) \neq \sem{p'}(I)\right) \implies \Pr_{I \sim D_I}\left[\sem{p}(I) \neq \sem{p'}(I)\right] \geq 1 - \frac{1}{m}\right)
	$$
\end{example}

In the remainder of this paper, we implicitly assume that both Assumption \ref{ass:1} and Assumption \ref{ass:2} are true. At this time, as distributions $D_p$ and $D_I$ have been abstracted, we shall omit their usages for simplicity. For example, generalization function $\text{gen}[D_I, \mathcal S](p, \epsilon)$ will be abbreviated to $\text{gen}[\mathcal S](p, \epsilon)$.

\subsection{Case Study: Random Program V.S. Minimal Program} \label{section:gen-case}
In this section, we establish a case study for two primitive PBE solvers $\mathcal S_{\text{rand}}$ and $\mathcal S_{\text{min}}$. For any PBE task $T$, let $P(T) \subseteq P$ be the set of programs that are consistent with all examples in $T$:
\begin{itemize}
	\item $\mathcal S_{\text{rand}}$ is the most basic synthesizer that has no guarantee on the quality of the result: It just uniformly returns a program from $P(T)$:
	$\forall p \in P(T), \Pr\left[\mathcal S_{\text{rand}}(T) = p\right] = |P(T)|^{-1}$.
	\item $\mathcal S_{\text{min}}$ regards a PBE task a an optimization problem, and always returns the smallest program in $P(T)$:
	$\mathcal S_{\text{min}}(T) \coloneqq \arg \min_{p \in P(T)} \text{size}(p)$.
\end{itemize}
Specially, when $P(T)$ is empty, both $\mathcal S_{\text{rand}}$ and $\mathcal S_{\text{min}}$ are defined as $\top$.

$\mathcal S_{\text{min}}$ is a commonly used strategy for improving the generalizability of PBE solvers, and its effectiveness has been studied by \citet{PD2007The}. In this subsection, we shall use our abstracted model to analyse the generalizability of $\mathcal S_{\text{min}}$ and $\mathcal S_{\text{rand}}$, and theoretically prove the advantage of $\mathcal S_{\text{min}}$ against $\mathcal S_{\text{rand}}$.

\begin{lemma} \label{lemma:min}$\forall p \in \mathbb P, \forall \epsilon \in (0, 1), \text{gen}[\mathcal S_{\text{min}}](p, \epsilon) \leq \frac{1}{\alpha} \left( \ln \left(\text{rank}(p)\right) + \ln\left(\frac{1}{\epsilon}\right)\right)$, where $\text{rank}(p)$ is defined as $|\{p' \in \mathbb P\ |\ \text{size}(p') \leq \text{size}(p)\}|$, i.e., the number of programs in $\mathbb P$ that are no larger than $p$. 
\end{lemma}
\begin{proof} In the worst case, there is no other program in $\mathbb P$ that is semantically equivalent to the target program $p$. At this time, according to the definition, $\mathcal S_{\text{min}}$ is guaranteed to return a correct program only when all incorrect programs in $S(p)$ are excluded by the PBE task, where $S(p) \subseteq \mathbb P$ is the set of programs that are no larger than $p$. Therefore, when $n$ examples are given:
	\begin{align*}
		n \geq \text{gen}[\mathcal S_{\text{min}}](p, \epsilon) \Longleftarrow&\ \Pr_{I_1, \dots, I_n \sim D_I}\left[\mathcal S_{\text{min}}\big((I_1, \sem{p}(I_1)), \dots, (I_n, \sem{p}(I_n))\big) \not \sim_{\mathbb I} p\right] \leq \epsilon \\
		\Longleftarrow &\ \Pr_{I_1, \dots, I_n \sim D_I}\left[\exists p' \in S(p), \big(p' \not \sim_{\mathbb I} p \wedge \forall i \in [n], \sem{p}(I) = \sem{p'}(I)\big)\right] \leq \epsilon \\
		\text{(Union bound)} \Longleftarrow &\ \sum_{p' \in S(p), p' \not \sim_{\mathbb I} p} \left(\Pr_{I_1, \dots, I_n \sim D_I}\big[ \forall i \in [n], \sem{p}(I) = \sem{p'}(I)\big] \right) \leq \epsilon \\
		\Longleftarrow &\ \sum_{p' \in S(p), p' \not \sim_{\mathbb I} p} \left(1 - \Pr_{I \sim D_I}\left[\sem{p}(I) \neq \sem{p'}(I)\right] \right)^n \leq \epsilon \\
		\text{(Assumption }\ref{ass:2}\text{)}  \Longleftarrow &\ |S(p)| (1 - \alpha) ^n \leq \epsilon \Longleftarrow n \geq \frac{1}{\alpha}\left(\ln \left(\text{rank}(p)\right) + \ln\left(\frac{1}{\epsilon}\right)\right)
	\end{align*}
\end{proof}

Lemma \ref{lemma:min} provides a general upper bound for $\text{gen}[\mathcal S_{\text{min}}]$. When we regard $\epsilon$ as a constant, the generalizability of $\mathcal S_{\text{min}}$ can be proven to be $o\left(\ln |\mathbb P|\right)$ by applying Assumption \ref{ass:1}:
\begin{align*}
	\text{gen}[D_p, D_I, \mathcal S_{\text{min}}](p, \epsilon) &\leq \mathbb E_{p \sim D_p} \left[\frac{1}{\alpha}\left(\ln (\text{rank}(p)) + \ln\left(\frac{1}{\epsilon}\right)\right)\right] \\ 
	& \leq \frac{1}{\alpha}\left(\mathbb E_{p \sim D_p}\left[\ln (\text{rank}(p))\right] + \ln \left(\frac{1}{\epsilon}\right)\right) = o(\ln |\mathbb P|)
\end{align*}
The second inequality is given by Jensen's Inequality, as $\ln(x)$ is a concave function.

\begin{lemma} \label{lemma:rand} There exists a domain $(\mathbb P, \mathbb I, \mathbb O)$ and distribution $D_I$ such that:
	$$ \forall p \in \mathbb P, \forall \epsilon \in (0, 0.5), \text{gen}[\mathcal S_{\text{rand}}]\left(p, \epsilon\right) >  \log_{2} \left((|\mathbb P| - 1) \frac{1 - 2 \epsilon}{2 \epsilon + 2}\right)$$
\end{lemma}
\begin{proof} We construct the following domain $(\mathbb P_{n}^{\oplus}, \mathbb I_{m}^{\oplus}, \mathbb O_{m}^{\oplus})$ using \textit{exclusive-OR} ($\oplus$): 
	$$
	\mathbb P_{m}^{\oplus} = \left\{x_1 \oplus \dots \oplus x_i | i \in [1,m] \right\}\ \ \ \mathbb I_{m}^{\oplus} = \{0, 1\}^{m}\ \ \ \mathbb O_{m}^{\oplus} = \{0, 1\}
	$$
	where $x_1, \dots, x_m$ are $m$ input paramteters. Moreover, we assume the input distribution $D_I$ is a uniform distribution over $\mathbb I_{m}^{\oplus}$.  
	
	For any target program $p$, let $p_1, \dots, p_{m-1}$ be the remaining programs in $\mathbb P_{m}^{\oplus}$. We define a series of binary random variables $\mathcal E_{i, n}$ where $\mathcal E_{i, n}$ takes $1$ only when program $p_i$ is consistent with $n$ random examples. The main effect of our construction is to guarantee the following two properties: (1) $\mathbb E[\mathcal E_{i,j}] = 2^{-n}$; (2) $\forall n>0$, $\mathcal E_{1, n}, \dots, \mathcal E_{m-1, n}$ are totally independent.  
	
	\begin{align*}
		n < \text{gen}[\mathcal S_{\text{rand}}](p, \epsilon) \Longleftarrow&\  \Pr_{I_1, \dots, I_n \sim D_I}\left[\mathcal S_{\text{rand}}\big((I_1, \sem{p}(I_1)), \dots, (I_n, \sem{p}(I_n))\big) \not \sim_{\mathbb I} p\right] > \epsilon \\ 
		\Longleftarrow&\  \Pr_{I_1, \dots, I_n \sim D_I}\left[\exists p' \in \mathbb P_{m}^{\oplus}, \big(p' \not \sim_{\mathbb I_{m}^{\oplus}} p \wedge \forall i \in [n], \sem{p}(I) = \sem{p'}(I) \big)\right] > 2\epsilon \\
		\Longleftarrow&\  \Pr\left[\sum_{i=1}^{m-1} \mathcal E_{i,n} \geq 1\right] > 2\epsilon 
	\end{align*}
	
	Define random variable $X_n$ as  $\sum_{i=1}^{m-1} \mathcal E_{i,n}$. Then $\mathbb E[X_n] = (m-1)2^{-n}, \mathbb E[X_n^2] = (m-1)2^{-n} + (m-1)(m-2)2^{-2n}$. By Paley-Zygmund inequality, when $\mathbb E[X] > 1$: 
	\begin{align*} \Pr[X_n > 1] \geq \left(1 - \frac{1}{\mathbb E[X_n]}\right)^2 \frac{\mathbb E[X_n]^2}{\mathbb E[X_n^2]} = \left(1 - \frac{1}{(m-1)2^{-n}} \right)^2 \frac{(m-1)2^{-n}}{1 + (m - 2)2^{-n}} > \left(1 - \frac{2}{Y}\right) \frac{Y}{1 + Y}  
	\end{align*}
	where $Y = \mathbb E[X_n] = (m - 1)2^{-n}$. 
	
	Combining the above two inequalities, the intended lower bound is obtained:
	
	$$\left(1 - \frac{2}{Y}\right)\frac{Y}{1 + Y} > 2 \epsilon \iff Y > \frac{2 \epsilon + 2}{1 - 2\epsilon} \iff n < \log_{2}\left((m - 1) \frac{1 - 2 \epsilon}{2 \epsilon + 2}\right)$$
\end{proof}

Lemma \ref{lemma:rand} provides a worst-case lower bound for the generalizability of $\mathcal S_{\text{rand}}$. When we regard $\epsilon$ as a constant, Lemma \ref{lemma:rand} implies that: whatever distribution $D_p$ is, there always exists a domain such that $\text{gen}[D_p, D_I, \mathcal S_{\text{rand}}](p, \epsilon) = \Omega(\ln |\mathbb P|)$, which is asymptotically larger than the genralizability of $\mathcal S_{\text{min}}$. Therefore, our abstracted generalization model can discover the advantage of $\mathcal S_{\text{min}}$ against $\mathcal S_{\text{rand}}$ on the generalizability.

\subsection{Polynomial-Size  Generalizability} \label{section:gen-class}
In the previous section, our abstracted generalization model successfully discovers the advantage of $\mathcal S_{\text{min}}$ on the generalizability. Analogy with the time complexity, the analysis in the previous section is like to calculate and compare the number of instruments executed by two different algorithms. However, to guided the design of PBE solvers, such a fine analysis may be unnecessary: Just like the polynomial-time class $\mathsf P$, a coarse class of solvers with acceptable generalizability is already enough. Therefore, motivated by class $\mathsf P$, in this section, we introduce the class of \textit{polynomial-size generalizability}, which (1) constraints less, (2) is more friendly for analysis, (3) could still distinguish the generalizability of $\mathcal S_{\text{min}}$ with $\mathcal S_{\text{rand}}$.

By Lemma \ref{lemma:min}, $\text{gen}[\mathcal S_{\text{min}}](p, \epsilon)$ is bounded by $O\left(\ln(\text{rank}(p))\right) + O\left(\ln (1 / \epsilon)\right)$. We derive the definition of polynomial-size generalizability by relaxing this upper bound twice:
\begin{itemize}
	\item As $\text{rank}(p)$ greatly relies on the program domain $\mathbb P$, we replace it with $\text{size}(p)$ by Lemma \ref{lemma:size}. On the one hand, such a replacement cuts off the reliance on the program domain $\mathbb P$, as $\text{size}(p)$ depends only on the syntax of program $p$. On the other hand, as the number of programs usually grows exponentially when the size increases, this replacement does not relax the bound much. 
	\item Motivated by class $\mathsf P$, in our class, we allow the generalizability of a PBE solver to be polynomially worse than $\mathcal S_{\text{min}}$, and thus leaves a great space for optimizing other aspects of solvers, such as the time complexity.
\end{itemize}

To summary, we define the class of \textit{polynomial-size generalizability} as the following.

\begin{definition}[Polynomial-Size Generalizability] \label{def:poly-gen} For a family of domains $\mathcal F = \{(\mathbb P, \mathbb I, \mathbb O)\}$, a PBE solver $\mathcal S$ has \textit{polynomial-size generalizability} on $\mathcal F$, abbreviated as $\mathcal S \in \mathsf {PSG}[\mathcal F]$, if there exists a polynomial $g(x,y)$ such that:
	$$\forall (\mathbb P, \mathbb I, \mathbb O) \in \mathcal F, \forall p \in \mathbb P, \forall \epsilon (0, 1), \text{gen}[\mathcal S](p, \epsilon) \leq g(\text{size}(p), \ln(1 / \epsilon))$$
\end{definition}

Specially, we abbreviate $\mathcal S \in \mathsf {PSG}[\mathcal F]$ to $\mathcal S \in \mathsf {PSG}$ when $\mathcal F$ contains all possible domains. By Lemma \ref{lemma:min}, we know that $\mathcal S_{\text{min}} \in \mathsf {PSG}$. Moreover, by Lemma \ref{lemma:rand}, $\mathcal S_{\text{rand}} \not \in \mathsf{PSG}$, as the generalization function of $\mathcal S_{\text{rand}}$ can be as large as $\Omega(\ln |\mathbb P|)$, which is not bounded by $\text{size}(p)$.

\begin{theorem} $\mathcal S_{\text{min}} \in \mathsf {PSG}, \mathcal S_{\text{rand}} \not \in \mathsf {PSG}$. 
\end{theorem}

In the last part of this section, we provide a simple sufficient condition for a solver to be in $\mathsf {PSG}$. As a result of relaxing the bound of $S_{\text{min}}$, besides the solver that always returns the smallest valid program, $\mathsf{PSG}$ now includes all solvers of which the synthesized program is usually at most polynomially larger than the smallest one.

\begin{definition}[Size Preserving] \label{def:solver-sp}A PBE solver $\mathcal S$ is \textit{size-preserving} on a family of domains $\mathcal F$ if there exists a polynomial $s(x, y)$ such that: 
	\begin{align*}
		\forall (\mathbb P, \mathbb I, \mathbb O) \in \mathcal F,& \forall n > 0, \forall p \in \mathbb P, \forall \epsilon \in (0, 1), \\
		&\Pr_{I_1, \dots, I_n \sim D_{I}}\left[\text{size}\left( \mathcal S\big((I_1, \sem{p}(I_1)), \dots, (I_n, \sem{p}(I_n))\big)\right) > s\left(\text{size}(p),  \ln \left(\frac{1}{\epsilon}\right)\right)\right] \leq \epsilon
	\end{align*}
\end{definition}

\begin{theorem} \label{theorem:size-preserving} $\mathcal S$ is size-perserving on $\mathcal F$ $\implies S \in \mathsf{PSG}[\mathcal F]$.
\end{theorem}

==> sections/Generalization3.tex <==
%!TEX root = ../CLIA.tex
\section{Generalization Model} \label{section:model}
In this section, we introduce the abstracted generalization model used in this paper. At the beginning, we introduce some necessary preliminaries on programming-by-example in Section \ref{section:pre-pbe}. Then, we define a natural and concrete model of the generalizability in Section \ref{section:concrete-gen}, and then abstracted it using assumptions in Section \ref{section:abstracted-gen}. After that, in Section \ref{section:gen-case}, we establish a case study to show how our abstracted model compare the generalizability of two PBE solvers. At last, motivated by the polynomial-time class $\mathsf P$, we introduce a coarse class of solvers with acceptable generalizability, namely \textit{polynomial-size generalizability}, in Section \ref{section:gen-class}.

\subsection{Preliminaries: Programming by Example}\label{section:pre-pbe}
The problem of programming by example is usually discussed above an underlying domain $\mathbb D = (\mathbb P, \mathbb I, \mathbb O, \sem{.}_{\mathbb D})$, where $\mathbb P, \mathbb I, \mathbb O$ represent a program space, an input space, and an output space respectively, $\sem{.}_{\mathbb D}$ is an oracle function that associates a program $p \in \mathbb P$ and an input $I \in \mathbb I$ with an output in $\mathbb O$, denoted as $\sem{p}_{\mathbb D}(I)$. The domain limits the ranges of possibly used programs and concerned inputs, and provides the semantics of these programs.

For simplicity, in this paper, we make the following assumptions:
\begin{itemize}
	\item There is a universal oracle function $\sem{.}$ for any domains.
	\item The program space $\mathbb P$ is always given by a regular tree grammar $G$ (Definition \ref{def:tg}).
	\item The output space $\mathbb O$ is always induced by the program space $\mathbb P$, the input space $\mathbb I$, and the oracle function $\sem{.}$, i.e., $\mathbb O = \{\sem{p}(I)\ |\ p \in \mathbb P, I \in \mathbb I\}$.
\end{itemize}

\begin{definition}\label{def:tg} A \textit{regular tree grammar} $G$ is a four-tuple $\langle N, \Sigma, s_0, R \rangle$ where:
	\begin{itemize}
		\item $N$ is a set of non-terminal symbols.
		\item $\Sigma$ is a set of terminal symbols that is disjoint from $N$. In $\Sigma$, each symbol $f$ is associated with an arity $k_f$. Specially, the arity is defined as $0$ for constants and input variables.
		\item $s_0 \in N$ represents the start symbol.
		\item $R$ is a set of production rules. All rules in $R$ are in the form of $(s, f (x_1, \dots, x_{k_f}))$ where $s, x_1, \dots, x_{k_f} \in N, f \in \Sigma$.  Rule $(s, f (x_1, \dots, x_{k_f}))$ represents that nonterminal symbol $s$ can be expanded to a function using operator $f$ and taking symbols $x_1, \dots, x_{k_f}$ as parameters. 
	\end{itemize}
	A program $p$ is inside regular tree grammar $G$ if there is no non-terminal symbol remaining in $p$ and $p$ can be produced by the start symbol $s_0$ directly or indirectly.
\end{definition}

In the remainder of this paper, we abbreviate a domain as a pair $(\mathbb P, \mathbb I)$ of a program space and an input space. We shall use notation $\mathcal F$ to represent a family of domains, and thus discuss general properties of domains.

\textit{Programming by Example (PBE)} is a subproblem of program synthesis where the solver is required to learn a program from a set of given input-output examples.

\begin{definition}[Programming by Example] \label{def:pbe}Given a domain $\mathbb D = (\mathbb P, \mathbb I)$, a PBE task $T \in (\mathbb I \times \mathbb O)^*$ is a sequence of input-output examples, where $\mathbb O$ is the induced output space of $\mathbb D$.
	
	Correspondingly, function $\mathcal S: (\mathbb I \times \mathbb O)^* \rightarrow {\{\top\} \cup \mathbb P}$ is a valid PBE solver for domain $\mathbb D$ if $\mathcal S$ satisfies the following two conditions for any PBE task $T \in (\mathbb I \times \mathbb O)^*$:
	\begin{itemize}
		\item (Soundness) If $\mathcal S(T)$ is a program, $\mathcal S(T)$ must be consistent with all examples in $T$:
		$$\mathcal {S}(T) \in \mathbb P \implies \forall (I, O) \in T, \sem{\mathcal {S}(T)}(I) = O$$
		\item (Completeness) If $\mathcal S(T) = \top$, all programs in $\mathbb P$ must violate at least one example in $T$:
		$$\mathcal {S}(T) = \top \iff \forall p \in \mathbb P, \exists (I, O) \in T, \sem{p}(I) \neq O$$
	\end{itemize}
\end{definition}

\subsection{Generalizability} \label{section:concrete-gen}
\textit{Generalizability} is a property defined for PBE solvers. Intuitively, it represents the ability for a solver to learn the \textit{full} functionality of a hidden target program from a few number of examples. Obviously, PBE tasks on input domain $\mathbb I$ cannot distinguish two programs if they perform the same on all inputs in $\mathbb I$. Therefore, the best a PBE solver can do is to synthesize a program that is \textit{semantically equivalent} to the target program on the entire input domain. 

\begin{definition}[Semantically Equivalence] Two programs $p_1$ and $p_2$ are semantically equivalent on input domain $\mathbb I$, written as $p_1 \sim_{\mathbb I} p_2$ if and only if $\forall I \in \mathbb I, \sem{p_1}(I) = \sem{p_2}(I)$.
\end{definition}

In this paper, we model the PBE task over domain $\mathbb D$ as a random variable relying on two distributions $D_p$ and $D_I$, describing the probability for each program to be taken as the target, and the probability for each input to be provided as an example respectively.

Given distributions $D_p$, $D_I$, we assume a PBE task with $n$ examples is generated in three steps: 
\begin{enumerate}
	\item A program $p$ is randomly drawn from the program space $\mathbb P$ according to $D_p$.
	\item $n$ inputs $I_1, \dots, I_n$ are independently drawn from the input space $\mathbb I$ according to $D_I$.
	\item PBE task $(I_1, \sem{p}(I_1)), \dots, (I_n, \sem{p}(I_n))$ is returned as the result of the generation.
\end{enumerate}
For simplicity, we use notation $\mathcal G$ to denote a generation model $(\mathbb D, D_p, D_I)$ for PBE tasks. \yxcomment{Generation model is never explicitly defined.}

Given a generation model $\mathcal G$, we define the generalizability as the minimal number of examples such that given a random PBE task, with a high probability, the solver is guaranteed to synthesize a program semantically equivalent to the target one.

\begin{definition}[Generalizability] \label{def:gen} Given a generation model $\mathcal G$ and a PBE solver $\mathcal S$, the generalizability $\text{gen}[\mathcal G, \mathcal S]: [0, 1] \rightarrow \mathbb Z^+$ is a function where $\forall \epsilon \in (0, 1)$, $\text{gen}[\mathcal G, \mathcal S](\epsilon)$ is defined as the smallest integer such that:
	$$\forall n \geq \text{gen}[\mathcal G, \mathcal S](\epsilon), \Pr_{p \sim D_p, I_1, \dots, I_n \sim D_I} \left[ \mathcal S\big((I_1, \sem{p}(I_1)), \dots, (I_n, \sem{p}(I_n)) \big) \not \sim_{\mathbb I} p \right] \leq \epsilon
	$$
\end{definition}
\yxcomment{The above one is complex. Can you make it shorter? For example, by moving things into text and/or adding auxiliary definitions.}

When the solver is allowed to access distributions $(D_p, D_I)$, the following solver $S_{\text{opt}}[\mathcal G]$ achieves the optimal generalizability on model $\mathcal G$:
$$ \mathcal S_{\text{opt}}[\mathcal G](T) \coloneqq \arg\max_p D_p(p)\ \ s.t.\ \forall (I, O) \in T, \sem{p}(I) = O 
$$
Where $D_p(p)$ represents the probability of $p$ in distribution $D_p$. Specially, when there is no program that is consistent with all examples, $\mathcal S_{\text{opt}}[\mathcal G](T)$ is defined as $\top$.

\begin{theorem} \label{theorem:optimal} For any generation model $\mathcal G$, for any PBE solver $\mathcal S$ valid for $\mathcal G$, and for any $\epsilon \in (0, 1)$,
	$$\text{gen}[\mathcal G, \mathcal S_{\text{opt}}[\mathcal G]](\epsilon) \leq \text{gen}[\mathcal G, \mathcal S](\epsilon)
	$$
\end{theorem}

\subsection{Abstracted Generalizability} \label{section:abstracted-gen}
Though Definition \ref{def:gen} provides a natural definition for the generalizability, its usage is rather limited, as it requires distributions $D_p, D_I$ to be explicitly given. However, when designing a PBE solver, we would always expect the solver to be generally efficient for different tasks. As the distributions vary frequently from tasks to tasks, the current definition of generalizability is usually unavailable when we want to evaluate the overall efficiency of a solver. 

To improve this point, we abstract the distributions and domains with assumptions, and thus make the generalizability estimable when concrete values of $D_p, D_I$ are unavailable.

\subsubsection{Abstracting the program distribution} To reduce the reliance on the program distribution $D_p$, we use the principle of \textit{Ocam's Razor}: We assume that a realistic application scenario always prefer simpler programs than complex ones. Therefore, distribution $D_p$ should be biased to smaller programs. To formalize this assumption, we start by defining the size of a program.

\begin{definition} Given a regular tree grammar $\langle N, \Sigma, s_0, R \rangle$, the size $\text{size}_0(p)$ of program $p$ is defined as the number of production rules used to produce program $p$ from the start symbol $s_0$, i.e.:
	$$\text{size}_0(p)\coloneqq\left\{
	\begin{array}{lcl}
		1 &  & p \in N \\
		1 + \sum_{1}^{k_f} \text{size}_0(p_i) & & p = f(p_1, \dots, p_{k_f})
	\end{array}
	\right.
	$$
	The normalized size $\text{size}(p)$ of a program $p$ is defined as $\text{size}(p) \coloneqq \left(\ln |R|\right)\text{size}_0(p)$.
\end{definition}
The advantage of introducing \textit{normalized size} is that for any program $p$, the normalized size of $p$ provides an \yxcomment{logarithmic?} upper bound on the number of programs no larger than $p$.

\begin{lemma} \label{lemma:size}For any program domain $\mathbb P$, $\forall p \in \mathbb P$, 
	$ \left|\left\{p' \in \mathbb P\  |\ \text{size}(p') \leq \text{size}(p)\right\} \right| \leq \exp\left(\text{size}(p)\right)
	$.
\end{lemma} 

\begin{assumption}[Ocam's Razor] \label{ass:1} For a random program $p \sim D_p$, the expected number of programs no larger than $p$ is asymptotically smaller than the size of the program space in logarithmic unit:
	$$
	\ln \left( \mathbb E_{p \sim D_p} \big [\left|\left\{p'\ |\ \text{size}(p') \leq \text{size}(p)\right\}\right|\big] \right) = o\left(\ln |\mathbb P|\right)
	$$
	Specially, when $\mathbb P$ is an infinite program domain, we assume the expectation is bounded:
	$$
	\ln \left( \mathbb E_{p \sim D_p} \big [\left|\left\{p'\ |\ \text{size}(p') \leq \text{size}(p)\right\}\right|\big] \right) < + \infty
	$$
\end{assumption}
\yxcomment{I do not understand the above. (1) Why is this an assumption? Is it not a theorem? (2) What is the relation with Ocam's Razor? Explanation in natural language is needed.}

To remove the reliance on $D_p$ from the generalizability, we introduce the concept of \textit{generalization function},  which eliminates the usage of $D_p$ by assuming the target program is fixed.

\begin{definition}[Generalization Function] Given a generation model $\mathcal G$ and a PBE solver $\mathcal S$, the generalization function $\text{gen}[\mathcal G,\mathcal S]: \mathbb P \times [0, 1] \rightarrow \mathbb Z^+$ is a function where $\forall p \in \mathbb P, \forall \epsilon \in (0, 1)$, $\text{gen}[\mathcal G,\mathcal S](p, \epsilon)$ is defined as the smallest integer such that 
	$$
	\forall n \geq \text{gen}[\mathcal G, \mathcal S](p, \epsilon),  \Pr_{I_1, \dots, I_n \sim D_I} \left[ \mathcal S\big((I_1, \sem{p}(I_1)), \dots, (I_n, \sem{p}(I_n)) \big) \not \sim_{\mathbb I} p \right] \leq \epsilon 
	$$
\end{definition}

\yxcomment{The notation overloads with Generalizability. Also, same as generalizability, the above formula needs to be simplified. Furthermore, $p$ and $\epsilon$ are usually referred as ``given" rather than ``forall".}

\subsubsection{Abstracting the semantics.} To calculate the generalizability, we have to model the semantics of a program on a random example, and thus distribution $D_I$ and domain $\mathbb D$ are required. To improve this point, we observe that: In most generalizability calculations, the concrete semantics is only used to calculate the probability for a random example to distinguish two semantically different programs. The following example elaborates this observation via a simple domain.

\begin{example} \label{example:analysis}Suppose there are only two programs $\{p_1, p_2\} (p_1 \not \sim_{\mathbb I} p_2)$ in the domain, and the solver $\mathcal S$ perfers $p_1$ to $p_2$ when both programs are consistent with all examples. In the case that $p_2$ is selected as the target program, the generalizability of $\mathcal S$ is determined by the probability for a random example to distinguish $p_1$ with $p_2$:
	$$
	\text{gen}[D_I, \mathcal S](p_2, \epsilon) = \left \lceil \ln \epsilon \bigg{/} \ln\left(1 - \Pr_{I \sim D_I}\left[\sem{p_2}(I) \neq \sem{p_1}(I)\right]\right) \right \rceil
	$$
	\yxcomment{What is the difference between $gen$ and $\text{gen}$? The first parameter to $\text{gen}$ is not a generation model. Also, I am puzzled about the rule of defining parameters for $gen$.}
	Therefore, to obtain an upper bound for the generalization function, the only thing we need to know about the semantics is a lower bound for probability $\Pr_{I \sim D_I} \left[\sem{p_2}(I) \neq \sem{p_1}(I)\right]$. Suppose there is such a lower bound $\alpha \in (0, 1)$, then:
	
	$$
	\text{gen}[D_I, \mathcal S](p_2, \epsilon) \leq \left \lceil \frac{\ln \epsilon}{\ln \left(1 - \alpha\right)} \right \rceil \leq \left \lceil \frac{1}{\alpha} \ln \left(\frac{1}{\epsilon}\right) \right \rceil = O\left(\ln \left(\frac{1}{\epsilon}\right)\right)
	$$
\end{example}

Example \ref{example:analysis} shows that, to obtain an asymptotical upper bound for the generalizability, a probability lower bound can be used instead of concrete semantics. In this paper, to obtain an abstracted generalization model, we assume that there is a global lower bound $\alpha$ on the probability for a random input to distinguish any two semantically different programs.

\begin{assumption} \label{ass:2} There exists a constant $\alpha \in (0, 1)$ such that for any two programs $p_1, p_2$:
	$$
	p_1 \not \sim_{\mathbb I} p_2 \implies \Pr_{I \sim D_I} \left[\sem{p_1}(I) \neq \sem{p_2}(I)\right] \geq \alpha
	$$
\end{assumption}

When the size of the input domain $\mathbb I$ is limited by a constant $S_{\mathbb I}$, there is a trivial lower bound $\alpha = S_{\mathbb I}^{-1}$. Moreover, for some specific domains, there can be a much larger lower bound, as shown in Example \ref{example:bound}. However, in our abstracted model, we do not refer to these concrete values: We just treat this probability for any programs and domains equivalently as a constant $\alpha$, and tries to derive some general bound for the generalizability of some PBE solver.

\begin{example} \label{example:bound}Let $\left(\mathbb P^L_{n,m}, \mathbb I^{L}_{n,m}\right)$ be the domain of linear integer expressions with $n$ parameters: 
	$$
	\mathbb P^L_{n,m} = \left \{\lambda \left(x_1, \dots, x_n\right). \left(a_0 + \sum_{i=1}^n a_i x_i \right) \bigg| a_0, \dots, a_n \in \{0, 1, \dots, m\}\right\}\ \ \ \mathbb I ^L_{n,m} = \{0, 1, \dots, m \}^n
	$$
	For any distinguishable programs $p_1, p_2 \in \mathbb P^L_{n,m}$, the probability for a random example to distinguish them is at least $1 - \frac{1}{m}$:
	$$
	\forall p_1, p_2 \in \mathbb P^L_{n,m}, \left (p_1 \not \sim_{\mathbb I^L_{n,m}} p_2 \implies \Pr_{I \sim D_I}\left[\sem{p}(I) \neq \sem{p'}(I)\right] \geq 1 - \frac{1}{m}\right)
	$$
\end{example}

In the remainder of this paper, when we discuss a general property for a solver on a family of domains $\mathcal F$, we implicity assume Assumption \ref{ass:1} and Assumption \ref{ass:2} hold for all domains in $\mathcal F$. 

As the distributions $D_p$ and $D_I$ has been abstracted, in the remainder of this paper, we shall omit their usages for simplicity. For example, we shall use  $\text{gen}[\mathbb D, \mathcal S](p, \epsilon)$ instead of $\text{gen}[\mathcal G, \mathcal S](p, \epsilon)$ to represent a generalization function.

\subsection{Case Study: Random Program V.S. Minimal Program} \label{section:gen-case}
In this section, we establish a case study for two primitive PBE solvers $\mathcal S_{\text{rand}}$ and $\mathcal S_{\text{min}}$. For any PBE task $T$, let $\mathbb P(T) \subseteq \mathbb P$ be the set of programs that are consistent with all examples in $T$:
\begin{itemize}
	\item $\mathcal S_{\text{rand}}$ is the most trivial synthesizer that has no guarantee on the quality of the result: It just uniformly returns a program from $\mathbb P(T)$:
	$\forall p \in \mathbb P(T), \Pr\left[\mathcal S_{\text{rand}}(T) = p\right] = |\mathbb P(T)|^{-1}$.
	\item $\mathcal S_{\text{min}}$ regards a PBE task a an optimization problem, and always returns the smallest program in $\mathbb P(T)$:
	$\mathcal S_{\text{min}}(T) \coloneqq \arg \min_{p \in \mathbb P(T)} \text{size}(p)$.
\end{itemize}
Specially, when $\mathbb P(T)$ is empty, both $\mathcal S_{\text{rand}}$ and $\mathcal S_{\text{min}}$ are defined as $\top$.

\yxmodify{$\mathcal S_{\text{min}}$ is a common strategy for improving the generalizability of PBE solvers, and its effectiveness has been \yxcomment{empirically?} studied by \citet{PD2007The}.}{It is usually believed that $\mathcal S_{\text{min}}$ has better generalizability than $\mathcal S_{\text{rand}}$.} In this subsection, we shall use our abstracted model to analyse the generalizability of $\mathcal S_{\text{min}}$ and $\mathcal S_{\text{rand}}$, and prove the advantage of $\mathcal S_{\text{min}}$ against $\mathcal S_{\text{rand}}$.

\begin{lemma} \label{lemma:min}For any domain $\mathbb D$, $\forall p \in \mathbb P, \forall \epsilon \in (0, 1), \text{gen}[\mathbb D, \mathcal S_{\text{min}}](p, \epsilon) \leq \frac{1}{\alpha} \left( \ln \left(\text{rank}(p)\right) + \ln\left(\frac{1}{\epsilon}\right)\right)$, where $\text{rank}(p)$ is defined as $|\{p' \in \mathbb P\ |\ \text{size}(p') \leq \text{size}(p)\}|$, i.e., the number of programs in $\mathbb P$ that are no larger than $p$. 
\end{lemma}
\begin{proof} In the worst case, there is no other program in $\mathbb P$ that is semantically equivalent to the target program $p$. At this time, according to the definition, $\mathcal S_{\text{min}}$ is guaranteed to return a correct program only when all incorrect programs in $S(p)$ are excluded by the PBE task, where $S(p) \subseteq \mathbb P$ is the set of programs that are no larger than $p$. Therefore, when $n$ examples are given:
	\begin{align*}
		n \geq \text{gen}[\mathbb D,\mathcal S_{\text{min}}](p, \epsilon) \Longleftarrow&\ \Pr_{I_1, \dots, I_n \sim D_I}\left[\mathcal S_{\text{min}}\big((I_1, \sem{p}(I_1)), \dots, (I_n, \sem{p}(I_n))\big) \not \sim_{\mathbb I} p\right] \leq \epsilon \\
		\Longleftarrow &\ \Pr_{I_1, \dots, I_n \sim D_I}\left[\exists p' \in S(p), \big(p' \not \sim_{\mathbb I} p \wedge \forall i \in [n], \sem{p}(I) = \sem{p'}(I)\big)\right] \leq \epsilon \\
		\text{(Union bound)} \Longleftarrow &\ \sum_{p' \in S(p), p' \not \sim_{\mathbb I} p} \left(\Pr_{I_1, \dots, I_n \sim D_I}\big[ \forall i \in [n], \sem{p}(I) = \sem{p'}(I)\big] \right) \leq \epsilon \\
		\Longleftarrow &\ \sum_{p' \in S(p), p' \not \sim_{\mathbb I} p} \left(1 - \Pr_{I \sim D_I}\left[\sem{p}(I) \neq \sem{p'}(I)\right] \right)^n \leq \epsilon \\
		\text{(Assumption }\ref{ass:2}\text{)}  \Longleftarrow &\ |S(p)| (1 - \alpha) ^n \leq \epsilon \Longleftarrow n \geq \frac{1}{\alpha}\left(\ln \left(\text{rank}(p)\right) + \ln\left(\frac{1}{\epsilon}\right)\right)
	\end{align*}
\end{proof}

Lemma \ref{lemma:min} provides a general upper bound for $\text{gen}[\mathbb D, \mathcal S_{\text{min}}]$. When we regard $\epsilon$ as a constant, the generalizability of $\mathcal S_{\text{min}}$ can be proven to be $o\left(\ln |\mathbb P|\right)$ by applying Assumption \ref{ass:1}:
\begin{align*}
	\text{gen}[\mathcal G, \mathcal S_{\text{min}}](p, \epsilon) &\leq \mathbb E_{p \sim D_p} \left[\frac{1}{\alpha}\left(\ln (\text{rank}(p)) + \ln\left(\frac{1}{\epsilon}\right)\right)\right] \\ 
	& \leq \frac{1}{\alpha}\left(\mathbb E_{p \sim D_p}\left[\ln (\text{rank}(p))\right] + \ln \left(\frac{1}{\epsilon}\right)\right) = o(\ln |\mathbb P|)
\end{align*}
The second inequality is given by Jensen's Inequality, as $\ln(x)$ is a concave function.

\begin{lemma} \label{lemma:rand} There exists a generation model $\mathcal G$ such that:
	$$ \forall p \in \mathbb P, \forall \epsilon \in (0, 0.5), \text{gen}[\mathcal G, \mathcal S_{\text{rand}}]\left(p, \epsilon\right) >  \log_{2} \left((|\mathbb P| - 1) \frac{1 - 2 \epsilon}{2 \epsilon + 2}\right)$$
\end{lemma}
\begin{proof} We construct the following domain $\mathbb D_{n}^{\oplus} = (\mathbb P_{n}^{\oplus}, \mathbb I_{m}^{\oplus})$ using \textit{exclusive-OR} ($\oplus$): 
	$$
	\mathbb P_{m}^{\oplus} = \left\{x_1 \oplus \dots \oplus x_i \ |\ i \in [1,m] \right\}\ \ \ \mathbb I_{m}^{\oplus} = \{0, 1\}^{m}
	$$
	where $x_1, \dots, x_m$ are $m$ input paramteters. Moreover, we assume the input distribution $D_I$ is a uniform distribution over $\mathbb I_{m}^{\oplus}$.  
	
	For any target program $p$, let $p_1, \dots, p_{m-1}$ be the remaining programs in $\mathbb P_{m}^{\oplus}$. We define a series of binary random variables $\mathcal E_{i, n}$ where $\mathcal E_{i, n}$ takes $1$ only when program $p_i$ is consistent with $n$ random examples. The main effect of our construction is to guarantee the following two properties: (1) $\mathbb E[\mathcal E_{i,j}] = 2^{-n}$; (2) $\forall n>0$, $\mathcal E_{1, n}, \dots, \mathcal E_{m-1, n}$ are totally independent.  
	
	\begin{align*}
		n < \text{gen}[\mathcal G, \mathcal S_{\text{rand}}](p, \epsilon) \Longleftarrow&\  \Pr_{I_1, \dots, I_n \sim D_I}\left[\mathcal S_{\text{rand}}\big((I_1, \sem{p}(I_1)), \dots, (I_n, \sem{p}(I_n))\big) \not \sim_{\mathbb I} p\right] > \epsilon \\ 
		\Longleftarrow&\  \Pr_{I_1, \dots, I_n \sim D_I}\left[\exists p' \in \mathbb P_{m}^{\oplus}, \big(p' \not \sim_{\mathbb I_{m}^{\oplus}} p \wedge \forall i \in [n], \sem{p}(I) = \sem{p'}(I) \big)\right] > 2\epsilon \\
		\Longleftarrow&\  \Pr\left[\sum_{i=1}^{m-1} \mathcal E_{i,n} \geq 1\right] > 2\epsilon 
	\end{align*}
	
	Define random variable $X_n$ as  $\sum_{i=1}^{m-1} \mathcal E_{i,n}$. Then $\mathbb E[X_n] = (m-1)2^{-n}, \mathbb E[X_n^2] = (m-1)2^{-n} + (m-1)(m-2)2^{-2n}$. By Paley-Zygmund inequality, when $\mathbb E[X] > 1$: 
	\begin{align*} \Pr[X_n > 1] \geq \left(1 - \frac{1}{\mathbb E[X_n]}\right)^2 \frac{\mathbb E[X_n]^2}{\mathbb E[X_n^2]} = \left(1 - \frac{1}{(m-1)2^{-n}} \right)^2 \frac{(m-1)2^{-n}}{1 + (m - 2)2^{-n}} > \left(1 - \frac{2}{Y}\right) \frac{Y}{1 + Y}  
	\end{align*}
	where $Y = \mathbb E[X_n] = (m - 1)2^{-n}$. 
	
	Combining the above two inequalities, the intended lower bound is obtained:
	
	$$\left(1 - \frac{2}{Y}\right)\frac{Y}{1 + Y} > 2 \epsilon \iff Y > \frac{2 \epsilon + 2}{1 - 2\epsilon} \iff n < \log_{2}\left((m - 1) \frac{1 - 2 \epsilon}{2 \epsilon + 2}\right)$$
\end{proof}

Lemma \ref{lemma:rand} provides a worst-case lower bound for the generalizability of $\mathcal S_{\text{rand}}$. When we regard $\epsilon$ as a constant, Lemma \ref{lemma:rand} implies that: There exists a generation model such that $\text{gen}[\mathcal G, \mathcal S_{\text{rand}}](p, \epsilon) = \Omega(\ln |\mathbb P|)$, which is asymptotically larger than the upper bound on the genralizability of $\mathcal S_{\text{min}}$. Therefore, our abstracted generalization model can discover the advantage of $\mathcal S_{\text{min}}$ against $\mathcal S_{\text{rand}}$ on the generalizability.

\subsection{Polynomial-Size  Generalizability} \label{section:gen-class}
In the previous section, our abstracted generalization model discovers the advantage of $\mathcal S_{\text{min}}$ on the generalizability. However, in the previous section, we distinguish $\mathcal S_{\text{min}}$ with $\mathcal S_{\text{rand}}$ by analyzing a concrete lower/upper bound, which may be unnecessarily tedious. Analogy with the time complexity, the analysis in the previous section is like to calculate and compare the number of instruments executed by two different algorithms. However, in many cases, we only care about whether the algorithm is polynomial-time or not. Motivated by this point, in this section, we introduce the class of \textit{polynomial-size generalizability}, which (1) is relexed from the upper bound proviede by Lemma \ref{lemma:min} and thus provide great flexibility for designing an efficient program with acceptable generalizability, (2) is more friendly for analysis, (3) could still distinguish $\mathcal S_{\text{min}}$ with $\mathcal S_{\text{rand}}$.

By Lemma \ref{lemma:min}, $\text{gen}[\mathbb D, \mathcal S_{\text{min}}](p, \epsilon)$ is bounded by $O\left(\ln(\text{rank}(p))\right) + O\left(\ln (1 / \epsilon)\right)$. We derive the definition of polynomial-size generalizability by relaxing this upper bound twice:
\begin{itemize}
	\item As $\text{rank}(p)$ greatly relies on the program domain $\mathbb P$, we replace it with $\text{size}(p)$ by Lemma \ref{lemma:size}. On the one hand, such a replacement cuts off the reliance on the program domain $\mathbb P$, as $\text{size}(p)$ depends only on the syntax of program $p$. On the other hand, as the number of programs usually grows exponentially when the size increases, this replacement does not relax the bound much. 
	\item Motivated by the class of polynomial-time algorithms, in our class, we allow the generalizability of a PBE solver to be polynomially worse than $\mathcal S_{\text{min}}$, and thus leaves a great space for optimizing other aspects of solvers, such as the time complexity.
\end{itemize}

To summary, we define the class of \textit{polynomial-size generalizability} as the following.

\begin{definition}[Polynomial-Size Generalizability] \label{def:poly-gen} For a family of domains $\mathcal F$, a PBE solver $\mathcal S$ has \textit{polynomial-size generalizability} on $\mathcal F$, abbreviated as $\mathcal S \in \mathsf {PSG}[\mathcal F]$, if there exists a polynomial $g(x,y)$ such that:
	$$\forall \mathbb D \in \mathcal F, \forall p \in \mathbb P, \forall \epsilon (0, 1), \text{gen}[\mathbb D, \mathcal S](p, \epsilon) \leq g(\text{size}(p), \ln(1 / \epsilon))$$
\end{definition}

Specially, we abbreviate $\mathcal S \in \mathsf {PSG}[\mathcal F]$ to $\mathcal S \in \mathsf {PSG}$ when $\mathcal F$ contains all possible domains. By Lemma \ref{lemma:min}, we know that $\mathcal S_{\text{min}} \in \mathsf {PSG}$. Moreover, by Lemma \ref{lemma:rand}, $\mathcal S_{\text{rand}} \not \in \mathsf{PSG}$, as the generalization function of $\mathcal S_{\text{rand}}$ can be as large as $\Omega(\ln |\mathbb P|)$, which is not bounded by $\text{size}(p)$.

\begin{theorem} $\mathcal S_{\text{min}} \in \mathsf {PSG}, \mathcal S_{\text{rand}} \not \in \mathsf {PSG}$. 
\end{theorem}

In the last part of this section, we provide a simple sufficient condition for a solver to be in $\mathsf {PSG}$. As a result of relaxing the bound of $S_{\text{min}}$, besides the solver that always returns the smallest valid program, $\mathsf{PSG}$ now includes all solvers of which the synthesized program is usually at most polynomially larger than the smallest one.

\begin{definition}[Size Preserving] \label{def:solver-sp}A PBE solver $\mathcal S$ is \textit{size-preserving} on a family of domains $\mathcal F$ if there exists a polynomial $s(x, y)$ such that: 
	\begin{align*}
		\forall \mathbb D \in \mathcal F,& \forall n > 0, \forall p \in \mathbb P, \forall \epsilon \in (0, 1), \\
		&\Pr_{I_1, \dots, I_n \sim D_{I}}\left[\text{size}\left( \mathcal S\big((I_1, \sem{p}(I_1)), \dots, (I_n, \sem{p}(I_n))\big)\right) > s\left(\text{size}(p),  \ln \left(\frac{1}{\epsilon}\right)\right)\right] \leq \epsilon
	\end{align*}
\end{definition}

\begin{theorem} \label{theorem:size-preserving} $\mathcal S$ is size-perserving on $\mathcal F$ $\implies S \in \mathsf{PSG}[\mathcal F]$.
\end{theorem}

\yxcomment{I suppose this is not a necessary condition. Then how tight is the condition? Or, is there any condition for determining non-PSG classes?}

==> sections/Generalization4.tex <==
%!TEX root = ../CLIA.tex
\section{Generalization Model} \label{section:model}
In this section, we introduce the abstracted generalization model used in this paper. At the beginning, we introduce some necessary preliminaries on programming-by-example in Section \ref{section:pre-pbe}. Then, we define a natural and concrete model of the generalizability in Section \ref{section:concrete-gen}, and then abstracted it using assumptions in Section \ref{section:abstracted-gen}. At last, we introduce a  class of solvers to represent "good generalizability", namely \textit{polynomial-size generalizability}, in Section \ref{section:gen-class}.

\subsection{Preliminaries: Programming by Example}\label{section:pre-pbe}
The problem of programming by example is usually discussed above an underlying domain $\mathbb D = (\mathbb P, \mathbb I, \mathbb O, \sem{.}_{\mathbb D})$, where $\mathbb P, \mathbb I, \mathbb O$ represent a program space, an input space, and an output space respectively, $\sem{.}_{\mathbb D}$ is an oracle function that associates a program $p \in \mathbb P$ and an input $I \in \mathbb I$ with an output in $\mathbb O$, denoted as $\sem{p}_{\mathbb D}(I)$. The domain limits the ranges of possibly used programs and concerned inputs, and provides the semantics of these programs.

For simplicity, in this paper, we make the following assumptions:
\begin{itemize}
	\item There is a universal oracle function $\sem{.}$ for any domains.
	\item The output space $\mathbb O$ is always induced by the program space $\mathbb P$, the input space $\mathbb I$, and the oracle function $\sem{.}$, i.e., $\mathbb O = \{\sem{p}(I)\ |\ p \in \mathbb P, I \in \mathbb I\}$.
\end{itemize}
Therefore, in the remainder of this paper, we abbreviate a domain as a pair $(\mathbb P, \mathbb I)$ of a program space and an input space. We shall use notation $\mathcal F$ to represent a family of domains, and thus discuss general properties of domains.

\textit{Programming by Example (PBE)} is a subproblem of program synthesis where the solver is required to learn a program from a set of given input-output examples. As this paper focus on generalizability of PBE solvers, we assume that there is at least a program satisfying all given examples: The problem of determining whether there is a valid program is another domain of program synthesis, namely \textit{unrealizability}~\cite{DBLP:conf/pldi/HuCDR20,DBLP:journals/pacmpl/KimHDR21}, and is out of the scope of our paper.

\begin{definition}[Programming by Example] \label{def:pbe}Given a domain $\mathbb D$, a PBE task $T \in (\mathbb I \times \mathbb O)^*$ is a sequence of input-output examples, where $\mathbb O$ is the induced output space of $\mathbb D$. Define $\mathbb T(\mathbb D) \subseteq (\mathbb I \times  \mathbb O)^*$ be the set of PBE tasks where there is at least one program satifying all examples:
	$$\mathbb T(\mathbb D) \coloneqq \{T \in (\mathbb I \times \mathbb O)^*\ |\ \exists p \in \mathbb P, \forall (I,O) \in T, \sem{p}(I) = O\}$$
	
	PBE solver $\mathcal S$ is a function that takes a PBE task as the input, and returns a program satisfying all given examples, i.e., $\forall T \in \mathbb T(\mathbb D), \forall (I,O) \in T, \sem{\mathcal S(T)}(I) = O$.
\end{definition}

\subsection{Generalizability} \label{section:concrete-gen}
\textit{Generalizability} is a property defined for PBE solvers. Intuitively, it represents the ability for a solver to learn the \textit{full} functionality of a hidden target program from a few number of examples. Obviously, PBE tasks on input space $\mathbb I$ cannot distinguish two programs if they perform the same on all inputs in $\mathbb I$. Therefore, the best a PBE solver can do is to synthesize a program that is \textit{semantically equivalent} to the target program on the entire input domain. 

\begin{definition}[Semantically Equivalence] Two programs $p_1$ and $p_2$ are semantically equivalent on input domain $\mathbb I$, written as $p_1 \sim_{\mathbb I} p_2$ if and only if $\forall I \in \mathbb I, \sem{p_1}(I) = \sem{p_2}(I)$.
\end{definition}

In this paper, we model a PBE task over domain $\mathbb D$ as a random variable generated from a random target program and several independent random inputs.

\begin{definition}[Generation Model] A generation model $\mathcal G$ is a pair of domain $\mathbb D$ and a joint distribution $D$ over $\mathbb P \times \mathbb I$. For convenience, we denote $D_p$ as the marginal distribution over programs, and $D_I(p)$ as the conditional distribution on inputs when the program is take as $p$, i.e.: 
	$$
	\forall p \in \mathbb P, D_I(p) \coloneqq \sum_{I \in \mathbb I} D(p, I)\ \ \ \ \forall p \in \mathbb P, \forall I \in \mathbb I, D_I(p)(I) \coloneqq D(p, I) / D_p(p) 
	$$
	
	Under generation model $\mathcal G$, a PBE task with $n$ examples is generated in the following three steps:
	\begin{enumerate}
			\item A program $p$ is randomly drawn from distribution $D_p$, representing the target program.
			\item $n$ inputs $I_1, \dots, I_n$ are independently drawn from distribution $D_I(p)$.
			\item PBE task $(I_1, \sem{p}(I_1), \dots, (I_n, \sem{p}(I_n)))$ is returned as the result of the generation.
	\end{enumerate}
\end{definition}
For simplicity, we use notation $T(p, I_1, \dots, I_n)$ to represent the PBE task generated from program $p$ and inputs $I_1, \dots, I_n$ in the third step, i.e., task $(I_1, \sem{p}(I_1), \dots, (I_n, \sem{p}(I_n)))$.

Given a generation model $\mathcal G$, we define generalizability of a PBE solver $\mathcal S$ as the minimal number of examples required such that with a high probability, $\mathcal S$ is guaranteed to synthesize a program semantically equivalent to the target.

\begin{definition}[Generalizability] \label{def:gen} Given a generation model $\mathcal G$ and a PBE solver $\mathcal S$, generalizability $\text{gen}[\mathcal G, \mathcal S]: (0, 1) \rightarrow \mathbb Z^+$ is a function where $\forall \epsilon \in (0, 1)$, $\text{gen}[\mathcal G, \mathcal S](\epsilon)$ is defined as the smallest integer such that:
	$$\forall n \geq \text{gen}[\mathcal G, \mathcal S](\epsilon), \Pr_{p \sim D_p, I_1, \dots, I_n \sim D_I(p)} \left[ \mathcal S\big(T(p, I_1, \dots, I_n) \big) \not \sim_{\mathbb I} p \right] \leq \epsilon
	$$
\end{definition}

When the solver is allowed to access the joint distribution $D$, the following solver $S_{\text{opt}}[\mathcal G]$ achieves the optimal generalizability on generation model $\mathcal G$:
$$ \mathcal S_{\text{opt}}[\mathcal G](T) \coloneqq \mathop{\arg\max}_p \left(D_p(p)\prod_{(I,O) \in T} D_I(p)(I)\right)\ \ s.t.\ \forall (I, O) \in T, \sem{p}(I) = O 
$$
Intuitively, $\mathcal S_{\text{opt}}$ selects the program that is most probable to generate the observed PBE task $T$.

\begin{theorem} \label{theorem:optimal} For any generation model $\mathcal G$, for any PBE solver $\mathcal S$ and for $\epsilon \in (0, 1)$,
	$$\text{gen}[\mathcal G, \mathcal S_{\text{opt}}[\mathcal G]](\epsilon) \leq \text{gen}[\mathcal G, \mathcal S](\epsilon)
	$$
\end{theorem}

Due to space limit of the main text, we move all proofs to the appendix, which can be found in the supplementary material.

To improve the generalizability of PBE solvers, there have been a series of previous works use a learned function to rank programs, and returns only a probable (or the optimal) program~\cite{DBLP:conf/iclr/BalogGBNT17, DBLP:conf/iclr/KalyanMPBJG18, DBLP:journals/pacmpl/JiS0H20, DBLP:conf/cav/SinghG15, DBLP:conf/sigsoft/ChenMF19, DBLP:conf/icml/MenonTGLK13, DBLP:conf/icml/DevlinUBSMK17, DBLP:conf/pldi/LeeHAN18}. The effectiveness of these appraoches can be explained using Theorem \ref{theorem:optimal}: Ideally, if the learned function ranks programs as $\mathcal S_{\text{opt}}$ does, these approaches can achieve the theoretically optimal generalizability.

\subsection{Abstracted Generalizability} \label{section:abstracted-gen}
Though Definition \ref{def:gen} provides a definition for the generalizability, its usage is rather limited: Calculating $\text{gen}[\mathcal G](\epsilon)$ requires the generation model $\mathcal G$ to be explicitly given, which is usually unavailable while performing theoretical analysis. To improve this point, in this section, we abstract the usage of the generation model $\mathcal G$, and thus make the generalizability estimable when concrete value of $\mathcal G$ is unavailable. 

\subsubsection{Abstracting the semantics.} A natural idea is to define the abstracted generalizability of a PBE solver as a general upper bound on generalizability for all possible generation model. However, such a model cannot distinguish between any PBE solvers: We find that for some extreme generation model where there is an incorrect program that performs extremely close to the target, no matter what the PBE solver is, a large number of examples is always necessary to exclude this incorrect program. We shall use an example to illustrate this observation.

\begin{example} \label{example:analysis-2-first} Consider a simple program domain $\mathbb D_2$ with only two programs $\{p_1, p_2\}$, and a generation model $\mathcal G_2$ where the marginal distribution $D_p$ is uniform and the input distribution is independent with the target program, i.e., $D_p(p_1) = D_p(p_2) \wedge \forall I \in \mathbb I, D_I(p_1)(I) = D_I(p_2)(I)$. For any PBE solver $\mathcal S$, we can prove that generalizability of $\mathcal S$ is bounded by the difference between $p_1$ and $p_2$ on semantics:
	$$
	\text{gen}[\mathcal G_2, \mathcal S](\epsilon) \geq \left \lceil \ln (2\epsilon) \bigg{/} \ln\left(1 - \Pr_{I \sim D_I(p_1)}\left[\sem{p_1}(I) \neq \sem{p_2}(I)\right]\right) \right \rceil
	$$
	
	When there is no constraint on $D$, the difference $\Pr_{I \sim D_I(p_1)}\left[\sem{p_1}(I) \neq \sem{p_2}(I)\right]$ can be arbitrarily small, and thus the generalizability of $\mathcal S$ can be arbitrarily large. At this time, it is meaningless to discuss the general upper bound of generalizability, as whatever the PBE solver is, this upper bound is always infinite.
\end{example}

Therefore, to dicuss the general upper bound of generalizability, it is necessary to introduce some assumptions on the generation model. Motivated by Example \ref{example:analysis-2-first}, we assume that there is a global lower bound $\alpha$ on the semantic difference between the target and any incorrect program.

\begin{assumption} \label{ass:2} There is a constant $\alpha \in (0, 0.5)$ such that for any program $p \in \mathbb P$:
	$$
	\forall p' \in \mathbb P, \left (p \not \sim_{\mathbb I} p' \implies \Pr_{I \sim D_I(p)} \left[\sem{p}(I) \neq \sem{p'}(I)\right] \geq \alpha \right)
	$$
\end{assumption}

\begin{example}\label{example:analysis-2-second}
	Continue to Example \ref{example:analysis-2-first}. With the help of Assumption \ref{ass:2}, a general upper bound on generalizability can be estabilished:
	$$
	\text{gen}[\mathcal G, \mathcal S](\epsilon) \leq \left \lceil \frac{\ln (2\epsilon)}{\ln \left(1 - \alpha\right)} \right \rceil \leq \left \lceil \frac{1}{\alpha} \ln \left(\frac{1}{2\epsilon}\right) \right \rceil = O\left(\ln \left(\frac{1}{\epsilon}\right)\right)
	$$
\end{example}

When the size of the input domain $\mathbb I$ is limited by a constant $S_{\mathbb I}$ and the input distribution $D_I(p)$ is uniform, there is a trivial bound $\alpha = S_{\mathbb I}^{-1}$. Moreover, for some specific domains, there can be a much larger lower bound, as shown in Example \ref{example:bound}. 

\begin{example} \label{example:bound}Let $\left(\mathbb P^L_{n,m}, \mathbb I^{L}_{n,m}\right)$ be the domain of linear integer expressions with $n$ parameters: 
	$$
	\mathbb P^L_{n,m} = \left \{\lambda \left(x_1, \dots, x_n\right). \left(a_0 + \sum_{i=1}^n a_i x_i \right) \bigg| a_0, \dots, a_n \in \{0, 1, \dots, m\}\right\}\ \ \ \mathbb I ^L_{n,m} = \{0, 1, \dots, m \}^n
	$$
	When the input distribution is uniform, the semantic difference between any two semantically different programs is at least $1 - \frac{1}{m}$:
	$$
	\forall p_1, p_2 \in \mathbb P^L_{n,m}, \left (p_1 \not \sim_{\mathbb I^L_{n,m}} p_2 \implies \Pr_{I \sim D_I(p_1)}\left[\sem{p}(I) \neq \sem{p'}(I)\right] \geq 1 - \frac{1}{m}\right)
	$$
\end{example}

\subsubsection{Abstracting the program distribution} To evaluate the effectiveness of the abstracted model, we consider two primitive PBE solvers, $\mathcal S_{\text{rank}}$ and $\mathcal S_{\text{min}}$. Before formally defining these two approaches, we first introduce the concept of \textit{syntactic size}.

\begin{definition} \label{def:size} The size $\text{size}_0(p)$ of program $p$ if defined as the number of vertices on the abstracted syntax tree of $p$. Based on it, the normalized size $\text{size}(p)$ is defined as $\left(\ln N\right) \times \text{size}_0(p)$, where $N$ represents the number of different types of AST vertices in the corresponding domain.
\end{definition}

\begin{example} The size of program $x + 1$ is equal to $3$, and the normalized size of $x+1$ varies with domains. When only input variable $x$, operator $+$ and constants $1, 2$ are available, $\text{size}(x+1)$ is defined as $3 \ln 4$. When there are $a$ input variables, $b$ constants and $c$ different operators, $\text{size}(x + 1)$ is defined as $3 \ln (a + b + c)$.
\end{example}

The advantage of introducing \textit{normalized size} is that for any program $p$, the $\text{size}(p)$ provides an logarithmic upper bound on the number of programs no larger than $p$.

\begin{lemma} \label{lemma:size}For any domain $\mathbb D$, $\forall p \in \mathbb P$, 
	$ \left|\left\{p' \in \mathbb P\  |\ \text{size}(p') \leq \text{size}(p)\right\} \right| \leq \exp\left(\text{size}(p)\right)
	$.
\end{lemma} 

Now we move to solvers $\mathcal S_{\text{rand}}$ and $\mathcal S_{\text{min}}$. For any PBE task $T$, let $\mathbb P(T) \subseteq \mathbb P$ be the set of programs that are consistent with examples in $T$:
\begin{itemize}
	\item $\mathcal S_{\text{rand}}$ is the most trivial synthesizer that has no guarantee on the quality of the result: It just uniformly returns a program from $\mathbb P(T)$:
	$\forall p \in \mathbb P(T), \Pr\left[\mathcal S_{\text{rand}}(T) = p\right] = |\mathbb P(T)|^{-1}$.
	\item $\mathcal S_{\text{min}}$ regards a PBE task as an optimization problem, and always returns the syntactically smallest program in $\mathbb P(T)$:
	$\mathcal S_{\text{min}}(T) \coloneqq \arg \min_{p \in \mathbb P(T)} \text{size}(p)$.
\end{itemize}

By the empirical performance, it is usually believed that $\mathcal S_{\text{min}}$ has better generalizability than $\mathcal S_{\text{rand}}$. Therefore, the abstracted model is expected to discover the advantage of $\mathcal S_{\text{min}}$ against $\mathcal S_{\text{rand}}$.

By Assumption \ref{ass:2}, upper bounds on generalizability of these two solvers can be estabilished.

\begin{lemma}\label{lemma:2-upper} For any generation model $\mathcal G$ and any $\epsilon \in (0, 1)$:
	\begin{align*}
		\text{gen}[\mathcal G, \mathcal S_{\text{rand}}](\epsilon) \leq \frac{1}{\alpha} \left( \ln |\mathbb P| + \ln \left(\frac{1}{\epsilon}\right) \right)\ \ \ \text{gen}[\mathcal G, \mathcal S_{\text{min}}](\epsilon) \leq \frac{1}{\alpha}\left(\mathop{\mathbb E}_{p \sim D_p}\big[\ln \text{rank}(p)\big] + \ln\left(\frac{1}{\epsilon}\right)\right)
	\end{align*}
where $\text{rank}(p)$ is defined as the number of programs no larger than $p$, i.e., $\{p' \in \mathbb P\ |\ \text{size}(p') \leq \text{size}(p)\}$. 
\end{lemma}

Moreover, when $\epsilon$ is regarded as a constant, we could prove that the upper bound provided in Lemma \ref{lemma:2-upper} is asymptotically tight for both $\mathcal S_{\text{rand}}$ and $\mathcal S_{\text{min}}$. 

\begin{lemma}\label{lemma:2-lower} There is a generation model $\mathcal G$ such that for all $\epsilon \in \left(0, \frac{1}{2}\right)$:
		$$\text{gen}[\mathcal G, \mathcal S_{\text{rand}}]\left(\epsilon\right) >  \log_{2} \left((|\mathbb P| - 1) \frac{1 - 2 \epsilon}{2 \epsilon + 2}\right)\ \ \ \text{gen}[\mathcal G, \mathcal S_{\text{min}}]\left(\epsilon\right) >   \mathop{\mathbb E}_{p \sim D_p}\big[\log_2 \text{rank}(p)\big] + \log_{2} \left(\frac{1 - 2 \epsilon}{2 \epsilon + 2}\right)
		$$
\end{lemma}

By the definition of $\text{rank}(p)$, for any finite program space $\mathbb P$, there is always a program $p_l \in \mathbb P$ such that $\text{rank}(p_l) = |\mathbb P|$. Therefore, if there is no addtional assumption on the program distribution $D_p$, by Lemma \ref{lemma:2-upper} and Lemma \ref{lemma:2-lower}, the generalizability of $\mathcal S_{\text{rand}}$ and $\mathcal S_{\text{min}}$ can be asymptotically the same in some extreme cases, for example, when $D_p(p_l)$ is close to $1$.

However, as the advantage of $\mathcal S_{\text{min}}$ has been verified empirically in many different applications, and the idea of finding the simplest solution of a problem has been extensively accepted as the principle of \textit{Ocam's Razor}, in our abstracted model, we choose to regard these extreme program distributions as unrealistic, and introduce an assumption to exclude them.

\begin{assumption}\label{ass:1} For a random program $p \sim D_p$, the expected number of programs no larger than $p$ is asymptotically smaller than the size of the program space in logarithmic unit:
	$$
	\mathbb E_{p \sim D_p} \big [\ln \text{rank}(p)\big] = o\left(\ln |\mathbb P|\right)
	$$
	Specially, when $\mathbb P$ is infinite, we assume the expectation is bounded, i.e., 
	$
	\mathbb E_{p \sim D_p} \big [\ln \text{rank}(p)\big]  < + \infty
	$.
\end{assumption}

By Lemma \ref{lemma:2-upper} and Lemma \ref{lemma:2-lower}, Assumption \ref{ass:1} is the loosest assumption on the program distribution to ensure the advantage of $\mathcal S_{\text{min}}$. After introducing this assumption, we could prove that the generalizability of $\mathcal S_{\text{min}}$ is asymptotically smaller than $\mathcal S_{\text{rand}}$.

To remove the reliance on $D_p$ from the generalizability, we introduce the concept of \textit{generalization function}. which eliminates the usage of $D_p$ by assuming the target program $p$ is fixed.

\begin{definition}[Generalization Function] Given a generation model $\mathcal G$ and a PBE solver $\mathcal S$, the generalization function $\text{gen}_f[\mathcal G,\mathcal S]: \mathbb P \times [0, 1] \rightarrow \mathbb Z^+$ is a function where $\forall p \in \mathbb P, \forall \epsilon \in (0, 1)$, $\text{gen}_f[\mathcal G,\mathcal S](p, \epsilon)$ is defined as the smallest integer such that 
	$$
	\forall n \geq \text{gen}_f[\mathcal G, \mathcal S](p, \epsilon),  \Pr_{I_1, \dots, I_n \sim D_I(p)} \left[ \mathcal S\big(T(p, I_1, \dots, I_n) \big) \not \sim_{\mathbb I} p \right] \leq \epsilon 
	$$
\end{definition}

In the remainder of this paper, when we discuss a general property on a family of domains $\mathcal F$, we shall implicity assume Assumption \ref{ass:2} and Assumption \ref{ass:1} hold for all generation models on $\mathcal F$. 

\subsection{Polynomial-Size  Generalizability} \label{section:gen-class}
In the previous section, we introduce two moderate assumptions to the generation model, and thus make it able to distinguish between $\mathcal S_{\text{min}}$ and $\mathcal S_{\text{rand}}$ without knowing a concrete generation model. However, the way we distinguish these two solvers is to caculate concrete upper bounds (Lemma \ref{lemma:2-upper}) and lower bounds (Lemma \ref{lemma:2-lower}), which may be unnecessarily tedious. 

Analogy with time complexity, the detailed analysis in the previous section is like to calculate the number of instruments executed by an algorithm. However, in many cases, we only care about whether the algorithm is polynomial-time or not. Motivated by this point, just like polynomial-time algorithm is often taken as a target for "efficient algorithms", we introduce the class of \textit{polynomial-size generalizability} as a target representing "good generalizability".

By Lemma \ref{lemma:2-upper}, $\text{gen}_f[\mathcal G, \mathcal S_{\text{min}}](p, \epsilon)$ is bounded by $O\left(\ln(\text{rank}(p))\right) + O\left(\ln (1 / \epsilon)\right)$. We derive the definition of polynomial-size generalizability by relaxing this upper bound twice:
\begin{itemize}
	\item As $\text{rank}(p)$ greatly relies on the program space $\mathbb P$, we replace it with $\text{size}(p)$ by Lemma \ref{lemma:size}. On the one hand, such a replacement reduces the reliance on the program space $\mathbb P$, as $\text{size}(p)$ depends only on the syntax of program $p$ and the number of syntax components. On the other hand, as the number of programs usually grows exponentially when the size increases, the relaxed bound is usually asymptotically equivalent to the origin one. 
	\item Motivated by the class of polynomial-time algorithms, we allow the generalizability of a PBE solver to be at most polynomially worse than $\mathcal S_{\text{min}}$, and thus leaves a great space for optimizing other aspects of solvers, such as the time complexity.
\end{itemize}

To summary, we define the class of \textit{polynomial-size generalizability} as the following.

\begin{definition}[Polynomial-Size Generalizability] \label{def:poly-gen} For a family of domains $\mathcal F$, a PBE solver $\mathcal S$ has \textit{polynomial-size generalizability} on $\mathcal F$, abbreviated as $\mathcal S \in \mathsf {PSG}[\mathcal F]$, if there exists a polynomial $g(x,y)$ such that for any generation model $\mathcal G$ on $\mathcal F$: 
	$$ \forall p \in \mathbb P, \forall \epsilon \in (0, 1), \text{gen}_f[\mathcal G, \mathcal S](p, \epsilon) \leq g(\text{size}(p), \ln(1 / \epsilon))$$
\end{definition}

Specially, we abbreviate $\mathcal S \in \mathsf {PSG}[\mathcal F]$ to $\mathcal S \in \mathsf {PSG}$ when $\mathcal F$ contains all possible domains. By Lemma \ref{lemma:2-upper}, we know that $\mathcal S_{\text{min}} \in \mathsf {PSG}$. Moreover, by Lemma \ref{lemma:2-lower}, $\mathcal S_{\text{rand}} \not \in \mathsf{PSG}$, as the generalization function of $\mathcal S_{\text{rand}}$ can be as large as $\Omega(\ln |\mathbb P|)$, which is not bounded by $\text{size}(p)$.

\begin{theorem} \label{theorem:2-final} $\mathcal S_{\text{min}} \in \mathsf {PSG}, \mathcal S_{\text{rand}} \not \in \mathsf {PSG}$. 
\end{theorem}

To end this section, we provide a sufficient condition for a solver to be in $\mathsf {PSG}$. As a result of relaxing the generalization bound of $S_{\text{min}}$, which always returns the smallest valid program, $\mathsf{PSG}$ includes all solvers where with a high probability, the synthesized program is at most polynomially larger than the smallest one.

\begin{definition}[Size Preserving] \label{def:solver-sp}A PBE solver $\mathcal S$ is \textit{size-preserving} on a family of domains $\mathcal F$ if there exists a polynomial $s(x, y)$ such that for any generation model $\mathcal G$ on $\mathcal F$:
	\begin{align*}
		\forall n > 0, \forall p \in \mathbb P, \forall \epsilon \in (0, 1),
		\Pr_{I_1, \dots, I_n \sim D_{I}(p)}\left[\text{size}\left( \mathcal S\big(T(p, I_1, \dots, I_n)\big)\right) > s\left(\text{size}(p),  \ln \left(\frac{1}{\epsilon}\right)\right)\right] \leq \epsilon
	\end{align*}
\end{definition}

\begin{theorem} \label{theorem:size-preserving} $\mathcal S$ is size-perserving on $\mathcal F$ $\implies S \in \mathsf{PSG}[\mathcal F]$.
\end{theorem}

==> sections/Introduction.tex <==
%!TEX root = ../CLIA.tex
\section{Introduction} \label{section:introduction}
\begin{itemize}
	\item Oracle-guided inductive program synthesis is important. In OGIS, an oracle is queried with questions, such as whether a couterexample exists to show program $p$ is incorrect, or what output corresponds to input $i$. The oracle is usually an automated program, but can also be human.
	\item Two main types of oracle exists. The first type is able to verify whether a program is correct, and produces a couterexample if it is not. A typical algorithm for this type is CEGIS. The second type is able to provide input-output examples. This involves oracles that are blackbox, such as binary programs, or oracles that are programs too complex to analyze, such as repair, second-order symbolic execution, deobfuscation, etc.
	\item For either type, the generalizability of PBE is a key factor. In the former case, generalizability significantly affects the efficiency of the solver. In the latter case, generalizability determines correctness.
	\item To ensure generalizability, a widely-used general principle is to return the smallest program (many citations). This principle also corresponds to the general principle of Occam's Razor. However, implementing this principle requires to solve an optimization problem, which is difficult to solve efficiently. As a matter of fact, all existing synthesizers that minimize the resulting program all work on small domains (true?). On many important domains it is still very hard to find the smallest program. For example, in the domain of CLIA. (Analyzing why minimizing program size on CLIA is hard?)
	\item Our core insight of this paper is that we do not need to return the smallest program: returning a small enough program could already lead to good generalizability. To characterize whether a synthesizer returns a small enough program, we utilize a concept (generalizability class?) from the computational learning theory: Occam's learning. To demonstrate the effectiveness of Occam's learning, we show that $S_{min}$ and $S_{rand}$ could be distinguished.
	\item (not sure if a better motivation can be given to STUN and Eusolver) We analyze the generalizability of Eusolver, an efficient algorithm that works on the CLIA domain, based on Occam's learning. To perform this analysis, we extend Occam's learning to the STUN framework, the framework that Eusolver uses, and give a necessary condition for a STUN algorithm to be an Occam learning. Based on this extension, we show that neither eusolver nor any of its two components are Occam learning.
	\item We design a new STUN algorithm based on our extension, we prove that our algorithm is an Occam learning.
	\item We evaluate our approach on the CLIA benchmark, and found that...
	% \item However, designing an algorithm with good generalizability is hard. A fundamental difficulty raises from the fact that we still lack theoretical tools to compare the generalizability of different algorithms.
	% \item In this paper we give two theoretical contributions.
	% \begin{itemize}
	% 	\item Inspired by PAC, we propose a definition of generalizability for program synthesis. We found that the PAC setting that makes no assumption about the distribution of 
	% 	\item Inspired by complexity theory, we propose a polynomial-size generalizability class.
	% 	\item 
	% \end{itemize}
\end{itemize}

\textit{Programming by Example (PBE)}~\cite{DBLP:conf/ijcai/ShawWG75} is an important subproblem of program synthesis where the solver is required to learn a program from input-output examples. PBE is useful for three main reasons: 
% There are three main reasons for the prevalence of PBE: 
(1) In practice, input-output examples are usually easier to obtain than the general logic specifications, and many practical problems theirselves are instances of PBE; (2) For synthesizers and verifiers, the example-based specification in PBE is usually more tractable than general logic specifications; (3) In many cases, the general synthesis problem can be converted into PBE by CEGIS frameowrk~\cite{DBLP:conf/asplos/Solar-LezamaTBSS06}. After decades of development, many general PBE solvers have been proposed~\cite{DBLP:conf/cav/AlurCR15, DBLP:conf/cav/ReynoldsBNBT19, DBLP:journals/pacmpl/WangDS18, DBLP:conf/oopsla/PolozovG15}, and these techniques have been applied to different domains, such as string manipulation \cite{DBLP:conf/popl/Gulwani11, DBLP:conf/pldi/BarowyGHZ15}, data wrangling \cite{DBLP:conf/pldi/FengMGDC17, DBLP:conf/sigsoft/ChenMF19, DBLP:conf/pldi/YaghmazadehKDC16}, SQL queries \cite{DBLP:conf/pldi/WangCB17, DBLP:conf/kbse/ZhangS13}. 

Despite many existing applications, generalizability remains one of the main challenges to apply PBE techniques~\cite{polozov2016program}. Because the example-based specification in PBE constraints only for a few inputs, there may be many different programs satisfying all given examples. At this time, the PBE solver should be able to infer the correct program from all these remaining ones. In practice, as it is usually costly to collect input-output examples, it is important for a PBE solver to have good generalizability: The fewer examples required to synthesize a correct program, the less cost invoking the PBE solver will be, and thus the more effective the PBE solver will be in practice. 

There have been many heuristic methods proposed to improve the generalizability of PBE solvers. Some previous works guarantee the optimality of the synthesized program under some heuristic functions~\cite{DBLP:conf/icml/LiangJK10,DBLP:conf/popl/Gulwani11, DBLP:conf/popl/RaychevBVK16, DBLP:conf/icse/MechtaevYR15, DBLP:conf/cav/DAntoniSS16, DBLP:conf/sigsoft/LeCLGV17}, and some other works use learned models to guide the synthesis procedure, and thus focus only on probable programs~\cite{DBLP:conf/iclr/BalogGBNT17, DBLP:conf/iclr/KalyanMPBJG18, DBLP:journals/pacmpl/JiS0H20, DBLP:conf/cav/SinghG15, DBLP:conf/sigsoft/ChenMF19, DBLP:conf/icml/MenonTGLK13, DBLP:conf/icml/DevlinUBSMK17, DBLP:conf/pldi/LeeHAN18}. Though these approaches greatly improve the generalizability of PBE solvers in many applications, there is a lack of theory to explain their effectiveness. So far, the generalizability of a PBE solver can only be evaluated empirically on a dataset. Such a limitation makes it extremely difficult to design a generalizable PBE solver for those complex domains, where we have to make a trade-off between generalizability and other desired properties, such as efficiency.

To illustrate this point, we take the domain of \textit{Conditional Linear Integer Arithmetic (CLIA)} as an example. In CLIA, each program $p$ is either a linear expression over input variables or is in the form of $(\texttt{if }c\texttt{ then }p_1\texttt{ else }p_2)$, where $c$ is a linear inequality and $p_1, p_2$ are two programs in CLIA. Besides, all input variables and used constants are limited to integers. In practice, a CLIA program can be quite large, as it may use nested \texttt{if-then-else} operators to express a complex control flow. Therefore, CLIA is known to be a difficult domain for synthesizing, as it requires the synthesizer to be efficient enough to scale up to large programs. 

To design a PBE solver with good generalizability for CLIA, one main challenge is to make a trade-off between generalizability and efficiency. However, such a trade-off can be extremely difficult in practice, because we do not even have a theoretical definition for "good generalizability". 

\textit{Eusolver}~\cite{DBLP:conf/tacas/AlurRU17} is a state-of-the-art PBE solver for CLIA which takes generalizability as one of its design purposes. In \textit{Eusolver}, this trade-off is made in two steps: At first, \textit{Eusolver} uses \textit{STUN}~\cite{DBLP:conf/cav/AlurCR15}, a synthesis framework for nested \texttt{if-then-else} operators, to decompose the PBE task into two subproblems, and thus guarantee the efficiency. Secondly, to improve the generalizability, \textit{Eusolver} considers existing heuristics while solving subproblems. Though such a combination seems natural, we find that such a trade-off loses too much on generalizability. Let us take a simple synthesis task on CLIA as an example, where (1) $x$ is the only input variable, (2) the target program $p^*$ is $x + 1$, and (3) constants and inputs are limited within range $[0, 100]$. To synthesize $p^*$, \textit{Eusolver} uses $27.6$ random examples in average of $5$ invocations. In contrast, a heuristic solver that always selects the smallest program requires only $2$ examples on average. \todo{Wait for Jingtao to add results of CVC4}.

Motivated by these facts, in this paper, we set up a theoretical model for analyzing the generalizability of PBE solvers. In our model, we view a PBE task as a random variable generated from a random target program and a set of independent random inputs. Under such a perspective, the generalizability can be naturally defined as the least number of examples required by the PBE solver such that with a high probability, the synthesized program is gauranteed to be the target. 

However, such a definition is domain-specific. It relies on concrete distributions of the target program and the inputs, and concrete semantics of programs: All of them are usually unavailable while performing theoretical analysis. Therefore, the main challenge in modeling the generalizability is to propose an abstracted model, which (1) reflects the actual generalizability of PBE solvers, and at the same time, (2) is usable even when no concrete domain knowledge is provided. 

To ensure the effectiveness of the abstracted model, we keep in track of two primitive PBE solvers: the optimized solver $\mathcal S_{\text{min}}$, which always selects the smallest program satisfying all examples, and the random solver $\mathcal S_{\text{rand}}$, which returns a valid program randomly. There have been many evidences showing that the generalizability of $\mathcal S_{\text{min}}$ should be much better than $\mathcal S_{\text{rand}}$~\cite{DBLP:conf/icml/LiangJK10,DBLP:conf/popl/Gulwani11, DBLP:conf/popl/RaychevBVK16}, and thus we expect the abstracted model could discover the advantage of $\mathcal S_{\text{min}}$ against $\mathcal S_{\text{rand}}$ on generalizability.

One natural idea of the abstraction is to measure the maximal generalizability of a PBE solver on all possible distribution of PBE tasks. However, such an abstraction is meaningless, as there are some extreme distributions where generalizability of all possible solvers are extremely bad. Therefore, our abstracted model introduces two assumptions to exclude those extreme and unrealistic cases:
\begin{itemize}
	\item In some extreme cases, there may be an incorrect program that performs extremely close to the target. At this time, no matter what the PBE solver is, the number of examples used to distinguish between these two programs is always a bottleneck of the generalizability. Therefore, our first assumption excludes these  cases by assuming the probability for a random example to distinguish any two semantically different programs is at least a constant.
	\item We find that the generalizability of $\mathcal  S_{\text{min}}$ is better than $\mathcal S_{\text{rand}}$ only when the marginal distribution of the target program is biased to those syntactically small programs. Therefore, we take this condition as our second assumption to ensure the advantage of $\mathcal S_{\text{min}}$ in theory. Such an assumption can also be explained by the principle of Occam's Razor.
\end{itemize}

Then, under the abstracted model, we set up a target to represent "good generalizability". Motivated by the class of polynomial-time algorithms in the complexity theory, we propose the class of \textit{polynomial-size generalizability}, abbreviated as $\mathsf{PSG}$, containing all PBE solvers that are at most polynomially worse than $\mathcal S_{\text{min}}$ on generalizability. Though the constraints of $\mathsf{PSG}$ seems to be loose, we prove that $\mathsf{PSG}$ successfully distinguishes between $\mathcal S_{\text{min}}$ and $\mathcal S_{\text{rand}}$.

To evaluate the effectiveness of our abstracted model, we study the generalizability of the STUN framework in theory. On the one hand, we prove that $\textit{Eusolver}$ does not belong to $\mathsf{PSG}$. On the other hand, we prove a sufficient condition for the sub-solvers in the STUN framework to form a solver in $\mathsf{PSG}$. Guided by this sufficient condition, we design a STUN solver, namely \mainname, which is guaranteed to have polynomial-size generalizability in theory.

We instantiate \mainname to the domain CLIA, and evaluate~\todo{Wait for the evaluation}.

To sum up, this paper makes the following constributions:
\begin{itemize}
	\item An abstracted model that has ability to compare the general generalizability of PBE solvers in theory, and a class of PBE solvers, namely $\mathsf{PSG}$, which can be used as a target for "good generalizability" (Section \ref{section:model}).
	\item A theoretical study on the generalizability of the STUN framework (Section \ref{section:stun}).
	\item A novel STUN solver, \mainname, which is guaranteed to have polynomial-size generalizability (Section \ref{section:term-solver} and \ref{section:unifier}), and an instantiation of \mainname on CLIA (Section \ref{section:implementation}).
	\item \todo{Add Evaluation}.
\end{itemize}



==> sections/Introduction2.tex <==
%!TEX root = ../CLIA.tex
\section{Introduction} \label{section:introduction}
\textit{Programming by Example (PBE)}~\cite{DBLP:conf/ijcai/ShawWG75} is an important subproblem of program synthesis where the solver is required to learn a program from input-output examples. After decades of development, many general PBE solvers have been proposed~\cite{DBLP:conf/cav/AlurCR15, DBLP:conf/cav/ReynoldsBNBT19, DBLP:journals/pacmpl/WangDS18, DBLP:conf/oopsla/PolozovG15}, and these techniques have been applied to different domains\todo{citation}.%, such as string manipulation \cite{DBLP:conf/popl/Gulwani11, DBLP:conf/pldi/BarowyGHZ15}, data wrangling \cite{DBLP:conf/pldi/FengMGDC17, DBLP:conf/sigsoft/ChenMF19, DBLP:conf/pldi/YaghmazadehKDC16}, SQL queries \cite{DBLP:conf/pldi/WangCB17, DBLP:conf/kbse/ZhangS13}.

Oracle-guided inductive synthesis (OGIS)~\cite{DBLP:journals/acta/JhaS17} is a formal framework for modeling practical synthesis systems. In OGIS, the environment of a synthesizer is modeled as an oracle, and the synthesizer synthesizes programs by iteratively querying the oracle with questions such as whether a counter-example exists to show a given program is incorrect, or what is the correct output corresponding to a given input. Under the framework of OGIS, there are two major classes among applications of PBE techniques:
\begin{enumerate}[leftmargin=*]
	\item In the first class, the oracle can verify whether a given program is correct, and can provide a counter-example when the program is incorrect. A typical algorithm for this type is counter-example guided inductive synthesis (CEGIS)~\cite{DBLP:conf/asplos/Solar-LezamaTBSS06}, which iteratively convert an OGIS task into PBE tasks: In each term, CEGIS invokes a PBE solver to synthesize a program from existing examples, then it queries the oracle with the synthesized program. If it is wrong, a new example will be provided by the oracle, and then a new CEGIS iteration will start. \todo{add applications}
	\item In the second class, the oracle can provide the correct output for a given input. This class involves oracles that are black boxes, such as binary programs, or oracles that are programs too complex to analyze, such as program repair, second-order symbolic execution, deobfuscation. \todo{citation} At this time, a PBE solver is invoked on a few examples obtained from the oracle, and it is expected to synthesize a program that is correct on all possible inputs.
\end{enumerate}

For both cases, the generalizability of the PBE solver is a key fact on the practical performance. In the former case, generalizability significantly affects the efficiency of the solver: The fewer example required by the PBE solver to synthesize a correct program, the fewer CEGIS iterations will be, and thus the faster the whole OGIS system will be. In the latter case, the generalizability of the PBE solver determines the correctness of the whole OGIS system, as the oracle is not able to check whether a program is correct.

To improve generalizability for PBE solvers, a widely-used principle is to return the smallest program among all programs consistent with all examples~\cite{DBLP:conf/icml/LiangJK10,DBLP:conf/popl/Gulwani11, DBLP:conf/popl/RaychevBVK16}. This principle also corresponds to the general principle of Occam's Razor. However, applying this principle converts a synthesis task into an optimization task, which significantly increases the difficulty of designing efficient PBE solvers. As a result, this principle has not been adopted in many important domains due to the efficiency issue.

To illustrate this point, we take the domain of conditional linear integer arithmetic (CLIA) as an example. In CLIA, each program $p$ is either a linear expression over input variables or is in the form of $(\texttt{if }c\texttt{ then }p_1\texttt{ else }p_2)$, where $c$ is a linear inequality and $p_1, p_2$ are two programs in CLIA. Besides, all input variables and used constants are limited to integers. A distinguishing feature of CLIA is that a CLIA program can be very large in practice, as it may use nested \texttt{if-then-else} operators to express a complex control flow. Therefore, CLIA is known to be a difficult domain for synthesizing, as it requires the synthesizer to be efficient enough to scale up to large programs, and so far, applying the principle of synthesizing the minimal program to CLIA always leads to a significant loss on the performance:  According to the evaluation established by ~\citet{DBLP:conf/tacas/AlurRU17}, under a timeout set to one hour, \textit{Eusolver}~\cite{DBLP:conf/tacas/AlurRU17}, a state-of-the-art PBE solver on CLIA which does not always synthesize the minimal program, solves $117\%$ more benchmarks than \textit{Esolver}, the known best PBE solver on CLIA that guarantees the minimality of the result.

Our core insight of this paper is that to improve the generalizability, it is not necessary to require the synthesizer to return the smallest program: returning a small enough program could already lead to good generalizability. In this way, the requirement on the synthesized program is relaxed, and thus it is easier to design an efficient PBE solver. To formally characterize whether the synthesized program is small enough, we utilize a concept from the computational learning theory: Occam Learning~\cite{DBLP:journals/ipl/BlumerEHW87}.  Occam learning is also motivated by the principle of Occam's Razor, and its effectiveness has been widely justified in machine learning~\cite{DBLP:journals/ml/AngluinL87,DBLP:conf/stoc/KearnsL88,DBLP:journals/jcss/KearnsS94,DBLP:conf/colt/Natarajan93,DBLP:journals/iandc/AldousV95}. Under the scenario of PBE, a PBE solver is an Occam solver if the size of the synthesized program is guaranteed to be polynomial to the target program and sub-linear to the number of provided examples. The justify the effectiveness of Occam learning on PBE solvers, we prove that it can distinguish two primitive solvers: $\mathcal S_{\text{min}}$, which always synthesizes the smallest valid program, and $\mathcal S_{\text{rand}}$, which returns an arbitrary valid program randomly.

Based on Occam learning, we analyze the framework of \textit{synthesis through unification (STUN)}~\cite{DBLP:conf/cav/AlurCR15}, a state-of-the-art framework for synthesizing nested \texttt{if-then-else} operators, which is also the basis of \textit{Eusolver}. On the one hand, we prove that \textit{Eusolver} is not an Occam solver. On the other hand, we extend the concept of Occam learning to each component of STUN and provide a sufficient condition for these components to merge into an Occam solver. Guided by this sufficient condition, we design an Occam solver for the STUN framework, namely \mainname. \todo{explain the idea of \mainname, 4 parts decomposition}.

We instantiate \mainname to the domain CLIA, and evaluate~\todo{Wait for the evaluation}.


To sum up, this paper makes the following constributions:
\begin{itemize}
	\item We adopt the concept of Occam learning to the domain of PBE, and then estabilish a theoretical study on generalizability of the STUN framework and \textit{Eusolver} (Section \ref{section:stun}).
	\item We design a novel Occam solver for the STUN framework, namely \mainname (Section \ref{section:term-solver} and \ref{section:unifier}), and instantiatie \mainname to the domain of CLIA (Section \ref{section:implementation}).
	\item \todo{Add Evaluation}.
\end{itemize}
\endinput


\begin{itemize}
	%\item Oracle-guided inductive program synthesis is important. In OGIS, an oracle is queried with questions, such as whether a couterexample exists to show program $p$ is incorrect, or what output corresponds to input $i$. The oracle is usually an automated program, but can also be human.
	%\item Two main types of oracle exists. The first type is able to verify whether a program is correct, and produces a couterexample if it is not. A typical algorithm for this type is CEGIS. The second type is able to provide input-output examples. This involves oracles that are blackbox, such as binary programs, or oracles that are programs too complex to analyze, such as repair, second-order symbolic execution, deobfuscation, etc.
	%\item For either type, the generalizability of PBE is a key factor. In the former case, generalizability significantly affects the efficiency of the solver. In the latter case, generalizability determines correctness.
	%\item To ensure generalizability, a widely-used general principle is to return the smallest program (many citations). This principle also corresponds to the general principle of Occam's Razor. However, implementing this principle requires to solve an optimization problem, which is difficult to solve efficiently. As a matter of fact, all existing synthesizers that minimize the resulting program all work on small domains (true?). On many important domains it is still very hard to find the smallest program. For example, in the domain of CLIA. (Analyzing why minimizing program size on CLIA is hard?)
	%\item Our core insight of this paper is that we do not need to return the smallest program: returning a small enough program could already lead to good generalizability. To characterize whether a synthesizer returns a small enough program, we utilize a concept (generalizability class?) from the computational learning theory: Occam's learning. To demonstrate the effectiveness of Occam's learning, we show that $S_{min}$ and $S_{rand}$ could be distinguished.
	\item (not sure if a better motivation can be given to STUN and Eusolver) We analyze the generalizability of Eusolver, an efficient algorithm that works on the CLIA domain, based on Occam's learning. To perform this analysis, we extend Occam's learning to the STUN framework, the framework that Eusolver uses, and give a necessary condition for a STUN algorithm to be an Occam learning. Based on this extension, we show that neither eusolver nor any of its two components are Occam learning.
	\item We design a new STUN algorithm based on our extension, we prove that our algorithm is an Occam learning.
	\item We evaluate our approach on the CLIA benchmark, and found that...
	% \item However, designing an algorithm with good generalizability is hard. A fundamental difficulty raises from the fact that we still lack theoretical tools to compare the generalizability of different algorithms.
	% \item In this paper we give two theoretical contributions.
	% \begin{itemize}
	% 	\item Inspired by PAC, we propose a definition of generalizability for program synthesis. We found that the PAC setting that makes no assumption about the distribution of 
	% 	\item Inspired by complexity theory, we propose a polynomial-size generalizability class.
	% 	\item 
	% \end{itemize}
\end{itemize}

%\textit{Programming by Example (PBE)}~\cite{DBLP:conf/ijcai/ShawWG75} is an important subproblem of program synthesis where the solver is required to learn a program from input-output examples. PBE is useful for three main reasons: 
% There are three main reasons for the prevalence of PBE: 
%(1) In practice, input-output examples are usually easier to obtain than the general logic specifications, and many practical problems theirselves are instances of PBE; (2) For synthesizers and verifiers, the example-based specification in PBE is usually more tractable than general logic specifications; (3) In many cases, the general synthesis problem can be converted into PBE by CEGIS frameowrk~\cite{DBLP:conf/asplos/Solar-LezamaTBSS06}. After decades of development, many general PBE solvers have been proposed~\cite{DBLP:conf/cav/AlurCR15, DBLP:conf/cav/ReynoldsBNBT19, DBLP:journals/pacmpl/WangDS18, DBLP:conf/oopsla/PolozovG15}, and these techniques have been applied to different domains, such as string manipulation \cite{DBLP:conf/popl/Gulwani11, DBLP:conf/pldi/BarowyGHZ15}, data wrangling \cite{DBLP:conf/pldi/FengMGDC17, DBLP:conf/sigsoft/ChenMF19, DBLP:conf/pldi/YaghmazadehKDC16}, SQL queries \cite{DBLP:conf/pldi/WangCB17, DBLP:conf/kbse/ZhangS13}. 

%Despite many existing applications, generalizability remains one of the main challenges to apply PBE techniques~\cite{polozov2016program}. Because the example-based specification in PBE constraints only for a few inputs, there may be many different programs satisfying all given examples. At this time, the PBE solver should be able to infer the correct program from all these remaining ones. In practice, as it is usually costly to collect input-output examples, it is important for a PBE solver to have good generalizability: The fewer examples required to synthesize a correct program, the less cost invoking the PBE solver will be, and thus the more effective the PBE solver will be in practice. 

%There have been many heuristic methods proposed to improve the generalizability of PBE solvers. Some previous works guarantee the optimality of the synthesized program under some heuristic functions~\cite{DBLP:conf/icml/LiangJK10,DBLP:conf/popl/Gulwani11, DBLP:conf/popl/RaychevBVK16, DBLP:conf/icse/MechtaevYR15, DBLP:conf/cav/DAntoniSS16, DBLP:conf/sigsoft/LeCLGV17}, and some other works use learned models to guide the synthesis procedure, and thus focus only on probable programs~\cite{DBLP:conf/iclr/BalogGBNT17, DBLP:conf/iclr/KalyanMPBJG18, DBLP:journals/pacmpl/JiS0H20, DBLP:conf/cav/SinghG15, DBLP:conf/sigsoft/ChenMF19, DBLP:conf/icml/MenonTGLK13, DBLP:conf/icml/DevlinUBSMK17, DBLP:conf/pldi/LeeHAN18}. Though these approaches greatly improve the generalizability of PBE solvers in many applications, there is a lack of theory to explain their effectiveness. So far, the generalizability of a PBE solver can only be evaluated empirically on a dataset. Such a limitation makes it extremely difficult to design a generalizable PBE solver for those complex domains, where we have to make a trade-off between generalizability and other desired properties, such as efficiency.

%To illustrate this point, we take the domain of \textit{Conditional Linear Integer Arithmetic (CLIA)} as an example. In CLIA, each program $p$ is either a linear expression over input variables or is in the form of $(\texttt{if }c\texttt{ then }p_1\texttt{ else }p_2)$, where $c$ is a linear inequality and $p_1, p_2$ are two programs in CLIA. Besides, all input variables and used constants are limited to integers. In practice, a CLIA program can be quite large, as it may use nested \texttt{if-then-else} operators to express a complex control flow. Therefore, CLIA is known to be a difficult domain for synthesizing, as it requires the synthesizer to be efficient enough to scale up to large programs. 

%To design a PBE solver with good generalizability for CLIA, one main challenge is to make a trade-off between generalizability and efficiency. However, such a trade-off can be extremely difficult in practice, because we do not even have a theoretical definition for "good generalizability". 

%\textit{Eusolver}~\cite{DBLP:conf/tacas/AlurRU17} is a state-of-the-art PBE solver for CLIA which takes generalizability as one of its design purposes. In \textit{Eusolver}, this trade-off is made in two steps: At first, \textit{Eusolver} uses \textit{STUN}~\cite{DBLP:conf/cav/AlurCR15}, a synthesis framework for nested \texttt{if-then-else} operators, to decompose the PBE task into two subproblems, and thus guarantee the efficiency. Secondly, to improve the generalizability, \textit{Eusolver} considers existing heuristics while solving subproblems. Though such a combination seems natural, we find that such a trade-off loses too much on generalizability. Let us take a simple synthesis task on CLIA as an example, where (1) $x$ is the only input variable, (2) the target program $p^*$ is $x + 1$, and (3) constants and inputs are limited within range $[0, 100]$. To synthesize $p^*$, \textit{Eusolver} uses $27.6$ random examples in average of $5$ invocations. In contrast, a heuristic solver that always selects the smallest program requires only $2$ examples on average. \todo{Wait for Jingtao to add results of CVC4}.

Motivated by these facts, in this paper, we set up a theoretical model for analyzing the generalizability of PBE solvers. In our model, we view a PBE task as a random variable generated from a random target program and a set of independent random inputs. Under such a perspective, the generalizability can be naturally defined as the least number of examples required by the PBE solver such that with a high probability, the synthesized program is gauranteed to be the target. 

However, such a definition is domain-specific. It relies on concrete distributions of the target program and the inputs, and concrete semantics of programs: All of them are usually unavailable while performing theoretical analysis. Therefore, the main challenge in modeling the generalizability is to propose an abstracted model, which (1) reflects the actual generalizability of PBE solvers, and at the same time, (2) is usable even when no concrete domain knowledge is provided. 

To ensure the effectiveness of the abstracted model, we keep in track of two primitive PBE solvers: the optimized solver $\mathcal S_{\text{min}}$, which always selects the smallest program satisfying all examples, and the random solver $\mathcal S_{\text{rand}}$, which returns a valid program randomly. There have been many evidences showing that the generalizability of $\mathcal S_{\text{min}}$ should be much better than $\mathcal S_{\text{rand}}$~\cite{DBLP:conf/icml/LiangJK10,DBLP:conf/popl/Gulwani11, DBLP:conf/popl/RaychevBVK16}, and thus we expect the abstracted model could discover the advantage of $\mathcal S_{\text{min}}$ against $\mathcal S_{\text{rand}}$ on generalizability.

One natural idea of the abstraction is to measure the maximal generalizability of a PBE solver on all possible distribution of PBE tasks. However, such an abstraction is meaningless, as there are some extreme distributions where generalizability of all possible solvers are extremely bad. Therefore, our abstracted model introduces two assumptions to exclude those extreme and unrealistic cases:
\begin{itemize}
	\item In some extreme cases, there may be an incorrect program that performs extremely close to the target. At this time, no matter what the PBE solver is, the number of examples used to distinguish between these two programs is always a bottleneck of the generalizability. Therefore, our first assumption excludes these  cases by assuming the probability for a random example to distinguish any two semantically different programs is at least a constant.
	\item We find that the generalizability of $\mathcal  S_{\text{min}}$ is better than $\mathcal S_{\text{rand}}$ only when the marginal distribution of the target program is biased to those syntactically small programs. Therefore, we take this condition as our second assumption to ensure the advantage of $\mathcal S_{\text{min}}$ in theory. Such an assumption can also be explained by the principle of Occam's Razor.
\end{itemize}

Then, under the abstracted model, we set up a target to represent "good generalizability". Motivated by the class of polynomial-time algorithms in the complexity theory, we propose the class of \textit{polynomial-size generalizability}, abbreviated as $\mathsf{PSG}$, containing all PBE solvers that are at most polynomially worse than $\mathcal S_{\text{min}}$ on generalizability. Though the constraints of $\mathsf{PSG}$ seems to be loose, we prove that $\mathsf{PSG}$ successfully distinguishes between $\mathcal S_{\text{min}}$ and $\mathcal S_{\text{rand}}$.

To evaluate the effectiveness of our abstracted model, we study the generalizability of the STUN framework in theory. On the one hand, we prove that $\textit{Eusolver}$ does not belong to $\mathsf{PSG}$. On the other hand, we prove a sufficient condition for the sub-solvers in the STUN framework to form a solver in $\mathsf{PSG}$. Guided by this sufficient condition, we design a STUN solver, namely \mainname, which is guaranteed to have polynomial-size generalizability in theory.

We instantiate \mainname to the domain CLIA, and evaluate~\todo{Wait for the evaluation}.

To sum up, this paper makes the following constributions:
\begin{itemize}
	\item An abstracted model that has ability to compare the general generalizability of PBE solvers in theory, and a class of PBE solvers, namely $\mathsf{PSG}$, which can be used as a target for "good generalizability" (Section \ref{section:model}).
	\item A theoretical study on the generalizability of the STUN framework (Section \ref{section:stun}).
	\item A novel STUN solver, \mainname, which is guaranteed to have polynomial-size generalizability (Section \ref{section:term-solver} and \ref{section:unifier}), and an instantiation of \mainname on CLIA (Section \ref{section:implementation}).
	\item \todo{Add Evaluation}.
\end{itemize}



==> sections/Introduction3.tex <==
%!TEX root = ../CLIA.tex
\section{Introduction} \label{section:introduction}

%\smalltitle{OGIS, PBE and Generalizability}
In the past decades, oracle-guided inductive program synthesis (OGIS)~\cite{DBLP:journals/acta/JhaS17} receives much attention. In each iteration of OGIS, an oracle provides input-output examples to an inductive program synthesizer, or programming-by-example (PBE) synthesizer~\cite{DBLP:conf/ijcai/ShawWG75}, and the PBE synthesizer generates a program based on the examples. There are two typical types of OGIS problems. In the first type, the oracle is able to verify whether the synthesized program is correct, and provides a counter-example if the program is incorrect. The many applications under the counter-example guided inductive synthesis (CEGIS) framework\todo{citation} falls into this type. In the second type, the oracle cannot verify the correctness of the synthesized program but is only able to provide a set of input-output examples. This includes the applications where the oracle is a black-box program, such as binary programs\todo{citations}, and applications where the program is too complex to verify its correctness, e.g., the task involves system calls or complex loops, such as program repair, second-order execution, and deobfuscation\todo{citations}. 

In both type of problems, generalizability of the PBE solver is the key to synthesis performance. In the first type, generalizability significantly affects the efficiency: the fewer examples the solver needs to synthesize a correct program, the fewer CEGIS iterations the synthesis requires, and thus the faster the synthesis would be. In the second type, the generalizability of the PBE solver decides the correctness of the whole OGIS system.

However, so far in program synthesis studies the generalizability of a PBE solver is evaluated empirically. We still lack theoretical understanding of the generalizability of PBE solvers, and the design of the new PBE solvers were not accompanied by theoretical guarantee on generalizability.

% However, achieving generalizability is not easy. For example, a basic principle to generalizability is Occam's Razor, which requires to return the simplest solution. In the domain of program synthesis, simplicity is often measured by program size. However, to return the smallest program is to solve an optimization problem, which significantly increases the difficulty of designing efficient PBE solvers. As a result, in many important domains we do not have efficient PBE solvers that return the smallest program consistent with the input-output examples. 

% \smalltitle{STUN and Generalizability}
% In this paper we concern an important family of program synthesis approaches, \emph{synthesis through unification} (STUN)~\cite{DBLP:conf/cav/AlurCR15}, and shall demonstrate why it is difficult to build an efficient solver that returns the smallest program in the domain of STUN. STUN is a framework for synthesizing nested \code{if-then-else} programs, and the solvers based on STUN such as Eusolver~\cite{DBLP:conf/tacas/AlurRU17} and Euphony~\cite{DBLP:conf/pldi/LeeHAN18} achieve the state-of-the-art results on many important benchmarks such as the CLIA track in the SyGUS competition. 

In this paper, we adopt a concept from the computational learning theory, Occam learning~\cite{DBLP:journals/ipl/BlumerEHW87}. Occam learning is inspired by Occam's razor, and provides a condition to examine whether a synthesizer favors smaller program than larger programs, a principle that is widely-believed to lead to generalizability. \yxcomment{Please check if this contribution (the remaining sentences of this paragraph) is significant enough to appear in the introduction. The problem is that, this statement tries to justify the usefulness of Occam learning with only one example, and this example falls exactly into its definition. Yet removing this, the contribution of "adapting Occam learning" becomes too small to be stated as a general contribution to PBE.} We demonstrate that, Occam learning is able to distinguish two primitive PBE solvers: $\mathcal S_{\text{rand}}$, which returns an arbitrary valid program randomly, and $\mathcal S_{\text{min}}$, which always synthesizes the smallest valid program and is widely-recognized to be better generalizable than $\mathcal S_{\text{rand}}$. On the other hand, PAC learning, another widely-used condition for generalizability, is unable to distinguish the two solvers.

%\smalltitle{STUN}
In this paper we concern an important family of program synthesis approaches, \emph{synthesis through unification} (STUN)~\cite{DBLP:conf/cav/AlurCR15}. STUN is a framework for synthesizing nested \code{if-then-else} programs, and the solvers based on STUN such as Eusolver~\cite{DBLP:conf/tacas/AlurRU17} and Euphony~\cite{DBLP:conf/pldi/LeeHAN18} achieve the state-of-the-art results on many important benchmarks such as the CLIA track in the SyGUS competition. 

Based on Occam learning, we analyze a state-of-the-art STUN algorithm, Eusolver~\cite{DBLP:conf/tacas/AlurRU17}, and prove that \textit{Eusolver} is not an Occam solver, i.e., does not meet the condition of Occam learning. To design an Occam solver under the STUN framework, we further analyze the framework and divide the condition of Occam learning into a set of conditions, one for each component in the STUN framework, that together sufficiently guarantee the STUN solver to be an Occam solver. Guided by these conditions, we design an Occam solver based on STUN, namely \mainname, by designing each component individually to satisfy the respective condition.

We instantiate \mainname to the domain CLIA\yxcomment{Not sure if this name is a good one, as it is also a benchmark name, and the reader may confuse the two}, and evaluate~\todo{Wait for the evaluation}.

To sum up, this paper makes the following contributions:
\begin{itemize}
	\item {\it Theoretical contribution.} We adopt the concept of Occam learning to the domain of PBE, prove that \textit{Eusolver} is not an Occam solver, and provides a sufficient set of conditions for individual components in the STUN framework to form an Occam solver (Section \ref{section:stun}).
	%	and establish a theoretical study on generalizability of the STUN framework and \textit{Eusolver} (Section \ref{section:stun}).
	\item {\it Algorithmic contribution.} We design a novel Occam solver based on the STUN framework, namely \mainname (Section \ref{section:term-solver} and \ref{section:unifier}).
	\item {\it Empirical contribution.} We instantiate \mainname to the domain of CLIA (Section \ref{section:implementation}) and \todo{Add Evaluation}.
\end{itemize}
\endinput


\begin{itemize}
	%\item Oracle-guided inductive program synthesis is important. In OGIS, an oracle is queried with questions, such as whether a couterexample exists to show program $p$ is incorrect, or what output corresponds to input $i$. The oracle is usually an automated program, but can also be human.
	%\item Two main types of oracle exists. The first type is able to verify whether a program is correct, and produces a couterexample if it is not. A typical algorithm for this type is CEGIS. The second type is able to provide input-output examples. This involves oracles that are blackbox, such as binary programs, or oracles that are programs too complex to analyze, such as repair, second-order symbolic execution, deobfuscation, etc.
	%\item For either type, the generalizability of PBE is a key factor. In the former case, generalizability significantly affects the efficiency of the solver. In the latter case, generalizability determines correctness.
	%\item To ensure generalizability, a widely-used general principle is to return the smallest program (many citations). This principle also corresponds to the general principle of Occam's Razor. However, implementing this principle requires to solve an optimization problem, which is difficult to solve efficiently. As a matter of fact, all existing synthesizers that minimize the resulting program all work on small domains (true?). On many important domains it is still very hard to find the smallest program. For example, in the domain of CLIA. (Analyzing why minimizing program size on CLIA is hard?)
	%\item Our core insight of this paper is that we do not need to return the smallest program: returning a small enough program could already lead to good generalizability. To characterize whether a synthesizer returns a small enough program, we utilize a concept (generalizability class?) from the computational learning theory: Occam's learning. To demonstrate the effectiveness of Occam's learning, we show that $S_{min}$ and $S_{rand}$ could be distinguished.
	\item (not sure if a better motivation can be given to STUN and Eusolver) We analyze the generalizability of Eusolver, an efficient algorithm that works on the CLIA domain, based on Occam's learning. To perform this analysis, we extend Occam's learning to the STUN framework, the framework that Eusolver uses, and give a necessary condition for a STUN algorithm to be an Occam learning. Based on this extension, we show that neither eusolver nor any of its two components are Occam learning.
	\item We design a new STUN algorithm based on our extension, we prove that our algorithm is an Occam learning.
	\item We evaluate our approach on the CLIA benchmark, and found that...
	% \item However, designing an algorithm with good generalizability is hard. A fundamental difficulty raises from the fact that we still lack theoretical tools to compare the generalizability of different algorithms.
	% \item In this paper we give two theoretical contributions.
	% \begin{itemize}
	% 	\item Inspired by PAC, we propose a definition of generalizability for program synthesis. We found that the PAC setting that makes no assumption about the distribution of 
	% 	\item Inspired by complexity theory, we propose a polynomial-size generalizability class.
	% 	\item 
	% \end{itemize}
\end{itemize}

%\textit{Programming by Example (PBE)}~\cite{DBLP:conf/ijcai/ShawWG75} is an important subproblem of program synthesis where the solver is required to learn a program from input-output examples. PBE is useful for three main reasons: 
% There are three main reasons for the prevalence of PBE: 
%(1) In practice, input-output examples are usually easier to obtain than the general logic specifications, and many practical problems theirselves are instances of PBE; (2) For synthesizers and verifiers, the example-based specification in PBE is usually more tractable than general logic specifications; (3) In many cases, the general synthesis problem can be converted into PBE by CEGIS frameowrk~\cite{DBLP:conf/asplos/Solar-LezamaTBSS06}. After decades of development, many general PBE solvers have been proposed~\cite{DBLP:conf/cav/AlurCR15, DBLP:conf/cav/ReynoldsBNBT19, DBLP:journals/pacmpl/WangDS18, DBLP:conf/oopsla/PolozovG15}, and these techniques have been applied to different domains, such as string manipulation \cite{DBLP:conf/popl/Gulwani11, DBLP:conf/pldi/BarowyGHZ15}, data wrangling \cite{DBLP:conf/pldi/FengMGDC17, DBLP:conf/sigsoft/ChenMF19, DBLP:conf/pldi/YaghmazadehKDC16}, SQL queries \cite{DBLP:conf/pldi/WangCB17, DBLP:conf/kbse/ZhangS13}. 

%Despite many existing applications, generalizability remains one of the main challenges to apply PBE techniques~\cite{polozov2016program}. Because the example-based specification in PBE constraints only for a few inputs, there may be many different programs satisfying all given examples. At this time, the PBE solver should be able to infer the correct program from all these remaining ones. In practice, as it is usually costly to collect input-output examples, it is important for a PBE solver to have good generalizability: The fewer examples required to synthesize a correct program, the less cost invoking the PBE solver will be, and thus the more effective the PBE solver will be in practice. 

%There have been many heuristic methods proposed to improve the generalizability of PBE solvers. Some previous works guarantee the optimality of the synthesized program under some heuristic functions~\cite{DBLP:conf/icml/LiangJK10,DBLP:conf/popl/Gulwani11, DBLP:conf/popl/RaychevBVK16, DBLP:conf/icse/MechtaevYR15, DBLP:conf/cav/DAntoniSS16, DBLP:conf/sigsoft/LeCLGV17}, and some other works use learned models to guide the synthesis procedure, and thus focus only on probable programs~\cite{DBLP:conf/iclr/BalogGBNT17, DBLP:conf/iclr/KalyanMPBJG18, DBLP:journals/pacmpl/JiS0H20, DBLP:conf/cav/SinghG15, DBLP:conf/sigsoft/ChenMF19, DBLP:conf/icml/MenonTGLK13, DBLP:conf/icml/DevlinUBSMK17, DBLP:conf/pldi/LeeHAN18}. Though these approaches greatly improve the generalizability of PBE solvers in many applications, there is a lack of theory to explain their effectiveness. So far, the generalizability of a PBE solver can only be evaluated empirically on a dataset. Such a limitation makes it extremely difficult to design a generalizable PBE solver for those complex domains, where we have to make a trade-off between generalizability and other desired properties, such as efficiency.

%To illustrate this point, we take the domain of \textit{Conditional Linear Integer Arithmetic (CLIA)} as an example. In CLIA, each program $p$ is either a linear expression over input variables or is in the form of $(\texttt{if }c\texttt{ then }p_1\texttt{ else }p_2)$, where $c$ is a linear inequality and $p_1, p_2$ are two programs in CLIA. Besides, all input variables and used constants are limited to integers. In practice, a CLIA program can be quite large, as it may use nested \texttt{if-then-else} operators to express a complex control flow. Therefore, CLIA is known to be a difficult domain for synthesizing, as it requires the synthesizer to be efficient enough to scale up to large programs. 

%To design a PBE solver with good generalizability for CLIA, one main challenge is to make a trade-off between generalizability and efficiency. However, such a trade-off can be extremely difficult in practice, because we do not even have a theoretical definition for "good generalizability". 

%\textit{Eusolver}~\cite{DBLP:conf/tacas/AlurRU17} is a state-of-the-art PBE solver for CLIA which takes generalizability as one of its design purposes. In \textit{Eusolver}, this trade-off is made in two steps: At first, \textit{Eusolver} uses \textit{STUN}~\cite{DBLP:conf/cav/AlurCR15}, a synthesis framework for nested \texttt{if-then-else} operators, to decompose the PBE task into two subproblems, and thus guarantee the efficiency. Secondly, to improve the generalizability, \textit{Eusolver} considers existing heuristics while solving subproblems. Though such a combination seems natural, we find that such a trade-off loses too much on generalizability. Let us take a simple synthesis task on CLIA as an example, where (1) $x$ is the only input variable, (2) the target program $p^*$ is $x + 1$, and (3) constants and inputs are limited within range $[0, 100]$. To synthesize $p^*$, \textit{Eusolver} uses $27.6$ random examples in average of $5$ invocations. In contrast, a heuristic solver that always selects the smallest program requires only $2$ examples on average. \todo{Wait for Jingtao to add results of CVC4}.

Motivated by these facts, in this paper, we set up a theoretical model for analyzing the generalizability of PBE solvers. In our model, we view a PBE task as a random variable generated from a random target program and a set of independent random inputs. Under such a perspective, the generalizability can be naturally defined as the least number of examples required by the PBE solver such that with a high probability, the synthesized program is gauranteed to be the target. 

However, such a definition is domain-specific. It relies on concrete distributions of the target program and the inputs, and concrete semantics of programs: All of them are usually unavailable while performing theoretical analysis. Therefore, the main challenge in modeling the generalizability is to propose an abstracted model, which (1) reflects the actual generalizability of PBE solvers, and at the same time, (2) is usable even when no concrete domain knowledge is provided. 

To ensure the effectiveness of the abstracted model, we keep in track of two primitive PBE solvers: the optimized solver $\mathcal S_{\text{min}}$, which always selects the smallest program satisfying all examples, and the random solver $\mathcal S_{\text{rand}}$, which returns a valid program randomly. There have been many evidences showing that the generalizability of $\mathcal S_{\text{min}}$ should be much better than $\mathcal S_{\text{rand}}$~\cite{DBLP:conf/icml/LiangJK10,DBLP:conf/popl/Gulwani11, DBLP:conf/popl/RaychevBVK16}, and thus we expect the abstracted model could discover the advantage of $\mathcal S_{\text{min}}$ against $\mathcal S_{\text{rand}}$ on generalizability.

One natural idea of the abstraction is to measure the maximal generalizability of a PBE solver on all possible distribution of PBE tasks. However, such an abstraction is meaningless, as there are some extreme distributions where generalizability of all possible solvers are extremely bad. Therefore, our abstracted model introduces two assumptions to exclude those extreme and unrealistic cases:
\begin{itemize}
	\item In some extreme cases, there may be an incorrect program that performs extremely close to the target. At this time, no matter what the PBE solver is, the number of examples used to distinguish between these two programs is always a bottleneck of the generalizability. Therefore, our first assumption excludes these  cases by assuming the probability for a random example to distinguish any two semantically different programs is at least a constant.
	\item We find that the generalizability of $\mathcal  S_{\text{min}}$ is better than $\mathcal S_{\text{rand}}$ only when the marginal distribution of the target program is biased to those syntactically small programs. Therefore, we take this condition as our second assumption to ensure the advantage of $\mathcal S_{\text{min}}$ in theory. Such an assumption can also be explained by the principle of Occam's Razor.
\end{itemize}

Then, under the abstracted model, we set up a target to represent "good generalizability". Motivated by the class of polynomial-time algorithms in the complexity theory, we propose the class of \textit{polynomial-size generalizability}, abbreviated as $\mathsf{PSG}$, containing all PBE solvers that are at most polynomially worse than $\mathcal S_{\text{min}}$ on generalizability. Though the constraints of $\mathsf{PSG}$ seems to be loose, we prove that $\mathsf{PSG}$ successfully distinguishes between $\mathcal S_{\text{min}}$ and $\mathcal S_{\text{rand}}$.

To evaluate the effectiveness of our abstracted model, we study the generalizability of the STUN framework in theory. On the one hand, we prove that $\textit{Eusolver}$ does not belong to $\mathsf{PSG}$. On the other hand, we prove a sufficient condition for the sub-solvers in the STUN framework to form a solver in $\mathsf{PSG}$. Guided by this sufficient condition, we design a STUN solver, namely \mainname, which is guaranteed to have polynomial-size generalizability in theory.

We instantiate \mainname to the domain CLIA, and evaluate~\todo{Wait for the evaluation}.

To sum up, this paper makes the following constributions:
\begin{itemize}
	\item An abstracted model that has ability to compare the general generalizability of PBE solvers in theory, and a class of PBE solvers, namely $\mathsf{PSG}$, which can be used as a target for "good generalizability" (Section \ref{section:model}).
	\item A theoretical study on the generalizability of the STUN framework (Section \ref{section:stun}).
	\item A novel STUN solver, \mainname, which is guaranteed to have polynomial-size generalizability (Section \ref{section:term-solver} and \ref{section:unifier}), and an instantiation of \mainname on CLIA (Section \ref{section:implementation}).
	\item \todo{Add Evaluation}.
\end{itemize}



==> sections/MotivateExample.tex <==
%!TEX root = ../CLIA.tex
\section{Overview} \label{section:example}
In this section, we introduce the basic idea of our appraoch via an example adopted from benchmark \texttt{mpg\_ite2.sl} in the SyGuS competition. The target program $p^*$ is shown as the following, where $x, y, z$ are two integer inputs.%, and $\texttt{ite}$ represents the \texttt{if-then-else} operator. 
\begin{align*}
	%p^*(x, y, z) \coloneqq& \texttt{(ite (>= (+ x y) 1)}\\
	%&\ \ \ \  \texttt{(ite (>= (+ x z) 1) (+ x 1) (+ y 1))} \\
	%&\ \ \ \  \texttt{(ite (>= (+ y z) 1) (+ x 1) (+ y 1)))}
	p^*(x, y, z) \coloneqq & \texttt{ if }(x + y \geq 1)\texttt{ then }\{ \\
	& \ \ \ \ \texttt{ if }(x + z \geq 1)\texttt{ then }\{x + 1\}\texttt{ else }\{y + 1\} \\ 
	& \texttt{ }\}\texttt{ else }\{ \\
	& \ \ \ \ \texttt{ if }(y + z \geq 1)\texttt{ then }\{z + 1\}\texttt{ else }\{y + 1\} \\ 
	& \texttt{ }\}
\end{align*}   
We assume that there are $9$ input-output examples provided to the PBE solver. Table \ref{table:examples} lists these examples, where tuple $(x_0, y_0, z_0)$ in column $I$ represents an input where $x,y,z$ are set to $x_0,y_0,z_0$ respectively, and the \texttt{if}-term in column \textit{Term} represents the executed branch on each example.

\begin{table*}[!htbp]
	
	\caption{The input-output examples that are available for the PBE solver.} \label{table:examples}
	\begin{spacing}{1.1}
		\small
		\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
			\hline
			ID & $I$ & $O$ & Term & ID & $I$ & $O$ & Term & ID & $I$ & $O$ & Term\\
			\hline
			$e_1$ & $(0, 1, 2)$ & $1$ & \multirow{3}{*}{$x + 1$} &$e_4$ & $(0, 2, 0)$ & $3$ & \multirow{3}{*}{$y + 1$} &$e_7$ & $(0, 0, 1)$ & $2$ & \multirow{3}{*}{$y + 1$} \\
			\cline{1-3} \cline{5-7} \cline{9-11}
			$e_2$ & $(1, 0, 2)$ & $2$ & & $e_5$ & $(-1, 3, 0)$ & $4$ & & $e_8$ & $(-3, 3, -2)$ & $-1$ & \\
			\cline{1-3} \cline{5-7} \cline{9-11}
			$e_3$ & $(-1, 3, 2)$ & $0$ & & $e_6$ & $(-1, 1, -1)$ & $2$ & & $e_9$ & $(-1, 0, 4)$ & $5$ & \\
			\hline
		\end{tabular}
	\end{spacing}
\end{table*}

\subsection{\textit{Eusolver}}
In short, Occam Learning requires the PBE solver to return a program that is not much larger than the target program in size. In this section, we shall briefly show why \textit{Eusolver}, a state-of-the-art solver on CLIA, is not an Occam solver via the motivating example.

\textit{Eusolver} is based on the STUN framework. In STUN, programs with \texttt{if-then-else} operators are synthesized in two steps. At first, a term solver is invoked to synthesize a set of \texttt{if}-terms, which is enough to cover all given input-output examples. One ideal result of the term solver is the set of terms used by the target program, denoted as $P^*$. In this example, $P^* = \{x + 1, y +1, z + 1\}$. Then, a unifier is invoked to use \texttt{if-then-else} operators to unify these terms into a program satisfying all examples. In this example, one valid solution for term set $P^*$ is the target program $p^*$ itself.

In \textit{Eusolver}, the term solver $\mathcal T_E$ enumerates all possible terms in the increasing order of the size. A term will be included in the result if the set of examples it covers is different from all smaller terms. The enumeration ends when collected terms are enough to cover all given examples. As $\mathcal T_E$ does not control the number of collected terms, it may return an extremely large set: In this example, when the term is allowed to use $-1, \dots, 5$ as constants, $\mathcal T_E$ will return set $\{-1, 0, \dots, 5\}$, as the size of constants is smaller than expressions in $P^*$. To unify these constants into a valid program, \textit{Eusolver} has to use complex \texttt{if}-conditions, and thus the synthesized program can be much larger than $p^*$.

The unifier $\mathcal U_E$ in \textit{Eusolver} is based on \textit{ID3}, a learning algorithm for decision trees. As \textit{ID3} does not guarantee the learned decision tree to be small, the program synthesized by $\mathcal U_E$ can still be much larger than $p^*$ even when the term set is small. In this example, if the term set is exactly $P^*$ and there are only $4$ available \texttt{if}-conditions: $x + y \geq 1$, $x + z \geq 1$, $y + z \geq 1$ and $z \leq 0$, $\mathcal U_{\text{poly}}$ will misuse $z \leq 0$ as the outmost \texttt{if}-condition. As a result, $\mathcal U_E$ will use two extra \texttt{if-then-else} operators to form a valid program.

In summary, \textit{Eusolver} is not likely to be an Occam solver, as neither term solver $\mathcal T_E$ nor unifier $\mathcal U_E$ guarantees the result to be small. We formally prove this point in Section \ref{section:gen-eusolver}.

\subsection{Term solver $\mathcal T_{\text{poly}}$ in \mainname}
Our approach, \mainname, is also based on the STUN framework. Both the term solver $\mathcal T_{\text{poly}}$ and the unifier $\mathcal U_{\text{poly}}$ used in \mainname focus on small solutions, and thus \mainname is designed to be an Occam solver. In this section, we introduce the main idea of $\mathcal T_{\text{poly}}$ via the motivating example.

The goal of $\mathcal T_{\text{poly}}$ is to find a term set that is similar to $P^*$. Let $t^* \in P^*$ be the most effective term, i.e., $t^*$ is the term that covers the most examples among $P^*$. In the first step, $\mathcal T_{\text{poly}}$ would like to find a term $t_0$ that is similar to $t^*$:
\begin{enumerate}
	\item To reduce the number of synthesized terms, $t_0$ should cover as many examples as possible, and thus $t_0$ should be semantically close to $t^*$.
	\item To bound the size of synthesized terms, the size of $t_0$ should not be much larger than $t^*$.
\end{enumerate}
The main insight used by $\mathcal T_{\text{poly}}$ is that both of these requirements can be achieved via an Occam solver $\mathcal S_t$ on the term domain. If we invoked $\mathcal S_t$ on a PBE task corresponding to $t^*$, the synthesized term will satisfy these two conditions with a high probability, as an Occam solver is guaranteed to (1) have good generalizability, and (2) synthesize programs with bounded size.

In this example, $t^*$ can be taken as $x + 1$, and $\mathcal S_t$ can be implemented as an optimized PBE solver that always finds the simplest valid term via linear integer programming, as the \texttt{if}-terms can only be linear integer expressions. More details on this domain solver can be found in Section \ref{section:implementation}. Clearly, $t^*$ can be immediately obtained by invoking $\mathcal S_t$ on any two examples among $\{e_1, e_2, e_3\}$.

The only problem remaining is how to get a PBE task $T$ corresponding to $t^*$. On the one hand, by the generalizability of $\mathcal S_t$, a few examples are enough. On the other hand, as $t^*$ is the most effective term in $P^*$, there is a large portion of examples corresponding to $t^*$. Therefore, $\mathcal T_{\text{poly}}$ obtains $T$ by random sampling: In each turn, $\mathcal T_{\text{poly}}$ invokes $\mathcal S_t$ on a small set of random examples. When the number of sampling turns is large enough, with a high probability, there will be a valid invocation of $\mathcal S_t$ where all selected examples correspond to $t^*$. Moreover, in other cases where some example corresponding to another term is selected, the synthesis result $t$ can often be excluded using the following two prune-off rules:
\begin{itemize}
	\item $t$ should cover a large portion of examples. For example, when $\{e_1, e_8\}$ are selected, $t$ will be $2z-3$. However, as $t$ fails in covering any other examples, $t$ can be ignored directly.
	\item $t$ should not be very complex. For example, when $\{e_3, e_5, e_9\}$ are selected, $t$ will be $4x-y+z+5$. Such a $t$ is much more complex than many other candidates such as $x + 1$, and thus can be ignored temporarily.
\end{itemize}
Therefore, after the sampling process, $\mathcal T_{\text{poly}}$ obtains a small set of candidate terms. $\mathcal T_{\text{poly}}$ will recursively try each of them. For example, when the selected term is $x + 1$, $\mathcal T_{\text{poly}}$ will recurse into a subproblem where the examples are $\{e_4, e_5, \dots, e_9\}$. 
\subsection{Unifier $\mathcal U_{\text{poly}}$ in \mainname}
Instead of the decision tree used by \textit{Eusolver}, $\mathcal U_{\text{poly}}$ unifies the terms into a decision list, of which the structure of nested \texttt{if-then-else} operators is guaranteed to be linear. In this example, when the term set found by $\mathcal T_{\text{poly}}$ is exactly $P^*$, $\mathcal U_{\text{poly}}$ will synthesize two conditions $c_1, c_2$ and unifies $P^*$ into the following program:
\begin{align*}
	p(x, y, z) \coloneqq& \texttt{ if }(c_1)\texttt{ then }\{x + 1\}\texttt{ else if }(c_2)\texttt{ then }\{y + 1\}\texttt{ else }\{z + 1\} 
\end{align*}   
One valid solution here is that: 
$$c_1^*= (x + y \geq 1) \texttt{ and }(x +z \geq 1)\ \ \ \ \ c_2^* =  (x + y \geq 1) \texttt{ or }(y + z < 1)$$

At first, $\mathcal U_{\text{poly}}$ constructs PBE tasks for $e_1$ and $e_2$ in order. At first, as $x + 1$ only covers examples $e_1, e_2$ and $e_3$, $c_1$ should be \texttt{true} on $\{e_1, e_2, e_3\}$ and be \texttt{flase} on $\{e_4, e_5, \dots, e_9\}$. Similarly, $c_2$ should be \texttt{true} on $\{e_4, e_5, e_6\}$, and be \texttt{false} on $\{e_7,e_8,e_9\}$.

Then, $\mathcal U_{\text{poly}}$ solves these PBE tasks separately. In this example, we assume that there only $5$ literals $l_1, \dots, l_5$ available for $\mathcal U_{\text{poly}}$: $l_1 \coloneqq (x + y \geq 1), l_2\coloneqq (x + z \geq 1), l_3 \coloneqq (y + z < 1), l_4 \coloneqq (x + y \geq 0)$ and $l_5 \coloneqq (z \leq 0)$. $\mathcal U_{\text{poly}}$ synthesizes conditions in the disjuctive normal form, i.e., the result condition is always in the form of $\left(\texttt{or}_{C_i} \left(\texttt{and}_{l \in C_i}\ l\right)\right)$, where $C_i \subseteq \{l_1, \dots, l_5\}$ represents a series of clauses. To bound the size of the synthesized condition, $\mathcal U_{\text{poly}}$ requires an upper bound $k$ on the maximal number of clauses. In this example, for simplicity, we assume the value of $k$ is given, which is equal to $1$ for condition $c_1$ and euqal to $2$ for condition $c_2$.

\textbf{Synthesizing condition $c_1$}. Under upper bound $k = 1$, $\mathcal U_{\text{poly}}$ is required to synthesize a single clause $C \subseteq \{l_1, \dots, l_5\}$. As $c_1$ should be \texttt{true} on examples $\{e_1, e_2, e_3\}$, all literals in $C$ must also be \texttt{true} on these examples. Therefore, literal $l_3$ and $l_5$ can excluded. Besides, as $c_1$ should be \texttt{false} on examples $\{e_4, \dots, e_9\}$, for each negative example $e$ among them, there should be at least one literal in $C$ that takes \texttt{false} on $e$. Meanwhile, to bound the size of the synthesized condition, we would like the size of literal $C$ to be as small as possible. Such a problem is an instance of \textit{weighted set covering}, a well-known $\mathsf{NP}$-Hard problem. Therefore $\mathcal U_{\text{poly}}$ uses a standard greedy algorithm to find an approximated solution: In each turn, $\mathcal U_{\text{poly}}$ adds the literal that covers the most uncovered negative example on average of each unit size to the result clause. In this way, $\mathcal U_{\text{poly}}$ further exludes literal $l_4$, and synthesizes clause $\{l_1, l_2\}$ as the result, which is exactly the target conditon $c_1^*$. Because this approximation algorithm guarantees the total size of selected literals to be close to the optimal, $\mathcal U_{\text{poly}}$ is an Occam solver for clauses.

\textbf{Synthesizing condition $c_2$}. The PBE task on $c_2$ is relatively more complex, as $\mathcal U_{\text{poly}}$ is allowed to use two clauses $C_1$ and $C_2$. Here we only introduce the basic idea of $\mathcal U_{\text{poly}}$, and more details will be introduced in Section \ref{section:uni-full}. In the PBE task on $c_2$, there are three positiove examples $E_P = \{e_4,e_5,e_6\}$ and three negative examples $E_N = \{e_7,e_8,e_9\}$. Clearly, both $C_1$ and $C_2$ shoud be \texttt{flase} on $E_N$, and at least one of $C_1, C_2$ shoud le \texttt{true} on each positive example in $E_P$. Similar with $\mathcal T_{\text{poly}}$, $\mathcal U_{\text{poly}}$ start by synthesizing the clause that covers the most positive examples: Here, such a clause should cover at least $2$ examples in $E_P$. 

One problem is that the number of such clauses can be very large: For each clause, $C \subseteq \{l_1, \dots, l_5\}$ covers at least $2$ positive examples, all its subset must also cover at least $2$ positive examples. In this example, there are $8$ such clauses, corresponding to all subsets of clause $\{l_1, l_3, l_5\}$. To solve this problem, we use the fact that we already have an Occam solver for clauses: As we analyzed when discussing the term solver $\mathcal T_{\text{poly}}$, if we already get a set of examples on the target clause, invoking the Occam solver for clauses on these examples can produce a clause which is guaranteed to be close to the target in semantics and size. Therefore, instead of enumerating all clauses that cover at least $2$ examples, $\mathcal U_{\text{poly}}$ enumerate on those subsets of $E_P$ which (1) contains at least $2$ positive examples, and (2) is exactly the set of positive examples covered by some clause. There are only two such sets: $E_{P, 1} = \{e_4,e_5,e_6\}, E_{P, 2} = \{e_4, e_5\}$. After running the clause synthesis algorithm on positive examples $E_{P,i}$ and negative examples $E_N$, a single candidate clause $\{l_1\}$ is obtained. 

Then, the same as the term solver $\mathcal T_{\text{poly}}$, $\mathcal U_{\text{poly}}$ will recurse into the subproblem where $k$ is equal to $1$, $e_6$ is the only positive example, and $\{e_7,e_8,e_9\}$ are the negative examples. On this subproblem, $\mathcal U_{\text{poly}}$ finds the clause $\{l_2\}$. Therefore, the two clauses found by $\mathcal U_{\text{poly}}$ are $\{l_1\}$ and $\{l_3\}$, which is exactly the same with the target condition $c_2^*$.





==> sections/MotivateExample2.tex <==
%!TEX root = ../CLIA.tex
\section{Overview} \label{section:example}
In this section, we introduce the basic idea of our appraoch via a motivating example adopted from benchmark \texttt{mpg\_ite2.sl} in the SyGuS competition. The target program $p^*$ is shown as the following, where $x, y, z$ are three integer inputs.%, and $\texttt{ite}$ represents the \texttt{if-then-else} operator. 
\begin{align*}
	%p^*(x, y, z) \coloneqq& \texttt{(ite (>= (+ x y) 1)}\\
	%&\ \ \ \  \texttt{(ite (>= (+ x z) 1) (+ x 1) (+ y 1))} \\
	%&\ \ \ \  \texttt{(ite (>= (+ y z) 1) (+ x 1) (+ y 1)))}
	p^*(x, y, z) \coloneqq & \texttt{ if }(x + y \geq 1)\texttt{ then }\{ \\
	& \ \ \ \ \texttt{ if }(x + z \geq 1)\texttt{ then }\{x + 1\}\texttt{ else }\{y + 1\} \\ 
	& \texttt{ }\}\texttt{ else }\{ \\
	& \ \ \ \ \texttt{ if }(y + z \geq 1)\texttt{ then }\{z + 1\}\texttt{ else }\{y + 1\} \\ 
	& \texttt{ }\}
\end{align*}   
We assume that there are $9$ input-output examples provided to the PBE solver. Table \ref{table:examples} lists these examples, where tuple $(x_0, y_0, z_0)$ in column $I$ represents an input where $x,y,z$ are set to $x_0,y_0,z_0$ respectively, and the \texttt{if}-term in column \textit{Term} represents the executed branch on each example.

\begin{table*}[!htbp]
	
	\caption{The input-output examples that are available for the PBE solver.} \label{table:examples}
	\begin{spacing}{1.1}
		\small
		\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
			\hline
			ID & $I$ & $O$ & Term & ID & $I$ & $O$ & Term & ID & $I$ & $O$ & Term\\
			\hline
			$e_1$ & $(0, 1, 2)$ & $1$ & \multirow{3}{*}{$x + 1$} &$e_4$ & $(0, 2, 0)$ & $3$ & \multirow{3}{*}{$y + 1$} &$e_7$ & $(0, 0, 1)$ & $2$ & \multirow{3}{*}{$y + 1$} \\
			\cline{1-3} \cline{5-7} \cline{9-11}
			$e_2$ & $(1, 0, 2)$ & $2$ & & $e_5$ & $(-1, 3, 0)$ & $4$ & & $e_8$ & $(-3, 3, -2)$ & $-1$ & \\
			\cline{1-3} \cline{5-7} \cline{9-11}
			$e_3$ & $(-1, 3, 2)$ & $0$ & & $e_6$ & $(-1, 1, -1)$ & $2$ & & $e_9$ & $(-1, 0, 4)$ & $5$ & \\
			\hline
		\end{tabular}
	\end{spacing}
\end{table*}

\subsection{Occam Solver, \textit{STUN} and \textit{Eusolver}}
\indent \textbf{Occam Solver.} For an Occam solver, the size of the synthesized program should be polynomial to the size of the target program and sub-linear to the number of provided examples. In our motivating example, informally, we would like the synthesis result is not much larger than $p^*$. 

For simplicity, we use notation \textit{valid program} to denote those programs that are consistent with all given examples. To design an Occam solver, one intuitive way is to require the solver to synthesize the minimal valid program $p_s$: As the target $p^*$ itself is a valid program, $p_s$ must be no larger than $p^*$. This method matches the general principle of Occam's Razor and has been taken by many previous approaches~\todo{cite}. 

%However, the requirement on the minimality of the synthesized program converts a general synthesis task into an optimization task, which usually makes the problem more difficult: Even in our simple example, it is already difficult to answer whether there is a valid program smaller than $p^*$.

Because the requirement on the minimality converts a general synthesis task into an optimization task, the main issue of this method is scalability. Even in this simple example, it is already difficult to answer whether there is a valid program smaller than $p^*$.

\noindent \textbf{\emph{STUN}}. To improve the efficiency, one useful way is to decompose a hard task into several simpler sub-tasks, and then solves them separately. STUN is an efficient framework following this idea, where a program with \texttt{if-then-else} operators are synthesized via solving two subtasks:
\begin{itemize}
	\item \emph{A term finding task.} A term solver is invoked to synthesize a set of \texttt{if}-terms, which is enough to cover all given input-output examples. In this motivating example, one valid result of the term solver is the term set $\{x + 1, y +1, z + 1\}$. 
	\item \emph{An unification task.} A unifier is invoked to use \texttt{if-then-else} operators to unify these terms into a program satisfying all examples. For example, term set $\{x+1, y+1, z+1\}$ can be unified into the target program $p^*$ with \texttt{if}-conditions $\{x+y \geq 1, x+z \geq 1, y+z \geq 1\}$.
\end{itemize}

For PBE tasks, there is a trivial STUN solver which directly encoding all input-output examples into the synthesis result. In this solver, the term solver returns all possible outputs, and the unifier generates specific checks for each different example. For example, when $\{e_1,e_2,e_3\}$ are provided, the following program may be synthesized.
$$\texttt{if}\ (x = 0\ \texttt{and}\ y = 1\ \texttt{and}\ z =2)\ \texttt{then}\ 1\ \texttt{else}\ \texttt{if}\ (x = 1\ \texttt{and}\ y = 0\ \texttt{and}\ z =2)\ \texttt{then}\ 2\ \texttt{else}\ 0$$
Though such a solver can be extremely efficient, it is not a wanted solver, as it can hardly generalize from examples. Therefore, generalizability is important for a STUN solver on PBE tasks.

\noindent \textbf{\emph{Eusolver}}. \textit{Eusolver} is a state-of-the-art STUN solver for PBE tasks, which considers the generalizability by heuristically adopting the principle of Occam's Razor to the term solver. We shall briefly introduce the idea of \textit{Eusolver}, and show why it is not an Occam solver via the motivating example.

The term solver $\mathcal T_E$ in \textit{Eusolver} adopts the principle of Occam's Razor by considering all possible terms in the increasing order of the size. A term $t$ will be included in the result if the set of examples covered by $t$ is different from all smaller terms. $\mathcal T_E$ returns when collected terms are enough to cover all given examples. However, such usage of Occam's Razor does not guarantee the total size of the result term set to be small, as it does not limit the number of collected terms. In our motivating example, when constants $-1, \dots, 5$ are available, $\mathcal T_E$ will return set $\{-1, \dots, 5\}$ instead of $\{x+1, y+1, z+1\}$. Moreover, this set can be unboundedly larger as the number of examples and available constants increases.

The unifier $\mathcal U_E$ in \textit{Eusolver} is based on \textit{ID3}, a learning algorithm for decision trees. Given a set of avaliable conditions and a set of examples, $\mathcal U_E$ greedily selects the condition which provides the most information on the examples, or informally, $\mathcal U_E$ selects the condition that distinguishs the most pair of examples that corresponding to different \texttt{if}-terms. According to the selected condition, examples are partitioned into two sets, corresponding to the \texttt{then}-branch and the \texttt{else}-branch respectively, and thus can be dealt with recursively. As \textit{ID3} does not guarantee the result to be small, the program synthesized by $\mathcal U_E$ can still be much larger than $p^*$ even with a small term set. To illustrate this point, suppose the term set is $\{x+1,y+1,z+1\}$, and available \texttt{if}-conditions are $z \leq 0$, $x + y \geq 1$, $x + z \geq 1$ and $y + z \geq 1$. Then, both $z \leq 0$ and $x + y \geq 1$ are best condition according to \textit{ID3}: Both of them completely distinguish between examples corresponding to $x+1$ and $z+1$, and partition the examples corresponding to $y+1$ to two branches. Therefore, $\mathcal U_E$ may misuse $z \leq 0$ as the outmost \texttt{if}-condition. At this time, $\mathcal U_E$ has to use two extra \texttt{if-then-else} operators to form a valid program.

In summary, \textit{Eusolver} is not likely to be an Occam solver, as neither term solver $\mathcal T_E$ nor unifier $\mathcal U_E$ guarantees the synthesis result to be small. We shall formally prove this point in Section \ref{section:gen-eusolver}.

\subsection{\mainname}
To efficiently synthesize programs with \texttt{if-then-else} operators,  our approach \mainname uses the idea of decomposition and starts decomposing with the STUN framework. Different from \textit{Eusolver}, which considers the generalizability locally in sub-solvers, we take the condition of an Occam solver as a design purpose of \mainname, and thus obtain a theoretical guarantee on the generalizability. Each time when we decompose the synthesis task, we propagate the condition of an Occam solver into a sufficient set of conditions, where each condition is defined locally on a subtask.


To apply the STUN framework, we first provide a sufficient condition which propagates the condition for a STUN solver to be an Occam solver to its term solver and its unifier. Informally, this condition states that: a STUN solver must be an Occam solver if both its term solver and its unifier guarantee the size of the synthesis result to be polynomial to the size of the target program. In this way, the problem of designing an Occam STUN solver can be safely decomposed into two independent subproblems for designing a term solver and a unifier, each with polynomial bounds on the synthesis result.


\subsubsection{Term solver $\mathcal T_{\text{poly}}$ in \mainname}

Let $P^*$ be the set of terms used by an arbitrary target program, and $P$ be the set of terms synthesized by the term solver. After decomposing using STUN, the condition propagated to the term solver $\mathcal T_{\text{poly}}$ is that: the total size of terms in $P$ should be polynomial to the total size of terms in $P^*$. This condition can be equivalently decomposed into two parts: (1) $|P|$ should be polynomial to $|P^*|$, and (2) the maximal size of terms in $P$ should be polynomial to that of $P^*$. Note that the concrete value of $P^*$ remains unknown to $\mathcal T_{\text{poly}}$ at all time.

$\mathcal T_{\text{poly}}$ is a recursive procedure that determines terms in $P$ one by one. Given a set $E$ of examples, $\mathcal T_{\text{poly}}$ synthesizes a term $t$ and then recurses into a subproblem where all examples covered by $t$ are excluded. In our motivating example, when $x + 1$ is synthesized as the first term, $\mathcal T_{\text{poly}}$ will recurse into a subproblem where the example set is $\{e_4, \dots, e_9\}$.

This method decomposes the term finding task into several individual term synthesis task. Therefore we also propagate the condition on $\mathcal T_{\text{poly}}$ to each individual term $t$. We prove that $\mathcal T_{\text{poly}}$ is valid if $t$ always satisfies the following two conditions on example set $E$:
\begin{enumerate}
	\item \emph{Condition T-1}. $t$ covers at least a half of those examples covered by $t^*$.
	\item \emph{Conditoin T-2}. The size of $t$ is polynomial to the size of $t^*$.
\end{enumerate}
where $t^*$ is the term in $P^*$ that covers the most examples in $E$. Intuitively, condition \emph{T-1} ensures that $|P| = O(|P^*|\log |E|)$, because in each recursion, there is always a target term in $P^*$ of which the corresponding examples are excluded by at least a half. Condition \emph{T-2} ensures the maximal size of terms in $P$ to be polynomial to that of $P^*$.

Because PBE tasks for synthesizing a term is usually a much simpler task, $\mathcal T_{\text{poly}}$ assumes that there is an Occam solver $\mathcal S_t$ for PBE tasks on the term space. In our motivating example, when we assume \texttt{if}-terms can only be linear integer expressions, $\mathcal S_t$ can be implemented by finding the simplest valid term via linear integer programming, as we shall show in Section \ref{section:implementation}. $\mathcal T_{\text{poly}}$ finds a term satisfying both conditions by repeatedly running $\mathcal S_t$ on a random PBE task: In each turn, $\mathcal T_{\text{poly}}$ randomly draws $n_t$ examples from $E$ and collects the term synthesized by $\mathcal S$ on these examples. 

The main insight behind this algorithm is that: when all selected examples happen to correspond to term $t^*$, the term synthesized by $\mathcal S_t$ will have a great chance to satisfy both conditions \emph{T-1} and \emph{T-2}. On the one hand, by the definition of an Occam solver, the size of $t$ is guaranteed to be polynomial to the size of $t^*$, and thus condition \emph{T-2} is satisfied. On the other hand, by the guaranteed generalizability of an Occam solver, $S_t$ can find a generalizable term satisfying condition \emph{T-1} with a small number of examples, i.e., with a small $n_t$. For instance, in our motivating example, when the PBE task $\{e_1, e_2\}$ is selected, $\mathcal S_t$ could directly find $x + 1$, and generalize to the unseen example $e_3$. 

By the definition of $t^*$, $t^*$ must cover at least $|P^*|^{-1}$ portion of examples in $E$. Therefore, a random PBE task with $n_t$ examples corresponds to $t^*$ with a probability of at least $|P^*|^{-n_t}$. Therefore, after repeating sampling $O(|P^*|^{n_t})$ times, with a high probability, there will be a term satisfying both condition \textit{T-1} and \textit{T-2} among all terms $\mathcal T_{\text{poly}}$ collected. One detail is that $|P^*|$ and a proper value of $n_t$ are unknown for $\mathcal T_{\text{poly}}$. Therefore, $\mathcal T_{\text{poly}}$ will guess their value in an iterative way. This part will be discussed in Section \ref{section:term-algorithm}.

Recall that the target of $\mathcal T_{\text{poly}}$ is only to find a term set with a small total size. Therefore, it is unnecessary to determine which collected terms are valid. $\mathcal T_{\text{poly}}$ recursively tries among these terms found by $\mathcal S_t$ until a small enough term set is obtained. 

For efficiency, we use prune-off rules to exclude those terms that are invalid:
\begin{itemize}
	\item A valid term should cover a large portion of examples. For instance, when $\{e_1, e_8\}$ are selected, $\mathcal S_t$ will find $2z-3$. As this term fails in covering any other examples, it can be ignored directly.
	\item A valid term should not be very complex. For instance, when $\{e_3, e_5, e_9\}$ are selected, $4x-y+z+5$ will be found. Such a term is much more complex than many other candidates such as $x + 1$ and thus can be ignored.
\end{itemize}
\subsubsection{Unifier $\mathcal U_{\text{poly}}$ in \mainname}
As the structure of an arbitrary program with nested \texttt{if-then-else} operators is complex, $\mathcal U_{\text{poly}}$ assumes the target program is in a normal form, namely \textit{decision list}, where the structure of nested \texttt{if-then-else} opeartors is guranteed to be linear. Meanwhile, $\mathcal U_{\text{poly}}$ also unifies the terms into a decision list instead of an arbitrary program. 

In our motivating example, suppose the term set synthesized by $\mathcal T_{\text{poly}}$ is $\{x+1, y+1, z+1\}$. Then, $\mathcal U_{\text{poly}}$ will synthesize two conditions $c_1, c_2$ and unifies the terms into the following program:
\begin{align*}
	p_L(x, y, z) \coloneqq& \texttt{ if }(c_1)\texttt{ then }\{x + 1\}\texttt{ else if }(c_2)\texttt{ then }\{y + 1\}\texttt{ else }\{z + 1\} 
\end{align*}   
One valid solution here is that: 
$$c_1^*= (x + y \geq 1) \texttt{ and }(x +z \geq 1)\ \ \ \ \ c_2^* =  (x + y \geq 1) \texttt{ or }(y + z < 1)$$

After decomposing using STUN, the condition propagated to the unifier $\mathcal U_{\text{poly}}$ is that: the size of the unified program should be polynomial to the size of the target program and the total size of the term set. This condition is equivalent to its narrowed version where the target program is required to be a decision tree, because for any progtram with nested \texttt{if-then-else} operators, there is always a semantically equivalent decision list $l$ satisfying $\text{size}(l) = O(\text{size}(p)^2)$. We shall formally prove this property in Section \ref{section:unifier-over}.

On the top level, $\mathcal U_{\text{poly}}$ decomposes the unification task into several individual PBE task for \texttt{if}-conditions. In this motivating example, as $x + 1$ covers examples $\{e_1, e_2, e_1\}$, condition $c_1$ should be \texttt{true} on $\{e_1,e_2,3_3\}$ and be \texttt{false} on $\{e_4, e_5, \dots, e_9\}$. Therefore, we obtain a PBE task for condition $c_1$ with $9$ examples. Similarly, $c_2$ should be \texttt{true} on $\{e_4, e_5, e_6\}$ and be \texttt{false} on $\{e_7,e_8,e_9\}$. 

To make $\mathcal U_{\text{poly}}$ satisfies the condition propagated to the unifier, it is enough to solve these PBE tasks via an Occam solver. Because in a decision list, the \texttt{if}-conditions can be rather complex, $\mathcal U_{\text{poly}}$ further decomposes the condition synthesis task into clause synthesis task according to the structure of disjunctive normal forms. 

When synthesizing \texttt{if}-conditions, $\mathcal U_{\text{poly}}$ requires a set $L$ of literals, and always synthesize a disjunctive normal form comprised of literals in $L$, i.e., the synthesis result is always in the formal of $\left(\texttt{or}_{C_i} \left(\texttt{and}_{l \in C_i}\ l\right)\right)$, where $C_i \subseteq L$ represents a series of clauses. In $\mathcal U_{\text{poly}}$, set $L$ is determined iteratively at runtime. 

Then, $\mathcal U_{\text{poly}}$ solves these PBE tasks separately. In this example, we assume that there only $5$ literals $l_1, \dots, l_5$ available for $\mathcal U_{\text{poly}}$: $l_1 \coloneqq (x + y \geq 1), l_2\coloneqq (x + z \geq 1), l_3 \coloneqq (y + z < 1), l_4 \coloneqq (x + y \geq 0)$ and $l_5 \coloneqq (z \leq 0)$. $\mathcal U_{\text{poly}}$ synthesizes conditions in the disjuctive normal form, i.e., the result condition is always in the form of  To bound the size of the synthesized condition, $\mathcal U_{\text{poly}}$ requires an upper bound $k$ on the maximal number of clauses. In this example, for simplicity, we assume the value of $k$ is given, which is equal to $1$ for condition $c_1$ and euqal to $2$ for condition $c_2$.

\textbf{Synthesizing condition $c_1$}. Under upper bound $k = 1$, $\mathcal U_{\text{poly}}$ is required to synthesize a single clause $C \subseteq \{l_1, \dots, l_5\}$. As $c_1$ should be \texttt{true} on examples $\{e_1, e_2, e_3\}$, all literals in $C$ must also be \texttt{true} on these examples. Therefore, literal $l_3$ and $l_5$ can excluded. Besides, as $c_1$ should be \texttt{false} on examples $\{e_4, \dots, e_9\}$, for each negative example $e$ among them, there should be at least one literal in $C$ that takes \texttt{false} on $e$. Meanwhile, to bound the size of the synthesized condition, we would like the size of literal $C$ to be as small as possible. Such a problem is an instance of \textit{weighted set covering}, a well-known $\mathsf{NP}$-Hard problem. Therefore $\mathcal U_{\text{poly}}$ uses a standard greedy algorithm to find an approximated solution: In each turn, $\mathcal U_{\text{poly}}$ adds the literal that covers the most uncovered negative example on average of each unit size to the result clause. In this way, $\mathcal U_{\text{poly}}$ further exludes literal $l_4$, and synthesizes clause $\{l_1, l_2\}$ as the result, which is exactly the target conditon $c_1^*$. Because this approximation algorithm guarantees the total size of selected literals to be close to the optimal, $\mathcal U_{\text{poly}}$ is an Occam solver for clauses.

\textbf{Synthesizing condition $c_2$}. The PBE task on $c_2$ is relatively more complex, as $\mathcal U_{\text{poly}}$ is allowed to use two clauses $C_1$ and $C_2$. Here we only introduce the basic idea of $\mathcal U_{\text{poly}}$, and more details will be introduced in Section \ref{section:uni-full}. In the PBE task on $c_2$, there are three positiove examples $E_P = \{e_4,e_5,e_6\}$ and three negative examples $E_N = \{e_7,e_8,e_9\}$. Clearly, both $C_1$ and $C_2$ shoud be \texttt{flase} on $E_N$, and at least one of $C_1, C_2$ shoud le \texttt{true} on each positive example in $E_P$. Similar with $\mathcal T_{\text{poly}}$, $\mathcal U_{\text{poly}}$ start by synthesizing the clause that covers the most positive examples: Here, such a clause should cover at least $2$ examples in $E_P$. 

One problem is that the number of such clauses can be very large: For each clause, $C \subseteq \{l_1, \dots, l_5\}$ covers at least $2$ positive examples, all its subset must also cover at least $2$ positive examples. In this example, there are $8$ such clauses, corresponding to all subsets of clause $\{l_1, l_3, l_5\}$. To solve this problem, we use the fact that we already have an Occam solver for clauses: As we analyzed when discussing the term solver $\mathcal T_{\text{poly}}$, if we already get a set of examples on the target clause, invoking the Occam solver for clauses on these examples can produce a clause which is guaranteed to be close to the target in semantics and size. Therefore, instead of enumerating all clauses that cover at least $2$ examples, $\mathcal U_{\text{poly}}$ enumerate on those subsets of $E_P$ which (1) contains at least $2$ positive examples, and (2) is exactly the set of positive examples covered by some clause. There are only two such sets: $E_{P, 1} = \{e_4,e_5,e_6\}, E_{P, 2} = \{e_4, e_5\}$. After running the clause synthesis algorithm on positive examples $E_{P,i}$ and negative examples $E_N$, a single candidate clause $\{l_1\}$ is obtained. 

Then, the same as the term solver $\mathcal T_{\text{poly}}$, $\mathcal U_{\text{poly}}$ will recurse into the subproblem where $k$ is equal to $1$, $e_6$ is the only positive example, and $\{e_7,e_8,e_9\}$ are the negative examples. On this subproblem, $\mathcal U_{\text{poly}}$ finds the clause $\{l_2\}$. Therefore, the two clauses found by $\mathcal U_{\text{poly}}$ are $\{l_1\}$ and $\{l_3\}$, which is exactly the same with the target condition $c_2^*$.





==> sections/MotivateExample3.tex <==
%!TEX root = ../CLIA.tex
\section{Overview} \label{section:example}
In this section, we introduce the basic idea of our appraoch via a motivating example adopted from benchmark \texttt{mpg\_ite2.sl} in the SyGuS competition. The target program $p^*$ is shown as the following, where $x, y, z$ are three integer inputs.%, and $\texttt{ite}$ represents the \texttt{if-then-else} operator. 
\begin{align*}
	%p^*(x, y, z) \coloneqq& \texttt{(ite (>= (+ x y) 1)}\\
	%&\ \ \ \  \texttt{(ite (>= (+ x z) 1) (+ x 1) (+ y 1))} \\
	%&\ \ \ \  \texttt{(ite (>= (+ y z) 1) (+ x 1) (+ y 1)))}
	p^*(x, y, z) \coloneqq & \texttt{ if }(x + y \geq 1)\texttt{ then }\{ \\
	& \ \ \ \ \texttt{ if }(x + z \geq 1)\texttt{ then }\{x + 1\}\texttt{ else }\{y + 1\} \\ 
	& \texttt{ }\}\texttt{ else }\{ \\
	& \ \ \ \ \texttt{ if }(y + z \geq 1)\texttt{ then }\{z + 1\}\texttt{ else }\{y + 1\} \\ 
	& \texttt{ }\}
\end{align*}   
We assume that there are $9$ input-output examples provided to the PBE solver. Table \ref{table:examples} lists these examples, where tuple $(x_0, y_0, z_0)$ in column $I$ represents an input where $x,y,z$ are set to $x_0,y_0,z_0$ respectively, and the \texttt{if}-term in column \textit{Term} represents the executed branch on each example.

\begin{table*}[!htbp]
	
	\caption{The input-output examples that are available for the PBE solver.} \label{table:examples}
	\begin{spacing}{1.1}
		\small
		\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
			\hline
			ID & $I$ & $O$ & Term & ID & $I$ & $O$ & Term & ID & $I$ & $O$ & Term\\
			\hline
			$e_1$ & $(0, 1, 2)$ & $1$ & \multirow{3}{*}{$x + 1$} &$e_4$ & $(0, 2, 0)$ & $3$ & \multirow{3}{*}{$y + 1$} &$e_7$ & $(0, 0, 1)$ & $2$ & \multirow{3}{*}{$y + 1$} \\
			\cline{1-3} \cline{5-7} \cline{9-11}
			$e_2$ & $(1, 0, 2)$ & $2$ & & $e_5$ & $(-1, 3, 0)$ & $4$ & & $e_8$ & $(-3, 3, -2)$ & $-1$ & \\
			\cline{1-3} \cline{5-7} \cline{9-11}
			$e_3$ & $(-1, 3, 2)$ & $0$ & & $e_6$ & $(-1, 1, -1)$ & $2$ & & $e_9$ & $(-1, 0, 4)$ & $5$ & \\
			\hline
		\end{tabular}
	\end{spacing}
\end{table*}

\subsection{Occam Solver, \textit{STUN} and \textit{Eusolver}}
\indent \textbf{Occam Solver.} For an Occam solver, the size of the synthesized program should be polynomial to the size of the target program and sub-linear to the number of provided examples. In our motivating example, informally, we would like the synthesis result is not much larger than $p^*$. 

For simplicity, we use notation \textit{valid program} to denote programs that are consistent with all given examples. To design an Occam solver, one intuitive way is to require the solver to synthesize the minimal valid program $p_s$: As the target $p^*$ itself is a valid program, $p_s$ must be no larger than $p^*$. This method matches the general principle of Occam's Razor and has been taken by many previous approaches~\cite{DBLP:conf/icml/LiangJK10,DBLP:conf/popl/Gulwani11, DBLP:conf/popl/RaychevBVK16, DBLP:conf/icse/MechtaevYR15}. 

%However, the requirement on the minimality of the synthesized program converts a general synthesis task into an optimization task, which usually makes the problem more difficult: Even in our simple example, it is already difficult to answer whether there is a valid program smaller than $p^*$.

Because the requirement on the minimality converts a general synthesis task into an optimization task, the main issue of this method is scalability. Even in this simple example, it is already difficult to answer whether there is a valid program smaller than $p^*$.

\noindent \textbf{\emph{STUN}}. To improve the efficiency, one useful way is to decompose a hard task into several simpler sub-tasks, and then solves them separately. STUN is an efficient framework following this idea, where a program with \texttt{if-then-else} operators are synthesized via solving two subtasks:
\begin{itemize}
	\item \emph{A term finding task.} A term solver is invoked to synthesize a set of \texttt{if}-terms, which is enough to cover all given input-output examples. In this motivating example, one valid result of the term solver is the term set $\{x + 1, y +1, z + 1\}$. 
	\item \emph{An unification task.} A unifier is invoked to use \texttt{if-then-else} operators to unify these terms into a program satisfying all examples. For example, term set $\{x+1, y+1, z+1\}$ can be unified into the target program $p^*$ with \texttt{if}-conditions $\{x+y \geq 1, x+z \geq 1, y+z \geq 1\}$.
\end{itemize}

For PBE tasks, there is a trivial STUN solver which directly encoding all input-output examples into the synthesis result. In this solver, the term solver returns all possible outputs, and the unifier generates specific checks for each different example. For example, when $\{e_1,e_2,e_3\}$ are provided, the following program may be synthesized.
$$\texttt{if}\ (x = 0\ \texttt{and}\ y = 1\ \texttt{and}\ z =2)\ \texttt{then}\ 1\ \texttt{else}\ \texttt{if}\ (x = 1\ \texttt{and}\ y = 0\ \texttt{and}\ z =2)\ \texttt{then}\ 2\ \texttt{else}\ 0$$
Though such a solver can be extremely efficient, it is not a wanted solver, as it can hardly generalize from examples. Therefore, generalizability is important for a STUN solver on PBE tasks.

\noindent \textbf{\emph{Eusolver}}. \textit{Eusolver} is a state-of-the-art STUN solver for PBE tasks, which considers the generalizability by heuristically adopting the principle of Occam's Razor to the term solver. We shall briefly introduce the idea of \textit{Eusolver}, and show why it is not an Occam solver via the motivating example.

The term solver $\mathcal T_E$ in \textit{Eusolver} adopts the principle of Occam's Razor by considering all possible terms in the increasing order of the size. A term $t$ will be included in the result if the set of examples covered by $t$ is different from all smaller terms. $\mathcal T_E$ returns when collected terms are enough to cover all given examples. However, such usage of Occam's Razor does not guarantee the total size of the result term set to be small, as it does not limit the number of collected terms. In our motivating example, when constants $-1, \dots, 5$ are available, $\mathcal T_E$ will return set $\{-1, \dots, 5\}$ instead of $\{x+1, y+1, z+1\}$. Moreover, this set can be unboundedly larger as the number of examples and available constants increases.

The unifier $\mathcal U_E$ in \textit{Eusolver} is based on \textit{ID3}, a learning algorithm for decision trees. Given a set of avaliable conditions and a set of examples, $\mathcal U_E$ greedily selects the condition which provides the most information on the examples, or informally, $\mathcal U_E$ selects the condition that distinguishs the most pair of examples that corresponding to different \texttt{if}-terms. According to the selected condition, examples are partitioned into two sets, corresponding to the \texttt{then}-branch and the \texttt{else}-branch respectively, and thus can be dealt with recursively. As \textit{ID3} does not guarantee the result to be small, the program synthesized by $\mathcal U_E$ can still be much larger than $p^*$ even with a small term set. To illustrate this point, suppose the term set is $\{x+1,y+1,z+1\}$, and available \texttt{if}-conditions are $z \leq 0$, $x + y \geq 1$, $x + z \geq 1$ and $y + z \geq 1$. Then, both $z \leq 0$ and $x + y \geq 1$ are best condition according to \textit{ID3}: Both of them completely distinguish between examples corresponding to $x+1$ and $z+1$, and partition the examples corresponding to $y+1$ to two branches. Therefore, $\mathcal U_E$ may misuse $z \leq 0$ as the outmost \texttt{if}-condition. At this time, $\mathcal U_E$ has to use two extra \texttt{if-then-else} operators to form a valid program.

In summary, \textit{Eusolver} is not likely to be an Occam solver, as neither term solver $\mathcal T_E$ nor unifier $\mathcal U_E$ guarantees the synthesis result to be small. We shall formally prove this point in Section \ref{section:gen-eusolver}.

\subsection{\mainname}
\begin{figure}
	\includegraphics[width=\columnwidth]{pics/draft}
\end{figure}
\begin{itemize}
	\item \mainname generates a decision list program rather than a decision tree program (example).
	\item There are four main algorithms. The term solver uses disjunctive solver and domain solver. The unifier uses decision list solver, clause solver, and disjunctive solver. 
	\item For each solver, states (1) what does it do, (2) what is its role in the term solver and/or in the unifier (using the example to illustrate), (3) what it ensures (for the returned program), and (4) how it achieves this. An example follows.
	\begin{itemize}
		\item the disjucntive solver lifts an occam solver into a solver for a set of programs, each blah blah.
		\item the disjunctive solver ensures the synthesized program set blah blah. 
		\item the disjunctive solver is used in term solver for blah, and is used in the unifier for blah.
		\item the disjunctive solver perform the task in this rought steps.
	\end{itemize}
	\item illustrate how the example program is generated.
	\begin{itemize}
		\item first the disjunctive solver calls the domain solver to generate many terms.
		\item the disjunctive solver returns with a set covering all examples
		\item the decision list solver generates condition for each term.
		\item for each term, the disjunctive solver calls the clause solver to generate many predicates
		\item for each term, the disjunctive solver returns a DNF
	\end{itemize}
\end{itemize}








To efficiently synthesize programs with \texttt{if-then-else} operators,  Our approach \mainname uses the idea of decomposition and starts decomposing with the STUN framework. Different from \textit{Eusolver}, which considers the generalizability locally in sub-solvers, we take the condition of an Occam solver as a design purpose of \mainname, and thus obtain a theoretical guarantee on the generalizability. Each time when we decompose the synthesis task, we propagate the condition of an Occam solver into a sufficient set of conditions, where each condition is defined locally on a subtask.


To apply the STUN framework, we first provide a sufficient condition which propagates the condition for a STUN solver to be an Occam solver to its term solver and its unifier. Informally, this condition states that: a STUN solver must be an Occam solver if both its term solver and its unifier guarantee the size of the synthesis result to be polynomial to the size of the target program. In this way, the problem of designing an Occam STUN solver can be safely decomposed into two independent subproblems for designing a term solver and a unifier, each with polynomial bounds on the synthesis result.


\subsubsection{Term solver $\mathcal T_{\text{poly}}$ in \mainname}

Let $P^*$ be the set of terms used by an arbitrary target program, and $P$ be the set of terms synthesized by the term solver. After decomposing using STUN, the condition propagated to the term solver $\mathcal T_{\text{poly}}$ is that: the total size of terms in $P$ should be polynomial to the total size of terms in $P^*$. This condition can be equivalently decomposed into two parts: (1) $|P|$ should be polynomial to $|P^*|$, and (2) the maximal size of terms in $P$ should be polynomial to that of $P^*$. Note that the concrete value of $P^*$ remains unknown to $\mathcal T_{\text{poly}}$ at all time.

$\mathcal T_{\text{poly}}$ is a recursive procedure that determines terms in $P$ one by one. Given a set $E$ of examples, $\mathcal T_{\text{poly}}$ synthesizes a term $t$ and then recurses into a subproblem where all examples covered by $t$ are excluded. In our motivating example, when $x + 1$ is synthesized as the first term, $\mathcal T_{\text{poly}}$ will recurse into a subproblem where the example set is $\{e_4, \dots, e_9\}$.

This method decomposes the term finding task into several individual term synthesis task. Therefore we also propagate the condition on $\mathcal T_{\text{poly}}$ to each individual term $t$. We prove that $\mathcal T_{\text{poly}}$ is valid if $t$ always satisfies the following two conditions on example set $E$:
\begin{enumerate}
	\item \emph{Condition T-1}. $t$ covers at least a half of those examples covered by $t^*$.
	\item \emph{Conditoin T-2}. The size of $t$ is polynomial to the size of $t^*$.
\end{enumerate}
where $t^*$ is the term in $P^*$ that covers the most examples in $E$. Intuitively, condition \emph{T-1} ensures that $|P| = O(|P^*|\log |E|)$, because in each recursion, there is always a target term in $P^*$ of which the corresponding examples are excluded by at least a half. Condition \emph{T-2} ensures the maximal size of terms in $P$ to be polynomial to that of $P^*$.

Because PBE tasks for synthesizing a term is usually a much simpler task, $\mathcal T_{\text{poly}}$ assumes that there is an Occam solver $\mathcal S_t$ for PBE tasks on the term space. In our motivating example, when we assume \texttt{if}-terms can only be linear integer expressions, $\mathcal S_t$ can be implemented by finding the simplest valid term via linear integer programming, as we shall show in Section \ref{section:implementation}. $\mathcal T_{\text{poly}}$ finds a term satisfying both conditions by repeatedly running $\mathcal S_t$ on a random PBE task: In each turn, $\mathcal T_{\text{poly}}$ randomly draws $n_t$ examples from $E$ and collects the term synthesized by $\mathcal S$ on these examples. 

The main insight behind this algorithm is that: when all selected examples happen to correspond to term $t^*$, the term synthesized by $\mathcal S_t$ will have a great chance to satisfy both conditions \emph{T-1} and \emph{T-2}. On the one hand, by the definition of an Occam solver, the size of $t$ is guaranteed to be polynomial to the size of $t^*$, and thus condition \emph{T-2} is satisfied. On the other hand, by the guaranteed generalizability of an Occam solver, $S_t$ can find a generalizable term satisfying condition \emph{T-1} with a small number of examples, i.e., with a small $n_t$. For instance, in our motivating example, when the PBE task $\{e_1, e_2\}$ is selected, $\mathcal S_t$ could directly find $x + 1$, and generalize to the unseen example $e_3$. 

By the definition of $t^*$, $t^*$ must cover at least $|P^*|^{-1}$ portion of examples in $E$. Therefore, a random PBE task with $n_t$ examples corresponds to $t^*$ with a probability of at least $|P^*|^{-n_t}$. Therefore, after repeating sampling $O(|P^*|^{n_t})$ times, with a high probability, there will be a term satisfying both condition \textit{T-1} and \textit{T-2} among all terms $\mathcal T_{\text{poly}}$ collected. One detail is that $|P^*|$ and a proper value of $n_t$ are unknown for $\mathcal T_{\text{poly}}$. Therefore, $\mathcal T_{\text{poly}}$ will guess their value in an iterative way. This part will be discussed in Section \ref{section:term-algorithm}.

Recall that the target of $\mathcal T_{\text{poly}}$ is only to find a term set with a small total size. Therefore, it is unnecessary to determine which collected terms are valid. $\mathcal T_{\text{poly}}$ recursively tries among these terms found by $\mathcal S_t$ until a small enough term set is obtained. 

For efficiency, we use prune-off rules to exclude those terms that are invalid:
\begin{itemize}
	\item A valid term should cover a large portion of examples. For instance, when $\{e_1, e_8\}$ are selected, $\mathcal S_t$ will find $2z-3$. As this term fails in covering any other examples, it can be ignored directly.
	\item A valid term should not be very complex. For instance, when $\{e_3, e_5, e_9\}$ are selected, $4x-y+z+5$ will be found. Such a term is much more complex than many other candidates such as $x + 1$ and thus can be ignored.
\end{itemize}
\subsubsection{Unifier $\mathcal U_{\text{poly}}$ in \mainname}
As the structure of an arbitrary program with nested \texttt{if-then-else} operators is complex, $\mathcal U_{\text{poly}}$ assumes the target program to be in a normal form, namely \textit{decision list}, where the program structure is linear. At the same time, $\mathcal U_{\text{poly}}$ also unifies the terms into a decision list instead of an arbitrary program. 

In our motivating example, suppose the term set synthesized by $\mathcal T_{\text{poly}}$ is $\{x+1, y+1, z+1\}$. Then, $\mathcal U_{\text{poly}}$  synthesizes two conditions $c_1, c_2$ and unifies the terms into the following program:
\begin{align*}
	p_L(x, y, z) \coloneqq& \texttt{ if }(c_1)\texttt{ then }\{x + 1\}\texttt{ else if }(c_2)\texttt{ then }\{y + 1\}\texttt{ else }\{z + 1\} 
\end{align*}   
One valid solution here is that: 
$$c_1^*= (x + y \geq 1) \texttt{ and }(x +z \geq 1)\ \ \ \ \ c_2^* =  (x + y \geq 1) \texttt{ or }(y + z < 1)$$

After decomposing using STUN, the condition propagated to the unifier $\mathcal U_{\text{poly}}$ is that: the size of the unified program should be polynomial to the size of the target program and the total size of the term set. This condition is equivalent to its narrowed version where the target program is required to be a decision tree, because for any program with nested \texttt{if-then-else} operators, there is always a semantically equivalent decision list $l$ satisfying $\text{size}(l) = O(\text{size}(p)^2)$. We shall formally prove this property in Section \ref{section:unifier-over}.

In the first step, $\mathcal U_{\text{poly}}$ decomposes the unification task into several individual PBE task for \texttt{if}-conditions according to the structure of a decision list. In this motivating example, as term $x+1$ covers $\{e_1,e_2,e_3\}$ only, we know condition $c_1$ must be \texttt{true} on $\{e_1,e_2,e_3\}$ and \texttt{false} on $\{e_4, e_5, \dots, e_9\}$. Therefore, we obtain $9$ examples on $c_1$. Similarly, $c_2$ should be \texttt{true} on $\{e_4, e_5, e_6\}$ and be \texttt{false} on $\{e_7,e_8,e_9\}$, and thus $6$ examples on $c_2$ are obtained.

To make $\mathcal U_{\text{poly}}$ satisfies the condition propagated to the unifier, it is enough to solve these PBE tasks via an Occam solver. In consideration of efficiency, $\mathcal U_{\text{poly}}$ further decomposes the condition synthesis task into clause synthesis tasks according to the structure of disjunctive normal forms. Concretely, $\mathcal U_{\text{poly}}$ requires a set $L$ of literals, and always synthesizes in the formal of $\left(\texttt{or}_{C_i} \left(\texttt{and}_{l \in C_i}\ l\right)\right)$, where $C_i \subseteq L$ represents a series of clauses. Just like parameter $n_t$ used in $\mathcal T_{\text{poly}}$, set $L$ is determined iteratively by $\mathcal U_{\text{poly}}$ at runtime. Besides, literals in $L$ are allowed to use boolean operators such as \texttt{not}, \texttt{and}, \texttt{or}, which are rather different from the logic notation "literals". 

In our motivating example, suppose $L$ includes only $5$ literals $\{l_1, \dots, l_5\}$, where $l_1 \coloneqq (x + y \geq 1), l_2\coloneqq (x + z \geq 1), l_3 \coloneqq (y + z < 1), l_4 \coloneqq (x + y \geq 0)$ and $l_5 \coloneqq (z \leq 0)$. Then clause $\{l_1,l_2\}$ and clause set $\{\{l_1\},\{l_3\}\}$ are valid solutions for condition $c_1$ and $c_2$ respectively. 

It is easy to see the task of synthesizing a set of clauses has a similar form with the term finding task. By the semantics of operator $\texttt{or}$, $\mathcal U_{\text{poly}}$ needs to find a series of clauses such that (1) each positive example should be covered by at least one clause, (2) all clauses should cover all negative examples. Therefore, a similar way as $\mathcal T_{\text{poly}}$ can be adopted here to convert a condition synthesis task to clause synthesis tasks by sampling only on positive examples. In this way, the problem is reduced to designing an Occam solver for clauses.

We use an example to illustrate our clause solver. Suppose $\mathcal U_{\text{poly}}$ is going to synthesize $c_1$ as a single clause, and the available literals are still $\{l_1, \dots, l_5\}$ defined before. As $c_1$ should be \texttt{true} on examples $\{e_1, e_2, e_3\}$, all literals used by $c_1$ must also be \texttt{true} on these examples. Therefore, literals $l_3$ and $l_5$ can be excluded.  As $c_1$ should be \texttt{false} on examples $\{e_4, \dots, e_9\}$, for each negative example $e$ among them, there should be at least one literal in $c_1$ that takes \texttt{false} on $e$. Meanwhile, to build an Occam solver, we would like the size of $c_1$ to be as small as possible. Such a problem is an instance of \textit{weighted set covering}, a well-known $\mathsf{NP}$-Hard problem. Therefore $\mathcal U_{\text{poly}}$ uses a standard greedy algorithm to find an approximated solution: In each turn, $\mathcal U_{\text{poly}}$ adds the literal that covers the most uncovered negative example on average of each unit size to the result clause. Because this approximation algorithm guarantees the total size of selected literals to be at most $\ln n_N$ times larger than the optimal, where $n_N$ is the number of negative examples, $\mathcal U_{\text{poly}}$ is an Occam solver for clauses.

In this example, there are three available clauses $l_1, l_2, l_4$. The sizes of these clauses are the same, and the sets of negative examples they covered are $\{e_6,e_7,e_8,e_9\}, \{e_4, e_5, e_8\}$ and $\{e_9\}$. In the fisrt turn, $l_1$ is added to the result, as it covers the most negative examples. Then, there are $2$ negative examples $\{e_4,e_5\}$ remaining, and $l_2, l_4$ cover $\{e_4,e_5\}$ and $\emptyset$ respectively. Therefore, in the second turn, $l_2$ is added to the result, and then clause $\{l_1, l_2\}$ is synthsized for condition $c_1$.

Different from $\mathcal T_{\text{poly}}$, where domain solver $\mathcal S_t$ is provided as a black box, the clause solver in $\mathcal U_{\text{poly}}$ is concretely known. Therefore, we further optimize the efficiency of the random sampling by utilizing the properties of the clause solver. This optimization will be discussed in Section \ref{section:uni-full}.





==> sections/Related.tex <==
%!TEX root = ../CLIA.tex
\section{Related Work} \label{section:related}
\noindent \textbf{Generalizability of PBE Solvers.} Generalizability is known to be important for programming-by-example, and there have been many different approaches proposed to improve generalizability of PBE solvers from different aspects.

To select a program that is likely to generalize, many previous works convert the PBE task into an optimization task by introducing a heuristic function. \citet{DBLP:conf/icml/LiangJK10,DBLP:conf/popl/Gulwani11, DBLP:conf/popl/RaychevBVK16} select the syntactically shortest program;  \citet{DBLP:conf/icse/MechtaevYR15} and \citet{DBLP:conf/cav/DAntoniSS16} choose the program that is syntactically and semantically closest to a reference program respectively; \citet{DBLP:conf/sigsoft/LeCLGV17} chooses the best program by comprehensively considering 6 heuristics from the perspectives of syntax and semantics. However, for those difficult domains, such as CLIA, it is hard to design a solver that is efficient enough and guarantees the optimality of the program at the same time, as the requirement on the optimality greatly increases the difficulty of synthesis in theory. In contrast, we propose a new target, i.e., class $\mathsf{PSG}$, which constraints less for synthesizers and still has theoretical guarantees on generalizability. In this way, we succeed in designing a STUN solver that has guaranteed generalizability.

Besides, many previous works use learned models to guide the synthesis procedure, and thus focus on only probable programs \cite{DBLP:conf/iclr/BalogGBNT17, DBLP:conf/iclr/KalyanMPBJG18, DBLP:journals/pacmpl/JiS0H20, DBLP:conf/cav/SinghG15, DBLP:conf/sigsoft/ChenMF19, DBLP:conf/icml/MenonTGLK13, DBLP:conf/icml/DevlinUBSMK17, DBLP:conf/pldi/LeeHAN18}. In theory, the effects of these approaches can be explained using Theorem \ref{theorem:optimal}: The more accurate the learned model is, the close to the optimal the PBE solver will be on generalizability. However, learning an accurate model itself is a difficult task, and the effectiveness of current methods greatly relies on domain knowledge and representative datasets. In contrast, our abstracted model is based only on two moderate assumptions and is generally applicable to different domains.

%There are also related works on improving the quality of input examples: \citet{DBLP:conf/cav/Drachsler-Cohen17} enhances the specification by learning abstracted examples; \citet{DBLP:conf/iclr/LaichBV20, DBLP:conf/pldi/IyerJPRR19} utilize neural networks to infer additional examples and thus reduce the number of examples required by the whole synthesizer. These approaches are complementary to ours: In our abstracted model, we focus only on PBE solvers and always remain the examples abstracted.

\noindent \textbf{Analysis on the generalizability.} Analyzing the generalizability of learning algorithms is an important problem in machine learning and has been studied for decades. The \textit{probably approximately correct (PAC)} learnability framework \cite{DBLP:journals/cacm/Valiant84} firstly introduces concepts in computational complexity theory to machine learning, and thus enables mathematical analysis of generalizability. In the PAC framework, inputs are assumed to be drawn from an unknown distribution, and the generalizability is defined as the number of examples required to guarantee that with a probability of at least $1 - \epsilon$, the learner returns a function that performs the same with the target program on a random input with a probability of at least $1 - \delta$, where $\epsilon$ and $\delta$ are two given parameters. On the program synthesis side, the PAC framework has been applied to analyze the generalizability for synthesizing logic programs \cite{DBLP:journals/jair/Cohen95,DBLP:journals/jair/Cohen95a,DBLP:conf/colt/DzeroskiMR92}.  

In addition to analyzing specific domains, \citet{DBLP:journals/ipl/BlumerEHW87,DBLP:journals/jacm/BlumerEHW89} provides general bounds under the PAC framework: a union bound and a \textit{Vapnik-Chervonenkis Dimension (VCD)} bound are established for the cases where the hypothesis space (a concept equivalent to the program space in program synthesis) is finite and infinite respectively. These two bounds have also been utilized in the program synthesis side. \citet{DBLP:journals/ml/LauWDW03} utilizes the union bound to prove the generalizability of a synthesizer based on \textit{version space algebra (VSA)}, as VSA always represents a finite program space. \citet{DBLP:conf/cav/DrewsAD19} uses the VCD bound for synthesizing linear arithmetic expressions (without conditions) for holes given in a sketch. 

There are two differences between our abstracted model and the PAC framework: (1) In our model, the target program is regarded as a random variable drawn from a distribution biased to small programs, and we only consider the average generalizability of a synthesizer on a random target program. In contrast, in the PAC framework, the target hypothesis is not viewed as random, and the generalization bound is required to hold for all hypotheses. Introducing the distribution of the target program enables our model to perform a more refined analysis and to compare the generalizability of different solvers. As shown in Section \ref{section:gen-case}, we can distinguish the generalizability between $\mathcal S_{\text{min}}$ and $\mathcal S_{\text{rank}}$ only after the distribution on the target program and Assumption \ref{ass:1} are introduced. (2) In the domain of program synthesis, it is crucial to guarantee the correctness of the synthesized program: Any small deviation will result in a bug and may lead to serious consequences in practice. To reflect this point, our model does not tolerate a small error rate on the synthesized program, as the PAC framework does. Instead, we introduce Assumption \ref{ass:2} to enable abstracted analysis when concrete semantics are unknown. Our treatment can be regarded as a special case of the PAC framework where the error rate $\delta$ on the synthesized program is smaller than the semantics difference between any two programs.

Apart from the PAC framework, on the machine learning side, there have been other works on analyzing the generalizability of concrete learning algorithms, such as \textit{Stochastic Gradient Descent (SGD)}~\cite{DBLP:conf/icml/HardtRS16, DBLP:conf/nips/London17}, and \textit{Stochastic Gradient Langevin Dynamic (SGLD)}~\cite{DBLP:conf/colt/Mou0Z018}. However, these works rely on specific properties of different learning algorithms and thus is difficult to apply to the program synthesis side.

\noindent \textbf{Synthesizing CLIA Programs.} CLIA is an important subdomain of program synthesis, as CLIA programs generally exist in real-world project and have ability to express complex behaviors by using nested \texttt{if-then-else} operators. There have been many applications of CLIA synthersizers,  such as program repair~\cite{DBLP:conf/icse/MechtaevYR15, DBLP:conf/sigsoft/LeCLGV17}, automated parallelization~\cite{DBLP:conf/pldi/FarzanN17, DBLP:conf/pldi/MoritaMMHT07}. For PBE tasks in CLIA, there are two major techniques:
\begin{itemize}
	\item STUN based synthesizers~\cite{DBLP:conf/cav/AlurCR15} , represneted by \textit{Eusolver}~\cite{DBLP:conf/tacas/AlurRU17}, divide a nested \texttt{if}-program into \texttt{if}-terms and \texttt{if}-conditions, and then synthesize them separately.
	\item Refutation based synthesizers ~\cite{DBLP:conf/cav/ReynoldsBNBT19, DBLP:journals/fmsd/ReynoldsKTBD19}, represented by \textit{CVC4}~\cite{DBLP:conf/cav/ReynoldsBNBT19}, synthesize programs from unsatisfiability proofs given by theory solvers.
\end{itemize}
Our solver \mainname follows the STUN framework. We have evaluated \mainname against state-of-the-art solvers in both directions in Section \ref{section:evaluation}. The result demonstrates that \textit{Eusolver} achieves better generalizability than both approaches. \todo{add explanation on the speed}.

Outside programming-by-example, there are other techniques proposed for synthesizing CLIA programs. \textit{DryadSynth}~\cite{DBLP:conf/pldi/HuangQSW20} reconciles enumerative and deductive synthesis techniques, and can be applied to synthesize CLIA programs. However, as the deductive techniques in \textit{DryadSynth} requires a logic specificaion, it is not suitable for PBE tasks. \textit{NAY}~\cite{DBLP:conf/pldi/HuCDR20} determines whether a PBE task on CLIA is realizable, i.e., whether there is a program satisfying all given examples, which is complementary to our solvers. \mainname is not guaranteed to terminate on an unrealizable PBE task. Therefore, \textit{NAY} can be used to pre-check whether the given PBE task is realizable, and thus guarantee the terminality of the whole solver.



==> sections/STUN.tex <==
%!TEX root = ../CLIA.tex
\section{Synthesis Through Unification}
To evaluate the effectiveness of our abstarcted generalization model and class $\mathsf{PSG}$, in the second part of this paper, we study the framework of \textit{synthesis through unification (STUN)}. STUN is deigned for synthesizing programs with nested \texttt{if-then-else} operators quickly, and it does not take the generalizability into consider. As a result, though the STUN framework achieves great success on the speed, the generalizability of existing STUN solvers is unsatisfiable: As shown in Section \ref{section:eusolver-gen}, even the state-of-the-art STUN solver is not inside $\mathsf {PSG}$.
\todo{move this part to the introduction.}

In this section, we study the generalizability of STUN and its solvers. In Section \ref{section:stun-pre} and \ref{section:eusolver-pre}, we introduce some necessary preliminaries on STUN and a state-of-the-art STUN solver, named \textit{Eusolver}, respectively. Then, in Section \ref{section:stun-gen}, we study the condition for a STUN solver to have polynomial-size generalizability. At last, in Section \ref{section:eusolver-gen}, we prove that \textit{Eusolver} is not inside $\mathsf{PSG}$.

\subsection{Preliminaries: Synthesis through Unification} \label{section:stun-pre}
The framework of \textit{synthesis through unification (STUN)} focuses on a special kind of synthesis tasks, where the program domain supports enough flexibility for \texttt{if-then-else} operators. Formally, STUN assumes that the program domain can be decomposed into two subdomains, for \texttt{if}-conditions and \texttt{if}-terms respectively. 

\begin{definition}A program domain $\mathbb P$ is a conditional program domain if and only if there exist two program domains $\mathbb P_c$ and $\mathbb P_t$ such that $\mathbb P$ is the smallest set of programs such that:
	$$
	\mathbb P = \mathbb P_t \cup \left\{\texttt{if}\ c\ \texttt{then}\ p_1\ \texttt{else}\ p_2\ |\ p_1, p_2 \in \mathbb P, c \in C(\mathbb P_c)  \right\}
	$$
	where $C(\mathbb P_c)$ is the set of all possible conditions formed by boolean expressions in $\mathbb P_c$, which is the smallest set satisfying:
	$$
	C(\mathbb P_c) = \mathbb P_c \cup \left\{c_1\ \texttt{and}\ c_2\ |\ c_1,c_2 \in C(\mathbb P_c)\right\} \cup  \left\{c_1\ \texttt{or}\ c_2\ |\ c_1,c_2 \in C(\mathbb P_c)\right\} \cup \{\texttt{not}\ c\ |\ c \in C(\mathbb P_c)\}
	$$
\end{definition}
For convenience, we use a pair of program domains $(\mathbb P_t, \mathbb P_c)$ to denote a conditional program domain derived from term domain $\mathbb P_t$ and condition domain $\mathbb P_c$, and use $\mathcal F_C$ to denote a family of domains with conditional program domains.

There are be many semantically equivalent programs in a conditional program domain, and thus $(\mathbb P_t, \mathbb P_c)$ is unnecessarily complex. Therefore, in most cases, only a small subset of programs is considered, namely \textit{normal form}, which contains all possible semantics in the whole domain. 

\begin{definition} For term domain $\mathbb P_t$ and condition domain $\mathbb P_c$, $(\mathbb P_t, \mathbb P_c)_N$ is a normal form if:
	$$
	(\mathbb P_t, \mathbb P_c)_N \subseteq (\mathbb P_t, \mathbb P_c) \wedge \forall p \in (\mathbb P_t, \mathbb P_c), \exists p' \in (\mathbb P_t, \mathbb P_c)_N, p \sim_{\mathbb I} p'
	$$
\end{definition}
Obviously, the join of two different normal forms is still a normal form. Given a family of domains $\mathcal F_C$, we use $\mathcal F_C^{\text{N}}$ to the corresponding family of domains where the program domians are in the form of $(\mathbb P_t, \mathbb P_c)_{\text{N}}$, i.e., $\mathcal F_C^{\text{N}} = \{((\mathbb P_t, \mathbb P_c)_{\text{N}}, \mathbb I, \mathbb O)\ |\ ((\mathbb P_t, \mathbb P_c), \mathbb I, \mathbb O) \in \mathcal F_C\}$.

A STUN solver designed for $\mathcal F_C^{\text{N}}$ synthesizes programs in two steps:
\begin{enumerate}
	\item A term solver is invoked to synthesize a set of programs $P \subseteq \mathbb P_t$ such that for any possible input $I$, there is always a program $p \in P$ such that $\sem{p}(I)$ is a valid output.
	\item A unifier is invoked to unify $P$ into a single program in the normal form $(P, \mathbb P_c)_{\text{N}}$ using \texttt{if-then-else} operators and \texttt{if}-conditions inside $C(\mathbb P_c)$.
\end{enumerate}
In this paper, we only consider the specialized version of the STUN framework on PBE tasks.

\begin{definition}[Term Solver] Given a term domain $\mathcal P_t$, a term solver $\mathcal T: (\mathbb I \times \mathbb O)^* \mapsto \{\top\} \cup \mathcal P(\mathbb P_t)$ is a function satisfying the following two conditions for any PBE task $T \in (\mathbb I, \mathbb O)^*$:
	\begin{itemize}
		\item (Soundness) If $\mathcal T(T)$ is a set of programs, for every example $e$ in $T$, there is always a program in $\mathcal T(T)$ consistent with $e$:
		$$\mathcal T(T) \subseteq \mathbb P_t \implies \forall (I,O) \in T, \exists p \in \mathcal T(T), \sem{T}(I) = O$$
		\item (Completeness) If $\mathcal T(T) = \top$,  all subsets of $\mathcal P_t$ must violate at least one example in $T$:
		$$\mathcal T(T) = \top \iff \forall P \subseteq \mathbb P_t, \exists (I,O) \in T, \forall p \in P, \sem{p}(I) \neq O$$
	\end{itemize}
	where $\mathcal P(\mathbb P_t)$ represents the power set of $\mathbb P_t$.
\end{definition}

\begin{definition}[Unifier] A unifier $\mathcal U_{\text{N}}$ designed for $\mathcal F_{C}^{\text{N}}$ is a function such that for any set of terms $P \subseteq \mathbb P_t$, $\mathcal U_{\text{N}}(P)$ is a PBE solver for normal form $(P, \mathbb P_c)_{\text{N}}$.
\end{definition}

In the STUN framework, a solver is comprised of a term solver $\mathcal T$ and a unifer $\mathcal U_{\text{N}}$. Given a PBE task $T$, the synthesizer simply returns $\mathcal U_{\text{N}}(\mathcal T(T))(T)$ as the result. 

The soundness of STUN is straight-forward from the soundness of $\mathcal T$ and $\mathcal U_{\text{N}}$. In contrast, the completeness of STUN is guaranteed only when the program domain is \textit{if-closed}:

\begin{definition}[If-Closed] A conditional program domain is \textit{if-closed} if: $$\forall p_1, p_2 \in \mathbb P_t, \exists c \in C(\mathbb P_c), \forall I \in \mathbb I, \left(\sem{c}(I) \iff \sem{p_1}(I) = \sem{p_2}(I)\right)$$
\end{definition}

\begin{theorem} \label{lemma:completeness}  For normal form $(\mathbb P_t, \mathbb P_c)_{\text{N}}$, the STUN framework is complete if the corresponding program domain $(\mathbb P_t, \mathbb P_c)$ is if-closed.
\end{theorem}

For other domains, STUN can be extended to complete by backtracking to the term solver when the unification fails, as done by related works ~\cite{DBLP:conf/cav/AlurCR15, DBLP:conf/tacas/AlurRU17}.

In the remainder of this paper, we focus on if-closed program domains only: We implicitly assume $\mathcal F_{C}^{\text{N}}$ only contains domains where the program domain is if-closed. 

\subsection{Preliminaries: \textit{EuSolver}} \label{section:eusolver-pre}
\textit{Eusolver}~\cite{DBLP:conf/tacas/AlurRU17} is a state-of-the-art synthesizer following the STUN framework. In this section, we shall briefly introduce the algorithm of \textit{Eusolver}.

\textit{Eusolver} is designed for normal form $\mathcal F_{C}^{\text{DT}}$, where only expressions in $\mathbb P_c$ is allowed to be used as \texttt{if}-conditions. Formally, $(\mathbb P_t, \mathbb P_c)_{\text{DT}}$  is the smallest set of programs such that:
$$
(\mathbb P_t, \mathbb P_c)_{\text{DT}}= \mathbb P_t \cup \left\{\texttt{if}\ c\ \texttt{then}\ p_1\ \texttt{else}\ p_2\ |\ p_1, p_2 \in (\mathbb P_t, \mathbb P_c)_{\text{DT}}, c \in \mathbb P_c  \right\}
$$

\SetKwFunction{Enum}{Enumerate}
\SetKwFunction{Covered}{Covered}
\SetKwFunction{Learn}{LearnDT}
\SetKwFunction{Select}{SelectCond}

Algorithm \ref{alg:eusolver-term} shows the pseudo code of the term solver in \textit{Eusolver}. The term solver enumerates programs in domain $\mathbb P_t$ in the increasing order of the size (Line 4). For each program $p$, if there is not a visited program that satisfies exactly the same subset of examples as $p$, $p$ will be included into the result (Lines 6-8). The enumeration ends when the enumerated programs are enough to cover all examples in $T$ (Line 9).

Algorithm \ref{alg:eusolver-uni} shows the pseudo code of the unifier in \textit{Eusolver}, which is from \textit{ID3}~\cite{DBLP:journals/ml/Quinlan86}, a standard multi-label decision tree learning algorithm. The unifier uses function \Learn{\variable{examples}} to recursively synthesize a program satisfying all examples in \variable{examples} (Lines 1-11). In each step, the unifier firstly tries to use a term to cover all examples (Lines 2-4). Then, it picks up a condition $c$ in $\mathbb P_c$ based on some greedy strategy, and synthesizes a program in the form of \texttt{if} $(c)$ \texttt{then} $t$ \texttt{else} $f$ (Line $5$).  To form a correct program, program $t$ and $f$ must satisfy all examples on which $c$ is evaluated to true and false respectively (Lines 6-7). Therefore, the unifier recursively invokes $\Learn$ to synthesize proper programs $t$ and $f$ (Line $9$). 

\begin{figure}[t]
	\begin{minipage}{.46\linewidth}
		\begin{algorithm}[H]
			\small
			\caption{The term solver in \textit{Eusolver}.}
			\label{alg:eusolver-term}
			\LinesNumbered
			\KwIn{PBE task $T$ and domain $\mathbb P_t$.}
			\KwOut{A set of programs in $\mathbb P_t$ or $\top$.}
			\SetKwProg{Fn}{Function}{:}{}
			\Fn{\Covered{$p, T$}}{\Return $\left\{(I,O)\ |\ (I,O) \in T \wedge \sem{p}(I) = O\right \}$;}
			\variable{covered} $\gets \emptyset$; \ \ \variable{result} $\gets \emptyset$; \\
			\For{each $p \in \Enum{$\mathbb P_t$}$}{
				\If {$\forall p' \in \variable{result}, \Covered{$p, T$} \neq \Covered{$p', T$}$}{
					$\variable{covered} \gets \variable{covered} \cup \Covered{$p, T$}$; \\
					$\variable{result} \gets \variable{result} \cup \{p\}$;
				}
				\lIf {$\variable{covered} = T$}{\Return \variable{covered}}
			}
			\Return $\top$;
		\end{algorithm}
		\ \ 
	\end{minipage}
	\begin{minipage}{.49\linewidth}
		\begin{algorithm}[H]
			\small
			\caption{The unifier in \textit{Eusolver}.}
			\label{alg:eusolver-uni}
			\LinesNumbered
			\KwIn{PBE task $T$, terms $P$, condition domain $\mathbb P_c$.}
			\KwOut{A valid program in $(P, \mathbb P_c)_{\text{DT}}$ or $\top$.}{
				\SetKwProg{Fn}{Function}{:}{}
				\Fn{\Learn{$\variable{examples}$}}{
					\If {$\exists p \in P, \variable{examples} \subseteq \Covered{p, T} $}{\Return $p$;}	
					$c \gets \Select{$\variable{examples}, \mathbb P_c$}$; \\
					$\variable{tE} \gets \{(I, O) \in \variable{examples}\ |\ \sem{c}(I)\}$; \\
					$\variable{fE} \gets \{(I, O) \in \variable{examples}\ |\ \neg \sem{c}(I) \}$; \\
					\lIf {$\variable{tE} = \emptyset \vee \variable{fE} = \emptyset$}{\Return $\top$}
					$t \gets \Learn{$tE$};$\ \
					$f \gets \Learn{$fE$};$ \\
					\lIf {$t = \top \wedge f = \top$}{\Return $\top$}
					\Return \texttt{if} $(c)$ \texttt{then} $t$ \texttt{else} $f$; \\
				}
				\Return {\Learn{$T$}};
			}
		\end{algorithm}
	\end{minipage}
\end{figure}
\todo{Example}

\subsection{Generalizability of STUN} \label{section:stun-gen}
In this section, we study the generalizability of the STUN framework. As mentioned before, a STUN solver is a combination of a term solver $\mathcal T$ and a unifier $\mathcal U_{\text{N}}$. Therefore, in this section, we would like to answer the question that: Under what conditions, term solver $\mathcal T$ and unifier $\mathcal U_{\text{N}}$ form a STUN solver with polynomial-size generalizability.

At first, we extend the concept of \textit{polynomial-size generalizability} to term solvers and unifiers: For a term solver in $\mathsf {PSG}$, there should be a polynomial that bounds the number of examples required to capture all behaviors of the target program; For a unifier in $\mathsf {PSG}$, there should be a universal polynomial that bounds the generation function for any set of terms.

\begin{definition} For normal form $\mathcal F_{C}^{\text{N}}$, term solver $\mathcal T$ has \textit{polynomial-size generalizability}, abbreviated as $\mathcal T \in \mathsf {PSG}[\mathcal F_C^{\text{N}}]$, if there exists a pollynomial $g(x, y)$ such that:
	\begin{align*}
		\forall ((\mathbb P_t, \mathbb P_c)_{\text{N}}, \mathbb I, \mathbb O) \in \mathcal F_{C}^{\text{N}}, \forall p \in (\mathbb P_t, \mathbb P_c)_{\text{N}}, &\forall \epsilon \in (0, 1), \forall n \geq g(\text{size}(p), \ln(1 / \epsilon)), \\ &\Pr_{I_1, \dots, I_n \sim D_I} \left[ \mathcal T\big((I_1, \sem{p}(I_1)), \dots, (I_n, \sem{p}(I_n)) \big) \not \triangleright_{\mathbb I} p\right] \leq \epsilon
	\end{align*}
	where $P \triangleright_{\mathbb I} p$ represents that program set $P$ covers the outputs of $p$ on all inputs in $\mathbb I$:
	$$
	P \triangleright_{\mathbb I} p \iff \forall I \in \mathbb I, \exists p' \in P, \sem{p}(I) = \sem{p'}(I)
	$$
\end{definition}

\begin{definition}\label{def:poly-unifier} For normal form $\mathcal F_{C}^{\text{N}}$, unifier $\mathcal U_{\text{N}}$ has  \textit{polynomial-size generalizability}, abbreviated as $\mathcal U_{\text{N}} \in \mathsf {PSG}[\mathcal F_C^{\text{N}}]$,  if there exists a polynomial $g(x, y)$ such that :
	$$ \forall P \subseteq \mathbb P_t, \forall p \in (P, \mathbb P_c)_{\text{N}}, \forall \epsilon \in (0, 1), \text{gen}[\mathcal U_{\text{N}}(P)](p, \epsilon) \leq g(\max(\text{tsize}(P), \text{size}(p)), \ln(1 / \epsilon))
	$$
	where $\text{tsize}(P)$ is defined as the total size of programs in $P$, i.e., $\sum_{p' \in P} \text{size}(p')$.
\end{definition}

Note that in Definition \ref{def:poly-unifier}, besides the size of the target program, the polynomial bound is also allowed to refer the total size of programs in the term set $P$. Such a relaxation allows the unifier to use more examples when an extremely large term set is provided.

However, a STUN solver merged by a term solver in $\mathsf {PSG}[\mathcal F_C^{\text{N}}]$ and a unifier in $\mathsf {PSG}[\mathcal F_C^{\text{N}}]$ are not guaranteed to have polynomial-size generalizability for normal form $\mathcal F_C^{\text{N}}$. The main reason is that, the term solver may produce an extremely large set $P$ of terms, and thus makes the size of the smallest valid program in $(P, \mathbb P_c)$ exponentially larger than the target program. Such a defect can be fixed by extending the concept of \textit{size-preserving} to term solvers.

\begin{definition} \label{def:size-preserve}A term solver $\mathcal T$ is \textit{size-preserving} for normal form $\mathcal F_{C}^{\text{N}}$ if there exists a polynomial $s(x, y)$ such that:
	\begin{align*}
		\forall ((\mathbb P_c, \mathbb P_t)_{\text{N}}, \mathbb I, \mathbb O) \in \mathcal F_{C}^{\text{N}},& \forall n > 0, \forall p \in (\mathbb P_t, \mathbb P_c), \forall \epsilon \in (0, 1), \\
		&Pr\left[\text{tsize}\left( \mathcal T\big((I_1, \sem{p}(I_1)), \dots, (I_n, \sem{p}(I_n))\big)\right) > s\left(\text{size}(p),  \ln \left(1/\epsilon\right)\right)\right] \leq \epsilon
	\end{align*}
\end{definition}

\begin{theorem} \label{theorem:gen-stun}Given a term solver $\mathcal T$ and a unifir $\mathcal U_{\text{N}}$, define $\mathcal T'$ and $\mathcal U_{\text{N}}'$ as a term solver and a unifier constructed as following:
	$$
	\mathcal T'(e_1, \dots, e_n) = \mathcal T\left(e_1, \dots, e_{\lfloor \frac{n}{2}\rfloor}\right)\ \ \ \ \mathcal U_{\text{N}}'(P)(e_1, \dots, e_n) = \mathcal U_{\text{N}}(P)\left(e_{\lfloor \frac{n}{2} \rfloor + 1}, \dots, e_{n}\right)
	$$
	The STUN solver induced by $\mathcal T'$ and $\mathcal U_{\text{N}}'$ has polynomial-size generalizability on $\mathcal F_{C}^{\text{N}}$ if (1) $\mathcal T$ is size-preserving for $\mathcal F_{C}^N$; (2) $\mathcal U_{\text{N}}$ has polynomial-size generalizability for $\mathcal F_{C}^{\text{N}}$, i.e., $\mathcal U_{\text{N}} \in \mathsf{PSG}[\mathcal F_{C}^{\text{N}}]$.
\end{theorem}

\subsection{Generalizability of \textit{Eusolver}} \label{section:eusolver-gen}
In this section, we analysize the generalizability of \textit{Eusolver} using the abstracted generation model. There are two main defects on the generalizability of \textit{Eusolver}.

The first defect is that the term solver in \textit{Eusolver} may return a term set that is exponentially larger than the terms used by the target program.

\begin{lemma} \label{lemma:eusolver-size} The term solver in \textit{Eusolver} (Algorithm \ref{alg:eusolver-term}) is not size-preserving for $\mathcal F_{C}^{\text{DT}}$.
\end{lemma}
\begin{proof} Consider the following term domain $\mathbb P_t^n$, input domain $\mathbb I_t^n$ and target program $p$:
	$$
	\mathbb P_t^n = \{2, 3, \dots, 2n, x + y\}\ \ \ \mathbb I_t^n = \big\{(x_0, y_0)\ \big|\ x_0, y_0 \in [1, n]\big\}\ \ \ p = x+ y
	$$
	As $x + y$ is the largest program in $\mathbb P_t^n$, when the number of examples is large enough, the term solver in \textit{Eusolver} will return $P = \{2, 3, \dots, 2n\}$ as the result instead of the term set $\{x + y\}$ used by the target program.  According to the definition of the size, $\text{tsize}(P) = \Omega(n \log n)$, $\text{size}(p) = O(\log n)$. Therefore, the returned term set can be exponentially larger than the the target program, and thus the term solver in \textit{Eusolver} is not size-preserving for $\mathcal F_{C}^{\text{DT}}$.
\end{proof}

The construction in Lemma \ref{lemma:eusolver-size} can also be used to prove that the generalizability of \textit{Eusolver} is not polynomial for normal form $\mathcal F_C^{\text{DT}}$.

\begin{theorem}\label{theorem:gen-eusolver} $\textit{Eusolver} \not \in \mathsf {PSG}[\mathcal F_{C}^{\text{DT}}]$.
\end{theorem}
\begin{proof} \todo{Complete the proof}.
\end{proof}

The second shortage of \textit{Eusolver }is that the expressiveness of normal form $\mathcal F_{C}^{\text{DT}}$ is not enough: $\mathcal F_{C}^{\text{DT}}$ may use an exponentially larger program to implement some common programs in a conditional program domain, as shown in the following example.

\begin{example} \label{example:uni-eusolver}
	Consider a series of tasks $\texttt{max}_n = (\mathbb P_t^n, \mathbb P_c^n, p_n)$ constructed as the following:
	$$
	\mathbb P_t^n = \{x_1, \dots, x_n\}\ \ \ \mathbb P_c^n = \{x_i\leq x_j\ |\ 1 \leq i,j \leq n\}\ \ \ \sem{p_n}(x_1, \dots, x_n) = \max(x_1, \dots, x_n)
	$$
	
	In domain $(\mathbb P_t^n, \mathbb P_c^n)$, $p_n$ can be implemented as a program of size $O(n^2\log n)$:
	\begin{align*}
		p_n = &\ \texttt{if}\ ((x_2 \leq x_1)\ \texttt{and}\ (x_3 \leq x_1)\ \texttt{and}\ \dots\ \texttt{and}\ (x_n \leq x_1))\ \texttt{then}\ x_1 \\
		& \ \texttt{else if}\ ((x_3 \leq x_2)\ \texttt{and}\ (x_4 \leq x_2)\ \texttt{and}\ \dots\ \texttt{and}\ (x_n \leq x_2))\ \texttt{then}\ x_2 \\
		&\ \dots \\
		&\ \texttt{else if}\ (x_{n-1} \leq x_n)\ \texttt{then}\ x_{n-1}\ \texttt{else}\ x_n
	\end{align*}
	
	Let $p'_n$ be the smallest program in $(\mathbb P_t^n, \mathbb P_c^n)_{\text{DT}}$ that is semantically equivalent to $p_n$, and let $t$ be a term used in $p'_n$. Suppose $t$ is constrained by $m$ \texttt{if}-conditions, and the corresponding conditions are $c_1, \dots, c_m$. According to the definition of $()_{\text{DT}}$, $c_i$ is either an expression in $\mathbb P_c^n$ or the negation of an expression in $\mathbb P_c^n$, corresponding to the \texttt{then}-branch and the \texttt{else}-branch respecitively.
	
	We make the following two claims:
	
	\textit{Claim 1: } There exists an input satisfying $c_1 \wedge \dots \wedge c_m$. Otherwise, term $t$ can be removed from $p'_n$, resulting in a strictly smaller program equivalent to $p_n$. This is conflict with the definition of $p'_n$.
	
	\textit{Claim 2: } $m \geq n - 1$. As $\mathbb P_c^n$ contains only simple comparisons, each $c_i$ can only constrain the relative order between two input variables. Therefore, when $m < n - 1$, there must exists two different variables $x_i, x_j$ such that there is no direct or indirect constraint on their relative order. Without loss of generality, let $x_i$ be different from $t$. By claim 1, there exists an input satisfying $c_1 \wedge \dots \wedge c_m$. Therefore, there must be an input satisfying $c_1 \wedge \dots \wedge c_m \wedge x_j > t$, as the relative order between $x_i, x_j$ is not constraned. This is conflict with $p'_n \sim_{\mathbb I} p_n$.
	
	By Claim $2$, all terms used in $p'_n$ is constrained by at least $n-1$ \texttt{if}-conditions. Therefore, these must be at least $2^{n-1}-1$ \texttt{if-then-else} operators in $p'_n$. Hense, $\text{size}(p') = \Omega(2^n \log n)$, which is exponentially larger than $p_n$.
	
	Further, as the unifier in \textit{Eusolver} returns immediately when there is a term covering all examples, there must be at least two examples remaining when synthesizing each \texttt{if} condition. Therefore, to solve $\texttt{max}_n$, \textit{Eusolver} requires at least $2^n - 2$ examples.
\end{example}

\subsection{Overview for \mainname}
Guiuded by the two defects of \textit{Eusolver} and Lemma \ref{theorem:gen-stun}, \mainname improves the generalizability of \textit{Eusolver} in two aspects:
\begin{itemize}
	\item Different from \textit{Eusolver}, the term solver $\mathcal T_{\text{poly}}$ in \mainname is designed to be size-preserving. 
	\item The unifier $\mathcal U_{\text{poly}}$ is designed for a new normal form $\mathcal F_{C}^{\text{DNF}}$, which is more compact than $\mathcal F_{C}^{\text{DT}}$. Moreover, $\mathcal U_{\text{poly}}$ is designed to have polynomial-size generalizability to enable Theorem \ref{theorem:gen-stun}.
\end{itemize}

The DNF normal form $(\mathbb P_t, \mathbb P_C)_{\text{DNF}}$ used by \mainname requires the program structre to be linear, and requires all \texttt{if}-conditions in the program to be disjunctive normal forms. Formally, $(\mathbb P_t, \mathbb P_c)_{\text{DNF}}$ is the smallest set of programs such that:
$$
(\mathbb P_t, \mathbb P_c)_{\text{DNF}}= \mathbb P_t \cup \left\{\texttt{if}\ c\ \texttt{then}\ t\ \texttt{else}\ p\ |\ t \in \mathbb P_t, p \in (\mathbb P_t, \mathbb P_c)_{\text{DNF}}, c \in \text{DNF}(\mathbb P_c) \right\}
$$
where $\text{DNF}(\mathbb P_c)$ is the set of all disjunctive normal form formed by boolean expressions in $\mathbb P_c$, which is the smallest set satisfying:
$$
\text{DNF}(\mathbb P_c) = \left\{\texttt{and}_{p \in P}\ p\ \big |\ P \subseteq \mathbb P_c\right\} \cup \left\{\left(\texttt{and}_{p \in P}\ p\right)\ \texttt{or}\ d\ \big |\ P \subseteq \mathbb P_c, d \in \text{DNF}(\mathbb P_c)\right\}
$$

The following theorem shows that the expressiveness of $\mathcal F_C^{\text{DNF}}$ is no worse than $\mathcal F_C^{\text{DT}}$ in the terms of polynomial-size generalizability: Any PBE solver in $\mathsf {PSG}[\mathcal F_{C}^{\text{DNF}}]$ can also be used as a solver with polynomial-size generalizability for $\mathcal F_C^{\text{DT}}$.

\begin{theorem} Define normal form $\mathcal F_C^{\text{M}}$ as the join of $\mathcal F_C^{\text{DT}}$ and $\mathcal F_C^{\text{DNF}}$, i.e., $(\mathbb P_t, \mathbb P_c)_{\text{M}} \coloneqq (\mathbb P_t, \mathbb P_c)_{\text{DT}} \cup (\mathbb P_t, \mathbb P_c)_{\text{DNF}}$. For any PBE solver $\mathcal S$, $\mathcal S \in \mathsf {PSG}[\mathcal F_{C}^{\text{DNF}}] \implies \mathcal S \in \mathsf {PSG}[\mathcal F_{C}^{\text{M}}]$.
\end{theorem}

Moreover, Example \ref{example:dnf} shows that the expressiveness of $\mathcal F_C^{\text{DNF}}$ is strictly stronger than $\mathcal F_C^{\text{DT}}$.

\begin{example} \label{example:dnf}Program $p_n$ introduced in Example \ref{example:uni-eusolver} is included in $(\mathbb P_t^n, \mathbb P_c^n)_{\text{DNF}}$. Therefore, to solve task $\texttt{max}_n$, $\mathcal F_C^{\text{DNF}}$ can use a program that is exponentially smaller than $\mathcal F_C^{\text{DT}}$.
\end{example}

Therefore, the generalizability of \mainname is better than \textit{Eusolver} in two levels: (1) \mainname has polynomial-size generalizability on its normal form but \textit{Eusolver} does not; (2) The normal form used by \mainname is strictly better than \textit{Eusolver} for the generalizability.

\endinput

==> sections/STUN2.tex <==
%!TEX root = ../CLIA.tex
\section{Synthesis Through Unification} \label{section:stun}
To evaluate the effectiveness of our abstarcted generalization model and class $\mathsf{PSG}$, in the second part of this paper, we study the framework of \textit{synthesis through unification (STUN)}. STUN is deigned for synthesizing programs with nested \texttt{if-then-else} operators quickly, and it does not take the generalizability into consider. As a result, though the STUN framework achieves great success on the speed, the generalizability of existing STUN solvers is unsatisfiable: As shown in Section \ref{section:eusolver-gen}, even the state-of-the-art STUN solver is not inside $\mathsf {PSG}$.
\todo{move this part to the introduction.}

In this section, we study the generalizability of STUN and its solvers. In Section \ref{section:stun-pre} and \ref{section:eusolver-pre}, we introduce some necessary preliminaries on STUN and a state-of-the-art STUN solver, named \textit{Eusolver}, respectively. Then, in Section \ref{section:stun-gen}, we study the condition for a STUN solver to have polynomial-size generalizability. At last, in Section \ref{section:eusolver-gen}, we prove that \textit{Eusolver} is not inside $\mathsf{PSG}$.

\subsection{Preliminaries: Synthesis through Unification} \label{section:stun-pre}
The framework of \textit{synthesis through unification (STUN)} focuses on a special kind of synthesis tasks, where the program space supports enough flexibility for \texttt{if-then-else} operators. Formally, STUN assumes that the program space can be decomposed into two subspaces, for \texttt{if}-conditions and \texttt{if}-terms respectively. 

\begin{definition}A program space $\mathbb P$ is a conditional program space if and only if there exist two program spaces $\mathbb P_c$ and $\mathbb P_t$ such that $\mathbb P$ is the smallest set of programs such that:
	$$
	\mathbb P = \mathbb P_t \cup \left\{\texttt{if}\ c\ \texttt{then}\ p_1\ \texttt{else}\ p_2\ |\ p_1, p_2 \in \mathbb P, c \in \mathbb P_c  \right\}
	$$
\end{definition}
For convenience, we use a pair of program spaces $(\mathbb P_t, \mathbb P_c)$ to denote a conditional program space derived from term space $\mathbb P_t$ and condition space $\mathbb P_c$. Besides, we call a domain $\mathbb D$ \textit{conditional} if the corresponding program space is conditional.

A STUN solver synthesizes programs in two steps:
\begin{enumerate}
	\item A term solver is invoked to synthesize a set of programs $P \subseteq \mathbb P_t$ such that for any possible input $I$, there is always a program $p \in P$ such that $\sem{p}(I)$ is a valid output.
	\item A unifier is invoked to unify $P$ into a single program in the normal form $(P, \mathbb P_c)_{\text{N}}$ \yxcomment{Has the normal form been defined?} using \texttt{if-then-else} operators and \texttt{if}-conditions inside $C(\mathbb P_c)$.
\end{enumerate}
In this paper, we only consider the specialized version of the STUN framework on PBE tasks.

\begin{definition}[Term Solver] Given a conditional domain $\mathbb D$, a term solver $\mathcal T: (\mathbb I \times \mathbb O)^* \mapsto \{\top\} \cup \mathcal P(\mathbb P_t)$ is a function satisfying the following two conditions for any PBE task $T \in (\mathbb I, \mathbb O)^*$:
	\begin{itemize}
		\item (Soundness) If $\mathcal T(T)$ is a set of programs, for every example $e$ in $T$, there is always a program in $\mathcal T(T)$ consistent with $e$:
		$$\mathcal T(T) \subseteq \mathbb P_t \implies \forall (I,O) \in T, \exists p \in \mathcal T(T), \sem{T}(I) = O$$
		\item (Completeness) If $\mathcal T(T) = \top$,  all subsets of $\mathcal P_t$ must violate at least one example in $T$:
		$$\mathcal T(T) = \top \iff \forall P \subseteq \mathbb P_t, \exists (I,O) \in T, \forall p \in P, \sem{p}(I) \neq O$$
	\end{itemize}
	where $\mathcal P(\mathbb P_t)$ represents the power set of $\mathbb P_t$.
\end{definition}

\begin{definition}[Unifier] Given a conditional domain $\mathbb D$, a unifier $\mathcal U_{\text{N}}$ is a function such that for any set of terms $P \subseteq \mathbb P_t$, $\mathcal U_{\text{N}}(P)$ is a valid PBE solver for $(P, \mathbb P_c)$.
\end{definition}

In the STUN framework, a solver is comprised of a term solver $\mathcal T$ and a unifer $\mathcal U$. Given a PBE task $T$, the synthesizer simply returns $\mathcal U(\mathcal T(T))(T)$ as the result. 

The soundness of STUN is straight-forward from the soundness of $\mathcal T$ and $\mathcal U$. In contrast, the completeness of STUN is guaranteed only when the domain is \textit{if-closed}. Intuitively, a domain is if-closed if the condition space can express the condition for any two terms to perform the same.

\begin{definition}[If-Closed] A conditional domain $\mathbb D$ is \textit{if-closed} if: $$\forall p_1, p_2 \in \mathbb P_t, \exists c \in C(\mathbb P_c), \forall I \in \mathbb I, \left(\sem{c}(I) \iff \sem{p_1}(I) = \sem{p_2}(I)\right)$$
where $C(\mathbb P_C)$ represents all conditions comprised of $\mathbb P_C$, i.e., $C(\mathbb P_C)$ is the smallest subset such that:
$$
C(\mathbb P_c) = \mathbb P_c \cup \left\{c_1\ \texttt{and}\ c_2\ |\ c_1,c_2 \in C(\mathbb P_c)\right\} \cup  \left\{c_1\ \texttt{or}\ c_2\ |\ c_1,c_2 \in C(\mathbb P_c)\right\} \cup \{\texttt{not}\ c\ |\ c \in C(\mathbb P_c)\}
$$
\end{definition}

\begin{theorem} \label{lemma:completeness}  STUN is complete on conditional domain $\mathbb D$ if the program space is if-closed.
\end{theorem}

For other domains, STUN can be extended to complete by backtracking to the term solver when the unification fails, as done by related works ~\cite{DBLP:conf/cav/AlurCR15, DBLP:conf/tacas/AlurRU17}.

In the remainder of this paper, we focus on if-closed program domains only. We use $\mathcal F_{C}$ to denote a family of if-closed conditional domains.

\subsection{Preliminaries: \textit{EuSolver}} \label{section:eusolver-pre}
\textit{Eusolver}~\cite{DBLP:conf/tacas/AlurRU17} is a state-of-the-art synthesizer following the STUN framework. In this section, we shall briefly introduce the algorithm of \textit{Eusolver}.

\SetKwFunction{Enum}{Enumerate}
\SetKwFunction{Covered}{Covered}
\SetKwFunction{Learn}{LearnDT}
\SetKwFunction{Select}{SelectCond}

Algorithm \ref{alg:eusolver-term} shows the pseudo code of the term solver in \textit{Eusolver}. The term solver enumerates programs in domain $\mathbb P_t$ in the increasing order of the size (Line 4). For each program $p$, if there is not a visited program that satisfies exactly the same subset of examples as $p$, $p$ will be included into the result (Lines 6-8). The enumeration ends when the enumerated programs are enough to cover all examples in $T$ (Line 9).

Algorithm \ref{alg:eusolver-uni} shows the pseudo code of the unifier in \textit{Eusolver}, which is from \textit{ID3}~\cite{DBLP:journals/ml/Quinlan86}, a standard multi-label decision tree learning algorithm. The unifier uses function \Learn{\variable{examples}} to recursively synthesize a program satisfying all examples in \variable{examples} (Lines 1-11). In each step, the unifier firstly tries to use a term to cover all examples (Lines 2-4). Then, it picks up a condition $c$ in $\mathbb P_c$ based on some greedy strategy, and synthesizes a program in the form of \texttt{if} $(c)$ \texttt{then} $t$ \texttt{else} $f$ (Line $5$).  To form a correct program, program $t$ and $f$ must satisfy all examples on which $c$ is evaluated to true and false respectively (Lines 6-7). Therefore, the unifier recursively invokes $\Learn$ to synthesize proper programs $t$ and $f$ (Line $9$). 

\begin{figure}[t]
	\begin{minipage}{.46\linewidth}
		\begin{algorithm}[H]
			\small
			\caption{The term solver in \textit{Eusolver}.}
			\label{alg:eusolver-term}
			\LinesNumbered
			\KwIn{PBE task $T$ and domain $\mathbb P_t$.}
			\KwOut{A set of programs in $\mathbb P_t$ or $\top$.}
			\SetKwProg{Fn}{Function}{:}{}
			\Fn{\Covered{$p, T$}}{\Return $\left\{(I,O)\ |\ (I,O) \in T \wedge \sem{p}(I) = O\right \}$;}
			\variable{covered} $\gets \emptyset$; \ \ \variable{result} $\gets \emptyset$; \\
			\For{each $p \in \Enum{$\mathbb P_t$}$}{
				\If {$\forall p' \in \variable{result}, \Covered{$p, T$} \neq \Covered{$p', T$}$}{
					$\variable{covered} \gets \variable{covered} \cup \Covered{$p, T$}$; \\
					$\variable{result} \gets \variable{result} \cup \{p\}$;
				}
				\lIf {$\variable{covered} = T$}{\Return \variable{covered}}
			}
			\Return $\top$;
		\end{algorithm}
		\ \ 
	\end{minipage}
	\begin{minipage}{.49\linewidth}
		\begin{algorithm}[H]
			\small
			\caption{The unifier in \textit{Eusolver}.}
			\label{alg:eusolver-uni}
			\LinesNumbered
			\KwIn{PBE task $T$, terms $P$, condition domain $\mathbb P_c$.}
			\KwOut{A valid program in $(P, \mathbb P_c)$ or $\top$.}{
				\SetKwProg{Fn}{Function}{:}{}
				\Fn{\Learn{$\variable{examples}$}}{
					\If {$\exists p \in P, \variable{examples} \subseteq \Covered{p, T} $}{\Return $p$;}	
					$c \gets \Select{$\variable{examples}, \mathbb P_c$}$; \\
					$\variable{tE} \gets \{(I, O) \in \variable{examples}\ |\ \sem{c}(I)\}$; \\
					$\variable{fE} \gets \{(I, O) \in \variable{examples}\ |\ \neg \sem{c}(I) \}$; \\
					\lIf {$\variable{tE} = \emptyset \vee \variable{fE} = \emptyset$}{\Return $\top$}
					$t \gets \Learn{$tE$};$\ \
					$f \gets \Learn{$fE$};$ \\
					\lIf {$t = \top \wedge f = \top$}{\Return $\top$}
					\Return \texttt{if} $(c)$ \texttt{then} $t$ \texttt{else} $f$; \\
				}
				\Return {\Learn{$T$}};
			}
		\end{algorithm}
	\end{minipage}
\end{figure}
\todo{Example}

\subsection{Generalizability of STUN} \label{section:stun-gen}
In this section, we study the generalizability of the STUN framework. As mentioned before, a STUN solver is a combination of a term solver $\mathcal T$ and a unifier $\mathcal U$. Therefore, in this section, we would like to answer the question that: Under what conditions, term solver $\mathcal T$ and unifier $\mathcal U$ form a STUN solver with polynomial-size generalizability.

At first, we extend the concept of \textit{polynomial-size generalizability} to term solvers and unifiers: For a term solver in $\mathsf {PSG}$, there should be a polynomial that bounds the number of examples required to cover the outputs of $p$ on all possible inputs; For a unifier in $\mathsf {PSG}$, there should be a universal polynomial that bounds the generation function for any set of terms.

\begin{definition} For a family of domains $\mathcal F_C$, term solver $\mathcal T$ has \textit{polynomial-size generalizability}, abbreviated as $\mathcal T \in \mathsf {PSG}[\mathcal F_C]$, if there exists a pollynomial $g(x, y)$ such that:
	\begin{align*}
		\forall \mathbb D \in \mathcal F_{C}, \forall p \in (\mathbb P_t, \mathbb P_c), &\forall \epsilon \in (0, 1), \forall n \geq g(\text{size}(p), \ln(1 / \epsilon)), \\ &\Pr_{I_1, \dots, I_n \sim D_I} \left[ \mathcal T\big((I_1, \sem{p}(I_1)), \dots, (I_n, \sem{p}(I_n)) \big) \not \triangleright_{\mathbb I} p\right] \leq \epsilon
	\end{align*}
	where $P \triangleright_{\mathbb I} p$ represents that program set $P$ covers the outputs of $p$ on all inputs in $\mathbb I$:
	$$
	P \triangleright_{\mathbb I} p \iff \forall I \in \mathbb I, \exists p' \in P, \sem{p}(I) = \sem{p'}(I)
	$$
\end{definition}

\begin{definition}\label{def:poly-unifier} For a family of domains $\mathcal F_C$ unifier $\mathcal U$ has  \textit{polynomial-size generalizability}, abbreviated as $\mathcal U_{\text{N}} \in \mathsf {PSG}[\mathcal F_C]$,  if there exists a polynomial $g(x, y)$ such that :
	\begin{align*} \forall \mathbb D \in \mathcal F_C, &\forall P \subseteq \mathbb P_t, \forall p \in (P, \mathbb P_c), \forall \epsilon \in (0, 1), \\ &\text{gen}[((P, \mathbb P_c), \mathbb I), \mathcal U(P)](p, \epsilon) \leq g(\max(\text{tsize}(P), \text{size}(p)), \ln(1 / \epsilon))
	\end{align*}
	where  $\text{tsize}(P)$ is defined as the total size of programs in $P$, i.e., $\sum_{p' \in P} \text{size}(p')$.
\end{definition}

Note that in Definition \ref{def:poly-unifier}, besides the size of the target program, the polynomial bound is also allowed to refer the total size of programs in the term set $P$. Such a relaxation allows the unifier to use more examples when an extremely large term set is provided.

However, a STUN solver merged by a term solver in $\mathsf {PSG}[\mathcal F_C]$ and a unifier in $\mathsf {PSG}[\mathcal F_C]$ is not guaranteed to have polynomial-size generalizability for $\mathcal F_C$. The main reason is that, the term solver may produce an extremely large set $P$ of terms, and thus makes the size of the smallest valid program in $(P, \mathbb P_c)$ exponentially larger than the target program. Such a defect can be fixed by extending the concept of \textit{size-preserving} to term solvers.

\begin{definition} \label{def:size-preserve}A term solver $\mathcal T$ is \textit{size-preserving} for $\mathcal F_{C}$ if there is a polynomial $s(x, y)$ such that:
	\begin{align*}
		\forall \mathbb D \in \mathcal F_{C},& \forall n > 0, \forall p \in (\mathbb P_t, \mathbb P_c), \forall \epsilon \in (0, 1), \\
		&Pr\left[\text{tsize}\left( \mathcal T\big((I_1, \sem{p}(I_1)), \dots, (I_n, \sem{p}(I_n))\big)\right) > s\left(\text{size}(p),  \ln \left(1/\epsilon\right)\right)\right] \leq \epsilon
	\end{align*}
\end{definition}

\begin{theorem} \label{theorem:gen-stun}Given a term solver $\mathcal T$ and a unifir $\mathcal U$, define $\mathcal T'$ and $\mathcal U'$ as the following:
	$$
	\mathcal T'(e_1, \dots, e_n) = \mathcal T\left(e_1, \dots, e_{\lfloor \frac{n}{2}\rfloor}\right)\ \ \ \ \mathcal U'(P)(e_1, \dots, e_n) = \mathcal U(P)\left(e_{\lfloor \frac{n}{2} \rfloor + 1}, \dots, e_{n}\right)
	$$
	The STUN solver induced by $\mathcal T'$ and $\mathcal U'$ has polynomial-size generalizability for $\mathcal F_{C}$ if (1) $\mathcal T$ is size-preserving for $\mathcal F_{C}$; (2) $\mathcal U_{\text{N}}$ has polynomial-size generalizability for $\mathcal F_{C}$, i.e., $\mathcal U \in \mathsf{PSG}[\mathcal F_{C}]$.
\end{theorem}

\subsection{Generalizability of \textit{Eusolver}} \label{section:eusolver-gen}
In this section, we analysize the generalizability of \textit{Eusolver} using the abstracted generation model. There are two main defects on the generalizability of \textit{Eusolver}.

The first defect is that the term solver in \textit{Eusolver} may return a term set that is exponentially larger than the terms used by the target program.

\begin{lemma} \label{lemma:eusolver-size} Let $\mathcal F_{C}^A$ be the family of all conditional domains. The term solver in \textit{Eusolver} (Algorithm \ref{alg:eusolver-term}) is not size-preserving for $\mathcal F_{C}^A$.
\end{lemma}
\begin{proof} Consider the following term domain $\mathbb P_t^n$, input domain $\mathbb I_t^n$ and target program $p$:
	$$
	\mathbb P_t^n = \{2, 3, \dots, 2n, x + y\}\ \ \ \mathbb I_t^n = \big\{(x_0, y_0)\ \big|\ x_0, y_0 \in [1, n]\big\}\ \ \ p = x+ y
	$$
	As $x + y$ is the largest program in $\mathbb P_t^n$, when the number of examples is large enough, the term solver in \textit{Eusolver} will return $P = \{2, 3, \dots, 2n\}$ as the result instead of the term set $\{x + y\}$ used by the target program.  According to the definition of the size, $\text{tsize}(P) = \Omega(n \log n)$, $\text{size}(p) = O(\log n)$. Therefore, the returned term set can be exponentially larger than the the target program, and thus the term solver in \textit{Eusolver} is not size-preserving for $\mathcal F_{C}^A$.
\end{proof}

The construction in Lemma \ref{lemma:eusolver-size} can also be used to prove that the generalizability of \textit{Eusolver} is not polynomial for $\mathcal F_C^A$.

\begin{theorem}\label{theorem:gen-eusolver} $\textit{Eusolver} \not \in \mathsf {PSG}[\mathcal F_{C}^A]$.
\end{theorem}
\begin{proof} \todo{Complete the proof}.
\end{proof}

The second shortage of \textit{Eusolver} is actually from the definition of conditional domains. As the conditional domain requires that only conditions in $\mathcal P_c$ can be used as \texttt{if}-conditions, it may use an extremely large program to implement some common functionality, as shown in Example \ref{example:uni-eusolver}.

\begin{example} \label{example:uni-eusolver}
	Consider tasks $\texttt{max}_n = (\mathbb D^n = ((\mathbb P_t^n, \mathbb P_c^n), \mathbb I), p_n)$ constructed as the following:
	\begin{align*}
	\mathbb P_t^n = \{x_1, \dots, x_n\}&\ \ \ \ \mathbb P_c^n = \{x_i\leq x_j\ |\ 1 \leq i,j \leq n\}\ \ \ \ \mathbb I^n = \{0, 1, \dots, 2n\}^{n} \\ &\sem{p_n}(x_1, \dots, x_n) = \max(x_1, \dots, x_n)
	\end{align*}
	
	%In domain $(\mathbb P_t^n, \mathbb P_c^n)$, $p_n$ can be implemented as a program of size $O(n^2\log n)$:
	
	We start by showing that a program with a size exponentially to $n$ is necessary to implement $p_n$ in conditional program space $(\mathbb P_t^n, \mathbb P_c^n)$.
	
	Let $p'_n$ be the smallest program in $(\mathbb P_t^n, \mathbb P_c^n)$ that implements $p_n$, and let $t$ be an arbitary term used in $p'_n$. Suppose $t$ is constrained by $m$ \texttt{if}-conditions, and the corresponding conditions are $c_1, \dots, c_m$. By the definition of the conditional program space, $c_i$ is either a condition in $\mathbb P_c^n$ or the negation of a condition in $\mathbb P_c^n$, corresponding to the \texttt{then}-branch and the \texttt{else}-branch respecitively.
	
	To obtain a lower bound on $\text{size}(p'_n)$, we make the following two claims:
	
	\textit{Claim 1: } There is an input satisfying $c_1 \wedge \dots \wedge c_m$. Otherwise, term $t$ can be removed from $p'_n$, resulting in a strictly smaller program equivalent to $p_n$. This is conflict with the definition of $p'_n$.
	
	\textit{Claim 2: } $m \geq n - 1$. As $\mathbb P_c^n$ contains only simple comparisons, each $c_i$ can only constrain the relative order between two input variables. Therefore, when $m < n - 1$, there must exists two different variables $x_i, x_j$ such that there is no direct or indirect constraint on their relative order. Without loss of generality, let $x_i$ be different from $t$. By claim 1, there exists an input satisfying $c_1 \wedge \dots \wedge c_m$. Therefore, there must be an input satisfying $c_1 \wedge \dots \wedge c_m \wedge x_j > t$, as the relative order between $x_i, x_j$ is not constraned. This is conflict with $p'_n \sim_{\mathbb I} p_n$.
	
	By Claim $2$, all terms used in $p'_n$ is constrained by at least $n-1$ \texttt{if}-conditions. Therefore, these must be at least $2^{n-1}-1$ \texttt{if-then-else} operators in $p'_n$. Hense, $\text{size}(p') = \Omega(2^n \log n)$, which is exponentially larger than $p_n$.
	
	As the unifier in \textit{Eusolver} returns immediately when there is a term covering all examples, there must be at least two examples remaining when synthesizing each \texttt{if} condition. Therefore, to solve $\texttt{max}_n$, \textit{Eusolver} requires at least $2^n - 2$ examples.
	
	However, the size required to implement $p_n$ can be exponentially reduced if we allow boolean operators \texttt{and}, \texttt{or} and \texttt{not} to be used in \texttt{if}-conditions. Concretely, the following program $p''_n$ implements $p_n$ and the size of $p''_n$ is only $O(n^2 \log n)$. 
	\begin{align*}
		p_n'' = &\ \texttt{if}\ ((x_2 \leq x_1)\ \texttt{and}\ (x_3 \leq x_1)\ \texttt{and}\ \dots\ \texttt{and}\ (x_n \leq x_1))\ \texttt{then}\ x_1 \\
		& \ \texttt{else if}\ ((x_3 \leq x_2)\ \texttt{and}\ (x_4 \leq x_2)\ \texttt{and}\ \dots\ \texttt{and}\ (x_n \leq x_2))\ \texttt{then}\ x_2 \\
		&\ \dots \\
		&\ \texttt{else if}\ (x_{n-1} \leq x_n)\ \texttt{then}\ x_{n-1}\ \texttt{else}\ x_n
	\end{align*}
\end{example}

\subsection{Overview for \mainname}
Motivated by the two defects of \textit{Eusolver} dicussed in the previous section, \mainname improves the generalizability of \textit{Eusolver} in two aspects:
\begin{itemize}
	\item Different from \textit{Eusolver}, the term solver $\mathcal T_{\text{poly}}$ of \mainname is designed to be size-preserving.
	\item The unifier $\mathcal U_{\text{poly}}$ is not only designed to have polynomial-size generalizability for conditional program spaces, but also for a more compact intermediate form, namely \textit{linear disjunctive normal form (LDNF)}. 
\end{itemize}

In the remainder of this section, we shall introduce the linear disjunctive normal form used by $\mathcal U_{\text{poly}}$. The concrete algorithms of $\mathcal T_{\text{poly}}$ and $\mathcal U_{\text{poly}}$ will be left to Section \ref{section:term-solver} and Section \ref{section:unifier} respectively.

\begin{definition} For conditional program domian $\mathbb D$, a program $p$ is of \textit{linear disjunctive normal form (LDNF)} if is satisfies the following three conditions:
	\begin{itemize}
		\item The structure of $p$ is linear, i.e., $p$ is in the form of:
		$$
		\texttt{if}\ (c_1)\ \texttt{then}\ t_1\ \texttt{else}\ \texttt{if}\ (c_2)\ \texttt{then}\ t_2\ \texttt{else} \dots \texttt{if}\  (c_{n})\ \texttt{then}\ t_{n}\ \texttt{else}\ \texttt{dummy}
		$$
		where \texttt{dummy} is a dummy value that is never used.
		\item \texttt{if}-terms $t_1, \dots, t_n$ used in $p$ are all from term space $\mathbb P_t$, and \texttt{if}-conditions $c_1, \dots, c_n$ used in $p$ are all from $\text{DNF}(\mathbb P_c)$, disjuctive normal forms comprised of $\mathbb P_c$. $\text{DNF}(\mathbb P_c)$ is defined in three steps:
		\begin{enumerate}
			\item $\text{L}(\mathbb P_c)$ is the set of literals comprised of $\mathbb P_c$, i.e., $\text{L}(\mathbb P_c) = \{\texttt{not } p\ |\ p \in \mathbb P_c\} \cup \mathbb P_c$
			\item $\text{CL}(\mathbb P_c)$ is the set of clauses compised of $\mathbb P_c$. $\text{CL}(\mathbb P_c)$ is the smallest set such that:
			$$\text{CL}(\mathbb P_c) = \{\texttt{true}\} \cup \{l\ \texttt{and}\ c\ |\ l \in \text{L}(\mathbb P_c), c \in \text{CL}(\mathbb P_c)\}$$
			\item $\text{DNF}(\mathbb P_c)$ is the smallest set such that:
			$$\text{DNF}(\mathbb P_c) = \{\texttt{false}\} \cup \{c\ \texttt{or}\ d\ |\ c \in \text{CL}(\mathbb P_c), d \in \text{DNF}(\mathbb P_c)\}$$
		\end{enumerate}
		\item  \texttt{if}-conditions $c_1, \dots, c_n$ are disjoint and the union of them covers the entire input space:
		$$
		\left(\forall I \in \mathbb I, \exists i \in [1, n], \sem{c_j}(I)\right) \wedge \left(\forall 1 \leq i < j < n, \forall I \in \mathbb I, \neg \left(\sem{c_i}(I) \wedge \sem{c_j}(I)\right)\right)
		$$
	\end{itemize}
\end{definition}

LDNF is designed to be more compact than the conditonal program space in the terms of polynomial-size generalizability. On the one hand, as shown in Lemma \ref{lemma:ldnf}, any program in a conditional domain can be converted to an LDNF of which the size is at most squared. On the other hand, as shown in Example \ref{example:ldnf}, the LDNF may be exponentially smaller than the origin program.

\begin{lemma} \label{lemma:ldnf} For any conditional domain $\mathbb D$ and any program $p \in \mathbb P$, these exists an LDNF of $p$, denoted as $p'$, satisfying that $\text{size}(p') \leq 3\text{size}(p)^2$.
\end{lemma}

\begin{example} \label{example:ldnf} Continue to Example \ref{example:uni-eusolver}, for task $\texttt{max}_n$, the following program $\overline{p}_n$ is a LDNF semantically equivalent to the target program $p_n$:
	\begin{align*}
		\overline{p}_n = &\ \texttt{if}\ ((x_2 \leq x_1)\ \texttt{and}\ (x_3 \leq x_1)\ \texttt{and}\ \dots\ \texttt{and}\ (x_n \leq x_1))\ \texttt{then}\ x_1 \\
		& \ \texttt{else if}\ ((x_1 < x_2)\ \texttt{and}\ (x_3 \leq x_2)\ \texttt{and}\ \dots\ \texttt{and}\ (x_n \leq x_2))\ \texttt{then}\ x_2 \\
		&\ \dots \\
		&\ \texttt{else if}\ ((x_1 < x_{n-1})\ \texttt{and}\ \dots\ \texttt{and}\ (x_{n-2} < x_{n - 1})\ \texttt{and}\ (x_{n-1} \leq x_n))\ \texttt{then}\ x_{n-1} \\ 
		&\ \texttt{else if}\ ((x_1 < x_{n})\ \texttt{and}\ \dots\ \texttt{and}\ (x_{n-1} < x_{n}))\ \texttt{then}\ x_{n}\ \texttt{else}\ \texttt{dummy}
	\end{align*}
The size of $\overline{p}_n$ is $O(n^2 \log n)$, which is exponentially smaller than the smallest program implementing $p_n$ in the conditional program space.
\end{example}

With the definition of LDNF, the generalizability of \mainname is better than \textit{Eusolver} in two levels. At first, \mainname has polynomial-size generalizability for conditonal domains but \textit{Eusolver} does not. Secondly, \mainname still has polynomial-size generazalibility when the target program is given in LDNF: By Lemma \ref{lemma:ldnf} and Example \ref{example:ldnf}, such a guarantee is strictly stronger than the polynomial-size generalizability for conditional domains.

==> sections/STUN3.tex <==
%!TEX root = ../CLIA.tex
\section{Synthesis Through Unification} \label{section:stun}

To evaluate the effectiveness of our abstracted generalization model, in this section we study the framework of \textit{synthesis through unification (STUN)}~\cite{DBLP:conf/cav/AlurCR15}, a state-of-the-art framework for synthesizing nested \texttt{if-then-else} operators. In Section \ref{section:stun-pre}, we introduce some necessary preliminaries on STUN and \textit{Eusolver}, a state-of-the-art STUN solver. Then, in Section \ref{section:stun-gen}, we study the generaliazbility of the STUN framework and \textit{Eusolver}.

\subsection{Preliminaries: Synthesis Sthrough Unification}
The framework of \textit{synthesis through unification (STUN)} focuses on a special kind of synthesis tasks, where the program space supports enough flexibility for \texttt{if-then-else} operators. Formally, STUN assumes that the program space can be decomposed into two subspaces, for \texttt{if}-conditions and \texttt{if}-terms respectively. 

\begin{definition}A program space $\mathbb P$ is a conditional program space if and only if there exist two program spaces $\mathbb P_c$ and $\mathbb P_t$ such that $\mathbb P$ is the smallest set of programs such that:
	$$
	\mathbb P = \mathbb P_t \cup \left\{\texttt{if}\ c\ \texttt{then}\ p_1\ \texttt{else}\ p_2\ |\ p_1, p_2 \in \mathbb P, c \in \mathbb P_c  \right\}
	$$
\end{definition}
For convenience, we use a pair of program spaces $(\mathbb P_t, \mathbb P_c)$ to denote a conditional program space derived from term space $\mathbb P_t$ and condition space $\mathbb P_c$. Besides, we call a domain $\mathbb D$ \textit{conditional} if the program space in $\mathbb D$ is conditional.

A STUN solver synthesizes programs in two steps:
\begin{enumerate}
	\item A term solver is invoked to synthesize a set of programs $P \subseteq \mathbb P_t$ such that for any example, there is always a consistent program in $P$.
	\item A unifier is invoked to synthesize a valid program from conditional program space $(P, \mathbb P_c)$. 
\end{enumerate}
In this paper, we only consider the specialized version of the STUN framework on PBE tasks.

\begin{definition}[Term Solver] Given a conditional domain $\mathbb D$, term solver $\mathcal T: \mathbb T(\mathbb D) \rightarrow \mathcal P(\mathbb P_t)$ takes a PBE task as the input, and returns a set of terms covering all given examples, i.e.:
	$$\forall T \in \mathbb T(\mathbb D), \forall (I,O) \in T, \exists p \in \mathcal T(T), \sem{p}(I) = O$$
	where $\mathcal P(\mathbb P_t)$ represents the power set of $\mathbb P_t$.
\end{definition}

\begin{definition}[Unifier] Given a conditional domain $\mathbb D$, a unifier $\mathcal U$ is a function such that for any set of terms $P \subseteq \mathbb P_t$, $\mathcal U(P)$ is a valid PBE solver for $(P, \mathbb P_c)$.
\end{definition}

A STUN solver is comprised of a term solver $\mathcal T$ and a unifer $\mathcal U$. Given a PBE task $T$, the solver returns $\mathcal U(\mathcal T(T))(T)$ as the synthesis result. \citet{DBLP:conf/cav/AlurCR15} proves that such a combination is complete when the conditiona domain is \textit{if-closed}. For other domains, STUN can be extended to complete by backtracking to the term solver when the unfier fails~\cite{DBLP:conf/cav/AlurCR15, DBLP:conf/tacas/AlurRU17}.

\begin{definition}[If-Closed] A conditional domain $\mathbb D$ is \textit{if-closed} if: $$\forall p_1, p_2 \in \mathbb P_t, \exists c \in \mathbb P_c, \forall I \in \mathbb I, \left(\sem{c}(I) \iff \sem{p_1}(I) = \sem{p_2}(I)\right)$$
\end{definition}

For simplicity, in the reminder of this paper, we implicitly assume the conditional program space is if-closed, and we use notation $\mathcal F_{C}$ to denote a family of if-closed conditional domains.

Now, we move to \textit{Eusolver}~\cite{DBLP:conf/tacas/AlurRU17}, a state-of-the-art PBE solver following the STUN framework. \textit{Eusolver} takes both efficiency and generalizability as its design purpose, and makes a trade-off between these two goals heuristically.

The term solver in \textit{Eusolver} is motivated by the success of $\mathcal S_{\text{min}}$ on generalizability. The term solver enumerates terms in $\mathbb P_t$ in the increasing order of the size. For each term $t$, if there is not a smaller term that performs the same with $p$ on all examples, $t$ will be included into the result. When collected terms are enough to colver all examples, the term solver returns them as the result.

The unifer in \textit{Eusolver} regards nested \texttt{if-then-else} operators as a decision tree, and uses \textit{ID3}~\cite{DBLP:journals/ml/Quinlan86}, a standard decision-tree learning algorithm, to unify the terms. The unifier learns a decision tree recursively from the top down: In each recursion, it firstly tries to use a term to cover all remaining examples. If there is no such term, the unifier will pick up a condition $c$ from $\mathbb P_c$ as the \texttt{if}-condition. According to the semantics of $c$, the examples will be divided into two parts, which will be used to synthesize the \texttt{then}-branch and the \texttt{else}-branch respectively.

\subsection{Generalizability of STUN} \label{section:stun-gen}
In this section, we study the generalizability of the STUN framework and \textit{Eusolver}. To start, we extend the concept of \textit{size-preserving} and \textit{polynomial-size generalizability} to term solvers and unifiers respectively: For a \textit{size-preserving} term solver, there should be a polynomial that bounds the total size of returned terms; and for a unifier in $\mathsf{PSG}$, there should be a universal polynomial that bounds the generation function on any set of terms.

\begin{definition} \label{def:size-preserve}A term solver $\mathcal T$ is \textit{size-preserving} on $\mathcal F_{C}$ if there is a polynomial $s(x, y)$ such that for any generation model $\mathcal G$ on $\mathcal F_C$:
	\begin{align*}
		\forall n > 0, \forall p \in (\mathbb P_t, \mathbb P_c), \forall \epsilon \in (0, 1), 
		\Pr_{I_1, \dots, I_n \sim D_I(p)}\left[\text{tsize}\left( \mathcal T\big(T(p, I_1, \dots, I_n)\big)\right) > s\left(\text{size}(p),  \ln \left(\frac{1}{\epsilon}\right)\right)\right] \leq \epsilon
	\end{align*}
where $\text{tsize}(P)$ is the total size of terms in term set $P$, i.e., $\sum_{t \in P} \text{size}(t)$.
\end{definition}

\begin{definition}\label{def:poly-unifier} Unifier $\mathcal U$ has  \textit{polynomial-size generalizability} on $\mathcal F_C$, abbreviated as $\mathcal U \in \mathsf {PSG}[\mathcal F_C]$,  if there exists a polynomial $g(x, y)$ such that for any generation model $\mathcal G$ on $\mathcal F_C$:
	\begin{align*} \forall P \subseteq \mathbb P_t, \forall p \in (P, \mathbb P_c), \forall \epsilon \in (0, 1), \text{gen}_f[\mathcal G(P), \mathcal U(P)](p, \epsilon) \leq g\left(\max(\text{tsize}(P), \text{size}(p)), \ln\left(\frac{1}{\epsilon}\right)\right)
	\end{align*}
	where $\mathcal G(P)$ is the induced generation model on program space $(P, \mathbb P_t)$.
\end{definition}

Note that in Definition \ref{def:poly-unifier}, besides the size of the target program, the polynomial bound also refers to the total size of $P$. Such a relaxation allows the unifier to use more examples when an extremely large term set is provided.

Based on above definitions, we prove that generalizability of a STUN solver can be guaranteed by size-preservability of the term solver and generalizability of the unifier.

\begin{theorem} \label{theorem:gen-stun}Given a term solver $\mathcal T$ and a unifir $\mathcal U$, define $\mathcal T'$ and $\mathcal U'$ as the following:
	$$
	\mathcal T'(e_1, \dots, e_n) = \mathcal T\left(e_1, \dots, e_{\lfloor \frac{n}{2}\rfloor}\right)\ \ \ \ \mathcal U'(P)(e_1, \dots, e_n) = \mathcal U(P)\left(e_{\lfloor \frac{n}{2} \rfloor + 1}, \dots, e_{n}\right)
	$$
	The STUN solver induced by $\mathcal T'$ and $\mathcal U'$ has polynomial-size generalizability on $\mathcal F_{C}$ if (1) $\mathcal T$ is size-preserving on $\mathcal F_{C}$; (2) $\mathcal U$ has polynomial-size generalizability on $\mathcal F_{C}$, i.e., $\mathcal U \in \mathsf{PSG}[\mathcal F_{C}]$.
\end{theorem}

Note that Theorem \ref{theorem:gen-stun} requires the term solver to be size-preserving rather than have polynomial-size generalizability. Actually, a term solver in $\mathsf{PSG}$ and a unifier in $\mathsf{PSG}$ is not guaranteed to merge into an STUN solver with polynomial-size generalizability, as the term solver may produce an extremely larger term set, and thus makes the smallest valid program for the unifier exponentially larger than the target.

The term solver in \textit{Eusolver} just fits into this case. Though \textit{Eusolver} simulates $\mathcal S_{\text{min}}$ to guarantee that all returned terms are syntactially small, it does not control the number of returned terms. To see this point, let us consider an extreme case where:
\begin{itemize}
	\item There are $n +1$ terms in $\mathbb P_t$, listed as $t_1, \dots, t_n, t^*$ in the increasing order of the size.
	\item The semantics of $t^*$ is covered by set $\{t_1, \dots, t_n\}$, i.e., $\forall I \in \mathbb I, \exists i \in [1,n], \sem{t_i}(I) = \sem{t^*}(I)$.
\end{itemize}
Recall that the term solver in \textit{Eusolver} enumerates the terms in the increasing order of the size. Therefore, when $t^*$ is taken as the target, \textit{Eusolver} will always returns a subset of $\{t_1, \dots, t_n\}$ and will never enumerates to $t^*$. By Lemma \ref{lemma:size}, $n$ can be as large as $\exp(\text{size}(t^*))$. Therefore, it is possible for the term sovler to return a term set exponentially larger than the target, and thus the term solver is not size-preserving.

Using the same extreme case, we can prove that the generalizability of $\textit{Eusolver}$ is unguaranteed.

\begin{theorem}\label{theorem:gen-eusolver} $\textit{Eusolver} \not \in \mathsf {PSG}[\mathcal F_{C}^A]$, where $\mathcal F_{C}^A$ is the family of all conditional domains.
\end{theorem}

Now we turn to the generalizability of the unifer in \textit{Eusolver}. As decision trees play important roles in learning theory and practical learning systems, there has been a series of work discussing whether decision trees can be learned efficiently. However, the theoretical results are rather negative: \citet{DBLP:conf/stacs/HancockJLT95} proves that there is no polynomial-time decision-learning algorithm that generalizes with a polynomial number of examples, unless $\mathsf{NP} = \mathsf{RP}$, the class of polynomial-time random algorithms with one-side error. Therefore, it is unlikely that \textit{ID3}, as well as other polynomial-time learning algorithms, have guaranteed generalizability.

\endinput
\subsection{Generalizability of \textit{Eusolver}}
In this section, we analysize the generalizability of \textit{Eusolver}. 


In this section, we analysize the state-of-the-art STUN solver \textit{Eusolver}, and prove that its generalizability is unsatisfying. Though the term solver in \textit{Eusolver} enumerates terms in the increasing order of the size and thus guarantees to return only small terms, it does not control the total size of the returned program. Therefore, the term solver may use a large number of examples to synthesize an extremely large set of terms, as shown in Example \ref{example:eusolver-size}.

\begin{example} \label{example:eusolver-size} Consider the following term space $\mathbb P_t^n$, input space $\mathbb I_t^n$ and target program $p$:
	$$
	\mathbb P_t^n = \{2, 3, \dots, 2n, x + y\}\ \ \ \mathbb I_t^n = \big\{(x_0, y_0)\ \big|\ x_0, y_0 \in [1, n]\big\}\ \ \ p = x+ y
	$$
	
	As $p$ is the largest term $\mathbb P_t^n$, for any input $(x_ 0, y_0) \in \mathbb I_t^n$, there is always a smaller term $c$ performs the same as $p$, where $c$ is a constant equal to $x_0 + y_0$. Therefore, whatever the PBE task, the term solver always returns a subset of $\{2,3, \dots, 2n\}$ and nevers enumerates to the target program $p$. 
	
	Let $P$ be the set of terms returned by the term solver. An necesseary condition for \textit{Eusolver} to synthesize a program semantically equivalent to $p$ is that, for any input in $\mathbb I_t^n$, there is always an term in $P$ performs the same with $p$, i.e., $\forall I \in \mathbb I_t^n, \exists t \in P, \sem{t}(I) = \sem{p}(I)$. As $P \subseteq \{2, 3, \dots, 2n\}$, the only possible term set satisfying this condition is $\{2, 3, \dots, 2n\}$.
	
	By Algorithm \ref{alg:eusolver-term}, the term solver return $\{2, 3, \dots, 2n\}$ only when the outputs of given examples cover all integers in range $[2, 2n]$. Therefore, the term solver requires at least $2n - 1$ examples. As the size of the target program is only $O(\log n)$, \textit{Eusolver} uses exponentially number of examples to syntehsize $p$ in this example.
\end{example}

Example \ref{example:eusolver-size} shows that the term solver in \textit{Eusolver} is not size-preserving, and also, \textit{Eusolver} does not have polynomial-size generalizability.

\endinput

\subsection{Overview for \mainname}
We design a STUN solver with polynomial-size generalizability, namely \mainname, according to Theorem \ref{theorem:gen-stun}:
\begin{itemize}
	\item Different from \textit{Eusolver}, the term solver $\mathcal T_{\text{poly}}$ of \mainname is designed to be size-preserving.
	\item The unifier $\mathcal U_{\text{poly}}$ is not only designed to have polynomial-size generalizability for conditional program spaces, but also for a more compact intermediate form, namely \textit{linear disjunctive normal form (LDNF)}. 
\end{itemize}

In the remainder of this section, we shall introduce the linear disjunctive normal form used by $\mathcal U_{\text{poly}}$. The concrete algorithms of $\mathcal T_{\text{poly}}$ and $\mathcal U_{\text{poly}}$ will be left to Section \ref{section:term-solver} and Section \ref{section:unifier} respectively.

\begin{definition} For conditional program domian $\mathbb D$, a program $p$ is of \textit{linear disjunctive normal form (LDNF)} if is satisfies the following three conditions:
	\begin{itemize}
		\item The structure of $p$ is linear, i.e., $p$ is in the form of:
		$$
		\texttt{if}\ (c_1)\ \texttt{then}\ t_1\ \texttt{else}\ \texttt{if}\ (c_2)\ \texttt{then}\ t_2\ \texttt{else} \dots \texttt{if}\  (c_{n})\ \texttt{then}\ t_{n}\ \texttt{else}\ \texttt{dummy}
		$$
		where \texttt{dummy} is a dummy value that is never used.
		\item \texttt{if}-terms $t_1, \dots, t_n$ used in $p$ are all from term space $\mathbb P_t$, and \texttt{if}-conditions $c_1, \dots, c_n$ used in $p$ are all from $\text{DNF}(\mathbb P_c)$, disjuctive normal forms comprised of $\mathbb P_c$. $\text{DNF}(\mathbb P_c)$ is defined in three steps:
		\begin{enumerate}
			\item $\text{L}(\mathbb P_c)$ is the set of literals comprised of $\mathbb P_c$, i.e., $\text{L}(\mathbb P_c) = \{\texttt{not } p\ |\ p \in \mathbb P_c\} \cup \mathbb P_c$
			\item $\text{CL}(\mathbb P_c)$ is the set of clauses compised of $\mathbb P_c$. $\text{CL}(\mathbb P_c)$ is the smallest set such that:
			$$\text{CL}(\mathbb P_c) = \{\texttt{true}\} \cup \{l\ \texttt{and}\ c\ |\ l \in \text{L}(\mathbb P_c), c \in \text{CL}(\mathbb P_c)\}$$
			\item $\text{DNF}(\mathbb P_c)$ is the smallest set such that:
			$$\text{DNF}(\mathbb P_c) = \{\texttt{false}\} \cup \{c\ \texttt{or}\ d\ |\ c \in \text{CL}(\mathbb P_c), d \in \text{DNF}(\mathbb P_c)\}$$
		\end{enumerate}
		\item  \texttt{if}-conditions $c_1, \dots, c_n$ are disjoint and the union of them covers the entire input space:
		$$
		\left(\forall I \in \mathbb I, \exists i \in [1, n], \sem{c_j}(I)\right) \wedge \left(\forall 1 \leq i < j < n, \forall I \in \mathbb I, \neg \left(\sem{c_i}(I) \wedge \sem{c_j}(I)\right)\right)
		$$
	\end{itemize}
\end{definition}

LDNF is designed to be more compact than the conditonal program space in the terms of polynomial-size generalizability. On the one hand, as shown in Lemma \ref{lemma:ldnf}, any program in a conditional domain can be converted to an LDNF of which the size is at most squared. On the other hand, as shown in Example \ref{example:ldnf}, the LDNF may be exponentially smaller than the origin program.

\begin{lemma} \label{lemma:ldnf} For any conditional domain $\mathbb D$ and any program $p \in \mathbb P$, these exists an LDNF of $p$, denoted as $p'$, satisfying that $\text{size}(p') \leq 3\text{size}(p)^2$.
\end{lemma}

\begin{example} \label{example:ldnf} Continue to Example \ref{example:uni-eusolver}, for task $\texttt{max}_n$, the following program $\overline{p}_n$ is a LDNF semantically equivalent to the target program $p_n$:
	\begin{align*}
		\overline{p}_n = &\ \texttt{if}\ ((x_2 \leq x_1)\ \texttt{and}\ (x_3 \leq x_1)\ \texttt{and}\ \dots\ \texttt{and}\ (x_n \leq x_1))\ \texttt{then}\ x_1 \\
		& \ \texttt{else if}\ ((x_1 < x_2)\ \texttt{and}\ (x_3 \leq x_2)\ \texttt{and}\ \dots\ \texttt{and}\ (x_n \leq x_2))\ \texttt{then}\ x_2 \\
		&\ \dots \\
		&\ \texttt{else if}\ ((x_1 < x_{n-1})\ \texttt{and}\ \dots\ \texttt{and}\ (x_{n-2} < x_{n - 1})\ \texttt{and}\ (x_{n-1} \leq x_n))\ \texttt{then}\ x_{n-1} \\ 
		&\ \texttt{else if}\ ((x_1 < x_{n})\ \texttt{and}\ \dots\ \texttt{and}\ (x_{n-1} < x_{n}))\ \texttt{then}\ x_{n}\ \texttt{else}\ \texttt{dummy}
	\end{align*}
The size of $\overline{p}_n$ is $O(n^2 \log n)$, which is exponentially smaller than the smallest program implementing $p_n$ in the conditional program space.
\end{example}

With the definition of LDNF, the generalizability of \mainname is better than \textit{Eusolver} in two levels. At first, \mainname has polynomial-size generalizability for conditonal domains but \textit{Eusolver} does not. Secondly, \mainname still has polynomial-size generazalibility when the target program is given in LDNF: By Lemma \ref{lemma:ldnf} and Example \ref{example:ldnf}, such a guarantee is strictly stronger than the polynomial-size generalizability for conditional domains.

==> sections/TermSolver.tex <==
%!TEX root = ../CLIA.tex
\section{Term Solver} \label{section:term-solver}
In this section, we introduce the term solver $\mathcal T_{\text{poly}}$ in \mainname, which is designed to be size-preserving, the family of domains where the program domain is conditional. We first dicuss the main idea of $\mathcal T_{\text{poly}}$ in Section \ref{section:term-main}, and then select proper parameters for the main algorithm in Section \ref{section:term-config}. At last, we finish the proofs of all wanted properties in Section \ref{section:term-property}.

\subsection{Main Algorithm} \label{section:term-main}
The main algorithm of $\mathcal T_{\text{poly}}$, denoted as $\mathcal T_{\text{main}}$, is motivated by the following lemma: A term solver is size-preserving if it seldom (1) takes large programs as terms, and (2) synthesizes a large term set.

\begin{lemma} \label{lemma:term-split} A term solver $\mathcal T$ is size-preserving for program domain $(\mathbb P_t, \mathbb P_c)$ if there exists a polynomial $s(x, y)$ such that for any $n > 0$, for any $p \in (\mathbb P_t, \mathbb P_c)$, for any $\epsilon \in (0, 1)$:
	\begin{enumerate}
		\item With a high probability, the size of the terms returned by $\mathcal T$ is bouned by polynomial $s$.
		$$
		\Pr_{I_1, \dots, I_n \sim D_I} \left[\max \left\{ \text{size(p)}\ \big |\ p \in \mathcal T \big((I_1, \sem{p}(I_1)), \dots, (I_n, \sem{p}(I_n))\big)\right\} > s(\text{size}(p), \ln(1 / \epsilon))\right] \leq \epsilon
		$$
		\item With a high probability, the size of the set returned by $\mathcal T$ is bounded by polynomial $s$.
		$$
		\Pr_{I_1, \dots, I_n \sim D_I} \left[\left|\mathcal T \big((I_1, \sem{p}(I_1)), \dots, (I_n, \sem{p}(I_n))\big)\right| > s(\text{size}(p), \ln(1 / \epsilon))\right] \leq \epsilon
		$$
	\end{enumerate}
\end{lemma}

We observe that the form of the first condition is like the guarantee provided by a size-preserving solver. Therefore, we design $\mathcal T_{\text{main}}$ as a meta-solver that takes a domain solver $\mathcal S_t$ as an input. For a term finding task, $\mathcal T_{\text{main}}$ firstly decomposes it into several standard PBE tasks, and then invokes $\mathcal S_t$ to synthesize terms with bounded sizes.

In a term finding task, different examples may correspond to different \texttt{if}-terms used by the target program. Therefore, to invokve the PBE solver $\mathcal S_t$, it is important to pick up several examples that are generated from the same term. To achieve this point, we observe that there is always a target term that covers a considerable portion of all examples, as shown in Lemma \ref{lemma:sample}.

\begin{lemma} \label{lemma:sample}Let $T$ be a PBE task, and let $P$ be a set of programs that covers all examples in $T$, i.e., $\forall (I, O) \in T, \exists p \in P, \left(\sem{p}(I) = O\right)$. There is always a program $p \in P$ such that:
	$$
	\left|\big\{(I, O) \in T\ \big|\ \sem{p}(I) = O\big\} \right| \geq \frac{|T|}{|P|}
	$$
\end{lemma}
Therefore, for an term finding task $T$ that takes $P^*$ as the target set, let $t^* \in P^*$ be the term that covers the most examples. According to Lemma \ref{lemma:sample}, if we randomly select $n_t$ examples from $T$, term $t^*$ will be consistent with all selected examples with a probability at least $|P^*|^{-n_t}$. Therefore, if  PBE solver $\mathcal S_t$ generalizes well over the term domain $\mathbb P_t$, running $\mathcal S_t$ on serveral random examples from task $T$ should have a great chance to find term $t^*$. 

For the second condition, $\mathcal T_{\text{main}}$ assumes that there is an upper bound $k$ on the number of terms, and $\mathcal T_{\text{main}}$ uses a backtracking to explore all possible set with at most $k$ terms. In this way, the second condition is guaranteed if the upper bound $k$ is selected properly: On the one hand, $k$ should not be too large to exceed the polynomial bound, and on the other hand, $k$ should be large enough to include the target set. We shall leave the problem of selecting a proper $k$ to Section \ref{section:term-config}.

\SetKwFunction{Search}{Search}
\SetKwFunction{Get}{GetCandidatePrograms}
\SetKwFunction{Covered}{Covered}

Algorithm \ref{alg:term-main} shows the pseudo code of $\mathcal T_{\text{main}}$. The algorithm is configured by 3 parameters: $\mathcal S_t$ is an underlying domain solver for $\mathbb P_t$, $k$ is the upper bound on the number terms, and $n_t$ is the number of random examples provided to the domain solver. 

Function $\Search{}$ (Lines 11-19) implements the backtracking for the second condition. It searches for a set of at most $\variable{sizeLimit}$ terms that covers all examples in $\variable{examples}$. In each step, \Search{} invokes function \Get{} to obtain a set of possibly used terms (Line 16), and then recursively tries each of them until a valid term set is found (Lines 17 - 18).

Function \Get{} implements the random sampling for the first condition (Lines 1-10). Guided by Lemma \ref{lemma:sample}, it returns a set of programs that covers at least $1/\variable{sizeLimit}$ portion of examples in $\variable{example}$. The body of \Get{} is a repeated sampling process (Line 3). In each turn, $n_t$ examples are sampled (Line 4), and solver $\mathcal S_t$ is invoked to synthesize a program from these sampled examples (Line 5). \Get{} collects all valid synthesis results (Line 7) and returns them to \Search{} (Line 10).

A detail worthy of note is that \Get{} only considers those programs of which the size is at most $n_t$ (Line 6). As all examples provided to $\mathcal S_t$ is randomly selected, these examples may happen to correspond some extremely complex programs. Even for a size-preserving $\mathcal S_t$, it is still possible for $\mathcal S_t$ to synthesize extremely large programs. Therefore, we add a special treatment to exclude large programs, and thus ensure the first condition of Lemma \ref{lemma:term-split}. 

\begin{algorithm}[t]
	\small
	\caption{The main algorithm $\mathcal T_{\text{main}}$ of $\mathcal T_{\text{poly}}$.}
	\label{alg:term-main}
	\LinesNumbered
	\KwIn{A PBE task $T$ and parameters $(\mathcal S_t, k, n_t)$.}
	\KwOut{$\top$ or a set of programs $P$ that contains at most $k$ programs and covers all examples.}
	\SetKwProg{Fn}{Function}{:}{}
	\Fn{\Get{\variable{examples}, \variable{sizeLimit}}}{
		$\variable{result} \gets \{\}$; \\
		\For{each $\variable{turn} \in [1, n_t \times \variable{sizeLimit}^{n_t}]$}{
			Uniformly and independently samples $n_t$ examples $e_1, \dots, e_{n_t}$ from $\variable{examples}$; \\
			$p \gets \mathcal S_t\left(e_1, \dots, e_{n_t}\right)$; \\
			\If {$p \neq \top \wedge |\Covered{p, \variable{examples}}| \geq |\variable{examples}|/ \variable{sizeLimit} \wedge \text{size}(p) \leq n_t$}{$\variable{result} \gets \variable{result} \cup \{p\}$;}
		}
		\Return $\variable{result}$;
	}
	\Fn{\Search{\variable{examples}, \variable{sizeLimit}}}{
		\lIf{(\variable{examples}, \variable{sizeLimit}) is visited before} {\Return $\top$}
		\If{\variable{sizeLimit} = 0}{
			\leIf{$|\variable{examples}| = 0$}{\Return $\{\}$}{\Return $\top$}	
		}
		\For{each $p \in \Get(\variable{examples}, \variable{sizeLimit})$}{
			\variable{searchResult} $\gets \Search{\variable{examples} - \Covered{$p, \variable{examples}$}, \variable{sizeLimit} - 1}$; \\
			\lIf{$\variable{searchResult} \neq$}{\Return $\{p\} \cup \variable{searchResult}$}
		}
	}
	\Return $\Search{$T, k$}$;
\end{algorithm}
\subsection{The Selection of Parameters} \label{section:term-config}
Guided by Lemma \ref{lemma:term-split}, $\mathcal T_{\text{main}}$ decomposes a trm finding task into standard PBE tasks. However, as a term solver, the performance of $\mathcal T_{\text{main}}$ depends on the choices of $k$ and $n_t$:
\begin{itemize}
	\item The value of $k$ should be moderate. If $k$ is so small that valid term sets are all excluded, the term solver will be incomplete. If $k$ is so large that the second condition of Lemma \ref{lemma:term-split} is violated, the term solver may not be size-preserving.
	\item The value of $n_t$ should not be too small. Otherwise, the synthesizer $\mathcal S_t$ may fail in generalizing to inteneded terms, or some necessary terms may be excluded as their sizes are larger then $n_t$. Either case will lead to an incomplete term solver.
\end{itemize}

As the proper values of $k$ and $n_t$ varies from tasks to tasks, $\mathcal T_{\text{main}}$ decides $k$ and $n_t$ iteratively, as shown in Algorithm \ref{alg:term-poly}. In each turn, $\mathcal T_{\text{poly}}$ tries all assignments to $(n,k)$ in a bounded range $[1, k_0] \times [1, n_0]$ (Line 3). If $\mathcal T_{\text{main}}$ is able to find a term set satisfying all examples in task $T$, this set will be returned by $\mathcal T_{\text{poly}}$ as the answer (Lines 5-6). Otherwise, range $k_0, n_0$ will be enlarged, and then a new turn will start (Line 9). Such an iteration ends when all possible assignments to $(n, k)$ have been explored (Line 2).
\begin{algorithm}[t]
	\small
	\caption{The main algorithm $\mathcal T_{\text{main}}$ of $\mathcal T_{\text{poly}}$.}
	\label{alg:term-poly}
	\LinesNumbered
	\KwIn{A PBE task $T$ and parameters $(\mathcal S_t, k_0, n_0)$.}
	\KwOut{A set of programs $P$ that covers all examples or $\top$.}
	\SetKwProg{Fn}{Function}{:}{}
	$k_0 \gets \min(k_0, |T|);\ \ n_0 \gets \min(k_0, |T|);$ \\
	\While {$k_0 \leq |T| \vee n_0 \leq |T|$}{
		\For {each $(k, n_t) \in [1, k_0] \times [1, n_0]$}{
			\If {$(k, n_t)$ has not been used before} {
				$P \gets \mathcal T_{\text{main}}(T, (\mathcal S_t, k, n_t))$; \\
				\lIf{$P \neq \top$}{\Return $P$}
			}
		}
		$k_0 \gets k_0 + 1; \ \ n_0 \gets n_0 + 1$; 
	}
\Return $\top$.
\end{algorithm}


\subsection{Properties of $\mathcal T_{\text{poly}}$} \label{section:term-property}
In this section, we discuss the properties of $\mathcal T_{\text{poly}}$. We start by showing $\mathcal T_{\text{poly}}$ is a valid term solver.

\begin{theorem}$\mathcal T_{\text{poly}}$ is sound and complete.
\end{theorem}
\begin{proof}
	The soundness of $\mathcal T_{\text{poly}}$ is naturally guaranteed as Algorithm \ref{alg:term-main} returns a program set only when it covers all examples.
	
	To show the completeness, suppose there exists a program set that covers all examples. At this time, for each example $e$ in the PBE task, there is always a program $p \in \mathbb P_t$ that is consistent with $e$. According to the completeness, $\mathcal S_t$ can successfully synthesize a program for each individual example. Therefore, under configuration $k = |T|, n_t = 1$, $\mathcal T_{\text{main}}$ is guaranteed to find a solution.  
\end{proof}

Besides, as a meta-solver, $\mathcal T_{\text{poly}}$ could inherient the size-preservability from domain solver $\mathcal S_t$. To prove this property, we start by introducing a lemma that bounds the probability for $\mathcal T_{\text{main}}$ to find a term set on a large enough $n$ and a large enough $k$.

\begin{lemma} \label{lemma:term-size-mid}For any size-preserving domain solver $\mathcal S_t$, there exists a polynomial $s(x)$ and a constant $\beta \in (0, 1)$ such that for any target program $p \in (\mathbb P_t, \mathbb P_c)$, for any $k, n_t > s(\text{size(p)})$, the probability for $\mathcal T_{\text{main}}$ to find a term set with configuration $(\mathcal S_t, k, n_t)$ is at least $\beta$. Formally, for any $n > 0$, for any $p \in (\mathbb P_t, \mathbb P_c)$:
	$$
	\forall k, n_t > s(\text{size}(p)), \Pr_{I_1, \dots, I_n \sim D_I}\left[\mathcal T_{\text{main}}\big((I_1, \sem{p}(I_1)), \dots, (I_n, \sem{p}(I_n)), (\mathcal S_t, k, n_t)\big) = \top\right] \leq \beta
	$$
\end{lemma}
\begin{proof} Let $P^*$ be the term set used by the target program $p$, and let $\epsilon$ be an arbitrary constrant in $(0, 1)$. As $\mathcal S_t$ is size-preserving, there exists a polynomial $f(x)$ such that the size of the program synthesized by $\mathcal S_t$ is bounded by polynomial $f$ except a probability at most $\epsilon$. 
	
We construct $s(x)$ as a polynomial satisfying $\forall x, s(x) \geq x \wedge s(x) \geq f(x)$. At this time, $k^*$ and $n_t$ are at least large as $\text{size}(p)$, and therefore they are larger than $|P^*|$ and the maximum size of programs in $P$ respectively.
	
We call an invocation of \Search{} \textit{correct} if all its ancestors on the recursion tree select programs in $P^*$.  Obviously, if $\mathcal{T_{\text{poly}}}$ fails in finding a term set, there must be no correct invocations of depth $|P^*|$, where the depth of the first invocation of \Search{} is defined as $0$. 
	
Let $S_i$ be the left-most invocation of depth $i$ on the recursion tree and let $\mathcal E_{i}$ be the random event that $S_i$ exists but $S_i$ does not recurse into a correct invocation of depth $i+1$. If $S_{|P^*|}$ does not exist, there must be at least one event among $\mathcal E_0, \dots, \mathcal E_{|P^*| - 1}$ happens.

For each $i$, there are only two possible reasons for $\mathcal E_{i}$ to happen:
\begin{itemize}
	\item Random event $\mathcal E_{i,1}$: There does not exist a sampling round that all examples are consistent with a program in $P^*$. According to Lemma \ref{lemma:sample}:
	$$
	\Pr[\mathcal E_{i, 1}] \leq \left(1 - \left(\frac{1}{|P^*| - i}\right)^{n_t}\right)^{n_t(k - i)^{n_t}} \leq \exp\left(- n_t(k - i)^{n_t}\left(\frac{1}{|P^*| - i}\right)^{n_t}\right) \leq e^{-n_t}
	$$
	\item Random event $\mathcal E_{i, 2}$: There exists a sampling round that all examples are consistent with a program in $P^*$, but $\mathcal S_t$ fail in synthesizing a program that is smaller than $n_t$. According to the definition of size-preserving, $\Pr[\mathcal E_{i,2}]$ is bounded by $\epsilon$.
\end{itemize}

Therefore, the probability for $\mathcal T_{\text{main}}$ to fail is bounded:
$$
\Pr\left[\mathcal T_{\text{main}}\text{ fails}\right] \leq \sum_{i=0}^{|P^*| - 1} \left(\Pr[\mathcal E_{i,1}] + \Pr[\mathcal E_{i,2}]\right) \leq |P^*| \left (e^{-n_t} + \epsilon \right) \leq \text{size}(p) \left(\exp(-s(\text{size}(p))) + \epsilon\right)
$$
This lemma is proved by selecting a small enough $\epsilon$ and a large enough $s(x)$.
\end{proof}

\begin{theorem}  \label{theorem:term-size}$\mathcal S_t$ is size-preserving $\implies \mathcal T_{\text{poly}}$ is size-preserving.
\end{theorem}
\begin{proof} Let $s_0(x), \beta$ be the polynomial and the upper bound provided by Lemma \ref{lemma:term-size-mid}. Let $\Delta$ be a constant, consider the probability for $\mathcal T_{\text{main}}$ not to return within the first $s_0(\text{size}(p)) + \Delta$ iterations:
	$$
	\Pr[\mathcal T_{\text{main}}\text{ does not returns within the first } s_0(\text{size}(p)) + \Delta \text{ iterations}] \leq \beta^{\Delta}
	$$ 
As $\beta$ is a constant, for any error rate $\epsilon$, it is enough to take $\Delta$ as $\frac{\ln(1 / \epsilon)}{\ln (1 / \beta)}$. This theorem is proved by applying Lemma \ref{lemma:term-split} with polynomial $s(x, y) = s_0(x) + \frac{1}{\ln(1 / \beta)}y$.
\end{proof}

At last, we discuss the time cost of the term solver. With a high probability, $\mathcal T_{\text{poly}}$ invokes $\mathcal T_{\text{main}}$ polynomial times. However, the time cost of $\mathcal T_{\text{main}}$ may not be polynomial. An invocation of \Search{} of depth $i$ on the recursion tree samples $n_t(k-i)^{n_t}$ times. In the worst case, $\mathcal S_t$ successfully synthesizes programs for all these samples, and the results are all different. At this time, \Search{} will recursively invoke itself for $n_t(k-i)^{n_t}$ times. Therefore, $\mathcal T_{\text{main}}$ invokes the domain solver $\mathcal S_t$ for $n_t^k(k!)^{n_t}$ times in the worst case.

However, in practice, $\mathcal T_{\text{poly}}$ is usually much faster than the worst case because:
\begin{itemize}
	\item The domain solver $\mathcal S_t$ usually fails when the random examples correspond to different domains, as the expressive ability of term domain $\mathbb P_t$ is usually limited.
	\item For those incorrect terms that are happened to be synthesized, they seldom satisfy the requirement on the size and the number of covered examples (Line 6 in Algorithmn \ref{alg:term-main}).
\end{itemize}	
Therefore, if we assume Function \Get{} never returns terms that are not used by the target program, the number for $\mathcal T_{\text{main}}$ to invoke $\mathcal S_t$ will be bounded within $n_t2^{k}k^{n_t}$. In practice, $\mathcal T_{\text{main}}$ seldom deals with large $n_t$ and $k$, as the generalizability of the domain solver is usually great and the number of terms used by the target program is usually small. Therefore, such a time complexity is actually acceptable in practice.

==> sections/TermSolver2.tex <==
%!TEX root = ../CLIA.tex
\section{Term Solver} \label{section:term-solver}
In this section, we introduce the term solver $\mathcal T_{\text{poly}}$ in \mainname, which is designed to be size-preserving, the family of domains where the program domain is conditional. We first dicuss the main idea of $\mathcal T_{\text{poly}}$ in Section \ref{section:term-main}, and then select proper parameters for the main algorithm in Section \ref{section:term-config}. At last, we finish the proofs of all wanted properties in Section \ref{section:term-property}.

\subsection{Overview} \label{section:term-main}
Term solver $\mathcal T_{\text{poly}}$ is motivated by the following lemma: A term solver is size-preserving if it seldom (1) takes large programs as terms, and (2) synthesizes a large term set.

\begin{lemma} \label{lemma:term-split} A term solver $\mathcal T$ is size-preserving for $\mathcal F_C$ if there exists a polynomial $s(x, y)$ such that for any $n > 0$, for any $\mathbb D \in \mathcal F_C$, for any $p \in (\mathbb P_t, \mathbb P_c)$, for any $\epsilon \in (0, 1)$:
	\begin{enumerate}
		\item With a high probability, the size of the terms returned by $\mathcal T$ is bouned by polynomial $s$.
		$$
		\Pr_{I_1, \dots, I_n \sim D_I} \left[\max \left\{ \text{size(p)}\ \big |\ p \in \mathcal T \big((I_1, \sem{p}(I_1)), \dots, (I_n, \sem{p}(I_n))\big)\right\} > s(\text{size}(p), \ln(1 / \epsilon))\right] \leq \epsilon
		$$
		\item With a high probability, the size of the set returned by $\mathcal T$ is bounded by polynomial $s$.
		$$
		\Pr_{I_1, \dots, I_n \sim D_I} \left[\left|\mathcal T \big((I_1, \sem{p}(I_1)), \dots, (I_n, \sem{p}(I_n))\big)\right| > s(\text{size}(p), \ln(1 / \epsilon))\right] \leq \epsilon
		$$
	\end{enumerate}
\end{lemma}

We observe that the form of the first condition is like the guarantee provided by a size-preserving solver. Therefore, we design $\mathcal T_{\text{poly}}$ as a meta-solver that takes a domain solver $\mathcal S_t$ as an input. For a term finding task, $\mathcal T_{\text{poly}}$ firstly decomposes it into several standard PBE tasks, and then invokes $\mathcal S_t$ to synthesize terms with bounded sizes.

In a term finding task, different examples may correspond to different \texttt{if}-terms used by the target program. Therefore, to invokve the PBE solver $\mathcal S_t$, it is important to pick up several examples that are generated from the same term. To achieve this point, we observe that there is always a target term that covers a considerable portion of all examples, as shown in Lemma \ref{lemma:sample}.

\begin{lemma} \label{lemma:sample}Let $T$ be a PBE task, and let $P$ be a set of programs that covers all examples in $T$, i.e., $\forall (I, O) \in T, \exists p \in P, \left(\sem{p}(I) = O\right)$. There is always a program $p \in P$ such that:
	$$
	\left|\big\{(I, O) \in T\ \big|\ \sem{p}(I) = O\big\} \right| \geq \frac{|T|}{|P|}
	$$
\end{lemma}
Therefore, for an term finding task $T$ that takes $P^*$ as the target set, let $t^* \in P^*$ be the term that covers the most examples. According to Lemma \ref{lemma:sample}, if we randomly select $n_t$ examples from $T$, term $t^*$ will be consistent with all selected examples with a probability at least $|P^*|^{-n_t}$. Therefore, if domain solver $\mathcal S_t$ generalizes well over the term domain $\mathbb P_t$, running $\mathcal S_t$ on serveral random examples from task $T$ should have a great chance to find term $t^*$. 

For the second condition, $\mathcal T_{\text{poly}}$ maintains an upper bound $k$ on the number of terms, and uses a backtracking to expore possible sets with at most $k$ terms. If no valid term set is found, $\mathcal T_{\text{poly}}$ will relax the bound $k$, and then restart the backtracking. In this way, the size of the term set synthesized by $\mathcal T_{\text{poly}}$ is guaranteed to be close to the smallest valid set.

\subsection{Algorithm}
\SetKwFunction{Search}{Search}
\SetKwFunction{Get}{GetCandidatePrograms}
\SetKwFunction{Covered}{Covered}
\begin{algorithm}[t]
	\small
	\caption{The main algorithm $\mathcal T_{\text{main}}$ of $\mathcal T_{\text{poly}}$.}
	\label{alg:term-main}
	\LinesNumbered
	\KwIn{A PBE task $T$ and parameters $(\mathcal S_t, k_0, n_0)$.}
	\KwOut{$\top$ or a set of programs $P$ that contains at most $k$ programs and covers all examples.}
	\SetKwProg{Fn}{Function}{:}{}
	\tcp{Part 1: Invoke the domain solver via sampling.}
	\Fn{\Get{\variable{examples}, $k$, $n_t$}}{
		$\variable{result} \gets \{\}$; \\
		\For{each $\variable{turn} \in [1, n_t \times k^{n_t}]$}{
			Uniformly and independently samples $n_t$ examples $e_1, \dots, e_{n_t}$ from $\variable{examples}$; \\
			$p \gets \mathcal S_t\left(e_1, \dots, e_{n_t}\right)$; \\
			\If {$p \neq \top \wedge |\Covered{p, \variable{examples}}| \geq |\variable{examples}|/k \wedge \text{size}(p) \leq n_t$}{$\variable{result} \gets \variable{result} \cup \{p\}$;}
		}
		\Return $\variable{result}$;
	}
	\tcp{Part 2: Backtrack to find a valid term set with at most $k$ terms. }
	\Fn{\Search{\variable{examples}, $k$, $n_t$}}{
		\lIf{(\variable{examples}, $k$) is visited before} {\Return $\top$}
		\lIf {$|\variable{examples}| = 0$}{\Return $\{\}$}
		\lIf {$k = 0$}{\Return $\top$}
		\For{each $p \in \Get{$\variable{examples}, k, n_t$}$}{
			\variable{searchResult} $\gets \Search{$\variable{examples} - \Covered{$p, \variable{examples}$}, k - 1, n_t$}$; \\
			\lIf{$\variable{searchResult} \neq \top$}{\Return $\{p\} \cup \variable{searchResult}$}
		}
		\Return $\top$;
	}
	\tcp{Part 3: Select proper values for parameters $n_t$ and $k$ iteratively.}
	$k_0 \gets \min(k_0, |T|);\ \ n_0 \gets \min(n_0, |T|);$ \\
	\While {$k_0 \leq |T|$}{
		\For {each $(k, n_t) \in [1, k_0] \times [1, n_0]$}{
			\If {$(k, n_t)$ has not been visited before} {
				$P \gets \Search{$T, k, n_t$}$; \\
				\lIf{$P \neq \top$}{\Return $P$}
			}
		}
		$k_0 \gets k_0 + 1; \ \ n_0 \gets n_0 + 1$; 
	}
	\Return $\top$.
\end{algorithm}

Algorithm \ref{alg:term-main} shows the pseudo code of $\mathcal T_{\text{poly}}$. The algorithm is configured by three parameters: $\mathcal S_t$ is an underlying domain solver for $\mathbb P_t$, $k_0, n_0$ are two integer constants that are used to specify an initial search range. 

The algorithm of $\mathcal T_{\text{poly}}$ is comprised of three parts. The first part implements the random sampling dicussed in the previous section, as function \Get{} (Lines 1-10).  \Get{} takes three inputs: $\variable{examples}$ is a set of examples, $k$ is an upper bound on the number of terms, and $n_t$ represents the number of examples required by the domain solver. Guided by Lemma \ref{lemma:sample}, \Get{} returns a set of programs that covers at least $k^{-1}$ portion of examples. 

The body of \Get{} is a repeated sampling process (Line 3). In each turn, $n_t$ examples are sampled (Line 4), and solver $\mathcal S_t$ is invoked to synthesize a program from these sampled examples (Line 5). \Get{} collects all valid synthesis results (Line 7) and returns them to \Search{} (Line 10).

A detail worthy of note is that \Get{} only considers those programs of which the size is at most $n_t$ (Line 6). As all examples provided to $\mathcal S_t$ is randomly selected, these examples may happen to correspond some extremely complex programs. It is still possible for $\mathcal S_t$ to synthesize extremely large programs: These programs may violate the first condition of Lemma \ref{lemma:term-split}. Therefore, $\mathcal T_{\text{poly}}$ sets this limitation on the size and rejects all programs that are too complex.

The second part implements the backtracking dicussed in the previous section, as function \Search{} (Lines 11-19). Given a set of examples $\variable{examples}$ and a size limit $k$, \Search{} searches for a set of at most $\variable{sizeLimit}$ terms that covers $\variable{examples}$ entirely. In each step, \Search{} invokes function \Get{} to obtain a set of possibly used terms (Line 15), and then recursively tries each of them until a valid term set is found (Lines 16 - 17).

The behavior of function \Search{} and \Get{} depends on the concrete values of parameters $k$ and $n_t$:
\begin{itemize} 
	\item If $k$ is too small, \Search{} may fail in finding a valid term set. If $k$ is too large, the second condition of Lemma \ref{lemma:term-split} may be violated.
	\item If $n_t$ is too small, domain solver $\mathcal S_t$ may fail in generalizaing to intended terms. If $n_t$ is too large, function \Get{} may be extremely slow.
\end{itemize}
The third part of $\mathcal T_{\text{poly}}$ selects proper values for $k$ and $n_t$ iteratively (Lines 20-30). Starting from an initial range $[1, k_0] \times [1, n_0]$, in each turn, $\mathcal T_{\text{poly}}$ tries all assignments to $(n,k)$ in this range (Line 22). If $\Search{}$ is able to find a valid term set, this result will be returned as the answer (Lines 24-25). Otherwise, range $k_0, n_0$ will be enlarged, and then a new turn will start (Line 28). Note that if there is a valid solution, $\Search{$T, |T|, 1$}$ must return with a valid term set: At this time, $\mathcal S_t$ is invoked to synthesize terms for each exampe individually. Therefore, if there is a valid solution, the iteration must exist before $k_0$ exceeds $|T|$. Hence it is safe to return $\top$ at Line 30.
\subsection{Properties of $\mathcal T_{\text{poly}}$} \label{section:term-property}
In this section, we discuss the properties of $\mathcal T_{\text{poly}}$. We start by showing $\mathcal T_{\text{poly}}$ is a valid term solver. 

\begin{theorem}$\mathcal S_{t}$ is valid for $T(\mathcal F_C) \implies \mathcal T_{\text{poly}}$ is valid for $\mathcal F_C$, where $T(\mathcal F_C)$ is a family of term domains induced from $\mathcal F_C$, i.e., $T(\mathcal F_C) \coloneqq \{(\mathbb P_t, \mathbb I')\ |\ ((\mathbb P_t, \mathbb P_c), \mathbb I) \in \mathcal F_C, \mathbb I' \subseteq \mathbb I\}$.
\end{theorem}
%\begin{proof}
%	The soundness of $\mathcal T_{\text{poly}}$ is naturally guaranteed as Algorithm \ref{alg:term-main} returns a program set only when it covers all examples.
	
%	To show the completeness, suppose there exists a program set that covers all examples. At this time, for each example $e$ in the PBE task, there is always a program $p \in \mathbb P_t$ that is consistent with $e$. According to the completeness, $\mathcal S_t$ can successfully synthesize a program for each individual example. Therefore, under configuration $k = |T|, n_t = 1$, $\mathcal T_{\text{main}}$ is guaranteed to find a solution.  
%\end{proof}

Besides, as a meta-solver, $\mathcal T_{\text{poly}}$ could inherient the size-preservability from domain solver $\mathcal S_t$. To prove this property, we start by introducing a lemma that bounds the probability for $\Search$ to find a term set on polynomial $k$ and $n_t$.

\begin{lemma} \label{lemma:term-size-mid}Given a family of conditional domains $\mathcal F_C$, if $\mathcal S_t$ is size-preserving for $T(\mathcal F_C)$, there exists a polynomial $s(x)$ and a constant $\beta \in (0, 1)$ such that $\forall \mathbb D \in \mathcal F_C, \forall p \in (\mathbb P_t, \mathbb P_c), \forall k, n_t > s(\text{size(p)})$, the probability for \Search{} to find a term set is at least $\beta$:
	$$
	\Pr_{I_1, \dots, I_n \sim D_I}\left[\mathcal T_{\text{main}}\big((I_1, \sem{p}(I_1)), \dots, (I_n, \sem{p}(I_n)), (\mathcal S_t, k, n_t)\big) = \top\right] \leq \beta
	$$
\end{lemma}
\begin{proof} Let $P^*$ be the term set used by the target program $p$, and let $\epsilon$ be an arbitrary constrant in $(0, 1)$. As $\mathcal S_t$ is size-preserving, there exists a polynomial $f(x)$ such that the size of the program synthesized by $\mathcal S_t$ is bounded by polynomial $f$ except a probability at most $\epsilon$. 
	
We construct $s(x)$ as a polynomial satisfying $\forall x, s(x) \geq x \wedge s(x) \geq f(x)$. At this time, $k^*$ and $n_t$ are at least large as $\text{size}(p)$, and therefore they are larger than $|P^*|$ and the maximum size of programs in $P$ respectively.
	
We call an invocation of \Search{} \textit{correct} if all its ancestors on the recursion tree select programs in $P^*$.  Obviously, if $\Search{}$ fails in finding a term set, there must be no correct invocations of depth $|P^*|$, where the depth of the first invocation of \Search{} is defined as $0$. 
	
Let $S_i$ be the left-most invocation of depth $i$ on the recursion tree and let $\mathcal E_{i}$ be the random event that $S_i$ exists but $S_i$ does not recurse into a correct invocation of depth $i+1$. If $S_{|P^*|}$ does not exist, there must be at least one event among $\mathcal E_0, \dots, \mathcal E_{|P^*| - 1}$ happens.

For each $i$, there are only two possible reasons for $\mathcal E_{i}$ to happen:
\begin{itemize}
	\item Random event $\mathcal E_{i,1}$: There does not exist a sampling round that all examples are consistent with a program in $P^*$. According to Lemma \ref{lemma:sample}:
	$$
	\Pr[\mathcal E_{i, 1}] \leq \left(1 - \left(\frac{1}{|P^*| - i}\right)^{n_t}\right)^{n_t(k - i)^{n_t}} \leq \exp\left(- n_t(k - i)^{n_t}\left(\frac{1}{|P^*| - i}\right)^{n_t}\right) \leq e^{-n_t}
	$$
	\item Random event $\mathcal E_{i, 2}$: There exists a sampling round that all examples are consistent with a program in $P^*$, but $\mathcal S_t$ fail in synthesizing a program that is smaller than $n_t$. According to the definition of size-preserving, $\Pr[\mathcal E_{i,2}]$ is bounded by $\epsilon$.
\end{itemize}

Therefore, the probability for $\mathcal T_{\text{main}}$ to fail is bounded:
$$
\Pr\left[\mathcal T_{\text{main}}\text{ fails}\right] \leq \sum_{i=0}^{|P^*| - 1} \left(\Pr[\mathcal E_{i,1}] + \Pr[\mathcal E_{i,2}]\right) \leq |P^*| \left (e^{-n_t} + \epsilon \right) \leq \text{size}(p) \left(\exp(-s(\text{size}(p))) + \epsilon\right)
$$
This lemma is proved by selecting a small enough $\epsilon$ and a large enough $s(x)$.
\end{proof}

\begin{theorem}  \label{theorem:term-size}$\mathcal S_t$ is size-preserving for $T(\mathcal F_C) \implies \mathcal T_{\text{poly}}$ is size-preserving for $\mathcal F_C$.
\end{theorem}
\begin{proof} Let $s_0(x), \beta$ be the polynomial and the upper bound provided by Lemma \ref{lemma:term-size-mid}. Let $\Delta$ be a constant, consider the probability for $\mathcal T_{\text{poly}}$ not to return within the first $s_0(\text{size}(p)) + \Delta$ iterations:
	$$
	\Pr[\mathcal T_{\text{poly}}\text{ does not returns within the first } s_0(\text{size}(p)) + \Delta \text{ iterations}] \leq \beta^{\Delta}
	$$ 
As $\beta$ is a constant, for any error rate $\epsilon$, it is enough to take $\Delta$ as $\frac{\ln(1 / \epsilon)}{\ln (1 / \beta)}$. This theorem is proved by applying Lemma \ref{lemma:term-split} with polynomial $s(x, y) = s_0(x) + \frac{1}{\ln(1 / \beta)}y$.
\end{proof}

At last, we discuss the time cost of the term solver. With a high probability, $\mathcal T_{\text{poly}}$ invokes $\Search{}$ polynomial times, but the time cost of $\Search{}$ may not be polynomial. An invocation of \Search{} of depth $i$ on the recursion tree samples $n_t(k-i)^{n_t}$ times. In the worst case, $\mathcal S_t$ successfully synthesizes programs for all these samples, and the results are all different. At this time, \Search{} will recursively invoke itself for $n_t(k-i)^{n_t}$ times. Therefore, for each $n_t, k$, the domain solver will be invoked $n_t^k(k!)^{n_t}$ times in the worst case.

However, in practice, $\mathcal T_{\text{poly}}$ is usually much faster than the worst case because:
\begin{itemize}
	\item The domain solver $\mathcal S_t$ usually fails when the random examples correspond to different domains, as the expressive ability of term domain $\mathbb P_t$ is usually limited.
	\item For those incorrect terms that are happened to be synthesized, they seldom satisfy the requirement on the size and the number of covered examples (Line 6 in Algorithmn \ref{alg:term-main}).
\end{itemize}	
Therefore, if we assume Function \Get{} never returns terms that are not used by the target program, invocations of $\mathcal S_t$ will be bounded within $n_t2^{k}k^{n_t}$ times. In practice, $\mathcal T_{\text{poly}}$ seldom deals with large $n_t$ and $k$, as the generalizability of the domain solver is usually great and the number of terms used by the target program is usually small. Therefore, such a time complexity is actually acceptable in practice.

==> sections/TermSolver3.tex <==
%!TEX root = ../CLIA.tex
\section{Term Solver} \label{section:term-solver}
In the remainder of this paper, we design a STUN solver with polynomial-size generalizability, named \mainname, guided by Theorem \ref{theorem:gen-stun}: \mainname is comprised of a size-preserving term solver $\mathcal T_{\text{poly}}$ and a unifier $\mathcal U_{\text{poly}}$ with polynomial-size generalizability. 

In this section, we focus on the term solver $\mathcal T_{\text{poly}}$ used in \mainname. We first show the main idea of $\mathcal T_{\text{poly}}$ in Section \ref{section:term-main}, and then introduce the detailed algorithm in Section \ref{section:term-algorithm}. At last, we show the properties of $\mathcal T_{\text{poly}}$ in Section \ref{section:term-property}. 

\subsection{Overview} \label{section:term-main}
Term solver $\mathcal T_{\text{poly}}$ is based on the following lemma: A term solver is size-preserving if it seldom (1) uses syntactically large terms, and (2) returns a large term set.

\begin{lemma} \label{lemma:term-split} A term solver $\mathcal T$ is size-preserving on $\mathcal F_C$ if there exists a polynomial $s(x, y)$ such that for any generation model $\mathcal G$ on $\mathcal F_C$, for any $n > 0$, for any $p \in (\mathbb P_t, \mathbb P_c)$, for any $\epsilon \in (0, 1)$:
	\begin{enumerate}
		\item With a high probability, the size of the terms returned by $\mathcal T$ is bouned by polynomial $s$.
		$$
		\Pr_{I_1, \dots, I_n \sim D_I(p)} \left[\max \left(\left\{ \text{size(p)}\ \big |\ p \in \mathcal T \big(T(p, I_1,\dots, I_n)\big)\right\}\right) > s\left(\text{size}(p), \ln\left(\frac{1}{\epsilon}\right)\right)\right] \leq \epsilon
		$$
		\item With a high probability, the size of the set returned by $\mathcal T$ is bounded by polynomial $s$.
		$$
		\Pr_{I_1, \dots, I_n \sim D_I} \left[\left|\mathcal T \big(T(p, I_1, \dots, I_n)\big)\right| > s\left(\text{size}(p), \ln\left(\frac{1}{\epsilon}\right)\right)\right] \leq \epsilon
		$$
	\end{enumerate}
\end{lemma}

We observe that the form of the first condition is like the guarantee provided by a size-preserving PBE solver. Therefore, we design $\mathcal T_{\text{poly}}$ as a meta-solver that takes a domain solver $\mathcal S_t$ as an input. For a term finding task, $\mathcal T_{\text{poly}}$ firstly decomposes it into several standard PBE tasks, and then invokes $\mathcal S_t$ to synthesize terms with bounded sizes.

In a term finding task, different examples may correspond to different \texttt{if}-terms used by the target program. Therefore, to invokve the PBE solver $\mathcal S_t$, the main challenge is to find enough examples corresponding to the same term. To achieve this goal, we observe that there is always a target term that covers a considerable portion of all examples, as shown in Lemma \ref{lemma:sample}.

\begin{lemma} \label{lemma:sample}Let $T$ be a PBE task, and let $P$ be a set of programs that covers all examples in $T$, i.e., $\forall (I, O) \in T, \exists p \in P, \left(\sem{p}(I) = O\right)$. There is always a program $p \in P$ such that:
	$$
	\left|\big\{(I, O) \in T\ \big|\ \sem{p}(I) = O\big\} \right| \geq \frac{|T|}{|P|}
	$$
\end{lemma}
Therefore, for a term finding task $T$ with target program $p^*$, let $P^*$ be the set of terms used by $p^*$, and $t^* \in P^*$ be the term that covers the most examples. According to Lemma \ref{lemma:sample}, the probability for $t^*$ to be consistent with $n_t$ random examples drawn from $T$ is at least $|P^*|^{-n_t}$. Therefore, if domain solver $\mathcal S_t$ generalizes well over the term domain $\mathbb P_t$, running $\mathcal S_t$ on serveral random examples from task $T$ should have a great chance to find term $t^*$. 

For the second condition, $\mathcal T_{\text{poly}}$ maintains an upper bound $k$ on the number of terms, and uses a backtracking to explore possible sets with at most $k$ terms. If no valid term set is found, $\mathcal T_{\text{poly}}$ will relax the bound $k$, and then restart the backtracking. In this way, the size of the term set synthesized by $\mathcal T_{\text{poly}}$ is guaranteed to be close to the smallest valid set.

\subsection{Algorithm} \label{section:term-algorithm}
\SetKwFunction{Search}{Search}
\SetKwFunction{Get}{GetCandidatePrograms}
\SetKwFunction{G}{Get}
\SetKwFunction{Covered}{Covered}
\begin{algorithm}[t]
	\small
	\caption{The term solver $\mathcal T_{\text{poly}}$ in \mainname.}
	\label{alg:term-main}
	\LinesNumbered
	\KwIn{A PBE task $T$ and parameters $(\mathcal S_t, k_0, n_0)$.}
	\KwOut{$\top$ or a set of programs $P$ that covers all examples.}
	\SetKwProg{Fn}{Function}{:}{}
	\tcp{Part 1: Invoke the domain solver via sampling.}
	\Fn{\Get{\variable{examples}, $k$, $n_t$}}{
		$\variable{result} \gets \{\}$; \\
		\For{each $\variable{turn} \in [1, n_t \times k^{n_t}]$}{
			Uniformly and independently samples $n_t$ examples $e_1, \dots, e_{n_t}$ from $\variable{examples}$; \\
			$p \gets \mathcal S_t\left(e_1, \dots, e_{n_t}\right)$; \\
			\If {$p \neq \top \wedge |\Covered{p, \variable{examples}}| \geq |\variable{examples}|/k \wedge \text{size}(p) \leq n_t$}{$\variable{result} \gets \variable{result} \cup \{p\}$;}
		}
		\Return $\variable{result}$;
	}
	\tcp{Part 2: Backtrack to find a valid term set with at most $k$ terms. }
	\Fn{\Search{\variable{examples}, $k$, $n_t$}}{
		\lIf{(\variable{examples}, $k$) is visited before} {\Return $\top$}
		\lIf {$|\variable{examples}| = 0$}{\Return $\{\}$}
		\lIf {$k = 0$}{\Return $\top$}
		\For{each $p \in \Get{$\variable{examples}, k, n_t$}$}{
			\variable{searchResult} $\gets \Search{$\variable{examples} - \Covered{$p, \variable{examples}$}, k - 1, n_t$}$; \\
			\lIf{$\variable{searchResult} \neq \top$}{\Return $\{p\} \cup \variable{searchResult}$}
		}
		\Return $\top$;
	}
	\tcp{Part 3: Select proper values for parameters $n_t$ and $k$ iteratively.}
	$k_0 \gets \min(k_0, |T|);\ \ n_0 \gets \min(n_0, |T|);$ \\
	\While {$k_0 \leq |T|$}{
		\For {each $(k, n_t) \in [1, k_0] \times [1, n_0]$}{
			\If {$(k, n_t)$ has not been visited before} {
				$P \gets \Search{$T, k, n_t$}$; \\
				\lIf{$P \neq \top$}{\Return $P$}
			}
		}
		$k_0 \gets k_0 + 1; \ \ n_0 \gets n_0 + 1$; 
	}
	\Return $\top$.
\end{algorithm}
The pseudo code of $\mathcal T_{\text{poly}}$ is shown as Algorithm \ref{alg:term-main}. $\mathcal T_{\text{poly}}$ is configured by three parameters: $\mathcal S_t$ is an underlying domain solver for $\mathbb P_t$, $k_0, n_0$ are two integer constants that are used to specify an initial search range. When there is no valid term set, $\mathcal T_{\text{poly}}$ returns symbol $\top$ instead.

The algorithm of $\mathcal T_{\text{poly}}$ is comprised of three parts. The first part implements the random sampling dicussed in the previous section, as function \Get{} (abbreviated as \G{}). \G{} takes three inputs: $\variable{examples}$ is a set of examples, $k$ is an upper bound on the number of terms, and $n_t$ represents the number of examples required by the domain solver. Guided by Lemma \ref{lemma:sample}, \G{} returns a set of programs that covers at least $k^{-1}$ portion of examples. The body of \G{} is a repeated sampling process (Line 3). In each turn, $n_t$ examples are sampled (Line 4), and solver $\mathcal S_t$ is invoked to synthesize a program from these sampled examples (Line 5). \G{} collects all valid synthesis results (Line 7) and returns them to \Search{} (Line 10).

Note that \G{} only considers those programs of which the size is at most $n_t$ (Line 6). As all examples provided to $\mathcal S_t$ is randomly selected, these examples may happen to correspond some extremely complex programs. It is still possible for $\mathcal S_t$ to synthesize extremely large programs: These programs may violate the first condition of Lemma \ref{lemma:term-split}. Therefore, $\mathcal T_{\text{poly}}$ sets this limitation on the size and rejects all programs that are too complex.

The second part implements the backtracking dicussed in the previous section, as function \Search{} (Lines 11-19). Given a set of examples $\variable{examples}$ and a size limit $k$, \Search{} searches for a set of at most $\variable{sizeLimit}$ terms that covers $\variable{examples}$ entirely. In each step, \Search{} invokes function \G{} to obtain a set of possibly used terms (Line 15), and then recursively tries each of them until a valid term set is found (Lines 16 - 17).

The behavior of \Search{} and \G{} depends on concrete values of parameters $k$ and $n_t$:
\begin{itemize} 
	\item If $k$ is too small, \Search{} may fail in finding a valid term set. If $k$ is too large, the second condition of Lemma \ref{lemma:term-split} may be violated.
	\item If $n_t$ is too small, domain solver $\mathcal S_t$ may fail in generalizaing to intended terms. If $n_t$ is too large, function \G{} may be extremely slow.
\end{itemize}
The third part of $\mathcal T_{\text{poly}}$ selects proper values for $k$ and $n_t$ iteratively (Lines 20-30). Starting from an initial range $[1, k_0] \times [1, n_0]$, in each turn, $\mathcal T_{\text{poly}}$ tries all assignments to $(n,k)$ in this range (Line 22). If $\Search{}$ is able to find a valid term set, this result will be returned as the answer (Lines 24-25). Otherwise, range $k_0, n_0$ will be enlarged, and then a new turn will start (Line 28). Note that if there is a valid solution, $\Search{$T, |T|, 1$}$ must return with a valid term set: At this time, $\mathcal S_t$ is invoked to synthesize terms for each exampe individually. Therefore, if there is a valid solution, the iteration must exist before $k_0$ exceeds $|T|$. Hence it is safe to return $\top$ at Line 30.
\subsection{Properties of $\mathcal T_{\text{poly}}$} \label{section:term-property}
In this section, we discuss the properties of $\mathcal T_{\text{poly}}$. We start by showing $\mathcal T_{\text{poly}}$ is a valid term solver. 

\begin{theorem}\label{theorem:term-valid}$\mathcal S_{t}$ is valid on $T(\mathcal F_C) \implies \mathcal T_{\text{poly}}$ is valid on $\mathcal F_C$, where $T(\mathcal F_C)$ is the family of term domains induced from $\mathcal F_C$, i.e., $T(\mathcal F_C) \coloneqq \{(\mathbb P_t, \mathbb I')\ |\ ((\mathbb P_t, \mathbb P_c), \mathbb I) \in \mathcal F_C, \mathbb I' \subseteq \mathbb I\}$.
\end{theorem}
%\begin{proof}
%	The soundness of $\mathcal T_{\text{poly}}$ is naturally guaranteed as Algorithm \ref{alg:term-main} returns a program set only when it covers all examples.

%	To show the completeness, suppose there exists a program set that covers all examples. At this time, for each example $e$ in the PBE task, there is always a program $p \in \mathbb P_t$ that is consistent with $e$. According to the completeness, $\mathcal S_t$ can successfully synthesize a program for each individual example. Therefore, under configuration $k = |T|, n_t = 1$, $\mathcal T_{\text{main}}$ is guaranteed to find a solution.  
%\end{proof}

Besides, as a meta-solver, $\mathcal T_{\text{poly}}$ could inherient the size-preservability from domain solver $\mathcal S_t$. By Algorithm  \ref{section:term-algorithm}, the total size of the term set found by \Search{$T,k,n_t$} is bounded by $kn_t$. Therefore, it is enough to prove that with a high probability, the outer loop (Lines 21-29 in Algorithm \ref{section:term-algorithm}) ends within a polynomial number of iterations. Lemma \ref{lemma:term-size-mid} shows that the probability for $\Search{}$ to return a term set will raise to a constant  after a polynomial number of iterations.


\begin{lemma} \label{lemma:term-size-mid}If $\mathcal S_t$ is size-preserving on term domains $T(\mathcal F_C)$, there exists a polynomial $s(x)$ and a constant $\beta \in (0, 1)$ such that for any generation model $\mathcal G$ on $\mathcal F_C$, for any target program $p \in (\mathbb P_t, \mathbb P_c), \forall k, n_t > s(\text{size(p)})$, the probability for \Search{} to find a term set is at least $\beta$:
	$$
	\Pr_{I_1, \dots, I_n \sim D_I(p)}\left[\texttt{Search}\big(T(p, I_1, \dots, I_n), (\mathcal S_t, k, n_t)\big) = \top\right] \leq \beta
	$$
\end{lemma}

Lemma \ref{lemma:term-size-mid} implies that after a polynomial number of iterations, the probability for $\mathcal T_{\text{poly}}$ still not to return will decrease exponentially when the number of extra iterations increases. This fact implies the size-preservability of $\mathcal T_{\text{poly}}$.

\begin{theorem}  \label{theorem:term-size}$\mathcal S_t$ is size-preserving on $T(\mathcal F_C) \implies \mathcal T_{\text{poly}}$ is size-preserving on $\mathcal F_C$.
\end{theorem}

At last, we discuss the time cost of $\mathcal T_{\text{poly}}$. With a high probability, $\mathcal T_{\text{poly}}$ invokes $\Search{}$ polynomial times, but the time cost of $\Search{}$ may not be polynomial. An invocation of \Search{} of depth $i$ on the recursion tree samples $n_t(k-i)^{n_t}$ times. In the worst case, $\mathcal S_t$ successfully synthesizes programs for all these samples, and the results are all different. At this time, \Search{} will recursively invoke itself for $n_t(k-i)^{n_t}$ times. Therefore, for each $n_t, k$, the domain solver will be invoked $n_t^k(k!)^{n_t}$ times in the worst case.

However, in practice, $\mathcal T_{\text{poly}}$ is usually much faster than the worst case because:
\begin{itemize}
	\item The domain solver $\mathcal S_t$ usually fails when the random examples correspond to different domains, as the expressive ability of term domain $\mathbb P_t$ is usually limited.
	\item For those incorrect terms that are happened to be synthesized, they seldom satisfy the requirement on the size and the number of covered examples (Line 6 in Algorithmn \ref{alg:term-main}).
\end{itemize}	
If we assume  \G{} never returns terms that are not used by the target program, invocations of $\mathcal S_t$ will be bounded within $n_t2^{k}k^{n_t}$ times, which is much smaller than the worst case.

==> sections/Unifier.tex <==
%!TEX root = ../CLIA.tex
\section{Unifier} \label{section:unifier}
In this section, we introduce the unifier $\mathcal U_{\text{poly}}$ used in \mainname, which is designed to have polynomial-size generalizability for $\mathcal F_C^{\text{DNF}}$. 

\subsection{Overview}
The main idea of $\mathcal U_{\text{poly}}$ is to decompose the unification task into several PBE tasks for disjuctive normal forms. $\mathcal F^{\text{DNF}}_C$ denote the boolean domains induced from $\mathcal F_C$.

\SetKwFunction{Covered}{Covered}
\SetKwFunction{SC}{SynthesizeDNF}
\SetKwFunction{AP}{Append}
\SetKwFunction{EP}{Expand}
The framework of $\mathcal U_{\text{poly}}$ is shown as Algorithm \ref{alg:uni-over}. $\mathcal U_{\text{poly}}$ unifies terms in two steps: $\mathcal U_{\text{poly}}$ firstly syntehsizes \texttt{if}-conditions for each term in $P$ (Lines 1-13), and then merges them together using \texttt{if-then-else} operators (Lines 14-17). However, the merged program $\variable{result}$ cannot be returned directly, as it may involve boolean operators $\texttt{and}, \texttt{or}$ and $\texttt{not}$, which are unavailable in $(\mathbb P_t, \mathbb P_c)$. Therefore, $\mathcal U_{\text{poly}}$ expands $\variable{result}$ and fits it into $(\mathbb P_c, \mathbb P_t)$ via $\EP{}$ (Line 18). However, in practice, the last step can be omitted as the semantics of these extra boolean operators are always avaliable: $\variable{result}$ is always executable in practice even though it is not inside $(\mathbb P_c, \mathbb P_t)$.

\begin{algorithm}[t]
	\small
	\caption{The framework of $\mathcal U_{\text{poly}}$.}
	\label{alg:uni-over}
	\LinesNumbered
	\KwIn{A term set $P = \{p_1, \dots, p_m\}$, a PBE task $T$ and a condition solver $\mathcal C$.}
	\KwOut{A program in $(P, \mathbb P_c)$ satisying all examples or $\top$.}
	\SetKwProg{Fn}{Function}{:}{}
	$\variable{conditionList} \gets \{\}$; \\
	\For {$i \gets 1$; $i < m$; $i \gets i + 1$}{
		$\variable{examples} \gets \emptyset$; \\
		\For {each $(I, O) \in T - \Covered{$p_i, T$}$} {
			$\variable{examples} \gets \variable{examples} \cup \{(I, \texttt{false})\}$;
		}
		\For {each $(I, O) \in \Covered{$p_i, T$} - \bigcup_{j ={i+1}}^{m} \Covered{$p_j, T$} $}{
			$\variable{examples} \gets \variable{examples} \cup \{(I, \texttt{true})\}$;
		}
		$\variable{condition} \gets \mathcal C(\variable{examples})$; \\
		\lIf {$\variable{condition} = \top$}{\Return $\top$}
		$\variable{conditionList}.\AP{\variable{condition}};\ \ T \gets \{(I, O) \in T\ |\ \sem{\variable{condition}}(I)\}$; \\
	}
	$\variable{result} \gets p_m$; \\
	\For {$i \gets m - 1$; $i > 0$; $i \gets i - 1$}{
		$\variable{result} \gets \texttt{if}\ \variable{conditionList}_i\ \texttt{then}\ p_i\ \texttt{else}\ \variable{result}$;
	}
	
	\Return \EP{\variable{result}};
\end{algorithm}

The core of $\mathcal U_{\text{poly}}$ is to synthesize conditions for terms (Lines 3-12). While synthesizing for term $p_i$, the conditions for $p_1, \dots, p_{i-1}$ have been determined, and there are only uncovered examples remained in $T$. For each remaining example $e = (I, O)$, there are three possible cases:
\begin{itemize} 
	\item if $p_i$ is not consistent with $e$, the \texttt{if}-condition of $p_i$ must be \texttt{False} on input $I$, and thus $e$ can be taken as a negative example for the condition (Lines 4-6).
	\item If $p_i$ is the only program in $p_i, \dots, p_n$ that is consistent with example $e$, the \texttt{if}-condition of $p_i$ must be \texttt{True} on input $I$, and thus $e$ can be taken as a positive example (Lines 7-9). 
	\item Otherwise, either the condition is evaluated to true or false is acceptable, as $p_i$ is not the last term satisfying this example. Therefore, $\mathcal U_{\text{poly}}$ ignores this example while synthesizing the condition: If the synthesized condition takes \texttt{false} on $e$, $e$ will be left to subsequent terms.
\end{itemize}

$\mathcal U_{\text{poly}}$ invokes condition solver $\mathcal C$ to synthesize a condition from examples (Line 10). $\mathcal U_{\text{poly}}$ excludes all examples that are covered by the new condition (Line 12) and then continue to the next term.

The following two theorems show that $\mathcal U_{\text{poly}}$ could inherient the soundness, the completeness and the generalizability from the condition solver $\mathcal C$. 

\begin{theorem} $\mathcal U_{\text{poly}}$ is complete and sound.
\end{theorem}

\begin{theorem} $\mathcal C \in \mathsf {PSG}[\mathcal F_C^{\text{DNF}}] \implies \mathcal U_{\text{poly}} \in \mathsf {PSG}^{\text{N}}[\mathcal F_C]$.
\end{theorem}

So far, the remaining problem is to design a condition solver with polynomial-size generalizability, and in the following two subsections, we shall show how to develop such a condition solver. We start by a simple case where the target condition can be implemented without using  disjuctions, i.e., operator \texttt{or}, in Section \ref{section:uni-simple}. Then, in Section \ref{section:uni-full}, we extend the algorithm to general disjunctive normal forms.

\subsection{Condition Synthesis for Clauses} \label{section:uni-simple}
In this section, for the simple case where disjunctions are banned, we develop a condition solver $\mathcal C_{\text{ND}}$ with polynomial-size generalizability. Formally, we assume the program domain are in the form of $\text{ND}(\mathbb P_c)$, where $\text{ND}(\mathbb P_c)$ is the smallest set satisfying:
$$
\text{ND}(\mathbb P_c) = \{\texttt{true}\} \cup \left\{c\ \texttt{and}\ p\ |\ c \in \overline{\mathbb P_c}, p \in \text{ND}(\mathbb P_c)\right\}
$$
where $\mathbb P_c$ is a domain of atomic conditions, and $\overline {\mathbb P_c}$ is defined as $\mathbb P_c \cup \{\texttt{not}\ c\ |\ c \in \mathbb P_c\}$. $\mathcal F^{\text{ND}}_C$ denote the boolean domains induced from $\mathcal F_C$.

\begin{algorithm}[t]
	\small
	\caption{Condition solver $\mathcal C_{\text{ND}}$ for the simple case where disjunctions are banned.}
	\label{alg:uni-over}
	\LinesNumbered
	\KwIn{A condition domain $\mathbb P_c$ and a PBE task $T$.}
	\KwOut{A program in $\text{ND}(\mathbb P_c)$ satisfying all examples or $\top$.}
	\SetKwProg{Fn}{Function}{:}{}
	$\forall p \in \overline{\mathbb P_c}, P(T, p) \gets \{(I, O) \in T\ |\ \sem{p}(I) = \texttt{true}\}$; \\
	$\forall p \in \overline{\mathbb P_c}, N(T, p) \gets \{(I, O) \in T\ |\ \sem{p}(I) = \texttt{false}\}$; \\
	$P(T) \gets \{(I, O) \in T\ |\ O = \texttt{true}\};\ \ N(T) \gets \{(I, O) \in T\ |\ O = \texttt{false}\};$ \\
	$\overline{\mathbb P_c}(T) \gets \{p \in \overline{\mathbb P_c}\ |\ P(T) \subseteq P(T, p)\}$; \\
	\lIf {$\left(\cap_p N(T, p) \text{ for } p \in \overline{\mathbb P_c}(T) \right)\not \subseteq N(T)$}{\Return $\top$}
	$\variable{result} \gets \overline{\mathbb P_c}(T)$; \\
	\For {each $p \in \overline{\mathbb P_c}(T)$ in the decreasing order of the size}{
		\If {$\left(\cap_p N(T, p) \text{ for } p \in \left(\variable{result} - \{p\}\right) \right)\not \subseteq N(T)$}{
			$\variable{result} \gets \variable{result} - \{p\}$;
		}
	}
	\Return $\texttt{and}_{p}\ p$ for $p \in \variable{result}$;
\end{algorithm} 

The pseudo code of $\mathcal C_{\text{ND}}$ is shown as Algorithm \ref{alg:uni-over}. For a PBE task $T$ and a program $p \in \text{ND}(\mathbb P_c)$, we use $P(T, p), N(T, p)$ to denote the set of examples where program $p$ are evaluated to $\texttt{true}$ and $\texttt{false}$ respectively (Lines 1-2). By the semantics of \texttt{and} operator:
\begin{equation} \label{eq:example}
	P(T, c\ \texttt{and}\ p) = P(T, c) \cap P(T, p)\ \ \ N(T, c\ \texttt{and}\ p) = N(T, c) \cup N(T, p)
\end{equation}

We use $P(T)$ and $N(T)$ to denote the set of positive examples and negative examples respectively (Line 3). The task for $\mathcal C_{\text{ND}}$ is to find a program $p$ such that $P(T) \subseteq P(T, p) \wedge N(T, p) \subseteq N(T)$. 

The main idea of $\mathcal C_{\text{ND}}$ is two parts. In the first part (Lines 4-5), we use the monotonicity of the semantics of $\text{ND}(\mathbb P_c)$. By the left of Equation \ref{eq:example}, for a program $p$, $P(T) \subseteq P(T, p)$ if and only if all conditions used by $p$ are in $\overline{\mathbb P_c}(T) = \{c \in \overline{\mathbb P_c}\ |\ P(T) \subseteq P(T, c)\}$, i.e., the set of conditions that are evaluated to \texttt{true} on all positive examples. Moreover, by the right side of Equation \ref{eq:example}, among all these programs, the conjunction of $\overline{\mathbb P_c}(T)$ is evalauted to \texttt{false} on most examples. Therefore, if there is a valid program in $\text{ND}(\mathbb P_c)$, the conjunction of $\overline{\mathbb P_c}(T)$ must be valid.

In the second part (Lines 6-11), $\mathcal C_{\text{ND}}$ searches for a valid program with a better generalizability. Though $\overline{\mathbb P_c}(T)$ is guaranteed to be a valid program, it may include many redundant programs and thus its size can be extremely large. $\mathcal C_{\text{poly}}$ recues the redundancy in a greedy way: It considers conditions in $\overline{\mathbb P_c}(T)$ in the decreasing order of the size (Line 7), and exludes the condition whenever possible (Lines 8-10). After this process, though the conjunction of $\variable{result}$ may not be the smallest solution, the largest conditioin used by $\variable{result}$ must be the minimum among all valid solutions: Such a property is crucial for proving the generalizability of $\mathcal C_{\text{ND}}$.

\begin{theorem} $\mathcal C_{\text{ND}} \in \mathcal PSG[\mathcal F_C^{\text{ND}}]$. 
\end{theorem}
\SetKwFunction{SR}{Search}
\SetKwFunction{GC}{GetPossibleClauses}
\SetKwFunction{SCS}{SimplifyClauseSet}
\SetKwFunction{VC}{IsValidClause}
\SetKwFunction{In}{Insert}
\subsection{Condition Synthesis for Disjunctive Normal Forms} \label{section:uni-full}
\begin{algorithm}[t]
	\small
	\caption{Condition solver $\mathcal C$ for disjunctive normal forms}
	\label{alg:uni-over}
	\LinesNumbered
	\KwIn{A condition domain $\mathbb P_c$ and a PBE task $T$.}
	\KwOut{A program in $\text{DNF}(\mathbb P_c)$ satisfying all examples or $\top$.}
	\SetKwProg{Fn}{Function}{:}{}
	\Fn{\VC{$\variable{clause} = \{p_1, \dots, p_m\}, E_P, E_N, \variable{sizeLimit}$}}{
		$P(\variable{clause}) = \cap_{i} P(T, p_i) \cap E_p; \ \ N(\variable{clause}) = \cup_{i} N(T, p_i)$; \\
		\Return $E_N \subseteq N(\variable{clause}) \wedge |P(\variable{clause})| \geq \variable{sizeLimit}^{-1}|E_P|$; 
	}
	\Fn{\SCS{$\variable{clauseSet}, E_P, E_N$}}{
		$\variable{result}$
	}
	\Fn{\GC{\variable{atomicSet}, $E_P$, $E_N$, \variable{sizeLimit}}}{
		$m \gets |\variable{atomSet}|;\ \ \ p_1, \dots, p_m \gets \variable{atomSet};$ \\ 
		\If {$|\variable{atomSet}| = 1$} {
			$\variable{result} \gets \{\emptyset\}$; \\
			\lIf {\VC{$\{p_1\}, E_P, E_N, \variable{sizeLimit}$}}{$\variable{result}.\In{$\{p_1\}$}$}
			\Return \SCS{$\variable{result}$}; \\
		}	
		$\variable{mid} \gets \lfloor m / 2 \rfloor;\ \ \variable{result} \gets \emptyset;$ \\
		$\variable{leftResult} \gets \GC{$\left\{p_1, \dots, p_{\variable{mid}}\right\}, E_P, E_N, \variable{sizeLimit}$}$; \\
		$\variable{rightResult} \gets \GC{$\left\{p_{\variable{mid} + 1}, \dots, p_{m}\right\}, E_P, E_N, \variable{sizeLimit}$}$;  \\
		\For {each $(\variable{leftClause}, \variable{rightClause}) \in \variable{leftResult} \times \variable{rightResult}$}{
			\If {\VC{$\variable{leftClsue} \cup \variable{rightClause}, E_P, E_N, \variable{sizeLimit}$}}{$\variable{result}.\In{$\variable{leftClause} \cup \variable{rightClause}$}$;}
		}
		\Return \SCS{\variable{result}};
	}
\end{algorithm} 

==> sections/Unifier2.tex <==
%!TEX root = ../CLIA.tex
\section{Unifier} \label{section:unifier}
In this section, we introduce the unifier $\mathcal U_{\text{poly}}$ used in \mainname, which is designed to have polynomial-size generalizability for LDNF. 

\subsection{Overview}
Given a term set $P = \{p_1, \dots, p_m\}$, unifier $\mathcal U_{\text{poly}}$ unifies $P$ into an intermidiate form:
$$
\texttt{if}\ (c_1)\ \texttt{then}\ p_1\ \texttt{else}\ \texttt{if}\ (c_2)\ \texttt{then}\ p_2\ \texttt{else} \dots \texttt{if}\  (c_{m-1})\ \texttt{then}\ p_{m-1}\ \texttt{else}\ p_m
$$
where $c_1, \dots, c_{m-1}$ are conditions in $\text{DNF}(\mathbb P_c)$, i.e., disjunctions normal forms comprised of $\mathbb P_c$. To achieve this, $\mathcal U_{\text{poly}}$ decomposes the unification task into $m-1$ PBE tasks for $c_1, \dots, c_{m-1}$ respectively.

\SetKwFunction{Covered}{Covered}
\SetKwFunction{SC}{SynthesizeDNF}
\SetKwFunction{AP}{Append}
\SetKwFunction{EP}{Expand}
\begin{algorithm}[t]
	\small
	\caption{The framework of $\mathcal U_{\text{poly}}$.}
	\label{alg:uni-over}
	\LinesNumbered
	\KwIn{A term set $P = \{p_1, \dots, p_m\}$, a PBE task $T$ and a condition solver $\mathcal C$.}
	\KwOut{A program in $(P, \mathbb P_c)$ satisying all examples or $\top$.}
	\SetKwProg{Fn}{Function}{:}{}
	$\variable{conditionList} \gets \{\}$; \\
	\For {$i \gets 1$; $i < m$; $i \gets i + 1$}{
		$\variable{examples} \gets \emptyset$; \\
		\For {each $(I, O) \in T - \Covered{$p_i, T$}$} {
			$\variable{examples} \gets \variable{examples} \cup \{(I, \texttt{false})\}$;
		}
		\For {each $(I, O) \in \Covered{$p_i, T$} - \bigcup_{j ={i+1}}^{m} \Covered{$p_j, T$} $}{
			$\variable{examples} \gets \variable{examples} \cup \{(I, \texttt{true})\}$;
		}
		$c_i \gets \mathcal C(\variable{examples})$; \\
		\lIf {$c_i = \top$}{\Return $\top$}
		$\variable{conditionList}.\AP{$c_i$};\ \ T \gets \{(I, O) \in T\ |\ \neg \sem{c_i}(I)\}$; \\
	}
	$\variable{result} \gets p_m$; \\
	\For {$i \gets m - 1$; $i > 0$; $i \gets i - 1$}{
		$\variable{result} \gets \texttt{if}\ \variable{conditionList}_i\ \texttt{then}\ p_i\ \texttt{else}\ \variable{result}$;
	}
	
	\Return \EP{\variable{result}};
\end{algorithm}

Algorithm \ref{alg:uni-over} shows the framework of $\mathcal U_{\text{poly}}$, which synthesizes conditions in order (Lines 2-13). For each term $p_i$ and each remaining example $e=(I, O)$, there are three possible cases:
\begin{itemize} 
	\item if $p_i$ is not consistent with $e$, the \texttt{if}-condition of $p_i$ must be \texttt{False} on input $I$, and thus $e$ can be taken as a negative example for $c_i$ (Lines 4-6).
	\item If $p_i$ is the only program in $p_i, \dots, p_n$ that is consistent with example $e$, the \texttt{if}-condition of $p_i$ must be \texttt{True} on input $I$, and thus $e$ can be taken as a positive example (Lines 7-9). 
	\item Otherwise, the value of $c_i$ does not matter, as $p_i$ is not the last term satisfying the example. Therefore, $\mathcal U_{\text{poly}}$ chooese to ignore this example: If the synthesized $c_i$ takes \texttt{false} on $e$, $e$ will be left to subsequent terms.
\end{itemize}
In this way, a PBE task for $c_i$ is obtained, and thus the task can be passed to a condition solver $\mathcal C$ (Line 10). After obtaining a valid $c_i$, $\mathcal U_{\text{poly}}$ excludes all examples covered by $c_i$ (Line 12) and then continue to the next term.  

Note that the intermidiate result (Lines 14-16) cannot be returned directly, as it may involve boolean operators $\texttt{and}, \texttt{or}$ and $\texttt{not}$, which are unavailable in $(\mathbb P_t, \mathbb P_c)$. Therefore, $\mathcal U_{\text{poly}}$ expands $\variable{result}$ and fits it into $(\mathbb P_c, \mathbb P_t)$ via $\EP{}$ (Line 18). However, in practice, the last step can be omitted as the semantics of these extra boolean operators are always avaliable: $\variable{result}$ is always executable in practice even though it is not inside $(\mathbb P_c, \mathbb P_t)$.

Just like $\mathcal U_{\text{poly}}$, unifier $\mathcal U_{\text{poly}}$ can also inherient useful properties from the condition solver $\mathcal C$.

\begin{theorem} $\mathcal C$ is valid for $\text{DNF}(\mathcal F_C) \implies \mathcal U_{\text{poly}}$ is valid for $\mathcal F_C$, where $\text{DNF}(\mathcal F_C)$ is a family of condition domains induced from $\mathcal F_C$, i.e., $\text{DNF}(\mathcal F_C) \coloneqq \{(\text{DNF}(\mathbb P_c), \mathbb I')\ |\ ((\mathbb P_t, \mathbb P_c), \mathbb I) \in \mathcal F_C \wedge \mathbb I' \subseteq \mathbb I\}$.
\end{theorem}

\begin{theorem} \label{theorem:unifier-gen} $\mathcal C \in \mathsf {PSG}[\text{DNF}(\mathcal F_C)] \implies \mathcal U_{\text{poly}} \in \mathsf {PSG}[\mathcal F_C]$.
\end{theorem}

By Theorem \ref{theorem:unifier-gen}, the only problem remaining is to design a condition solver with polynomial-size generalizability. We shall gradually build such a condition solver in the following three subsections. 

\subsection{Condition Synthesis for Clauses} \label{section:uni-simple}
In this section, we build a condition solver $\mathcal C_{\text{CL}}$ for the easy case where disjunctions are not allowed. Formally, $\mathcal C_{\text{CL}}$ is designed for $\text{CL}(\mathcal F_C)$, which is defined as $\{(\text{CL}(\mathbb P_c), \mathbb I')\ |\ ((\mathbb P_t, \mathbb P_c), \mathbb I) \in \mathcal F_C \wedge \mathbb I' \subseteq \mathbb I\}$.

For convenience, we start by involving some notations. For a PBE task $T$ and a condition $p$, we use $P(T, p), N(T, p)$ to denote the set of examples where condition $p$ are evaluated to \texttt{true} and \texttt{false} reslectively. By the semantics of \texttt{and} operator, we have:
\begin{equation} \label{eq:example}
	P(T, c_1\ \texttt{and}\ c_2) = P(T, c_1) \cap P(T, c_2)\ \ \ N(T, c_1\ \texttt{and}\ c_2) = N(T, c_1) \cup N(T, c_2)
\end{equation}
Besides, we use $P(T)$ and $N(T)$ to denote positive and negative examples in $T$ respectively. The task for $\mathcal C_{\text{CL}}$ is to find a clause $c$ such that $P(T) \subseteq (T, c) \wedge N(T, c) \subseteq N(T)$. 

\SetKwFunction{SC}{SimplifyClause}
\begin{algorithm}[t]
	\small
	\caption{Condition solver $\mathcal C_{\text{ND}}$ for the simple case where disjunctions are banned.}
	\label{alg:uni-over}
	\LinesNumbered
	\KwIn{A condition domain $\mathbb P_c$ and a PBE task $T$.}
	\KwOut{A program in $\text{CL}(\mathbb P_c)$ satisfying all examples or $\top$.}
	\SetKwProg{Fn}{Function}{:}{}
	\Fn{\SC{$\variable{clause}, T$}}{
		$\variable{result} \gets \variable{clause}$; \\
		\For {each $l \in \variable{clause}$ in the decreasing order of the size}{
			\lIf {$N(T) \subseteq \left(\cap_p N(T, l) \text{ for } l \in \left(\variable{result} - \{l\}\right) \right)$}{
				$\variable{result} \gets \variable{result} - \{l\}$
			}
		}
	\Return \variable{result};
	}
	$\variable{validLiterals} \gets \{l \in \text{L}(\mathbb P_c)\ |\ P(T) \subseteq P(T, l)\}$; \\
	\lIf {$\left(\cap_l N(T, l) \text{ for } l \in \variable{validLiterals} \right)\not \subseteq N(T)$}{\Return $\top$}
	\Return $\texttt{and}_{l}\ l$ for $l \in \SC{$\variable{result}, T$}$;
\end{algorithm} 

The pseudo code of $\mathcal C_{\text{CL}}$ is shown as Algorithm \ref{alg:uni-over}, which is comprised of two parts. In the first part (Lines 7-8), we use the monotonicity given by Equation \ref{eq:example}. By the left equation of Equation \ref{eq:example}, for a clause $c$, $P(T) \subseteq P(T, c)$ if and only if all literals used in $c$ are evaluated to \texttt{true} on all positive examples. $\mathcal C_{\text{CL}}$ finds all such literals and stores them in \variable{validLiterals} (Line 7).  By the right equation of Equation \ref{eq:example}, among all valid clauses, the conjunction of $\variable{validLiterals}$ is evalauted to \texttt{false} on most examples. Therefore, if there is a valid condition in $\text{CL}(\mathbb P_c)$, the conjunction of $\variable{validLiterals}$ must be valid (Line 8).

In the second part (Lines 1-7, 9), $\mathcal C_{\text{CL}}$ reduces the size of $\variable{validLiteral}$: Though the conjunction of $\variable{validLiteral}$ is guaranteed to be a valid condition, it may include many redundant programs and thus its size can be extremely large. $\mathcal C_{\text{poly}}$ use a greedy algorithm, implemented as function \SC{}, to reduce the size of $\variable{validLiteral}$: It considers literal in the decreasing order of the size (Line 3), and exludes them whenever possible (Lines 4). The advantage of this greedy algorithm is that: The literals used in the result is guaranteed to be the lexicographically smallest among all valid clauses.

\begin{lemma} Given a sclause $C$ and a PBE task $T$, let $\{l_1, \dots, l_m\} = \SC{$C,T$}$, and let $\{l'_1, \dots, l'_{m'}\} \subseteq C$ be any set satisfying $N(T) \subseteq \cap_{i} N(T, l'_i)$. Suppose both $l_i$ and $l'_i$ are listed in the decreasing order of the size, i.e., $\forall i, \text{size}(l_i) \geq \text{size}(l_{i + 1}) \wedge \forall i,  \text{size}(l_i') \geq \text{size}(l_{i + 1}')$. Then, list $[\text{size}(l_1), \dots, \text{size}(l_m)]$ is lexicographically smaller than list $[\text{size}(l'_1), \dots, \text{size}(l'_m)]$.
\end{lemma}

\begin{theorem} \label{theorem:cl-gen}For any domain $\mathbb D, (\text{CL}(\mathbb P_c), \mathbb I), \text{gen}[\mathbb D, \mathcal C_{\text{CL}}](p, \epsilon) = O(\ln |\mathbb P_c|) + O(\ln (1 / \epsilon))$.
\end{theorem}

Theorem \ref{theorem:cl-gen} implies that: If $\mathbb P_c$ contains only conditions of which the sizes are close to the target condition, the generalizability of $\mathcal C_{\text{CL}}$ can be bounded by the size of the target.
\subsection{Condition Synthesis for Disjunctive Normal Forms} \label{section:uni-full}
\SetKwFunction{SR}{Search}
\SetKwFunction{DAC}{DivideAndConquer}
\SetKwFunction{SCS}{SimplifyClauseSet}
\SetKwFunction{GC}{GetPossibleClause}
\SetKwFunction{VC}{IsValidClause}
\SetKwFunction{In}{Insert}
\SetKwFunction{Search}{Search}
\SetKwFunction{GPWS}{GetProgramsWithSizeBound}
In this section, we implement a condition solver $\mathcal C$ for disjunctive normal forms based on the simple sovler $\mathcal C_{\text{CL}}$ introduced in the previous section. 

\begin{algorithm}[t]
	\small
	\caption{Condition solver $\mathcal C$ for disjunctive normal forms}
	\label{alg:uni-dnf-main}
	\LinesNumbered
	\KwIn{A condition domain $\mathbb P_c$, a PBE task $T$ and parameters $(k_0, s_0)$.}
	\KwOut{A program in $\text{DNF}(\mathbb P_c)$ satisfying all examples or $\top$.}
	\SetKwProg{Fn}{Function}{:}{}
	\Fn{\Search{$\variable{literals}, T, k$}}{
		\lIf{$(\variable{literals}, T, k)$ is visited before} {\Return $\top$}
		\lIf {$|P(T)| = 0$}{\Return $\{\}$}
		\lIf {$k = 0$}{\Return $\top$}
		\For{each $\variable{clause} \in \GC{$\variable{literals}, T, k$}$}{
			$\variable{searchResult} \gets \Search{$\variable{literals}, T - \left(P(T) \cup P(T, \variable{clause})\right), k - 1$}$; \\
			\lIf{$\variable{searchResult} \neq \top$}{\Return $\{p\} \cup \variable{searchResult}$}
		}
		\Return $\top$;
	}
	$s_{\text{max}} = \max_p \text{size}(p)\text{ for } p \in \mathbb P_c;\ \ k_0 \gets \min(k_0, |T|);\ \ s_0 \gets \min(s_0, s_{\text{max}});$ \\
	\While {$k_0 \leq |T| \vee s_0 \leq s_{\text{max}}$}{
	\For {each $(k, s) \in [1, k_0] \times [1, s_0]$}{
		\If {$(k, s)$ has not been visited before} {
			$d \gets \Search{$\text{L}(\GPWS{$\mathbb P_c, s$}),T, k$}$; \\
			\lIf{$P \neq \top$}{\Return $\texttt{or}_{c}\ \left(\texttt{and}_p\ p\text{ for } p \in c\right)\text{ for } c \in d$}
		}
	}
	$k_0 \gets k_0 + 1; \ \ s_0 \gets s_0 + 1$; 
	}
	\Return $\top$.
\end{algorithm} 

For simplicity, we regard a DNF formula as a set of clauses, and use symbol $d, c$ to represent DNF formulas and clauses respectively. By the semantics of \texttt{or} operator, we have:
\begin{equation} \label{eq:or}
	P(T, d_1\ \texttt{or}\ d_1) = P(T, d_1) \cup P(T, d_2)\ \ \ N(T, d_1\ \texttt{or}\ d_2) = N(T, d_1) \cap N(T, d_2)
\end{equation}
Hence, we could obtain a lemma that is similiar with Lemma \ref{lemma:sample} in form. 
\begin{lemma}\label{lemma:or-sample} Let $T$ be a PBE task, and let $T$ be a DNF formula satisfying all examples in $T$, then:
\begin{itemize}
	\item All clauses in $d$ must be \texttt{false} on all negative examplesin $T$, i.e., $\forall c \in d, N(T, c) \subseteq N(T)$.
	\item There exists a clause in $d$ that is \texttt{true} on at least $|d|^{-1}$ portion of positive examples in $T$, i.e., $\exists c \in d, |P(T, c)| \geq |d|^{-1}|P(T)|$.
\end{itemize}
\end{lemma}
Lemma \ref{lemma:or-sample} allows $\mathcal C$ to decompose the condition synthesis task to clause synthesis tasks in a similiar way as $\mathcal T_{\text{poly}}$ (Lines 11-30 in Algorithm \ref{alg:term-main}).

Algorithm \ref{alg:uni-dnf-main} shows the pseudo code of $\mathcal C$, which is comprised of two parts. The first part is a backtracking on the set of clauses, implemented as Function \Search{} (Lines 1-9), which is almost the same as the second part of Algorithm \ref{alg:term-main}. Function \Search{} takes a set of literals $\variable{literals}$, a PBE task $T$ and an upper bound $k$ as the input, and its goal is to find a valid DNF formula comprised of at most $k$ clauses and literals in $\variable{literals}$. Guided by Lemma \ref{lemma:or-sample}, \Search{} invokes \GC{} to find a set of clauses that are evaluated to \texttt{false} on all negative examples, and are evaluated to \texttt{true} on at least $k^{-1}$ portion of postive examples (Line 14). Then, \Search{} recursively try all possible clauses until a valid DNF formula is found (Lines 6-7). 

The second part iteratively selects parameters for the backtracking (Lines 10-20). Besides the size limit $k$, $\mathcal C$ also iteratively determines the set of literals, as the generalizability of the clause solver $\mathcal C$ is polynomial-size only when the number of literals is bounded (according to Theorem \ref{theorem:cl-gen}). In each turn, $\mathcal C$ invokes function $\GPWS{}$ to obtain all conditions in $\mathbb P_c$ with a size at most $k$, and invokes $\Search{}$ with the corresponding set of literals (Line 14). 

Now, we go to the implementation of Function \GC{}. Actually, applying the sampling algorithm in $\mathcal T_{\text{poly}}$ here can already induce a condition solver with polynomial-size generalizability. But we do not do so, as a more efficient algorithm can be developed by opening the box of the clause solver $\mathcal C_{\text{CL}}$ and applying some domain specific optimizations.

\begin{algorithm}[t]
	\small
	\caption{Implementation of \texttt{GetPossibleClause()} in $\mathcal C$.}
	\label{alg:get-clause}
	\LinesNumbered
	\KwIn{A set of literals $\variable{literals}$, a PBE task $T$, and an upper bound $k$.}
	\KwOut{A set of possible clauses according to Lemma \ref{lemma:or-sample}.}
	\SetKwProg{Fn}{Function}{:}{}
	\Fn{\VC{$\variable{clause} = \{p_1, \dots, p_m\}, T, k$}}{
		\Return $|P(T, \variable{clause}) \cap P(T)| \geq k^{-1}|P(T)|$; 
	}
	\Fn{\SCS{$\variable{clauseSet}, T, k$}}{
		$\variable{result} \gets \{\variable{clause} \in \variable{clauseSet}\ |\ \VC{$\variable{clause}, T, k$}\}$; \\
		\For {each $\variable{clause} \in \variable{clauseSet}$}{
			\If {$\exists \variable{clause}' \in \variable{result}, \left(\left(P(T, \variable{clause}') \cap P(T)\right) =  \left(P(T, \variable{clause}) \cap P(T)\right) \wedge \variable{clause} \subset \variable{clause'}\right)$}{
				$\variable{result} \gets \variable{result} - \{\variable{clause}\}$;
			}
		}
		\Return \variable{result};
	}
	\Fn{\DAC{\variable{literals}, $T$, $k$}}{
		$m \gets |\variable{literals}|;\ \ \ p_1, \dots, p_m \gets \variable{literals};$ \\ 
		\lIf {$|\variable{literals}| = 1$} {
			\Return \SCS{$\{\emptyset, \variable{literals}\}, T, k$}
		}	
		$\variable{mid} \gets \lfloor m / 2 \rfloor;\ \ \variable{result} \gets \emptyset;$ \\
		$\variable{leftResult} \gets \DAC{$\left\{p_1, \dots, p_{\variable{mid}}\right\}, T, k$}$; \\
		$\variable{rightResult} \gets \DAC{$\left\{p_{\variable{mid} + 1}, \dots, p_{m}\right\}, T, k$}$;  \\
		$\variable{result} \gets \{\variable{leftClause} \cup \variable{rightClause}\ |\ \variable{leftClause} \in \variable{leftResult} \wedge \variable{rightClause} \in \variable{rightResult}\}$; \\
		\Return \SCS{\variable{result}};
	}
	$\variable{result} \gets \{\variable{clause} \in \DAC{$\variable{literals}, T, k$}\ |\ N(T) \subseteq N(T, \variable{clause})\}$; \\
	\Return $\{\SC{\variable{clause}}\ |\ \variable{clause} \in \variable{result}\}$; \\
\end{algorithm} 

==> sections/Unifier3.tex <==
%!TEX root = ../CLIA.tex
\section{Unifier} \label{section:unifier}
In this section, we introduce the unifier $\mathcal U_{\text{poly}}$ used in \mainname, which is designed to have polynomial-size generalizability for LDNF. 

\subsection{Overview}
Given a term set $P = \{p_1, \dots, p_m\}$, unifier $\mathcal U_{\text{poly}}$ unifies $P$ into an intermidiate form:
$$
\texttt{if}\ (c_1)\ \texttt{then}\ p_1\ \texttt{else}\ \texttt{if}\ (c_2)\ \texttt{then}\ p_2\ \texttt{else} \dots \texttt{if}\  (c_{m-1})\ \texttt{then}\ p_{m-1}\ \texttt{else}\ p_m
$$
where $c_1, \dots, c_{m-1}$ are conditions in $\text{DNF}(\mathbb P_c)$, i.e., disjunctions normal forms comprised of $\mathbb P_c$. To achieve this, $\mathcal U_{\text{poly}}$ decomposes the unification task into $m-1$ PBE tasks for $c_1, \dots, c_{m-1}$ respectively.

\SetKwFunction{Covered}{Covered}
\SetKwFunction{SC}{SynthesizeDNF}
\SetKwFunction{AP}{Append}
\SetKwFunction{EP}{Expand}
\begin{algorithm}[t]
	\small
	\caption{The framework of $\mathcal U_{\text{poly}}$.}
	\label{alg:uni-over}
	\LinesNumbered
	\KwIn{A term set $P = \{p_1, \dots, p_m\}$, a PBE task $T$ and a condition solver $\mathcal C$.}
	\KwOut{A program in $(P, \mathbb P_c)$ satisying all examples or $\top$.}
	\SetKwProg{Fn}{Function}{:}{}
	$\variable{conditionList} \gets \{\}$; \\
	\For {$i \gets 1$; $i < m$; $i \gets i + 1$}{
		$\variable{examples} \gets \emptyset$; \\
		\For {each $(I, O) \in T - \Covered{$p_i, T$}$} {
			$\variable{examples} \gets \variable{examples} \cup \{(I, \texttt{false})\}$;
		}
		\For {each $(I, O) \in \Covered{$p_i, T$} - \bigcup_{j ={i+1}}^{m} \Covered{$p_j, T$} $}{
			$\variable{examples} \gets \variable{examples} \cup \{(I, \texttt{true})\}$;
		}
		$c_i \gets \mathcal C(\variable{examples})$; \\
		\lIf {$c_i = \top$}{\Return $\top$}
		$\variable{conditionList}.\AP{$c_i$};\ \ T \gets \{(I, O) \in T\ |\ \neg \sem{c_i}(I)\}$; \\
	}
	$\variable{result} \gets p_m$; \\
	\For {$i \gets m - 1$; $i > 0$; $i \gets i - 1$}{
		$\variable{result} \gets \texttt{if}\ \variable{conditionList}_i\ \texttt{then}\ p_i\ \texttt{else}\ \variable{result}$;
	}
	
	\Return \EP{\variable{result}};
\end{algorithm}

Algorithm \ref{alg:uni-over} shows the framework of $\mathcal U_{\text{poly}}$, which synthesizes conditions in order (Lines 2-13). For each term $p_i$ and each remaining example $e=(I, O)$, there are three possible cases:
\begin{itemize} 
	\item if $p_i$ is not consistent with $e$, the \texttt{if}-condition of $p_i$ must be \texttt{False} on input $I$, and thus $e$ can be taken as a negative example for $c_i$ (Lines 4-6).
	\item If $p_i$ is the only program in $p_i, \dots, p_n$ that is consistent with example $e$, the \texttt{if}-condition of $p_i$ must be \texttt{True} on input $I$, and thus $e$ can be taken as a positive example (Lines 7-9). 
	\item Otherwise, the value of $c_i$ does not matter, as $p_i$ is not the last term satisfying the example. Therefore, $\mathcal U_{\text{poly}}$ chooese to ignore this example: If the synthesized $c_i$ takes \texttt{false} on $e$, $e$ will be left to subsequent terms.
\end{itemize}
In this way, a PBE task for $c_i$ is obtained, and thus the task can be passed to a condition solver $\mathcal C$ (Line 10). After obtaining a valid $c_i$, $\mathcal U_{\text{poly}}$ excludes all examples covered by $c_i$ (Line 12) and then continue to the next term.  

Note that the intermidiate result (Lines 14-16) cannot be returned directly, as it may involve boolean operators $\texttt{and}, \texttt{or}$ and $\texttt{not}$, which are unavailable in $(\mathbb P_t, \mathbb P_c)$. Therefore, $\mathcal U_{\text{poly}}$ expands $\variable{result}$ and fits it into $(\mathbb P_c, \mathbb P_t)$ via $\EP{}$ (Line 18). However, in practice, the last step can be omitted as the semantics of these extra boolean operators are always avaliable: $\variable{result}$ is always executable in practice even though it is not inside $(\mathbb P_c, \mathbb P_t)$.

Just like $\mathcal U_{\text{poly}}$, unifier $\mathcal U_{\text{poly}}$ can also inherient useful properties from the condition solver $\mathcal C$.

\begin{theorem} $\mathcal C$ is valid for $\text{DNF}(\mathcal F_C) \implies \mathcal U_{\text{poly}}$ is valid for $\mathcal F_C$, where $\text{DNF}(\mathcal F_C)$ is a family of condition domains induced from $\mathcal F_C$, i.e., $\text{DNF}(\mathcal F_C) \coloneqq \{(\text{DNF}(\mathbb P_c), \mathbb I')\ |\ ((\mathbb P_t, \mathbb P_c), \mathbb I) \in \mathcal F_C \wedge \mathbb I' \subseteq \mathbb I\}$.
\end{theorem}

\begin{theorem} \label{theorem:unifier-gen} $\mathcal C \in \mathsf {PSG}[\text{DNF}(\mathcal F_C)] \implies \mathcal U_{\text{poly}} \in \mathsf {PSG}[\mathcal F_C]$.
\end{theorem}

By Theorem \ref{theorem:unifier-gen}, the only problem remaining is to design a condition solver with polynomial-size generalizability. We shall gradually build such a condition solver in the following three subsections. 

\subsection{Condition Synthesis for Clauses} \label{section:uni-simple}
Before discussing the condition solver $\mathcal C$, we introduce some useful notations first:
\begin{itemize}
	\item We regard a DNF formula $d$ as a set of clauses, regard a clause $c$ as a set of literals, and use notation $p_c(c)$ and $p_d(d)$ to represent the corresponding program, $\left(\texttt{and}_l\ l\text{ for }l \in c\right)$ and $\left(\texttt{or}_c\ \left(\texttt{and}_l\ l\text{ for }l \in c\right)\text{ for }c \in d\right)$, respectively. 
	\item For an input space $\mathbb I$ and a condition $p$, we use $P(\mathbb I, p)$ and $N(\mathbb I, p)$ to denote the set of inputs where $p$ is evaluated to \texttt{true} and \texttt{false} respectively, i.e.:
	$$P(\mathbb I, p) \coloneqq \{I \in \mathbb I\ |\ \sem{p}(I) = \texttt{true}\}\ \ \ N(\mathbb I, p) \coloneqq \{I \in \mathbb I\ |\ \sem{p}(I) = \texttt{false}\}$$
	\item For a PBE task $T$, we use $\mathbb I(T)$, $\mathbb I_P(T)$ and $\mathbb I_N(T)$ to denote the inputs of examples, positive examples and negative examples in $T$ respectively, i.e.:
	$$\mathbb I(T) \coloneqq \{I\ |\ (I, O) \in T\}\ \ \ \mathbb I_P(T) \coloneqq \{I\ |\ (I, \texttt{true}) \in T\}\ \ \ \mathbb I_N(T) \coloneqq \{I\ |\ (I, \texttt{false}) \in T\}$$
\end{itemize}
For a PBE task $T$ on condition domain $(\text{DNF}(\mathbb P_c), \mathbb I)$, a valid condition $p$ should satisfy two conditions: (1) $\mathbb I_P(T) \subseteq P(\mathbb I(T), p)$; (2) $\mathbb I_N(T) \subseteq N(\mathbb I(T), p)$. They will be frequently used when designing solver. 

\begin{algorithm}[t]
	\small
	\caption{The pseudo code of clause solver $\mathcal C_{\text{CL}}$.}
	\label{alg:uni-over}
	\LinesNumbered
	\KwIn{A condition domain $\mathbb P_c$ and a PBE task $T$.}
	\KwOut{A program in $\text{CL}(\mathbb P_c)$ satisfying all examples or $\top$.}
	\SetKwProg{Fn}{Function}{:}{}

	$c^* \gets \{l \in \text{L}(\mathbb P_c)\ |\ \mathbb I_P(T) \subseteq P(\mathbb I(T), l)\}$; \\
	\lIf {$\mathbb I_N(T) \subseteq N(\mathbb I(T), c^*) $}{\Return $p_c(c^*)$}
	\Return $\top$;
\end{algorithm} 

In this section, we focus on a subproblem of condition synthesis, where the target condition is assumed to be a single clause. Algorithm \ref{alg:uni-over} shows the pseudo code of a simple solver $\mathcal C_{\text{CL}}$.

$\mathcal C_{\text{CL}}$ starts with the first condition of a valid clause: $\mathbb I_P(T) \subseteq P(\mathbb I(T), c)$. By the semantics of operator $\texttt{and}$, for any clause $c$ and any literal $l \in c$, $P(\mathbb I(T), c)$ must a subset of $P(\mathbb I(T), l)$. Therefore, only those literals that covers all positive examples can be used in the result. $\mathcal C_{\text{CL}}$ constructs a clause $c^*$ that includes all possible literals (Line 1). Obviously, $c^*$ itself satisfies the first condition, and all valid clauses must be a subset of $c^*$. By the semantic of operator \texttt{and}, for any two clauses $c_1$ and $c_2$, $c_1 \subseteq c_2 \implies N(\mathbb I(T), c_1) \subseteq N(\mathbb I(T), c_2)$. Therefore, if $c^*$ does not satisfy the second condition, neither does any subset of $c^*$ (Lines 2-3).

The generalizability of $\mathcal C_{\text{CL}}$ is bounded. For input space $\mathbb I$ and target clause $c$, we say a literal $l$ is incorrect for target clause $c$ if $P(\mathbb I, c) \not \subseteq P(\mathbb I, l)$. According to Algorithmn \ref{alg:uni-over}, $\mathcal C_{\text{CL}}$ generalizes to the target $c$ when all incorrect literals are excluded. As the number of incorrect literals is bounded by $|\text{L}(\mathbb P_c)| \leq 2|\mathbb P_C|$, and the probability for each incorrect literal to be excluded is guaranteed by our second assumption, the generalizability of $\mathcal C_{\text{CL}}$ is bounded by $O(\ln |\mathbb P_C|)$.

\begin{theorem} \label{theorem:cl-gen}For any domain $\mathbb D = (\text{CL}(\mathbb P_c), \mathbb I), \text{gen}[\mathbb D, \mathcal C_{\text{CL}}](p, \epsilon) \leq \frac{1}{\alpha}\left(\ln \left(2|\mathbb P_C|\right) + \ln(1 / \epsilon)\right)$.
\end{theorem}

Theorem \ref{theorem:cl-gen} implies that: If $\mathbb P_c$ contains only conditions of which the sizes are close to the target condition, the generalizability of $\mathcal C_{\text{CL}}$ can be bounded by the size of the target.
\subsection{Condition Synthesis for Disjunctive Normal Forms} \label{section:uni-full}
In this section, we implement a condition solver $\mathcal C$ with guaranteed generalizability for disjunctive normal forms. By the semantics of operator \texttt{or}, we could obtain a lemma that is similiar with Lemma \ref{lemma:sample} in form. 

\begin{lemma}\label{lemma:or-sample} Let $T$ be a PBE task and $d$ be a DNF formula satisfying all examples in $T$, then:
	\begin{itemize}
		\item All clauses in $d$ must be \texttt{false} on all negative examplesin $T$, i.e., $\forall c \in d, \mathbb I_N(T) \subseteq N(\mathbb I(T), c)$.
		\item There exists a clause in $d$ that is \texttt{true} on at least $|d|^{-1}$ portion of positive examples in $T$, i.e., $\exists c \in d, |P(\mathbb I(T), c)| \geq |d|^{-1}|\mathbb I_P(T)|$.
	\end{itemize}
\end{lemma}
Lemma \ref{lemma:or-sample} allows $\mathcal C$ to decompose the condition synthesis task to clause synthesis tasks in a similiar way as $\mathcal T_{\text{poly}}$ (Lines 11-30 in Algorithm \ref{alg:term-main}).

\SetKwFunction{SR}{Search}
\SetKwFunction{DAC}{DivideAndConquer}
\SetKwFunction{SCS}{SimplifyClauseSet}
\SetKwFunction{GC}{GetPossibleClause}
\SetKwFunction{VC}{IsValidClause}
\SetKwFunction{In}{Insert}
\SetKwFunction{De}{Delete}
\SetKwFunction{G}{Get}
\SetKwFunction{Search}{Search}
\SetKwFunction{GPWS}{GetProgramsWithSizeBound}

\begin{algorithm}[t]
	\small
	\caption{Condition solver $\mathcal C$ for disjunctive normal forms}
	\label{alg:uni-dnf-main}
	\LinesNumbered
	\KwIn{A condition domain $\mathbb P_c$, a PBE task $T$ and parameters $(k_0, s_0)$.}
	\KwOut{A DNF formula in $\text{DNF}(\mathbb P_c)$ satisfying all examples or $\top$.}
	\SetKwProg{Fn}{Function}{:}{}
	\Fn{\Search{$\variable{literals}, T, k$}}{
		\lIf{$(\variable{literals}, T, k)$ is visited before} {\Return $\top$}
		\lIf {$|\mathbb I_P(T)| = 0$}{\Return $\{\}$}
		\lIf {$k = 0$}{\Return $\top$}
		\For{each $c \in \GC{$\variable{literals}, T, k$}$}{
			$\variable{searchResult} \gets \Search{$\variable{literals}, T - \left\{(I, \texttt{true}) \in T\ |\ \sem{p_c(c)}(I) = \texttt{true} \right\}, k - 1$}$; \\
			\lIf{$\variable{searchResult} \neq \top$}{\Return $\{c\} \cup \variable{searchResult}$}
		}
		\Return $\top$;
	}
	$s_{\text{max}} = \max_p \text{size}(p)\text{ for } p \in \mathbb P_c;\ \ k_0 \gets \min(k_0, |T|);\ \ s_0 \gets \min(s_0, s_{\text{max}});$ \\
	\While {$k_0 \leq |T| \vee s_0 \leq s_{\text{max}}$}{
	\For {each $(k, s) \in [1, k_0] \times [1, s_0]$}{
		\If {$(k, s)$ has not been visited before} {
			$d \gets \Search{$\text{L}(\GPWS{$\mathbb P_c, s$}),T, k$}$; \\
			\lIf{$P \neq \top$}{\Return $p_d(d)$}
		}
	}
	$k_0 \gets k_0 + 1; \ \ s_0 \gets s_0 + 1$; 
	}
	\Return $\top$.
\end{algorithm} 

Algorithm \ref{alg:uni-dnf-main} shows the pseudo code of $\mathcal C$, which is comprised of two parts. The first part is a backtracking on the set of clauses, implemented as Function \Search{} (Lines 1-9), which is almost the same as the second part of Algorithm \ref{alg:term-main}. Function \Search{} takes a set of literals $\variable{literals}$, a PBE task $T$ and an upper bound $k$ as the input, and its goal is to find a valid DNF formula comprised of at most $k$ clauses with literals inside $\variable{literals}$. Guided by Lemma \ref{lemma:or-sample}, \Search{} invokes \GC{} to find a set of clauses that are evaluated to \texttt{false} on all negative examples, and are evaluated to \texttt{true} on at least $k^{-1}$ portion of postive examples (Line 14). Then, \Search{} recursively try all possible clauses until a valid DNF formula is found (Lines 6-7). 

The second part iteratively selects parameters for the backtracking (Lines 10-20). Besides the size limit $k$, $\mathcal C$ also iteratively determines the set of literals, as the generalizability of the clause solver $\mathcal C$ is polynomial-size only when the number of literals is bounded (according to Theorem \ref{theorem:cl-gen}). In each turn, $\mathcal C$ invokes function $\GPWS{}$ to obtain all conditions in $\mathbb P_c$ with a size at most $k$, and invokes $\Search{}$ with the corresponding set of literals (Line 14). 

Now, we go to the implementation of \GC{} (abbreviated as \G{}). To guarantee the generalizability of $\mathcal C_{\text{CL}}$, \G{} should satisfy the following two requirements:
\begin{itemize}
	\item Under a small number of examples, which is at most polynomial to $\ln |\mathbb P_c|$, \G{} should guarantee that with a high probability, at least one intended clause is found. Otherwise, the probability for $
	\mathcal C_{\text{CL}}$ to miss the target condition may be unbounded.
	\item The number of clauses returned by \G{} should be small, of which the logarithm should be at most polynomial to $\ln |\mathbb P_c|$. Otherwise, the search alrgoithm may expand to too many search branches, and thus it may require a lot of examples to guarantee the first valid DNF formula is semantically equivalent to the target one.
\end{itemize}

Actually, applying the sampling algorithm in $\mathcal T_{\text{poly}}$ with the clause solver $\mathcal C_{\text{CL}}$ already satisfies both requirements. In condition solver $\mathcal C$, we make some optimization by opening the box of the clause solver $\mathcal C$. More concretely, our implementation of \G{} finds all possible results of $\mathcal C_{\text{CL}}$, denoted as a representative set, and returns them as the result. According to Algorithm \ref{alg:uni-over}, though there may be many clauses corresponding to each semantics on the space of positive examples, only the largest clause to each semantics is possible to be returned by $\mathcal C_{\text{CL}}$.

We formalize this idea with some additional notations. Given an input space $\mathbb I$ and a set of literals $L$, the relationship of semantically equivalence $\sim_{\mathbb I}$ divides the clause space $\text{CL}(L)$ into several equivalent classes. We denote the set of those classes as $[\text{CL}(L)]_{\mathbb I}$, and the equivalent class of clause $c$ as $[c]_{\mathbb I}$. It is easy to show that each class $[c]_{\mathbb I}$ contains a globally largest clause that is the union of all its elements, i.e., $\exists c' \in [c]_{\mathbb I},  c' = \left(\cup_{x}\ x\text{ for } x \in [c]_{\mathbb I}\right)$. 

\begin{definition}[Representative Clauses] 
	Given a input space $\mathbb I$, a size limit $k$, and a set of literals $L$, representative set $R(\mathbb I, k, L) \subseteq \text{CL}(L)$ includes all clause $c$ satisfying: (1) $c$ is the largest element in $[c]_{\mathbb I}$, (2) $c$ satisfying at least $k^{-1}$ portion of positive examples, i.e., $|P(\mathbb I_P(T), c)| \geq k^{-1} |\mathbb I_T(P)|$.
\end{definition}

The following lemma shows that $R(T, k, L)$ succesfully captures all wanted results of $\mathcal C_{\text{CL}}$.

\begin{lemma} For any PBE task $T$, size limit $k$, and set $L$ of literals, for any subset of examples $T' \subseteq T$, if the clause synthesized by $\mathcal C_{\text{CL}}$ on subtask $T'$ satisfies at least $k^{-1}$ portion of positive examples in $T$, this clause must be inside $R(T, k, L)$, i.e.,
	$$
	\forall T' \subseteq T, \left(\big|P\big(\mathbb I_P(T), \mathcal C_{\text{CL}}[L](T')\big)\big| \geq \frac{|\mathbb I_P(T)|}{k} \implies \mathcal C_{\text{CL}}[L](T') \in R(\mathbb I_P(T), k, L)\right)
	$$
\end{lemma}

\begin{algorithm}[t]
	\small
	\caption{Implementation of \texttt{GetPossibleClause()} in $\mathcal C$.}
	\label{alg:get-clause}
	\LinesNumbered
	\KwIn{A set of literals $\variable{literals}$, a PBE task $T$, and an upper bound $k$.}
	\KwOut{A set of possible clauses according to Lemma \ref{lemma:or-sample}.}
	$\variable{result} \gets \{\emptyset\}$; \\
	\For {each $l \in \variable{literals}$}{
		\For {each $c \in \variable{result}$}{
			\lIf{$\left|P(\mathbb I_P(T), c \cup \{l\})\right| \geq k^{-1}\left|\mathbb I_P(T)\right|$}{$\variable{result}.\In{$c \cup \{l\}$}$}
		}
		\For {each $c \in \variable{result}$}{
			\lIf{$\exists c' \in \variable{result}, \left(P(\mathbb I_P(T), c) = P(\mathbb I_P(T), c') \wedge c \subset c'\right)$}{$\variable{result}.\De{$c$}$}
		}
	}
	\Return $\left\{c \in \variable{result}\ |\  \mathbb I_N(T) \subseteq N(\mathbb I (T),c)\right\}$
\end{algorithm} 

Our implementation of \G{} is shown as Algorithm \ref{alg:get-clause}. \G{} maintains set \variable{result} which is equal to $R(\mathbb I_P(T), k, L)$ for some hidden literal set $L$. Initially, $L$ is empty and thus $\variable{result}$ includes only an empty clause, i.e., \texttt{true} (Line 1). \G{} considers all literals in order (Lines 2-9). In each turn, a new literal is inserted to $L$ and thus \variable{result} is updated correspondingly (Lines 3-8). At last, $\variable{result}$ is equal to $R(\mathbb I_P(T), k, \variable{literal})$, and thus \G{} returns all valid clause in $\variable{result}$ (Line 10).

Now, we shall informally show why \G{} satisfies the two requirements. The full proof can be found in the appendix. The first requirement is obvious: As \G{} returns all possible results of $\mathcal C_{\text{CL}}$ on a subset of examples, the probability for \G{} to find an inteneded clause must be larger than the sampling algorithm in $\mathcal T_{\text{poly}}$, which has been proved to satisfy this condition. 

To prove the second requirement, we need to bound the size of $R(\mathbb I_P(T), k, L)$. Let $\mathbb I_P \subseteq \mathbb I$ be the entire set of inputs where the target condition is \texttt{true}. As $\mathbb I_P(T) \subseteq \mathbb I_P$, relation $\sim_{\mathbb I_P}$ can be regarded as a refinement of $\sim_{\mathbb I_P(T)}$. Therefore, $|R(\mathbb I_P(T), k, L)|$ is no larger than the number of classes $[c]_{\mathbb I_P}$ in $[\text{CL}(L)]_{\mathbb I_P}$ with $|P(\mathbb I_P(T), c)| \geq k^{-1}|\mathbb I_P(T)|$. Clearly, the more inputs in $\mathbb I_P$ are covered by $c$, the more probable for equivalent class $[c]_{\mathbb I_P}$ to satisfy at least $k^{-1}$ portion of examples in $T$. The following lemma bounds the number of equivalent classes in $[\text{CL}(L)]_{\mathbb I_P}$ that covers a large enough number of examples, and limits the size of the representative set $R(\mathbb I_P(T), k, L)$ to be small.

\begin{lemma} Let $t = \frac{1}{\alpha}\ln(4|L|)$, the number of equivalent classes $[c]_{\mathbb I_P}$ in $[\text{CL}(L)]_{\mathbb I_P}$, where the probability for $c$ to be \texttt{true} on a random example in $\mathbb I_P$ is at least $\beta$, is at most $2\beta^{-t}$, i.e.,:
	$$\left|\left\{[c]_{\mathbb I_P} \in [\text{CL}(L)]_{\mathbb I_P}\ \big|\ \Pr_{I \sim {D_I}} \left[\sem{c}(I)\ |\ I \in \mathbb I_P\right] \geq \beta\right\}\right| \leq 2\left(\frac{1}{\beta}\right)^t
	$$ 
\end{lemma}

Therefore, we could prove that the generalizability of $\mathcal C$ is polynomial.
\begin{theorem} \label{theorem:condition-solver}$\mathcal C \in \mathsf{PSG}[\text{DNF}(\mathcal F_C)]$.
\end{theorem}

Combining Theorem \ref{theorem:condition-solver} with Theorem \ref{theorem:unifier-gen} and Theorem \ref{theorem:gen-stun}, we prove the generalizability of $\mathcal U_{\text{poly}}$ and \mainname are all polynomial
\begin{theorem} $\mathcal U_{\text{poly}}$ implemented with condition solver $\mathcal C$ is inside $\mathsf{PSG}[\mathcal F_C]$.
\end{theorem}
\begin{theorem}\label{theorem:main} Domain solver $\mathcal S_t$ is size-preserving for $T(\mathcal F_C) \implies \mainname \in \mathsf{PSG}[\mathcal F_C]$.
\end{theorem}



==> sections/Unifier4.tex <==
%!TEX root = ../CLIA.tex
\section{Unifier} \label{section:unifier}
In this section, we introduce the unifier $\mathcal U_{\text{poly}}$ used in \mainname. Guided by Theorem \ref{theorem:gen-stun}, $\mathcal U_{\text{poly}}$ is designed to have polynomial-size generalizability to guarantee generalizability of $\mainname$.

\subsection{Overview}
As the structure of a decision tree is rather complex, $\mathcal U_{\text{poly}}$ unifies $P$ into a decision list, a form of nested \texttt{if-then-else} operators with a linear structure. Formally, given a term set $P = \{p_1, \dots, p_m\}$, unifier $\mathcal U_{\text{poly}}$ unifies $P$ into an intermidiate form:
$$
\texttt{if}\ (c_1)\ \texttt{then}\ p_1\ \texttt{else}\ \texttt{if}\ (c_2)\ \texttt{then}\ p_2\ \texttt{else} \dots \texttt{if}\  (c_{m-1})\ \texttt{then}\ p_{m-1}\ \texttt{else}\ p_m
$$
Specially, $c_1, \dots, c_{m-1}$ are required to be disjunctive normal forms comprised of $\mathbb P_c$, denoted as $\text{DNF}(\mathbb P_c)$. $\text{DNF}(\mathbb P_c)$ is defined in three steps:
\begin{enumerate}
	\item $\text{L}(\mathbb P_c)$ represents the set of literals comprised of $\mathbb P_c$, i.e., $\text{L}(\mathbb P_c) = \{\texttt{not } p\ |\ p \in \mathbb P_c\} \cup \mathbb P_c$
	\item $\text{CL}(\mathbb P_c)$ represents the set of clauses compised of $\mathbb P_c$. $\text{CL}(\mathbb P_c)$ is the smallest set such that:
	$$\text{CL}(\mathbb P_c) = \{\texttt{true}\} \cup \{l\ \texttt{and}\ c\ |\ l \in \text{L}(\mathbb P_c), c \in \text{CL}(\mathbb P_c)\}$$
	\item $\text{DNF}(\mathbb P_c)$ is defined as the smallest set such that:
	$$\text{DNF}(\mathbb P_c) = \{\texttt{false}\} \cup \{c\ \texttt{or}\ d\ |\ c \in \text{CL}(\mathbb P_c), d \in \text{DNF}(\mathbb P_c)\}$$
\end{enumerate}

We use notation $(\mathbb P_t, \mathbb P_c)_{\text{L}}$ to denote the set of these decision lists where \texttt{if}-terms and \texttt{if}-conditions are from $\mathbb P_t$ and $\text{DNF}(\mathbb P_c)$ respectively. Lemma \ref{lemma:decision-tree-size} shows that converting a program from $(\mathbb P_t, \mathbb P_c)$ to $(\mathbb P_t, \mathbb P_c)_{\text{L}}$ would not increase its size much.

\begin{lemma} \label{lemma:decision-tree-size}For any condition domain $\mathbb D$ and any program $p \in (\mathbb P_t, \mathbb P_c)$, there always exists a program $p' \in (\mathbb P_t, \mathbb P_c)_{\text{L}}$ such that $p \sim_{\mathbb I} p' \wedge \text{size}(p') \leq 2\text{size}(p)^2$.
\end{lemma}

\SetKwFunction{Covered}{Covered}
\SetKwFunction{SC}{SynthesizeDNF}
\SetKwFunction{AP}{Append}
\SetKwFunction{EP}{Expand}
\begin{algorithm}[t]
	\small
	\caption{The framework of $\mathcal U_{\text{poly}}$.}
	\label{alg:uni-over}
	\LinesNumbered
	\KwIn{A term set $P = \{p_1, \dots, p_m\}$, a PBE task $T$ and a condition solver $\mathcal C$.}
	\KwOut{A program in $(P, \mathbb P_c)$ satisying all examples or $\top$.}
	\SetKwProg{Fn}{Function}{:}{}
	$\variable{conditionList} \gets \{\}$; \\
	\For {$i \gets 1$; $i < m$; $i \gets i + 1$}{
		$\variable{examples} \gets \emptyset$; \\
		\For {each $(I, O) \in T - \Covered{$p_i, T$}$} {
			$\variable{examples} \gets \variable{examples} \cup \{(I, \texttt{false})\}$;
		}
		\For {each $(I, O) \in \Covered{$p_i, T$} - \bigcup_{j ={i+1}}^{m} \Covered{$p_j, T$} $}{
			$\variable{examples} \gets \variable{examples} \cup \{(I, \texttt{true})\}$;
		}
		$c_i \gets \mathcal C(\variable{examples})$; \\
		\lIf {$c_i = \top$}{\Return $\top$}
		$\variable{conditionList}.\AP{$c_i$};\ \ T \gets \{(I, O) \in T\ |\ \neg \sem{c_i}(I)\}$; \\
	}
	$\variable{result} \gets p_m$; \\
	\For {$i \gets m - 1$; $i > 0$; $i \gets i - 1$}{
		$\variable{result} \gets \texttt{if}\ \variable{conditionList}_i\ \texttt{then}\ p_i\ \texttt{else}\ \variable{result}$;
	}
	
	\Return \EP{\variable{result}};
\end{algorithm}

$\mathcal U_{\text{poly}}$ decomposes the unification task into $m-1$ PBE tasks for $c_1, \dots, c_{m-1}$ respectively. Algorithm \ref{alg:uni-over} shows the framework of $\mathcal U_{\text{poly}}$, which synthesizes conditions in order (Lines 2-13). For each term $p_i$ and each remaining example $e=(I, O)$, there are three possible cases:
\begin{itemize} 
	\item if $p_i$ is not consistent with $e$, the \texttt{if}-condition of $p_i$ must be \texttt{False} on input $I$, and thus $e$ can be taken as a negative example for $c_i$ (Lines 4-6).
	\item If $p_i$ is the only program in $p_i, \dots, p_n$ that is consistent with example $e$, the \texttt{if}-condition of $p_i$ must be \texttt{True} on input $I$, and thus $e$ can be taken as a positive example (Lines 7-9). 
	\item Otherwise, the value of $c_i$ does not matter, as $p_i$ is not the last term satisfying the example. Therefore, $\mathcal U_{\text{poly}}$ choose to ignore this example: If the synthesized $c_i$ takes \texttt{false} on $e$, $e$ will be left to subsequent terms.
\end{itemize}
In this way, a PBE task for $c_i$ is obtained, and thus the task can be passed to a condition solver $\mathcal C$ (Line 10). After obtaining a valid $c_i$, $\mathcal U_{\text{poly}}$ excludes all examples covered by $c_i$ (Line 12) and then continue to the next term.  

Note that the intermidiate result (Lines 14-16) cannot be returned directly, as it may involve boolean operators $\texttt{and}, \texttt{or}$ and $\texttt{not}$, which are unavailable in $(\mathbb P_t, \mathbb P_c)$. Therefore, $\mathcal U_{\text{poly}}$ expands $\variable{result}$ and fits it into $(\mathbb P_c, \mathbb P_t)$ via $\EP{}$ (Line 18). However, in practice, the last step can be omitted as $\variable{result}$ is always executable in practice even though it is not inside $(\mathbb P_c, \mathbb P_t)$.

Just like $\mathcal T_{\text{poly}}$, unifier $\mathcal U_{\text{poly}}$ can also inherient useful properties from the condition solver $\mathcal C$.

\begin{theorem} $\mathcal C$ is valid for $\text{DNF}(\mathcal F_C) \implies \mathcal U_{\text{poly}}$ is valid for $\mathcal F_C$, where $\text{DNF}(\mathcal F_C)$ is a family of condition domains induced from $\mathcal F_C$, i.e., $\text{DNF}(\mathcal F_C) \coloneqq \{(\text{DNF}(\mathbb P_c), \mathbb I')\ |\ ((\mathbb P_t, \mathbb P_c), \mathbb I) \in \mathcal F_C \wedge \mathbb I' \subseteq \mathbb I\}$.
\end{theorem}

\begin{theorem} \label{theorem:unifier-gen} $\mathcal C \in \mathsf {PSG}[\text{DNF}(\mathcal F_C)] \implies \mathcal U_{\text{poly}} \in \mathsf {PSG}[\mathcal F_C]$.
\end{theorem}

By Theorem \ref{theorem:unifier-gen}, the only problem remaining is to design a condition solver with polynomial-size generalizability. We shall gradually build such a condition solver in the following three subsections. 

\subsection{Condition Synthesis for Clauses} \label{section:uni-simple}
Before discussing the condition solver $\mathcal C$, we introduce some useful notations first:
\begin{itemize}
	\item We regard a DNF formula $d$ as a set of clauses, regard a clause $c$ as a set of literals, and use notation $p_c(c)$ and $p_d(d)$ to represent the corresponding program, $\left(\texttt{and}_l\ l\text{ for }l \in c\right)$ and $\left(\texttt{or}_c\ \left(\texttt{and}_l\ l\text{ for }l \in c\right)\text{ for }c \in d\right)$, respectively. 
	\item For an input space $\mathbb I$ and a condition $p$, we use $P(\mathbb I, p)$ and $N(\mathbb I, p)$ to denote the set of inputs where $p$ is evaluated to \texttt{true} and \texttt{false} respectively, i.e.:
	$$P(\mathbb I, p) \coloneqq \{I \in \mathbb I\ |\ \sem{p}(I) = \texttt{true}\}\ \ \ N(\mathbb I, p) \coloneqq \{I \in \mathbb I\ |\ \sem{p}(I) = \texttt{false}\}$$
	\item For a PBE task $T$, we use $\mathbb I(T)$, $\mathbb I_P(T)$ and $\mathbb I_N(T)$ to denote the inputs of examples, positive examples and negative examples in $T$ respectively, i.e.:
	$$\mathbb I(T) \coloneqq \{I\ |\ (I, O) \in T\}\ \ \ \mathbb I_P(T) \coloneqq \{I\ |\ (I, \texttt{true}) \in T\}\ \ \ \mathbb I_N(T) \coloneqq \{I\ |\ (I, \texttt{false}) \in T\}$$
\end{itemize}
For a PBE task $T$ on condition domain $(\text{DNF}(\mathbb P_c), \mathbb I)$, a valid condition $p$ should satisfy two conditions: (1) $\mathbb I_P(T) \subseteq P(\mathbb I(T), p)$; (2) $\mathbb I_N(T) \subseteq N(\mathbb I(T), p)$.

\begin{algorithm}[t]
	\small
	\caption{The pseudo code of clause solver $\mathcal C_{\text{CL}}$.}
	\label{alg:uni-over}
	\LinesNumbered
	\KwIn{A condition domain $\mathbb P_c$ and a PBE task $T$.}
	\KwOut{A program in $\text{CL}(\mathbb P_c)$ satisfying all examples or $\top$.}
	\SetKwProg{Fn}{Function}{:}{}

	$c^* \gets \{l \in \text{L}(\mathbb P_c)\ |\ \mathbb I_P(T) \subseteq P(\mathbb I(T), l)\}$; \\
	\lIf {$\mathbb I_N(T) \subseteq N(\mathbb I(T), c^*) $}{\Return $p_c(c^*)$}
	\Return $\top$;
\end{algorithm} 

In this section, we focus on a subproblem of condition synthesis, where the target condition is assumed to be a single clause. Algorithm \ref{alg:uni-over} shows the pseudo code of a simple solver $\mathcal C_{\text{CL}}$.

$\mathcal C_{\text{CL}}$ starts with the first condition of a valid clause: $\mathbb I_P(T) \subseteq P(\mathbb I(T), c)$. By the semantics of operator $\texttt{and}$, for any clause $c$ and any literal $l \in c$, $P(\mathbb I(T), c)$ must be a subset of $P(\mathbb I(T), l)$. Therefore, only those literals that covers all positive examples can be used in the result. $\mathcal C_{\text{CL}}$ constructs a clause $c^*$ that includes all possible literals (Line 1). Obviously, $c^*$ itself satisfies the first condition, and all valid clauses must be a subset of $c^*$. By the semantic of operator \texttt{and}, for any two clauses $c_1$ and $c_2$, $c_1 \subseteq c_2 \implies N(\mathbb I(T), c_1) \subseteq N(\mathbb I(T), c_2)$. Therefore, if $c^*$ does not satisfy the second condition, neither does any subset of $c^*$ (Lines 2-3).

The generalizability of $\mathcal C_{\text{CL}}$ is bounded. For input space $\mathbb I$ and target clause $c$, we say a literal $l$ is incorrect for target clause $c$ if $P(\mathbb I, c) \not \subseteq P(\mathbb I, l)$. According to Algorithmn \ref{alg:uni-over}, $\mathcal C_{\text{CL}}$ generalizes to the target $c$ when all incorrect literals are excluded. As the number of incorrect literals is bounded by $|\text{L}(\mathbb P_c)| \leq 2|\mathbb P_C|$, and the probability for each incorrect literal to be excluded is guaranteed by Assumption \ref{ass:2}, the generalizability of $\mathcal C_{\text{CL}}$ is bounded by $O(\ln |\mathbb P_C|)$.

\begin{theorem} \label{theorem:cl-gen}For any domain $\mathbb D = (\text{CL}(\mathbb P_c), \mathbb I), \text{gen}[\mathbb D, \mathcal C_{\text{CL}}](p, \epsilon) \leq \frac{1}{\alpha}\left(\ln \left(2|\mathbb P_C|\right) + \ln(1 / \epsilon)\right)$.
\end{theorem}

Theorem \ref{theorem:cl-gen} implies that: If $\mathbb P_c$ contains only conditions of which the sizes are close to the target condition, the generalizability of $\mathcal C_{\text{CL}}$ can be bounded by the size of the target.
\subsection{Condition Synthesis for Disjunctive Normal Forms} \label{section:uni-full}
In this section, we implement a condition solver $\mathcal C$ with guaranteed generalizability for disjunctive normal forms. By the semantics of operator \texttt{or}, we could obtain a lemma that is similiar with Lemma \ref{lemma:sample} in form. 

\begin{lemma}\label{lemma:or-sample} Let $T$ be a PBE task and $d$ be a DNF formula satisfying all examples in $T$, then:
	\begin{itemize}
		\item All clauses in $d$ must be \texttt{false} on all negative examplesin $T$, i.e., $\forall c \in d, \mathbb I_N(T) \subseteq N(\mathbb I(T), c)$.
		\item There exists a clause in $d$ that is \texttt{true} on at least $|d|^{-1}$ portion of positive examples in $T$, i.e., $\exists c \in d, |P(\mathbb I(T), c)| \geq |d|^{-1}|\mathbb I_P(T)|$.
	\end{itemize}
\end{lemma}
Lemma \ref{lemma:or-sample} allows $\mathcal C$ to decompose the condition synthesis task to clause synthesis tasks in a similiar way as $\mathcal T_{\text{poly}}$ (Lines 11-30 in Algorithm \ref{alg:term-main}).

\SetKwFunction{SR}{Search}
\SetKwFunction{DAC}{DivideAndConquer}
\SetKwFunction{SCS}{SimplifyClauseSet}
\SetKwFunction{GC}{GetPossibleClause}
\SetKwFunction{VC}{IsValidClause}
\SetKwFunction{In}{Insert}
\SetKwFunction{De}{Delete}
\SetKwFunction{G}{Get}
\SetKwFunction{Search}{Search}
\SetKwFunction{GPWS}{GetProgramsWithSizeBound}

\begin{algorithm}[t]
	\small
	\caption{Condition solver $\mathcal C$ for disjunctive normal forms}
	\label{alg:uni-dnf-main}
	\LinesNumbered
	\KwIn{A condition domain $\mathbb P_c$, a PBE task $T$ and parameters $(k_0, s_0)$.}
	\KwOut{A DNF formula in $\text{DNF}(\mathbb P_c)$ satisfying all examples or $\top$.}
	\SetKwProg{Fn}{Function}{:}{}
	\Fn{\Search{$\variable{literals}, T, k$}}{
		\lIf{$(\variable{literals}, T, k)$ is visited before} {\Return $\top$}
		\lIf {$|\mathbb I_P(T)| = 0$}{\Return $\{\}$}
		\lIf {$k = 0$}{\Return $\top$}
		\For{each $c \in \GC{$\variable{literals}, T, k$}$}{
			$\variable{searchResult} \gets \Search{$\variable{literals}, T - \left\{(I, \texttt{true}) \in T\ |\ \sem{p_c(c)}(I) = \texttt{true} \right\}, k - 1$}$; \\
			\lIf{$\variable{searchResult} \neq \top$}{\Return $\{c\} \cup \variable{searchResult}$}
		}
		\Return $\top$;
	}
	$s_{\text{max}} = \max_p \text{size}(p)\text{ for } p \in \mathbb P_c;\ \ k_0 \gets \min(k_0, |T|);\ \ s_0 \gets \min(s_0, s_{\text{max}});$ \\
	\While {$k_0 \leq |T| \vee s_0 \leq s_{\text{max}}$}{
	\For {each $(k, s) \in [1, k_0] \times [1, s_0]$}{
		\If {$(k, s)$ has not been visited before} {
			$d \gets \Search{$\text{L}(\GPWS{$\mathbb P_c, s$}),T, k$}$; \\
			\lIf{$P \neq \top$}{\Return $p_d(d)$}
		}
	}
	$k_0 \gets k_0 + 1; \ \ s_0 \gets s_0 + 1$; 
	}
	\Return $\top$.
\end{algorithm} 

Algorithm \ref{alg:uni-dnf-main} shows the pseudo code of $\mathcal C$, which is comprised of two parts. The first part is a backtracking on the set of clauses, implemented as Function \Search{} (Lines 1-9), which is almost the same as the second part of Algorithm \ref{alg:term-main}. Function \Search{} takes a set of literals $\variable{literals}$, a PBE task $T$ and an upper bound $k$ as the input, and its goal is to find a valid DNF formula comprised of at most $k$ clauses with literals inside $\variable{literals}$. Guided by Lemma \ref{lemma:or-sample}, \Search{} invokes \GC{} to find a set of clauses that are evaluated to \texttt{false} on all negative examples, and are evaluated to \texttt{true} on at least $k^{-1}$ portion of postive examples (Line 14). Then, \Search{} recursively try all possible clauses until a valid DNF formula is found (Lines 6-7). 

The second part iteratively selects parameters for the backtracking (Lines 10-20). Besides the size limit $k$, $\mathcal C$ also iteratively determines the set of literals, as the generalizability of the clause solver $\mathcal C$ is polynomial-size only when the number of literals is bounded (according to Theorem \ref{theorem:cl-gen}). In each turn, $\mathcal C$ invokes function $\GPWS{}$ to obtain all conditions in $\mathbb P_c$ with a size at most $k$, and invokes $\Search{}$ with the corresponding set of literals (Line 14). 

Now, we go to the implementation of \GC{} (abbreviated as \G{}). To guarantee the generalizability of $\mathcal C$, \G{} should satisfy the following two requirements:
\begin{itemize}
	\item Under a small number of examples, which is at most polynomial to $\ln |\mathbb P_c|$, \G{} should guarantee that with a high probability, at least one intended clause is found. Otherwise, the probability for $
	\mathcal C_{\text{CL}}$ to miss the target condition may be unbounded.
	\item The number of clauses returned by \G{} should be small, of which the logarithm should be at most polynomial to $\ln |\mathbb P_c|$. Otherwise, the search alrgoithm may expand to too many search branches, and thus it may require a lot of examples to guarantee the first valid DNF formula is semantically equivalent to the target one.
\end{itemize}

Actually, applying the sampling algorithm in $\mathcal T_{\text{poly}}$ with the clause solver $\mathcal C_{\text{CL}}$ already satisfies both requirements. In condition solver $\mathcal C$, we make some optimization by opening the box of the clause solver $\mathcal C_{\text{CL}}$. More concretely, our implementation of \G{} finds all possible results of $\mathcal C_{\text{CL}}$, denoted as a representative set, and returns them as the result. According to Algorithm \ref{alg:uni-over}, though there may be many clauses corresponding to each semantics on the space of positive examples, only the largest clause corresponding to each semantics is possible to be returned by $\mathcal C_{\text{CL}}$.

We formalize this idea with some additional notations. Given an input space $\mathbb I$ and a set of literals $L$, the relationship of semantically equivalence $\sim_{\mathbb I}$ divides the clause space $\text{CL}(L)$ into several equivalent classes. We denote the set of those classes as $[\text{CL}(L)]_{\mathbb I}$, and the equivalent class of clause $c$ as $[c]_{\mathbb I}$. It is easy to show that each class $[c]_{\mathbb I}$ contains a globally largest clause that is the union of all its elements, i.e., $\exists c' \in [c]_{\mathbb I},  c' = \left(\cup_{x}\ x\text{ for } x \in [c]_{\mathbb I}\right)$. 

\begin{definition}[Representative Clauses] 
	Given a input space $\mathbb I$, a size limit $k$, and a set of literals $L$, representative set $R(\mathbb I, k, L) \subseteq \text{CL}(L)$ includes all clause $c$ satisfying: (1) $c$ is the largest element in $[c]_{\mathbb I}$, (2) $c$ is consistent with least $k^{-1}$ portion of positive examples, i.e., $|P(\mathbb I_P(T), c)| \geq k^{-1} |\mathbb I_P(T)|$.
\end{definition}

The following lemma shows that $R(T, k, L)$ succesfully captures all wanted results of $\mathcal C_{\text{CL}}$.

\begin{lemma} \label{lemma:rp-set}For any PBE task $T$, size limit $k$, and set $L$ of literals, for any subset of examples $T' \subseteq T$, if the clause synthesized by $\mathcal C_{\text{CL}}$ on subtask $T'$ satisfies at least $k^{-1}$ portion of positive examples in $T$, this clause must be inside $R(T, k, L)$, i.e.,
	$$
	\forall T' \subseteq T, \left(\big|P\big(\mathbb I_P(T), \mathcal C_{\text{CL}}[L](T')\big)\big| \geq \frac{|\mathbb I_P(T)|}{k} \implies \mathcal C_{\text{CL}}[L](T') \in R(\mathbb I_P(T), k, L)\right)
	$$
\end{lemma}

\begin{algorithm}[t]
	\small
	\caption{Implementation of \texttt{GetPossibleClause()} in $\mathcal C$.}
	\label{alg:get-clause}
	\LinesNumbered
	\KwIn{A set of literals $\variable{literals}$, a PBE task $T$, and an upper bound $k$.}
	\KwOut{A set of possible clauses according to Lemma \ref{lemma:or-sample}.}
	$\variable{result} \gets \{\emptyset\}$; \\
	\For {each $l \in \variable{literals}$}{
		\For {each $c \in \variable{result}$}{
			\lIf{$\left|P(\mathbb I_P(T), c \cup \{l\})\right| \geq k^{-1}\left|\mathbb I_P(T)\right|$}{$\variable{result}.\In{$c \cup \{l\}$}$}
		}
		\For {each $c \in \variable{result}$}{
			\lIf{$\exists c' \in \variable{result}, \left(P(\mathbb I_P(T), c) = P(\mathbb I_P(T), c') \wedge c \subset c'\right)$}{$\variable{result}.\De{$c$}$}
		}
	}
	\Return $\left\{c \in \variable{result}\ |\  \mathbb I_N(T) \subseteq N(\mathbb I (T),c)\right\}$
\end{algorithm} 

Our implementation of \G{} is shown as Algorithm \ref{alg:get-clause}. \G{} maintains set \variable{result} which is equal to $R(\mathbb I_P(T), k, L)$ for some hidden literal set $L$. Initially, $L$ is empty and thus $\variable{result}$ includes only an empty clause, i.e., \texttt{true} (Line 1). \G{} considers all literals in order (Lines 2-9). In each turn, a new literal is inserted to $L$ and thus \variable{result} is updated correspondingly (Lines 3-8). At last, $\variable{result}$ is equal to $R(\mathbb I_P(T), k, \variable{literal})$, and thus \G{} returns all valid clause in $\variable{result}$ (Line 10).

Now, we shall informally show why \G{} satisfies the two requirements. The full proof can be found in the appendix. The first requirement is obvious: As \G{} returns all possible results of $\mathcal C_{\text{CL}}$ on a subset of examples, the probability for \G{} to find an inteneded clause must be larger than the sampling algorithm in $\mathcal T_{\text{poly}}$, which has been proved to satisfy this condition. 

To prove the second requirement, we need to bound the size of $R(\mathbb I_P(T), k, L)$. Let $\mathbb I_P \subseteq \mathbb I$ be the entire set of inputs where the target condition is \texttt{true}. As $\mathbb I_P(T) \subseteq \mathbb I_P$, relation $\sim_{\mathbb I_P}$ is a refinement of relation $\sim_{\mathbb I_P(T)}$, i.e., $\forall c_1, c_2 \in \text{CL}(\mathbb P_c)$, $p_c(c_1) \sim_{\mathbb I_P} p_c(c_2)\implies p_c(c_1) \sim_{\mathbb I_P(T)} p_c(c_2)$. Hence $|R(\mathbb I_P(T), k, L)|$ is no larger than the number of classes $[c]_{\mathbb I_P}$ in $[\text{CL}(L)]_{\mathbb I_P}$ with $|P(\mathbb I_P(T), c)| \geq k^{-1}|\mathbb I_P(T)|$. Intuitively, the more inputs in $\mathbb I_P$ are covered by clause $c$, the more probable for equivalent class $[c]_{\mathbb I_P}$ to satisfy at least $k^{-1}$ portion of examples in $T$. The following lemma formally bounds the number of equivalent classes in $[\text{CL}(L)]_{\mathbb I_P}$ that covers a large enough number of examples, and thus limits the size of the representative set $R(\mathbb I_P(T), k, L)$.

\begin{lemma} \label{lemma:class-size}Let $t = \frac{1}{\alpha}\ln(4|L|)$, the number of equivalent classes $[c]_{\mathbb I_P}$ in $[\text{CL}(L)]_{\mathbb I_P}$, where the probability for $c$ to be \texttt{true} on a random example in $\mathbb I_P$ is at least $\beta$, is at most $2\beta^{-t}$, i.e.,:
	$$\left|\left\{[c]_{\mathbb I_P} \in [\text{CL}(L)]_{\mathbb I_P}\ \big|\ \Pr_{I \sim {D_I}} \left[\sem{c}(I)\ |\ I \in \mathbb I_P\right] \geq \beta\right\}\right| \leq 2\left(\frac{1}{\beta}\right)^t
	$$ 
\end{lemma}

Theorem \ref{theorem:condition-solver} formally states that $\mathcal C$ has polynomial-size generalizability.
\begin{theorem} \label{theorem:condition-solver}$\mathcal C \in \mathsf{PSG}[\text{DNF}(\mathcal F_C^A)]$.
\end{theorem}

Combining Theorem \ref{theorem:condition-solver} with Theorem \ref{theorem:unifier-gen} and Theorem \ref{theorem:gen-stun}, we prove the generalizability of $\mathcal U_{\text{poly}}$ and \mainname are all polynomial
\begin{theorem} $\mathcal U_{\text{poly}}$ implemented with condition solver $\mathcal C$ is inside $\mathsf{PSG}[\mathcal F_C^A]$.
\end{theorem}
\begin{theorem}\label{theorem:main} $\mathcal S_t$ is size-preserving on $T(\mathcal F_C) \implies \mainname \in \mathsf{PSG}[\mathcal F_C]$.
\end{theorem}


